Quantum Emission From Hexagonal Boron Nitride Monolayers

Atomically thin van der Waals crystals have recently enabled new scientific and technological breakthroughs across a variety of disciplines in materials science, nanophotonics and physics. However, non-classical photon emission from these materials has not been achieved to date. Here we report room temperature quantum emission from hexagonal boron nitride nanoflakes. The single photon emitter exhibits a combination of superb quantum optical properties at room temperature that include the highest brightness reported in the visible part of the spectrum, narrow line width, absolute photo-stability, a short excited state lifetime and a high quantum efficiency. Density functional theory modeling suggests that the emitter is the antisite nitrogen vacancy defect that is present in single and multi-layer hexagonal boron nitride. Our results constitute the unprecedented potential of van der Waals crystals for nanophotonics, optoelectronics and quantum information processing.

==> Photonics <==
% This file was created with JabRef 2.10.
% Encoding: UTF8


@Article{Abass2014,
  Title                    = {Active liquid crystal tuning of metallic nanoantenna enhanced light emission from colloidal quantum dots},
  Author                   = {Abass, A. and Rodriguez, S. R. and Ako, T. and Aubert, T. and Verschuuren, M. and Van Thourhout, D. and Beeckman, J. and Hens, Z. and Gomez Rivas, J. and Maes, B.},
  Journal                  = {Nano Lett},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {5555-60},
  Volume                   = {14},

  Abstract                 = {A system comprising an aluminum nanoantenna array on top of a luminescent colloidal quantum dot waveguide and covered by a thermotropic liquid crystal (LC) is introduced. By heating the LC above its critical temperature, we demonstrate that the concomitant refractive index change modifies the hybrid plasmonic-photonic resonances in the system. This enables active control of the spectrum and directionality of the narrow-band ( approximately 6 nm) enhancement of quantum dot photoluminescence by the metallic nanoantennas.},
  Doi                      = {10.1021/nl501955e},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25237822}
}

@Article{Adiga2009,
  Title                    = {Mechanical stiffness and dissipation in ultrananocrystalline diamond microresonators},
  Author                   = {Adiga, V. and Sumant, A. and Suresh, S. and Gudeman, C. and Auciello, O. and Carlisle, J. and Carpick, R.},
  Journal                  = {Physical Review B},
  Year                     = {2009},
  Number                   = {24},
  Volume                   = {79},

  Doi                      = {10.1103/PhysRevB.79.245403},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Aharonovich2010,
  Title                    = {Photophysics of chromium-related diamond single-photon emitters},
  Author                   = {Aharonovich, I. and Castelletto, S. and Simpson, D. A. and Greentree, A. D. and Prawer, S.},
  Journal                  = {Phys. Rev. A},
  Year                     = {2010},
  Number                   = {4},
  Pages                    = {043813},
  Volume                   = {81},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevA.81.043813}
}

@Article{Aharonovich2009,
  Title                    = {Two-Level Ultrabright Single Photon Emission from Diamond Nanocrystals},
  Author                   = {Aharonovich, Igor and Castelletto, Stefania and Simpson, David A. and Stacey, Alastair and McCallum, Jeff and Greentree, Andrew D. and Prawer, Steven},
  Journal                  = {Nano Lett.},
  Year                     = {2009},
  Number                   = {9},
  Pages                    = {3191-3195},
  Volume                   = {9},

  Doi                      = {10.1021/nl9014167},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl9014167}
}

@Article{Aharonovich2011,
  Title                    = {Diamond-based single-photon emitters},
  Author                   = {Aharonovich, I. and Castelletto, S. and Simpson, D. A. and Su, C. H. and Greentree, A. D. and Prawer, S.},
  Journal                  = {Reports on Progress in Physics},
  Year                     = {2011},
  Number                   = {7},
  Pages                    = {076501},
  Volume                   = {74},

  Doi                      = {10.1088/0034-4885/74/7/076501},
  ISSN                     = {0034-4885
1361-6633},
  Type                     = {Journal Article}
}

@Article{Aharonovich2011a,
  Title                    = {Diamond photonics},
  Author                   = {Aharonovich, Igor and Greentree, Andrew D. and Prawer, Steven},
  Journal                  = {Nat Photon},
  Year                     = {2011},
  Number                   = {7},
  Pages                    = {397-405},
  Volume                   = {5},

  ISSN                     = {1749-4885},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nphoton.2011.54}
}

@Article{Aharonovich2014,
  Title                    = {Diamond Nanophotonics},
  Author                   = {Aharonovich, Igor and Neu, Elke},
  Journal                  = {Adv. Opt. Mater.},
  Year                     = {2014},
  Pages                    = {911-928},

  Doi                      = {10.1002/adom.201400189},
  ISSN                     = {21951071},
  Type                     = {Journal Article}
}

@Article{Ahmad2014,
  Title                    = {Synthesis of Boron Nitride Microtubes and Formation of Boron Nitride Nanosheets},
  Author                   = {Ahmad, Pervaiz and Khandaker, Mayeen Uddin and Amin, Yusoff Mohd and Khan, Ziaul Raza},
  Journal                  = {Materials and Manufacturing Processes},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {184-188},
  Volume                   = {30},

  Doi                      = {10.1080/10426914.2014.952041},
  ISSN                     = {1042-6914},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1080/10426914.2014.952041}
}

@Article{Ahn2013,
  Title                    = {Localized plasmon resonances of bimetallic AgAuAg nanorods},
  Author                   = {Ahn, S. H. and Kim, D. S. and Seo, D. and Choi, W. and Yi, G. R. and Song, H. and Park, Q. H. and Kim, Z. H.},
  Journal                  = {Phys Chem Chem Phys},
  Year                     = {2013},
  Number                   = {12},
  Pages                    = {4190-4},
  Volume                   = {15},

  Abstract                 = {We investigated the localized surface plasmon resonances of individual AgAuAg nanorods (NRs) using the dark-field spectro-microscopy technique. We find that the scattering spectra of such hetero-NRs show longitudinal resonance wavelengths that are nearly insensitive to the relative composition of Ag and Au. Instead, the resonance is mostly governed by the overall length of the nanorod. This shows that the plasmons oscillate along the entire length of the NR without the significant perturbation at the Ag-Au interfaces. The results demonstrate that the overall geometry as well as the composition determine the tunability of the hetero-metallic nanostructures, and provide an important design rule for the composition-tunable bimetallic plasmon structures.},
  Doi                      = {10.1039/c2cp43365f},
  ISSN                     = {1463-9084 (Electronic)
1463-9076 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23247539}
}

@Article{Ahn2013a,
  Title                    = {Demonstration of Efficient On-Chip Photon Transfer in Self-Assembled Optoplasmonic Networks},
  Author                   = {Ahn, Wonmi and Hong, Yan and Boriskina, Svetlana V. and Reinhard, BjÃ¶rn M.},
  Journal                  = {ACS Nano},
  Year                     = {2013},
  Number                   = {5},
  Pages                    = {4470-4478},
  Volume                   = {7},

  Doi                      = {10.1021/nn401062b},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn401062b}
}

@Article{Akimov2007,
  Title                    = {Generation of single optical plasmons in metallic nanowires coupled to quantum dots},
  Author                   = {Akimov, A. V. and Mukherjee, A. and Yu, C. L. and Chang, D. E. and Zibrov, A. S. and Hemmer, P. R. and Park, H. and Lukin, M. D.},
  Journal                  = {Nature},
  Year                     = {2007},
  Number                   = {7168},
  Pages                    = {402-6},
  Volume                   = {450},

  Abstract                 = {Control over the interaction between single photons and individual optical emitters is an outstanding problem in quantum science and engineering. It is of interest for ultimate control over light quanta, as well as for potential applications such as efficient photon collection, single-photon switching and transistors, and long-range optical coupling of quantum bits. Recently, substantial advances have been made towards these goals, based on modifying photon fields around an emitter using high-finesse optical cavities. Here we demonstrate a cavity-free, broadband approach for engineering photon-emitter interactions via subwavelength confinement of optical fields near metallic nanostructures. When a single CdSe quantum dot is optically excited in close proximity to a silver nanowire, emission from the quantum dot couples directly to guided surface plasmons in the nanowire, causing the wire's ends to light up. Non-classical photon correlations between the emission from the quantum dot and the ends of the nanowire demonstrate that the latter stems from the generation of single, quantized plasmons. Results from a large number of devices show that efficient coupling is accompanied by more than 2.5-fold enhancement of the quantum dot spontaneous emission, in good agreement with theoretical predictions.},
  Doi                      = {10.1038/nature06230},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/18004381}
}

@Article{Akinwande2014,
  Title                    = {Two-dimensional flexible nanoelectronics},
  Author                   = {Akinwande, D. and Petrone, N. and Hone, J.},
  Journal                  = {Nat Commun},
  Year                     = {2014},
  Pages                    = {5678},
  Volume                   = {5},

  Abstract                 = {2014/2015 represents the tenth anniversary of modern graphene research. Over this decade, graphene has proven to be attractive for thin-film transistors owing to its remarkable electronic, optical, mechanical and thermal properties. Even its major drawback--zero bandgap--has resulted in something positive: a resurgence of interest in two-dimensional semiconductors, such as dichalcogenides and buckled nanomaterials with sizeable bandgaps. With the discovery of hexagonal boron nitride as an ideal dielectric, the materials are now in place to advance integrated flexible nanoelectronics, which uniquely take advantage of the unmatched portfolio of properties of two-dimensional crystals, beyond the capability of conventional thin films for ubiquitous flexible systems.},
  Doi                      = {10.1038/ncomms6678},
  ISSN                     = {2041-1723 (Electronic)
2041-1723 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25517105}
}

@Article{Alegre2007,
  Title                    = {Polarization-selective excitation of nitrogen vacancy centers in diamond},
  Author                   = {Alegre, Thiago P. Mayer and Santori, Charles and Medeiros-Ribeiro, Gilberto and Beausoleil, Raymond G.},
  Journal                  = {Physical Review B},
  Year                     = {2007},
  Number                   = {16},
  Volume                   = {76},

  Doi                      = {10.1103/PhysRevB.76.165205},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Almeida2003,
  Title                    = {Nanotaper for compact mode conversion},
  Author                   = {Almeida, V. R. and Panepucci, R. R. and Lipson, M.},
  Journal                  = {Optics Letters},
  Year                     = {2003},
  Number                   = {15},
  Pages                    = {1302-1304},
  Volume                   = {28},

  Abstract                 = {We propose and demonstrate an efficient coupler for compact mode conversion between a fiber and a submicrometer waveguide. The coupler is composed of high-index-contrast materials and is based on a short taper with a nanometer-sized tip. We show that the micrometer-long silicon-on-insulator-based nanotaper coupler is able to efficiently convert both the mode field profile and the effective index, with a total length as short as 40 mum. We measure an enhancement of the coupling efficiency between an optical fiber and a waveguide by 1 order of magnitude due to the coupler. (C) 2003 Optical Society of America.},
  Doi                      = {10.1364/ol.28.001302},
  ISSN                     = {0146-9592},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000184256400004}
}

@Article{Ambrose1994,
  Title                    = {Alterations of Single Molecule Fluorescence Lifetimes in Near-Field Optical Microscopy},
  Author                   = {Ambrose, W. Patrick and Goodwin, Peter M. and Keller, Richard A. and Martin, John C.},
  Journal                  = {Science},
  Year                     = {1994},
  Number                   = {5170},
  Pages                    = {364-367},
  Volume                   = {265},

  Abstract                 = {Fluorescence lifetimes of single Rhodamine 6G molecules on silica surfaces were measured with pulsed laser excitation, time-correlated single photon counting, and near-field scanning optical microscopy (NSOM). The fluorescence lifetime varies with the position of a molecule relative to a near-field probe. Qualitative features of lifetime decreases are consistent with molecular excited state quenching effects near metal surfaces. The technique of NSOM provides a means of altering the environment of a single fluorescent molecule and its decay kinetics in a repeatable fashion.},
  Doi                      = {10.1126/science.265.5170.364},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/265/5170/364.abstract}
}

@Article{Aoki2008,
  Title                    = {Coupling of quantum-dot light emission with a three-dimensional photonic-crystal nanocavity},
  Author                   = {Aoki, Kanna and Guimard, Denis and Nishioka, Masao and Nomura, Masahiro and Iwamoto, Satoshi and Arakawa, Yasuhiko},
  Journal                  = {Nature Photonics},
  Year                     = {2008},
  Number                   = {11},
  Pages                    = {688-692},
  Volume                   = {2},

  Doi                      = {10.1038/nphoton.2008.202},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Aouani2014,
  Title                    = {Third-harmonic-upconversion enhancement from a single semiconductor nanoparticle coupled to a plasmonic antenna},
  Author                   = {Aouani, H. and Rahmani, M. and Navarro-Cia, M. and Maier, S. A.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2014},
  Number                   = {4},
  Pages                    = {290-4},
  Volume                   = {9},

  Abstract                 = {The ability to convert low-energy quanta into a quantum of higher energy is of great interest for a variety of applications, including bioimaging, drug delivery and photovoltaics. Although high conversion efficiencies can be achieved using macroscopic nonlinear crystals, upconverting light at the nanometre scale remains challenging because the subwavelength scale of materials prevents the exploitation of phase-matching processes. Light-plasmon interactions that occur in nanostructured noble metals have offered alternative opportunities for nonlinear upconversion of infrared light, but conversion efficiency rates remain extremely low due to the weak penetration of the exciting fields into the metal. Here, we show that third-harmonic generation from an individual semiconductor indium tin oxide nanoparticle is significantly enhanced when coupled within a plasmonic gold dimer. The plasmonic dimer acts as a receiving optical antenna, confining the incident far-field radiation into a near field localized at its gap; the indium tin oxide nanoparticle located at the plasmonic dimer gap acts as a localized nonlinear transmitter upconverting three incident photons at frequency omega into a photon at frequency 3omega. This hybrid nanodevice provides third-harmonic-generation enhancements of up to 10(6)-fold compared with an isolated indium tin oxide nanoparticle, with an effective third-order susceptibility up to 3.5 x 10(3) nm V(-2) and conversion efficiency of 0.0007%. We also show that the upconverted third-harmonic emission can be exploited to probe the near-field intensity at the plasmonic dimer gap.},
  Doi                      = {10.1038/nnano.2014.27},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24608232}
}

@Article{Arcizet2011,
  Title                    = {A single nitrogen-vacancy defect coupled to a nanomechanical oscillator},
  Author                   = {Arcizet, O. and Jacques, V. and Siria, A. and Poncharal, P. and Vincent, P. and Seidelin, S.},
  Journal                  = {Nature Physics},
  Year                     = {2011},
  Number                   = {11},
  Pages                    = {879-883},
  Volume                   = {7},

  Doi                      = {10.1038/nphys2070},
  ISSN                     = {1745-2473
1745-2481},
  Type                     = {Journal Article}
}

@Article{Arenal2006,
  Title                    = {Raman Spectroscopy of Single-Wall Boron Nitride Nanotubes},
  Author                   = {Arenal, R. and Ferrari, A. C. and Reich, S. and Wirtz, L. and Mevellec, J.-Y. and Lefrant, S. and Rubio, A. and Loiseau, A.},
  Journal                  = {Nano Letters},
  Year                     = {2006},
  Number                   = {8},
  Pages                    = {1812-1816},
  Volume                   = {6},

  __markedentry            = {[Toan:6]},
  Doi                      = {10.1021/nl0602544},
  Eprint                   = { 
 http://dx.doi.org/10.1021/nl0602544
 
},
  Owner                    = {Toan},
  Timestamp                = {2015.04.01},
  Url                      = { 
 http://dx.doi.org/10.1021/nl0602544
 
}
}

@Article{Aspetti2014,
  Title                    = {Studies of hot photoluminescence in plasmonically coupled silicon via variable energy excitation and temperature-dependent spectroscopy},
  Author                   = {Aspetti, C. O. and Cho, C. H. and Agarwal, R. and Agarwal, R.},
  Journal                  = {Nano Lett},
  Year                     = {2014},
  Number                   = {9},
  Pages                    = {5413-22},
  Volume                   = {14},

  Abstract                 = {By integrating silicon nanowires ( approximately 150 nm diameter, 20 mum length) with an Omega-shaped plasmonic nanocavity, we are able to generate broadband visible luminescence, which is induced by high order hybrid nanocavity-surface plasmon modes. The nature of this super bandgap emission is explored via photoluminescence spectroscopy studies performed with variable laser excitation energies (1.959 to 2.708 eV) and finite difference time domain simulations. Furthermore, temperature-dependent photoluminescence spectroscopy shows that the observed emission corresponds to radiative recombination of unthermalized (hot) carriers as opposed to a resonant Raman process.},
  Doi                      = {10.1021/nl502606q},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25120156}
}

@Article{Attaccalite2011,
  Title                    = {Coupling of excitons and defect states in boron-nitride nanostructures},
  Author                   = {Attaccalite, C. and Bockstedte, M. and Marini, A. and Rubio, A. and Wirtz, L.},
  Journal                  = {Phys. Rev. B},
  Year                     = {2011},
  Number                   = {14},
  Pages                    = {144115},
  Volume                   = {83},

  Doi                      = {10.1103/PhysRevB.83.144115},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Atwater2007,
  Title                    = {The Promise of Plasmonics},
  Author                   = {Atwater, H. A.},
  Journal                  = {Scientific American},
  Year                     = {2007},
  Pages                    = {56-63},

  Type                     = {Journal Article}
}

@Article{Awschalom2013,
  Title                    = {Quantum Spintronics: Engineering and Manipulating Atom-Like Spins in Semiconductors},
  Author                   = {Awschalom, David D. and Bassett, Lee C. and Dzurak, Andrew S. and Hu, Evelyn L. and Petta, Jason R.},
  Journal                  = {Science},
  Year                     = {2013},
  Number                   = {6124},
  Pages                    = {1174--1179},
  Volume                   = {339},

  Doi                      = {10.1126/science.1231364},
  Oi                       = {Petta, Jason/0000-0002-6416-0789},
  Owner                    = {Toan},
  Pm                       = {23471400},
  Ri                       = {Petta, Jason/J-6663-2013},
  Sn                       = {0036-8075},
  Tc                       = {64},
  Timestamp                = {2015.04.09},
  Ut                       = {WOS:000315709900039},
  Z8                       = {1},
  Z9                       = {65},
  Zb                       = {9},
  Zs                       = {0}
}

@Article{Awschalom2007,
  Title                    = {The diamond age of spintronics - Quantum electronic devices that harness the spins of electrons might one day enable room-temperature quantum computers - made of diamond},
  Author                   = {Awschalom, David D. and Epstein, Ryan and Hanson, Ronald},
  Journal                  = {Scientific American},
  Year                     = {2007},
  Number                   = {4},
  Pages                    = {84-+},
  Volume                   = {297},

  ISSN                     = {0036-8733},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000249677500035}
}

@Article{Babinec2010,
  Title                    = {A diamond nanowire single-photon source},
  Author                   = {Babinec, T. M. and Hausmann, B. J. and Khan, M. and Zhang, Y. and Maze, J. R. and Hemmer, P. R. and Loncar, M.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2010},
  Number                   = {3},
  Pages                    = {195-9},
  Volume                   = {5},

  Abstract                 = {The development of a robust light source that emits one photon at a time will allow new technologies such as secure communication through quantum cryptography. Devices based on fluorescent dye molecules, quantum dots and carbon nanotubes have been demonstrated, but none has combined a high single-photon flux with stable, room-temperature operation. Luminescent centres in diamond have recently emerged as a stable alternative, and, in the case of nitrogen-vacancy centres, offer spin quantum bits with optical readout. However, these luminescent centres in bulk diamond crystals have the disadvantage of low photon out-coupling. Here, we demonstrate a single-photon source composed of a nitrogen-vacancy centre in a diamond nanowire, which produces ten times greater flux than bulk diamond devices, while using ten times less power. This result enables a new class of devices for photonic and quantum information processing based on nanostructured diamond, and could have a broader impact in nanoelectromechanical systems, sensing and scanning probe microscopy.},
  Doi                      = {10.1038/nnano.2010.6},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20154687}
}

@Article{Baffou2014,
  Title                    = {Nanoplasmonics for chemistry},
  Author                   = {Baffou, G. and Quidant, R.},
  Journal                  = {Chem Soc Rev},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {3898-907},
  Volume                   = {43},

  Abstract                 = {Noble metal nanoparticles supporting plasmonic resonances behave as efficient nanosources of light, heat and energetic electrons. Owing to these properties, they offer a unique playground to trigger chemical reactions on the nanoscale. In this tutorial review, we discuss how nanoplasmonics can benefit chemistry and review the most recent developments in this new and fast growing field of research.},
  Doi                      = {10.1039/c3cs60364d},
  ISSN                     = {1460-4744 (Electronic)
0306-0012 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24549257}
}

@Article{Bahari2013,
  Title                    = {Effect of shell thickness on propagation of surface hybrid modes in metallic cylindrical nanoshells},
  Author                   = {Bahari, Ali and Amraie, Elham},
  Journal                  = {Physica Scripta},
  Year                     = {2013},
  Number                   = {3},
  Pages                    = {035707},
  Volume                   = {88},

  Doi                      = {10.1088/0031-8949/88/03/035707},
  ISSN                     = {0031-8949
1402-4896},
  Type                     = {Journal Article}
}

@Article{Bakker2008,
  Title                    = {Nanoantenna array-induced fluorescence enhancement and reduced lifetimes},
  Author                   = {Bakker, Reuben M. and Drachev, Vladimir P. and Liu, Zhengtong and Yuan, Hsiao-Kuan and Pedersen, Rasmus H. and Boltasseva, Alexandra and Chen, Jiji and Irudayaraj, Joseph and Kildishev, Alexander V. and Shalaev, Vladimir M.},
  Journal                  = {New Journal of Physics},
  Year                     = {2008},
  Number                   = {12},
  Pages                    = {125022},
  Volume                   = {10},

  Doi                      = {10.1088/1367-2630/10/12/125022},
  ISSN                     = {1367-2630},
  Type                     = {Journal Article}
}

@Article{Balasubramanian2008,
  Title                    = {Nanoscale imaging magnetometry with diamond spins under ambient conditions},
  Author                   = {Balasubramanian, G. and Chan, I. Y. and Kolesov, R. and Al-Hmoud, M. and Tisler, J. and Shin, C. and Kim, C. and Wojcik, A. and Hemmer, P. R. and Krueger, A. and Hanke, T. and Leitenstorfer, A. and Bratschitsch, R. and Jelezko, F. and Wrachtrup, J.},
  Journal                  = {Nature},
  Year                     = {2008},
  Number                   = {7213},
  Pages                    = {648-51},
  Volume                   = {455},

  Abstract                 = {Magnetic resonance imaging and optical microscopy are key technologies in the life sciences. For microbiological studies, especially of the inner workings of single cells, optical microscopy is normally used because it easily achieves resolution close to the optical wavelength. But in conventional microscopy, diffraction limits the resolution to about half the wavelength. Recently, it was shown that this limit can be partly overcome by nonlinear imaging techniques, but there is still a barrier to reaching the molecular scale. In contrast, in magnetic resonance imaging the spatial resolution is not determined by diffraction; rather, it is limited by magnetic field sensitivity, and so can in principle go well below the optical wavelength. The sensitivity of magnetic resonance imaging has recently been improved enough to image single cells, and magnetic resonance force microscopy has succeeded in detecting single electrons and small nuclear spin ensembles. However, this technique currently requires cryogenic temperatures, which limit most potential biological applications. Alternatively, single-electron spin states can be detected optically, even at room temperature in some systems. Here we show how magneto-optical spin detection can be used to determine the location of a spin associated with a single nitrogen-vacancy centre in diamond with nanometre resolution under ambient conditions. By placing these nitrogen-vacancy spins in functionalized diamond nanocrystals, biologically specific magnetofluorescent spin markers can be produced. Significantly, we show that this nanometre-scale resolution can be achieved without any probes located closer than typical cell dimensions. Furthermore, we demonstrate the use of a single diamond spin as a scanning probe magnetometer to map nanoscale magnetic field variations. The potential impact of single-spin imaging at room temperature is far-reaching. It could lead to the capability to probe biologically relevant spins in living cells.},
  Doi                      = {10.1038/nature07278},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/18833276}
}

@Article{Balasubramanian2009,
  Title                    = {Ultralong spin coherence time in isotopically engineered diamond},
  Author                   = {Balasubramanian, G. and Neumann, P. and Twitchen, D. and Markham, M. and Kolesov, R. and Mizuochi, N. and Isoya, J. and Achard, J. and Beck, J. and Tissler, J. and Jacques, V. and Hemmer, P. R. and Jelezko, F. and Wrachtrup, J.},
  Journal                  = {Nat Mater},
  Year                     = {2009},
  Number                   = {5},
  Pages                    = {383-7},
  Volume                   = {8},

  Abstract                 = {As quantum mechanics ventures into the world of applications and engineering, materials science faces the necessity to design matter to quantum grade purity. For such materials, quantum effects define their physical behaviour and open completely new (quantum) perspectives for applications. Carbon-based materials are particularly good examples, highlighted by the fascinating quantum properties of, for example, nanotubes or graphene. Here, we demonstrate the synthesis and application of ultrapure isotopically controlled single-crystal chemical vapour deposition (CVD) diamond with a remarkably low concentration of paramagnetic impurities. The content of nuclear spins associated with the (13)C isotope was depleted to 0.3% and the concentration of other paramagnetic defects was measured to be <10(13) cm(-3). Being placed in such a spin-free lattice, single electron spins show the longest room-temperature spin dephasing times ever observed in solid-state systems (T2=1.8 ms). This benchmark will potentially allow observation of coherent coupling between spins separated by a few tens of nanometres, making it a versatile material for room-temperature quantum information processing devices. We also show that single electron spins in the same isotopically engineered CVD diamond can be used to detect external magnetic fields with a sensitivity reaching 4 nT Hz(-1/2) and subnanometre spatial resolution.},
  Doi                      = {10.1038/nmat2420},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Keywords                 = {Carbon Isotopes
Chemical Engineering/*methods
Diamond/*chemistry
Nitrogen/chemistry
Quantum Theory},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/19349970}
}

@Article{Baranov2011,
  Title                    = {Silicon vacancy in SiC as a promising quantum system for single-defect and single-photon spectroscopy},
  Author                   = {Baranov, Pavel G. and Bundakova, Anna P. and Soltamova, Alexandra A. and Orlinskii, Sergei B. and Borovykh, Igor V. and Zondervan, Rob and Verberk, Rogier and Schmidt, Jan},
  Journal                  = {Physical Review B},
  Year                     = {2011},
  Number                   = {12},
  Volume                   = {83},

  Doi                      = {10.1103/PhysRevB.83.125203},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Baranov2008,
  Title                    = {Identification of the carbon antisite in SiC: EPR of C13 enriched crystals},
  Author                   = {Baranov, Pavel G. and Ilyin, Ivan V. and Soltamova, Alexandra A. and Mokhov, Eugene N.},
  Journal                  = {Physical Review B},
  Year                     = {2008},
  Number                   = {8},
  Pages                    = {085120},
  Volume                   = {77},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.77.085120}
}

@Article{Barclay2005,
  Title                    = {Nonlinear response of silicon photonic crystal microresonators excited via an integrated waveguide and fiber taper},
  Author                   = {Barclay, Paul and Srinivasan, Kartik and Painter, Oskar},
  Journal                  = {Optics Express},
  Year                     = {2005},
  Number                   = {3},
  Pages                    = {801-820},
  Volume                   = {13},

  Abstract                 = {A technique is demonstrated which efficiently transfers light between a tapered standard single-mode optical fiber and a high-Q, ultra-small mode volume, silicon photonic crystal resonant cavity. Cavity mode quality factors of 4.7??104 are measured, and a total fiber-to-cavity coupling efficiency of 44% is demonstrated. Using this efficient cavity input and output channel, the steady-state nonlinear absorption and dispersion of the photonic crystal cavity is studied. Optical bistability is observed for fiber input powers as low as 250 ÂµW, corresponding to a dropped power of 100 ÂµW and 3 fJ of stored cavity energy. A high-density effective free-carrier lifetime for these silicon photonic crystal resonators of ~ 0.5 ns is also estimated from power dependent loss and dispersion measurements.},
  Doi                      = {10.1364/OPEX.13.000801},
  Keywords                 = {Buffers, couplers, routers, switches, and multiplexers
Integrated optics devices
Bistability
Nonlinear optics, integrated optics},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-13-3-801}
}

@Article{Barnes2004,
  Title                    = {Surface Plasmon Polaritons and Their Role in the Enhanced Transmission of Light through Periodic Arrays of Subwavelength Holes in a Metal Film},
  Author                   = {Barnes, W. and Murray, W. and Dintinger, J. and Devaux, E. and Ebbesen, T.},
  Journal                  = {Physical Review Letters},
  Year                     = {2004},
  Number                   = {10},
  Volume                   = {92},

  Doi                      = {10.1103/PhysRevLett.92.107401},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Barnes2003,
  Title                    = {Surface plasmon subwavelength optics},
  Author                   = {Barnes, William L. and Dereux, Alain and Ebbesen, Thomas W.},
  Journal                  = {Nature},
  Year                     = {2003},
  Number                   = {6950},
  Pages                    = {824-830},
  Volume                   = {424},

  ISSN                     = {0028-0836},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nature01937}
}

@Article{Basche1992,
  Title                    = {Photon antibunching in the fluorescence of a single dye molecule trapped in a solid},
  Author                   = {Basche, Th. and Moerner, W. E. and Orrit, M. and Talon, H.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {1992},
  Pages                    = {1516--1519},
  Volume                   = {69},

  Doi                      = {10.1103/PhysRevLett.69.1516},
  Issue                    = {10},
  Numpages                 = {0},
  Owner                    = {Toan},
  Publisher                = {American Physical Society},
  Timestamp                = {2015.04.06},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.69.1516}
}

@Article{Batalov2008,
  Title                    = {Temporal Coherence of Photons Emitted by Single Nitrogen-Vacancy Defect Centers in Diamond Using Optical Rabi-Oscillations},
  Author                   = {Batalov, A. and Zierl, C. and Gaebel, T. and Neumann, P. and Chan, I. Y. and Balasubramanian, G. and Hemmer, P. R. and Jelezko, F. and Wrachtrup, J.},
  Journal                  = {Physical Review Letters},
  Year                     = {2008},
  Number                   = {7},
  Volume                   = {100},

  Doi                      = {10.1103/PhysRevLett.100.077401},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Batson2012,
  Title                    = {Plasmonic Modes Revealed},
  Author                   = {Batson, Philip E.},
  Journal                  = {Science},
  Year                     = {2012},
  Number                   = {6064},
  Pages                    = {47-48},
  Volume                   = {335},

  Doi                      = {10.1126/science.1215588},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000298846200044}
}

@Article{Belacel2013,
  Title                    = {Controlling spontaneous emission with plasmonic optical patch antennas},
  Author                   = {Belacel, C. and Habert, B. and Bigourdan, F. and Marquier, F. and Hugonin, J. P. and de Vasconcellos, S. M. and Lafosse, X. and Coolen, L. and Schwob, C. and Javaux, C. and Dubertret, B. and Greffet, J. J. and Senellart, P. and Maitre, A.},
  Journal                  = {Nano Lett},
  Year                     = {2013},
  Number                   = {4},
  Pages                    = {1516-21},
  Volume                   = {13},

  Abstract                 = {We experimentally demonstrate the control of the spontaneous emission rate and the radiation pattern of colloidal quantum dots deterministically positioned in a plasmonic patch antenna. The antenna consists of a thin gold microdisk separated from a planar gold layer by a few tens of nanometers thick dielectric layer. The emitters are shown to radiate through the entire patch antenna in a highly directional and vertical radiation pattern. Strong acceleration of spontaneous emission is observed, depending on the antenna geometry. Considering the double dipole structure of the emitters, this corresponds to a Purcell factor up to 80 for dipoles perpendicular to the disk.},
  Doi                      = {10.1021/nl3046602},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Colloids/*chemistry
Equipment Design
Gold/*chemistry
Light
Nanostructures/chemistry
Nanotechnology
Optics and Photonics
*Quantum Dots
Surface Plasmon Resonance},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23461679}
}

@Article{Belford1972,
  Title                    = {Dynamics of Fluorescence Polarization in Macromolecules},
  Author                   = {Belford, G. G. and Belford, R. L. and Weber, G.},
  Journal                  = {Proceedings of the National Academy of Sciences},
  Year                     = {1972},
  Number                   = {6},
  Pages                    = {1392-1393},
  Volume                   = {69},

  Abstract                 = {Reexamination of the theory of fluorescence time dependence owing to rotational diffusion of rigid macromolecules reveals deficiencies or hidden restrictions in each of the previous treatments. The correct master equation has five exponential decay terms, with preexponential factors that depend upon the diffusion constants and, in a completely symmetrical fashion, upon the orientations of absorbing and emitting dipoles.},
  Owner                    = {Toan},
  Timestamp                = {2015.04.10},
  Url                      = {http://www.pnas.org/content/69/6/1392.abstract}
}

@Article{Benson2011,
  Title                    = {Assembly of hybrid photonic architectures from nanophotonic constituents},
  Author                   = {Benson, O.},
  Journal                  = {Nature},
  Year                     = {2011},
  Number                   = {7376},
  Pages                    = {193-9},
  Volume                   = {480},

  Abstract                 = {The assembly of hybrid nanophotonic devices from different fundamental photonic entities--such as single molecules, nanocrystals, semiconductor quantum dots, nanowires and metal nanoparticles--can yield functionalities that exceed those of the individual subunits. Combining these photonic elements requires nanometre-scale fabrication precision and potentially involves a material diversity that is incompatible with standard nanotechnological processes. Although merging these different systems on a single hybrid platform is at present challenging, it promises improved performance and novel devices. Particularly rapid progress is seen in the combination of plasmonic-dielectric constituents with quantum emitters that can be assembled on demand into fundamental model systems for future optical elements.},
  Doi                      = {10.1038/nature10610},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Keywords                 = {Nanostructures/chemistry
Nanotechnology/*instrumentation
Optics and Photonics/*instrumentation/*methods
Photons},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22158243}
}

@Article{Bera2010,
  Title                    = {Quantum Dots and Their Multimodal Applications: A Review},
  Author                   = {Bera, Debasis and Qian, Lei and Tseng, Teng-Kuan and Holloway, Paul H.},
  Journal                  = {Materials},
  Year                     = {2010},
  Number                   = {4},
  Pages                    = {2260-2345},
  Volume                   = {3},

  Doi                      = {10.3390/ma3042260},
  ISSN                     = {1996-1944},
  Type                     = {Journal Article}
}

@Article{Bernard1993,
  Title                    = {Photon bunching in the fluorescence from single molecules: A probe for intersystem crossing},
  Author                   = {Bernard, J. and Fleury, L. and Talon, H. and Orrit, M.},
  Journal                  = {The Journal of Chemical Physics},
  Year                     = {1993},
  Number                   = {2},
  Pages                    = {850-859},
  Volume                   = {98},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.464249},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/jcp/98/2/10.1063/1.464249}
}

@Article{Bernard2014,
  Title                    = {Nanostructured and architectured boron nitride from boron, nitrogen and hydrogen-containing molecular and polymeric precursors},
  Author                   = {Bernard, S. and Miele, P.},
  Journal                  = {Materials Today},
  Year                     = {2014},
  Number                   = {9},
  Pages                    = {443-450},
  Volume                   = {17},

  Doi                      = {10.1016/j.mattod.2014.07.006},
  ISSN                     = {13697021},
  Type                     = {Journal Article}
}

@Article{Berthel2015,
  Title                    = {Photophysics of single nitrogen-vacancy centers in diamond nanocrystals},
  Author                   = {Berthel, Martin and Mollet, Oriane and Dantelle, GÃ©raldine and Gacoin, Thierry and Huant, Serge and Drezet, AurÃ©lien},
  Journal                  = {Physical Review B},
  Year                     = {2015},
  Number                   = {3},
  Pages                    = {035308},
  Volume                   = {91},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.91.035308}
}

@Article{Betzig1993,
  Title                    = {Single Molecules Observed by Near-Field Scanning Optical Microscopy},
  Author                   = {Betzig, Eric and Chichester, Robert J.},
  Journal                  = {Science},
  Year                     = {1993},
  Number                   = {5138},
  Pages                    = {1422-1425},
  Volume                   = {262},

  Abstract                 = {Individual carbocyanine dye molecules in a sub-monolayer spread have been imaged with near-field scanning optical microscopy. Molecules can be repeatedly detected and spatially localized (to âˆ¼Î»/50 where Î» is the wavelength of light) with a sensitivity of at least 0.005 molecules/(Hz)1/2 and the orientation of each molecular dipole can be determined. This information is exploited to map the electric field distribution in the near-field aperture with molecular spatial resolution.},
  Doi                      = {10.1126/science.262.5138.1422},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/262/5138/1422.abstract}
}

@Article{Beveratos2001,
  Title                    = {Nonclassical radiation from diamond nanocrystals},
  Author                   = {Beveratos, Alexios and Brouri, Rosa and Gacoin, Thierry and Poizat, Jean-Philippe and Grangier, Philippe},
  Journal                  = {Physical Review A},
  Year                     = {2001},
  Number                   = {6},
  Pages                    = {061802},
  Volume                   = {64},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevA.64.061802}
}

@Article{Beveratos2002,
  Title                    = {Room temperature stable single-photon source},
  Author                   = {Beveratos, A. and x000Fc and hn, S. and Brouri, R. and Gacoin, T. and Poizat, J. P. and Grangier, P.},
  Journal                  = {The European Physical Journal D - Atomic, Molecular and Optical Physics},
  Year                     = {2002},
  Number                   = {2},
  Pages                    = {191-196},
  Volume                   = {18},

  Doi                      = {10.1140/epjd/e20020023},
  ISSN                     = {1434-6060
1434-6079},
  Type                     = {Journal Article}
}

@Article{Blanco2000,
  Title                    = {Large-scale synthesis of a silicon photonic crystal with a complete three-dimensional bandgap near 1.5 micrometres},
  Author                   = {Blanco, Alvaro and Chomski, Emmanuel and Grabtchak, Serguei and Ibisate, Marta and John, Sajeev and Leonard, Stephen W. and Lopez, Cefe and Meseguer, Francisco and Miguez, Hernan and Mondia, Jessica P. and Ozin, Geoffrey A. and Toader, Ovidiu and van Driel, Henry M.},
  Journal                  = {Nature},
  Year                     = {2000},
  Number                   = {6785},
  Pages                    = {437-440},
  Volume                   = {405},

  ISSN                     = {0028-0836},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/35013024}
}

@Article{Boltasseva2011,
  Title                    = {Low-Loss Plasmonic Metamaterials},
  Author                   = {Boltasseva, Alexandra and Atwater, Harry A.},
  Journal                  = {Science},
  Year                     = {2011},
  Number                   = {6015},
  Pages                    = {290-291},
  Volume                   = {331},

  Doi                      = {10.1126/science.1198258},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000286636300023}
}

@Article{Bose2003,
  Title                    = {Quantum Communication through an Unmodulated Spin Chain},
  Author                   = {Bose, Sougato},
  Journal                  = {Physical Review Letters},
  Year                     = {2003},
  Number                   = {20},
  Volume                   = {91},

  Doi                      = {10.1103/PhysRevLett.91.207901},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Bourrellier2014,
  Title                    = {Nanometric Resolved Luminescence in h-BN Flakes: Excitons and Stacking Order},
  Author                   = {Bourrellier, Romain and Amato, Michele and GalvÃ£o Tizei, Luiz Henrique and Giorgetti, Christine and Gloter, Alexandre and Heggie, Malcolm I. and March, Katia and StÃ©phan, Odile and Reining, Lucia and Kociak, Mathieu and Zobelli, Alberto},
  Journal                  = {ACS Photonics},
  Year                     = {2014},
  Number                   = {9},
  Pages                    = {857-862},
  Volume                   = {1},

  Abstract                 = {The strong excitonic emission of hexagonal boron nitride (h-BN) makes this material one of the most promising candidate for light emitting devices in the far ultraviolet (UV). However, single excitons occur only in perfect monocrystals that are extremely hard to synthesize, while regular h-BN samples present a complex emission spectrum with several additional peaks. The microscopic origin of these additional emissions has not yet been understood. In this work we address this problem using an experimental and theoretical approach that combines nanometric resolved cathodoluminescence, high resolution transmission electron microscopy and state of the art theoretical spectroscopy methods. We demonstrate that emission spectra are strongly inhomogeneus within individual few layer flakes and that additional excitons occur at structural deformations, such as faceted plane folds, that lead to local changes of the h-BN layers stacking order.},
  Doi                      = {10.1021/ph500141j},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/ph500141j}
}

@Article{Bozhevolnyi2006,
  Title                    = {Channel plasmon subwavelength waveguide components including interferometers and ring resonators},
  Author                   = {Bozhevolnyi, S. I. and Volkov, V. S. and Devaux, E. and Laluet, J. Y. and Ebbesen, T. W.},
  Journal                  = {Nature},
  Year                     = {2006},
  Number                   = {7083},
  Pages                    = {508-11},
  Volume                   = {440},

  Abstract                 = {Photonic components are superior to electronic ones in terms of operational bandwidth, but the diffraction limit of light poses a significant challenge to the miniaturization and high-density integration of optical circuits. The main approach to circumvent this problem is to exploit the hybrid nature of surface plasmon polaritons (SPPs), which are light waves coupled to free electron oscillations in a metal that can be laterally confined below the diffraction limit using subwavelength metal structures. However, the simultaneous realization of strong confinement and a propagation loss sufficiently low for practical applications has long been out of reach. Channel SPP modes--channel plasmon polaritons (CPPs)--are electromagnetic waves that are bound to and propagate along the bottom of V-shaped grooves milled in a metal film. They are expected to exhibit useful subwavelength confinement, relatively low propagation loss, single-mode operation and efficient transmission around sharp bends. Our previous experiments showed that CPPs do exist and that they propagate over tens of micrometres along straight subwavelength grooves. Here we report the design, fabrication and characterization of CPP-based subwavelength waveguide components operating at telecom wavelengths: Y-splitters, Mach-Zehnder interferometers and waveguide-ring resonators. We demonstrate that CPP guides can indeed be used for large-angle bending and splitting of radiation, thereby enabling the realization of ultracompact plasmonic components and paving the way for a new class of integrated optical circuits.},
  Doi                      = {10.1038/nature04594},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/16554814}
}

@Article{Bradac2010,
  Title                    = {Observation and control of blinking nitrogen-vacancy centres in discrete nanodiamonds},
  Author                   = {Bradac, C. and Gaebel, T. and Naidoo, N. and Sellars, M. J. and Twamley, J. and Brown, L. J. and Barnard, A. S. and Plakhotnik, T. and Zvyagin, A. V. and Rabeau, J. R.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2010},
  Number                   = {5},
  Pages                    = {345-9},
  Volume                   = {5},

  Abstract                 = {Nitrogen-vacancy colour centres in diamond can undergo strong, spin-sensitive optical transitions under ambient conditions, which makes them attractive for applications in quantum optics, nanoscale magnetometry and biolabelling. Although nitrogen-vacancy centres have been observed in aggregated detonation nanodiamonds and milled nanodiamonds, they have not been observed in very small isolated nanodiamonds. Here, we report the first direct observation of nitrogen-vacancy centres in discrete 5-nm nanodiamonds at room temperature, including evidence for intermittency in the luminescence (blinking) from the nanodiamonds. We also show that it is possible to control this blinking by modifying the surface of the nanodiamonds.},
  Doi                      = {10.1038/nnano.2010.56},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20383128}
}

@Article{Bray2015,
  Title                    = {Enhanced photoluminescence from single nitrogen-vacancy defects in nanodiamonds coated with phenol-ionic complexes},
  Author                   = {Bray, K. and Previdi, R. and Gibson, B. C. and Shimoni, O. and Aharonovich, I.},
  Journal                  = {Nanoscale},
  Year                     = {2015},

  Abstract                 = {Fluorescent nanodiamonds are attracting major attention in the field of bio-sensing and bio-labeling. In this work we demonstrate a robust approach to achieve an encapsulation of individual nanodiamonds with phenol-ionic complexes that enhance the photoluminescence from single nitrogen vacancy (NV) centers. We show that single NV centres in the coated nanodiamonds also exhibit shorter lifetimes, opening another channel for high resolution sensing. We propose that the nanodiamond encapsulation reduces the non-radiative decay pathways of the NV color centers. Our results provide a versatile and assessable way to enhance photoluminescence from nanodiamond defects that can be used in a variety of sensing and imaging applications.},
  Doi                      = {10.1039/c4nr07510b},
  ISSN                     = {2040-3372 (Electronic)
2040-3364 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25655482}
}

@Article{Brenneis2014,
  Title                    = {Ultrafast electronic readout of diamond nitrogen-vacancy centres coupled to graphene},
  Author                   = {Brenneis, A. and Gaudreau, L. and Seifert, M. and Karl, H. and Brandt, M. S. and Huebl, H. and Garrido, J. A. and Koppens, F. H. and Holleitner, A. W.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2014},

  Abstract                 = {Non-radiative transfer processes are often regarded as loss channels for an optical emitter because they are inherently difficult to access experimentally. Recently, it has been shown that emitters, such as fluorophores and nitrogen-vacancy centres in diamond, can exhibit a strong non-radiative energy transfer to graphene. So far, the energy of the transferred electronic excitations has been considered to be lost within the electron bath of the graphene. Here we demonstrate that the transferred excitations can be read out by detecting corresponding currents with a picosecond time resolution. We detect electronically the spin of nitrogen-vacancy centres in diamond and control the non-radiative transfer to graphene by electron spin resonance. Our results open the avenue for incorporating nitrogen-vacancy centres into ultrafast electronic circuits and for harvesting non-radiative transfer processes electronically.},
  Doi                      = {10.1038/nnano.2014.276},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25437746}
}

@Article{Brolo2012,
  Title                    = {Plasmonics for future biosensors},
  Author                   = {Brolo, Alexandre G.},
  Journal                  = {Nature Photonics},
  Year                     = {2012},
  Number                   = {11},
  Pages                    = {709-713},
  Volume                   = {6},

  Doi                      = {10.1038/nphoton.2012.266},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Brouri2000,
  Title                    = {Photon antibunching in the fluorescence of individual color centers in diamond},
  Author                   = {Brouri, Rosa and Beveratos, Alexios and Poizat, Jean-Philippe and Grangier, Philippe},
  Journal                  = {Opt. Lett.},
  Year                     = {2000},
  Number                   = {17},
  Pages                    = {1294-1296},
  Volume                   = {25},

  Abstract                 = {We observed photon antibunching in the fluorescent light emitted from a single nitrogen-vacancy center in diamond at room temperature. The possibility of generating triggerable single photons with such a solid-state system is discussed.},
  Booktitle                = {Optics Letters},
  Keywords                 = {Photon counting, Confocal microscopy, Photon statistics},
  Owner                    = {Toan},
  Publisher                = {OSA},
  Timestamp                = {2015.04.10},
  Url                      = {http://ol.osa.org/abstract.cfm?URI=ol-25-17-1294}
}

@Article{Bulu2011,
  Title                    = {Plasmonic resonators for enhanced diamond NV- center single photon sources},
  Author                   = {Bulu, Irfan and Babinec, Thomas and Hausmann, Birgit and Choy, Jennifer T. and Loncar, Marko},
  Journal                  = {Optics Express},
  Year                     = {2011},
  Number                   = {6},
  Pages                    = {5268-5276},
  Volume                   = {19},

  Abstract                 = {We propose a novel source of non-classical light consisting of plasmonic aperture with single-crystal diamond containing a single Nitrogen-Vacancy (NV) color center. Theoretical calculations of optimal structures show that these devices can simultaneously enhance optical pumping by a factor of 7, spontaneous emission rates by Fp ~50 (Purcell factor), and offer collection efficiencies up to 40%. These excitation and collection enhancements occur over a broad range of wavelengths (~30nm), and are independently tunable with device geometry, across the excitation (~530nm) and emission (~600-800nm) spectrum of the NV center. Implementing this system with top-down techniques in bulk diamond crystals will provide a scalable architecture for a myriad of diamond NV center applications.},
  Doi                      = {10.1364/OE.19.005268},
  Keywords                 = {Surface plasmons
Quantum optics},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-19-6-5268}
}

@Article{Butun2015,
  Title                    = {Enhanced Light Emission from Large-Area Monolayer MoS Using Plasmonic Nanodisc Arrays},
  Author                   = {Butun, S. and Tongay, S. and Aydin, K.},
  Journal                  = {Nano Lett},
  Year                     = {2015},

  Abstract                 = {Single-layer direct band gap semiconductors such as transition metal dichalcogenides are quite attractive for a wide range of electronics, photonics, and optoelectronics applications. Their monolayer thickness provides significant advantages in many applications such as field-effect transistors for high-performance electronics, sensor/detector applications, and flexible electronics. However, for optoelectronics and photonics applications, inherent monolayer thickness poses a significant challenge for the interaction of light with the material, which therefore results in poor light emission and absorption behavior. Here, we demonstrate enhanced light emission from large-area monolayer MoS2 using plasmonic silver nanodisc arrays, where enhanced photoluminescence up to 12-times has been measured. Observed phenomena stem from the fact that plasmonic resonance couples to both excitation and emission fields and thus boosts the light-matter interaction at the nanoscale. Reported results allow us to engineer light-matter interactions in two-dimensional materials and could enable highly efficient photodetectors, sensors, and photovoltaic devices, where photon absorption and emission efficiency highly dictate the device performance.},
  Doi                      = {10.1021/acs.nanolett.5b00407},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25729895}
}

@Article{Cacciola2014,
  Title                    = {Ultrastrong Coupling of Plasmons and Excitons in a Nanoshell},
  Author                   = {Cacciola, Adriano and Di Stefano, Omar and Stassi, Roberto and Saija, Rosalba and Savasta, Salvatore},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {11483-11492},
  Volume                   = {8},

  Doi                      = {10.1021/nn504652w},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn504652w}
}

@Article{Cai2011,
  Title                    = {Electrically Controlled Nonlinear Generation of Light with Plasmonics},
  Author                   = {Cai, Wenshan and Vasudev, Alok P. and Brongersma, Mark L.},
  Journal                  = {Science},
  Year                     = {2011},
  Number                   = {6050},
  Pages                    = {1720-1723},
  Volume                   = {333},

  Abstract                 = {Plasmonics provides a route to develop ultracompact optical devices on a chip by using extreme light concentration and the ability to perform simultaneous electrical and optical functions. These properties also make plasmonics an ideal candidate for dynamically controlling nonlinear optical interactions at the nanoscale. We demonstrate electrically tunable harmonic generation of light from a plasmonic nanocavity filled with a nonlinear medium. The metals that define the cavity also serve as electrodes that can generate high direct current electric fields across the nonlinear material. A fundamental wave at 1.56 micrometers was frequency doubled and modulated in intensity by applying a moderate external voltage to the electrodes, yielding a voltage-dependent nonlinear generation with a normalized magnitude of similar to 7% per volt.},
  Doi                      = {10.1126/science.1207858},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000295121500034}
}

@Article{Caldwell2014,
  Title                    = {Sub-diffractional volume-confined polaritons in the natural hyperbolic material hexagonal boron nitride},
  Author                   = {Caldwell, Joshua D. and Kretinin, Andrey V. and Chen, Yiguo and Giannini, Vincenzo and Fogler, Michael M. and Francescato, Yan and Ellis, Chase T. and Tischler, Joseph G. and Woods, Colin R. and Giles, Alexander J. and Hong, Minghui and Watanabe, Kenji and Taniguchi, Takashi and Maier, Stefan A. and Novoselov, Kostya S.},
  Journal                  = {Nat. Commun.},
  Year                     = {2014},

  Month                    = oct,
  Pages                    = {--},
  Volume                   = {5},

  Abstract                 = {Strongly anisotropic media, where the principal components of the dielectric tensor have opposite signs, are called hyperbolic. Such materials exhibit unique nanophotonic properties enabled by the highly directional propagation of slow-light modes localized at deeply sub-diffractional length scales. While artificial hyperbolic metamaterials have been demonstrated, they suffer from high plasmonic losses and require complex nanofabrication, which in turn induces size-dependent limitations on optical confinement. The low-loss, mid-infrared, natural hyperbolic material hexagonal boron nitride is an attractive alternative. Here we report on three-dimensionally confined â€˜hyperbolic polaritonsâ€™ in boron nitride nanocones that support four series (up to the seventh order) modes in two spectral bands. The resonant modes obey the predicted aspect ratio dependence and exhibit high-quality factors (Q up to 283) in the strong confinement regime (up to Î»/86). These observations assert hexagonal boron nitride as a promising platform for studying novel regimes of lightâ€“matter interactions and nanophotonic device engineering.},
  Comment                  = {Supplementary information available for this article at http://www.nature.com/ncomms/2014/141017/ncomms6221/suppinfo/ncomms6221_S1.html},
  Owner                    = {Toan},
  Timestamp                = {2015.04.09},
  Url                      = {http://dx.doi.org/10.1038/ncomms6221}
}

@Article{Cang2011,
  Title                    = {Probing the electromagnetic field of a 15-nanometre hotspot by single molecule imaging},
  Author                   = {Cang, H. and Labno, A. and Lu, C. and Yin, X. and Liu, M. and Gladden, C. and Liu, Y. and Zhang, X.},
  Journal                  = {Nature},
  Year                     = {2011},
  Number                   = {7330},
  Pages                    = {385-8},
  Volume                   = {469},

  Abstract                 = {When light illuminates a rough metallic surface, hotspots can appear, where the light is concentrated on the nanometre scale, producing an intense electromagnetic field. This phenomenon, called the surface enhancement effect, has a broad range of potential applications, such as the detection of weak chemical signals. Hotspots are believed to be associated with localized electromagnetic modes, caused by the randomness of the surface texture. Probing the electromagnetic field of the hotspots would offer much insight towards uncovering the mechanism generating the enhancement; however, it requires a spatial resolution of 1-2 nm, which has been a long-standing challenge in optics. The resolution of an optical microscope is limited to about half the wavelength of the incident light, approximately 200-300 nm. Although current state-of-the-art techniques, including near-field scanning optical microscopy, electron energy-loss spectroscopy, cathode luminescence imaging and two-photon photoemission imaging have subwavelength resolution, they either introduce a non-negligible amount of perturbation, complicating interpretation of the data, or operate only in a vacuum. As a result, after more than 30 years since the discovery of the surface enhancement effect, how the local field is distributed remains unknown. Here we present a technique that uses Brownian motion of single molecules to probe the local field. It enables two-dimensional imaging of the fluorescence enhancement profile of single hotspots on the surfaces of aluminium thin films and silver nanoparticle clusters, with accuracy down to 1.2 nm. Strong fluorescence enhancements, up to 54 and 136 times respectively, are observed in those two systems. This strong enhancement indicates that the local field, which decays exponentially from the peak of a hotspot, dominates the fluorescence enhancement profile.},
  Doi                      = {10.1038/nature09698},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Keywords                 = {Aluminum/chemistry
*Electromagnetic Fields
Fluorescence
Fluorescent Dyes/analysis/chemistry
*Hot Temperature
Luminescent Measurements/*methods
Metal Nanoparticles/*chemistry
Microscopy, Fluorescence/*methods
Molecular Imaging/*methods
Motion
Quartz
Silver/chemistry
Surface Properties},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/21248848}
}

@Article{Cao2002,
  Title                    = {Negative Role of Surface Plasmons in the Transmission of Metallic Gratings with Very Narrow Slits},
  Author                   = {Cao, Qing and Lalanne, Philippe},
  Journal                  = {Physical Review Letters},
  Year                     = {2002},
  Number                   = {5},
  Volume                   = {88},

  Doi                      = {10.1103/PhysRevLett.88.057403},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Carbonera2009,
  Title                    = {Optically Detected Magnetic Resonance (ODMR) of photoexcited triplet states},
  Author                   = {Carbonera, D.},
  Journal                  = {Photosynth Res},
  Year                     = {2009},
  Number                   = {2-3},
  Pages                    = {403-14},
  Volume                   = {102},

  Abstract                 = {Optically Detected Magnetic Resonance (ODMR) is a double resonance technique which combines optical measurements (fluorescence, phosphorescence, absorption) with electron spin resonance spectroscopy. After the first triplet-state ODMR experiments in zero magnetic field reported in 1968 by Schmidt and van der Waals, the number of double resonance studies on excited triplet states grew rapidly. Photosynthesis has proven to be a fruitful field of application due to the intrinsic possibility of forming photo-induced pigment triplet states in many sites of the photosynthetic apparatus. The basic principles of this technique are described and examples of application in Photosynthesis are reported.},
  Doi                      = {10.1007/s11120-009-9407-5},
  ISSN                     = {1573-5079 (Electronic)
0166-8595 (Linking)},
  Keywords                 = {Chlorophyll/metabolism
*Light
Magnetic Resonance Spectroscopy/instrumentation/*methods
Molecular Conformation/*radiation effects
Photosynthesis/radiation effects
Plant Proteins/metabolism
Thylakoids/metabolism/radiation effects},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/19238576}
}

@Article{Castelletto2014,
  Title                    = {Quantum-confined single photon emission at room temperature from SiC tetrapods},
  Author                   = {Castelletto, S. and Bodrog, Z. and Magyar, A. P. and Gentle, A. and Gali, A. and Aharonovich, I.},
  Journal                  = {Nanoscale},
  Year                     = {2014},
  Number                   = {17},
  Pages                    = {10027-32},
  Volume                   = {6},

  Abstract                 = {Controlled engineering of isolated solid state quantum systems is one of the most prominent goals in modern nanotechnology. In this letter we demonstrate a previously unknown quantum system namely silicon carbide tetrapods. The tetrapods have a cubic polytype core (3C) and hexagonal polytype legs (4H)--a geometry that creates spontaneous polarization within a single tetrapod. Modeling of the tetrapod structures predicts that a bound exciton should exist at the 3C-4H interface. The simulations are confirmed by the observation of fully polarized and narrowband single photon emission from the tetrapods at room temperature. The single photon emission provides important insights into understanding the quantum confinement effects in non-spherical nanostructures. Our results pave the way to a new class of crystal phase nanomaterials that exhibit single photon emission at room temperature and therefore are suitable for sensing, quantum information and nanophotonics.},
  Doi                      = {10.1039/c4nr02307b},
  ISSN                     = {2040-3372 (Electronic)
2040-3364 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25031102}
}

@Article{Castelletto2013,
  Title                    = {Quantum Effects in Silicon Carbide Hold Promise for Novel Integrated Devices and Sensors},
  Author                   = {Castelletto, Stefania and Johnson, Brett C. and Boretti, Alberto},
  Journal                  = {Advanced Optical Materials},
  Year                     = {2013},
  Number                   = {9},
  Pages                    = {609-625},
  Volume                   = {1},

  Doi                      = {10.1002/adom.201300246},
  ISSN                     = {21951071},
  Type                     = {Journal Article}
}

@Article{Castelletto2014a,
  Title                    = {A silicon carbide room-temperature single-photon source},
  Author                   = {Castelletto, S. and Johnson, B. C. and IvÃ¡dy, V. and Stavrias, N. and Umeda, T. and Gali, A. and Ohshima, T.},
  Journal                  = {Nat Mater},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {151-156},
  Volume                   = {13},

  Doi                      = {10.1038/nmat3806
http://www.nature.com/nmat/journal/v13/n2/abs/nmat3806.html},
  ISSN                     = {1476-1122},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nmat3806}
}

@Article{Castelletto2014b,
  Title                    = {Room Temperature Quantum Emission from Cubic Silicon Carbide Nanoparticles},
  Author                   = {Castelletto, Stefania and Johnson, Brett C. and Zachreson, Cameron and Beke, David and Balogh, IstvÃ¡n and Ohshima, Takeshi and Aharonovich, Igor and Gali, Adam},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {8},
  Pages                    = {7938-7947},
  Volume                   = {8},

  Abstract                 = {The photoluminescence (PL) arising from silicon carbide nanoparticles has so far been associated with the quantum confinement effect or to radiative transitions between electronically active surface states. In this work we show that cubic phase silicon carbide nanoparticles with diameters in the range 45?500 nm can host other point defects responsible for photoinduced intrabandgap PL. We demonstrate that these nanoparticles exhibit single photon emission at room temperature with record saturation count rates of 7 ? 106 counts/s. The realization of nonclassical emission from SiC nanoparticles extends their potential use from fluorescence biomarker beads to optically active quantum elements for next generation quantum sensing and nanophotonics. The single photon emission is related to single isolated SiC defects that give rise to states within the bandgap.},
  Doi                      = {10.1021/nn502719y},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn502719y}
}

@Article{Chan1998,
  Title                    = {Quantum Dot Bioconjugates for Ultrasensitive Nonisotopic Detection},
  Author                   = {Chan, W. C.},
  Journal                  = {Science},
  Year                     = {1998},
  Number                   = {5385},
  Pages                    = {2016-2018},
  Volume                   = {281},

  Doi                      = {10.1126/science.281.5385.2016},
  Type                     = {Journal Article}
}

@Article{Chang2007,
  Title                    = {Strong coupling of single emitters to surface plasmons},
  Author                   = {Chang, D. and SÃ¸rensen, A. and Hemmer, P. and Lukin, M.},
  Journal                  = {Physical Review B},
  Year                     = {2007},
  Number                   = {3},
  Volume                   = {76},

  Doi                      = {10.1103/PhysRevB.76.035420},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Chang2006,
  Title                    = {Quantum Optics with Surface Plasmons},
  Author                   = {Chang, D. and SÃ¸rensen, A. and Hemmer, P. and Lukin, M.},
  Journal                  = {Physical Review Letters},
  Year                     = {2006},
  Number                   = {5},
  Volume                   = {97},

  Doi                      = {10.1103/PhysRevLett.97.053002},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Chang2007a,
  Title                    = {A single-photon transistor using nanoscale surface plasmons},
  Author                   = {Chang, Darrick E. and SÃ¸rensen, Anders S. and Demler, Eugene A. and Lukin, Mikhail D.},
  Journal                  = {Nature Physics},
  Year                     = {2007},
  Number                   = {11},
  Pages                    = {807-812},
  Volume                   = {3},

  Doi                      = {10.1038/nphys708},
  ISSN                     = {1745-2473
1745-2481},
  Type                     = {Journal Article}
}

@Article{Chang2008,
  Title                    = {Mass production and dynamic imaging of fluorescent nanodiamonds},
  Author                   = {Chang, Y. R. and Lee, H. Y. and Chen, K. and Chang, C. C. and Tsai, D. S. and Fu, C. C. and Lim, T. S. and Tzeng, Y. K. and Fang, C. Y. and Han, C. C. and Chang, H. C. and Fann, W.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2008},
  Number                   = {5},
  Pages                    = {284-8},
  Volume                   = {3},

  Abstract                 = {Fluorescent nanodiamond is a new nanomaterial that possesses several useful properties, including good biocompatibility, excellent photostability and facile surface functionalizability. Moreover, when excited by a laser, defect centres within the nanodiamond emit photons that are capable of penetrating tissue, making them well suited for biological imaging applications. Here, we show that bright fluorescent nanodiamonds can be produced in large quantities by irradiating synthetic diamond nanocrystallites with helium ions. The fluorescence is sufficiently bright and stable to allow three-dimensional tracking of a single particle within the cell by means of either one- or two-photon-excited fluorescence microscopy. The excellent photophysical characteristics are maintained for particles as small as 25 nm, suggesting that fluorescent nanodiamond is an ideal probe for long-term tracking and imaging in vivo, with good temporal and spatial resolution.},
  Doi                      = {10.1038/nnano.2008.99},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {Contrast Media/*chemistry
Crystallization/*methods
Diamond/*chemistry/*diagnostic use
HeLa Cells
Humans
Image Enhancement/*methods
Materials Testing
Microscopy, Fluorescence/*methods
Nanoparticles/*chemistry/*diagnostic use},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/18654525}
}

@Article{Chen2014,
  Title                    = {Spectral Tuning of Localized Surface Phonon Polariton Resonators for Low-Loss Mid-IR Applications},
  Author                   = {Chen, Yiguo and Francescato, Yan and Caldwell, Joshua D. and Giannini, Vincenzo and MaÃŸ, Tobias W. W. and Glembocki, Orest J. and Bezares, Francisco J. and Taubner, Thomas and Kasica, Richard and Hong, Minghui and Maier, Stefan A.},
  Journal                  = {ACS Photonics},
  Year                     = {2014},
  Number                   = {8},
  Pages                    = {718-724},
  Volume                   = {1},

  Doi                      = {10.1021/ph500143u},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/ph500143u}
}

@Article{Chen2010,
  Title                    = {Finite-element modeling of spontaneous emission of a quantum emitter at nanoscale proximity to plasmonic waveguides},
  Author                   = {Chen, Yuntian and Nielsen, Torben Roland and Gregersen, Niels and Lodahl, Peter and MÃ¸rk, Jesper},
  Journal                  = {Physical Review B},
  Year                     = {2010},
  Number                   = {12},
  Volume                   = {81},

  Doi                      = {10.1103/PhysRevB.81.125431},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Childress2013,
  Title                    = {Diamond NV centers for quantum computing and quantum networks},
  Author                   = {Childress, Lilian and Hanson, Ronald},
  Journal                  = {MRS Bulletin},
  Year                     = {2013},
  Number                   = {02},
  Pages                    = {134-138},
  Volume                   = {38},

  Keywords                 = {Diamond, optical, spintronic, optical properties},
  Type                     = {Journal Article}
}

@Article{Childress2006,
  Title                    = {Fault-Tolerant Quantum Communication Based on Solid-State Photon Emitters},
  Author                   = {Childress, L. and Taylor, J. and SÃ¸rensen, A. and Lukin, M.},
  Journal                  = {Physical Review Letters},
  Year                     = {2006},
  Number                   = {7},
  Volume                   = {96},

  Doi                      = {10.1103/PhysRevLett.96.070504},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Cho2013,
  Title                    = {Silicon coupled with plasmon nanocavity generates bright visible hot-luminescence},
  Author                   = {Cho, C. H. and Aspetti, C. O. and Park, J. and Agarwal, R.},
  Journal                  = {Nat Photonics},
  Year                     = {2013},
  Pages                    = {285-289},
  Volume                   = {7},

  Abstract                 = {Due to limitations in device speed and performance of silicon-based electronics, silicon optoelectronics has been extensively studied to achieve ultrafast optical-data processing1-3. However, the biggest challenge has been to develop an efficient silicon-based light source since indirect band-gap of silicon gives rise to extremely low emission efficiency. Although light emission in quantum-confined silicon at sub-10 nm lengthscales has been demonstrated4-7, there are difficulties in integrating quantum structures with conventional electronics8,9. It is desirable to develop new concepts to obtain emission from silicon at lengthscales compatible with current electronic devices (20-100 nm), which therefore do not utilize quantum-confinement effects. Here, we demonstrate an entirely new method to achieve bright visible light emission in "bulk-sized" silicon coupled with plasmon nanocavities from non-thermalized carrier recombination. Highly enhanced emission quantum efficiency (>1%) in plasmonic silicon, along with its size compatibility with present silicon electronics, provides new avenues for developing monolithically integrated light-sources on conventional microchips.},
  Doi                      = {10.1038/nphoton.2013.25},
  ISSN                     = {1749-4885 (Print)
1749-4885 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23710256}
}

@Article{Cho2011,
  Title                    = {Tailoring hot-exciton emission and lifetimes in semiconducting nanowires via whispering-gallery nanocavity plasmons},
  Author                   = {Cho, C. H. and Aspetti, C. O. and Turk, M. E. and Kikkawa, J. M. and Nam, S. W. and Agarwal, R.},
  Journal                  = {Nat Mater},
  Year                     = {2011},
  Number                   = {9},
  Pages                    = {669-75},
  Volume                   = {10},

  Abstract                 = {The manipulation of radiative properties of light emitters coupled with surface plasmons is important for engineering new nanoscale optoelectronic devices, including lasers, detectors and single photon emitters. However, so far the radiative rates of excited states in semiconductors and molecular systems have been enhanced only moderately, typically by a factor of 10-50, producing emission mostly from thermalized excitons. Here, we show the generation of dominant hot-exciton emission, that is, luminescence from non-thermalized excitons that are enhanced by the highly concentrated electromagnetic fields supported by the resonant whispering-gallery plasmonic nanocavities of CdS-SiO(2)-Ag core-shell nanowire devices. By tuning the plasmonic cavity size to match the whispering-gallery resonances, an almost complete transition from thermalized exciton to hot-exciton emission can be achieved, which reflects exceptionally high radiative rate enhancement of >10(3) and sub-picosecond lifetimes. Core-shell plasmonic nanowires are an ideal test bed for studying and controlling strong plasmon-exciton interaction at the nanoscale and opens new avenues for applications in ultrafast nanophotonic devices.},
  Doi                      = {10.1038/nmat3067},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Keywords                 = {Cadmium Compounds/chemistry
Electric Impedance
Light
Nanotechnology/*methods
*Nanowires
*Optical Processes
*Semiconductors
Silicon Dioxide/chemistry
Silver/chemistry
Sulfates/chemistry
Sulfides/chemistry
*Temperature
Time Factors},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/21765398}
}

@Article{Choy2011,
  Title                    = {Enhanced single-photon emission from a diamondâ€“silver aperture},
  Author                   = {Choy, Jennifer T. and Hausmann, Birgit J. M. and Babinec, Thomas M. and Bulu, Irfan and Khan, Mughees and Maletinsky, Patrick and Yacoby, Amir and LonÄ?ar, Marko},
  Journal                  = {Nature Photonics},
  Year                     = {2011},
  Number                   = {12},
  Pages                    = {738-743},
  Volume                   = {5},

  Doi                      = {10.1038/nphoton.2011.249},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Christ2003,
  Title                    = {Waveguide-Plasmon Polaritons: Strong Coupling of Photonic and Electronic Resonances in a Metallic Photonic Crystal Slab},
  Author                   = {Christ, A. and Tikhodeev, S. and Gippius, N. and Kuhl, J. and Giessen, H.},
  Journal                  = {Physical Review Letters},
  Year                     = {2003},
  Number                   = {18},
  Volume                   = {91},

  Doi                      = {10.1103/PhysRevLett.91.183901},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Chu2014,
  Title                    = {Coherent optical transitions in implanted nitrogen vacancy centers},
  Author                   = {Chu, Y. and de Leon, N. P. and Shields, B. J. and Hausmann, B. and Evans, R. and Togan, E. and Burek, M. J. and Markham, M. and Stacey, A. and Zibrov, A. S. and Yacoby, A. and Twitchen, D. J. and Loncar, M. and Park, H. and Maletinsky, P. and Lukin, M. D.},
  Journal                  = {Nano Lett},
  Year                     = {2014},
  Number                   = {4},
  Pages                    = {1982-6},
  Volume                   = {14},

  Abstract                 = {We report the observation of stable optical transitions in nitrogen-vacancy (NV) centers created by ion implantation. Using a combination of high temperature annealing and subsequent surface treatment, we reproducibly create NV centers with zero-phonon lines (ZPL) exhibiting spectral diffusion that is close to the lifetime-limited optical line width. The residual spectral diffusion is further reduced by using resonant optical pumping to maintain the NV(-) charge state. This approach allows for placement of NV centers with excellent optical coherence in a well-defined device layer, which is a crucial step in the development of diamond-based devices for quantum optics, nanophotonics, and quantum information science.},
  Doi                      = {10.1021/nl404836p},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24588353}
}

@Article{Chunlang2006,
  Title                    = {Single photon emission from SiV centres in diamond produced by ion implantation},
  Author                   = {Chunlang, Wang and Christian, Kurtsiefer and Harald, Weinfurter and Bernd, Burchard},
  Journal                  = {Journal of Physics B: Atomic, Molecular and Optical Physics},
  Year                     = {2006},
  Number                   = {1},
  Pages                    = {37},
  Volume                   = {39},

  Abstract                 = {We report the observation of single photon emission from single SiV (silicon-vacancy) centres in diamond produced by ion implantation. The high photostability and the narrow emission bandwidth of about 5 nm at room temperature make SiV centres interesting as a single photon source in practical quantum cryptography. We discuss problems that arise from the nonradiaditve transitions which lower the brightness of the source.},
  ISSN                     = {0953-4075},
  Type                     = {Journal Article},
  Url                      = {http://stacks.iop.org/0953-4075/39/i=1/a=005}
}

@Article{Ci2010,
  Title                    = {Atomic layers of hybridized boron nitride and graphene domains},
  Author                   = {Ci, Lijie and Song, Li and Jin, Chuanhong and Jariwala, Deep and Wu,
 Dangxin and Li, Yongjie and Srivastava, Anchal and Wang, Z. F. and
 Storr, Kevin and Balicas, Luis and Liu, Feng and Ajayan, Pulickel M.},
  Journal                  = {NATURE MATERIALS},
  Year                     = {2010},

  Month                    = {MAY},
  Number                   = {5},
  Pages                    = {430-435},
  Volume                   = {9},

  Doi                      = {{10.1038/nmat2711}},
  ISSN                     = {{1476-1122}},
  Orcid-numbers            = {{wang, zhengfei/0000-0002-0788-9725
 }},
  Owner                    = {Toan},
  Researcherid-numbers     = {{Li, cocaok/B-3357-2012
 Wu, Dangxin/E-5891-2012
 wang, zhengfei/E-8150-2011
 Song, Li/B-1950-2010
 Jariwala, Deep/E-9913-2013
 æ…ˆ, ç«‹æ�°/E-3485-2014}},
  Timestamp                = {2015.04.08},
  Unique-id                = {{ISI:000276953500024}}
}

@Article{Ciraci2012,
  Title                    = {Probing the Ultimate Limits of Plasmonic Enhancement},
  Author                   = {Ciraci, C. and Hill, R. T. and Mock, J. J. and Urzhumov, Y. and Fernandez-Dominguez, A. I. and Maier, S. A. and Pendry, J. B. and Chilkoti, A. and Smith, D. R.},
  Journal                  = {Science},
  Year                     = {2012},
  Number                   = {6098},
  Pages                    = {1072-1074},
  Volume                   = {337},

  Abstract                 = {Metals support surface plasmons at optical wavelengths and have the ability to localize light to subwavelength regions. The field enhancements that occur in these regions set the ultimate limitations on a wide range of nonlinear and quantum optical phenomena. We found that the dominant limiting factor is not the resistive loss of the metal, but rather the intrinsic nonlocality of its dielectric response. A semiclassical model of the electronic response of a metal places strict bounds on the ultimate field enhancement. To demonstrate the accuracy of this model, we studied optical scattering from gold nanoparticles spaced a few angstroms from a gold film. The bounds derived from the models and experiments impose limitations on all nanophotonic systems.},
  Doi                      = {10.1126/science.1224823},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000308125800040}
}

@Article{Coe2002,
  Title                    = {Electroluminescence from single monolayers of nanocrystals in molecular organic devices},
  Author                   = {Coe, Seth and Woo, Wing-Keung and Bawendi, Moungi and BuloviÄ‡, Vladimir},
  Journal                  = {Nature},
  Year                     = {2002},
  Number                   = {6917},
  Pages                    = {800-803},
  Volume                   = {420},

  Abstract                 = {The integration of organic and inorganic materials at the nanometre scale into hybrid optoelectronic structures enables active devices that combine the diversity of organic materials with the high-performance electronic and optical properties of inorganic nanocrystals. The optimization of such hybrid devices ultimately depends upon the precise positioning of the functionally distinct materials. Previous studies have already emphasized that this is a challenge, owing to the lack of well-developed nanometre-scale fabrication techniques. Here we demonstrate a hybrid light-emitting diode (LED) that combines the ease of processability of organic materials with the narrow-band, efficient luminescence of colloidal quantum dots (QDs). To isolate the luminescence processes from charge conduction, we fabricate a quantum-dot LED (QD-LED) that contains only a single monolayer of QDs, sandwiched between two organic thin films. This is achieved by a method that uses material phase segregation between the QD aliphatic capping groups and the aromatic organic materials. In our devices, where QDs function exclusively as lumophores, we observe a 25-fold improvement in luminescence efficiency (1.6 cd A(-1) at 2,000 cd m(-2)) over the best previous QD-LED results. The reproducibility and precision of our phase-segregation approach suggests that this technique could be widely applicable to the fabrication of other hybrid organic/inorganic devices.;},
  ISSN                     = {0028-0836},
  Type                     = {Journal Article},
  Url                      = {http://search.ebscohost.com/login.aspx?direct=true&db=mnh&AN=12490945&site=ehost-live}
}

@Article{Coe-Sullivan2005,
  Title                    = {Large-Area Ordered Quantum-Dot Monolayers via Phase Separation During Spin-Casting},
  Author                   = {Coe-Sullivan, S. and Steckel, J. â€‰S and Woo, W. K. and Bawendi, M. â€‰G and BuloviÄ‡, V.},
  Journal                  = {Advanced Functional Materials},
  Year                     = {2005},
  Number                   = {7},
  Pages                    = {1117-1124},
  Volume                   = {15},

  Abstract                 = {We investigate a new method for forming large-area (>â€‰cm2) ordered monolayers of colloidal nanocrystal quantum dots (QDs). The QD thin films are formed in a single step by spin-casting a mixed solution of aromatic organic materials and aliphatically capped QDs. The two different materials phase separate during solvent drying, and for a predefined set of conditions the QDs can assemble into hexagonally close-packed crystalline domains. We demonstrate the robustness and flexibility of this phase-separation process, as well as how the properties of the resulting films can be controlled in a precise and repeatable manner. Solution concentration, solvent ratio, QD size distribution, and QD aspect ratio affect the morphology of the cast thin-film structure. Controlling all of these factors allows the creation of colloidal-crystal domains that are square micrometers in size, containing tens of thousands of individual nanocrystals per grain. Such fabrication of large-area, engineered layers of nanoscale materials brings the beneficial properties of inorganic QDs into the realm of nanotechnology. For example, this technique has already enabled significant improvements in the performance of QD light-emitting devices.},
  Doi                      = {10.1002/adfm.200400468},
  ISSN                     = {1616-3028},
  Keywords                 = {Colloidal crystals
Light-emitting devices
Nanoparticles, inorganic
Quantum dots
Self-assembly
Thin films},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/adfm.200400468}
}

@Article{Coleman2011,
  Title                    = {Two-Dimensional Nanosheets Produced by Liquid Exfoliation of Layered Materials},
  Author                   = {Coleman, Jonathan N. and Lotya, Mustafa and Oâ€™Neill, Arlene and Bergin, Shane D. and King, Paul J. and Khan, Umar and Young, Karen and Gaucher, Alexandre and De, Sukanta and Smith, Ronan J. and Shvets, Igor V. and Arora, Sunil K. and Stanton, George and Kim, Hye-Young and Lee, Kangho and Kim, Gyu Tae and Duesberg, Georg S. and Hallam, Toby and Boland, John J. and Wang, Jing Jing and Donegan, John F. and Grunlan, Jaime C. and Moriarty, Gregory and Shmeliov, Aleksey and Nicholls, Rebecca J. and Perkins, James M. and Grieveson, Eleanor M. and Theuwissen, Koenraad and McComb, David W. and Nellist, Peter D. and Nicolosi, Valeria},
  Journal                  = {Science},
  Year                     = {2011},
  Number                   = {6017},
  Pages                    = {568-571},
  Volume                   = {331},

  Abstract                 = {If they could be easily exfoliated, layered materials would become a diverse source of two-dimensional crystals whose properties would be useful in applications ranging from electronics to energy storage. We show that layered compounds such as MoS2, WS2, MoSe2, MoTe2, TaSe2, NbSe2, NiTe2, BN, and Bi2Te3 can be efficiently dispersed in common solvents and can be deposited as individual flakes or formed into films. Electron microscopy strongly suggests that the material is exfoliated into individual layers. By blending this material with suspensions of other nanomaterials or polymer solutions, we can prepare hybrid dispersions or composites, which can be cast into films. We show that WS2 and MoS2 effectively reinforce polymers, whereas WS2/carbon nanotube hybrid films have high conductivity, leading to promising thermoelectric properties.},
  Doi                      = {10.1126/science.1194975},
  Owner                    = {Toan},
  Timestamp                = {2015.04.09}
}

@Article{Collins1983,
  Title                    = {Luminescence decay time of the 1.945 eV centre in type Ib diamond},
  Author                   = {Collins, A. T. and Thomaz, M. F. and Jorge, M. I. B.},
  Journal                  = {Journal of Physics C: Solid State Physics},
  Year                     = {1983},
  Number                   = {11},
  Pages                    = {2177},
  Volume                   = {16},

  Abstract                 = {The luminescence decay time of the 1.945 eV centre has been determined as 13+or-0.5 ns for natural type Ib diamonds. For synthetic diamonds the value is slightly lower, probably because of competitive non-radiative recombination in these relatively impure crystals. The similarity of the decay time to that for the H3 centre further supports the model proposed for the vacancy-enhanced aggregation of nitrogen in diamond. No temperature dependence of the 1.945 eV decay time has been detected in the range 77-700K, and this result is not inconsistent with the energy level scheme used to interpret ESR data for the 1.945 eV centre.},
  ISSN                     = {0022-3719},
  Type                     = {Journal Article},
  Url                      = {http://stacks.iop.org/0022-3719/16/i=11/a=020}
}

@Article{Colvin1994,
  Title                    = {Light-emitting diodes made from cadmium selenide nanocrystals and a semiconducting polymer},
  Author                   = {Colvin, V. L. and Schlamp, M. C. and Alivisatos, A. P.},
  Journal                  = {Nature},
  Year                     = {1994},
  Number                   = {6488},
  Pages                    = {354-357},
  Volume                   = {370},

  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/370354a0}
}

@Article{Comin2014,
  Title                    = {New materials for tunable plasmonic colloidal nanocrystals},
  Author                   = {Comin, Alberto and Manna, Liberato},
  Journal                  = {Chemical Society Reviews},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {3957-3975},
  Volume                   = {43},

  Abstract                 = {We present a review on the emerging materials for novel plasmonic colloidal nanocrystals. We start by explaining the basic processes involved in surface plasmon resonances in nanoparticles and then discuss the classes of nanocrystals that to date are particularly promising for tunable plasmonics: non-stoichiometric copper chalcogenides, extrinsically doped metal oxides, oxygen-deficient metal oxides and conductive metal oxides. We additionally introduce other emerging types of plasmonic nanocrystals and finally we give an outlook on nanocrystals of materials that could potentially display interesting plasmonic properties.},
  Doi                      = {10.1039/C3CS60265F},
  ISSN                     = {0306-0012},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1039/C3CS60265F}
}

@Article{Constantinescu2013,
  Title                    = {Stacking in Bulk and Bilayer Hexagonal Boron Nitride},
  Author                   = {Constantinescu, Gabriel and Kuc, Agnieszka and Heine, Thomas},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2013},

  Month                    = jul,
  Number                   = {3},
  Pages                    = {036104--},
  Volume                   = {111},

  Owner                    = {Toan},
  Publisher                = {American Physical Society},
  Refid                    = {10.1103/PhysRevLett.111.036104},
  Timestamp                = {2015.04.22},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.111.036104}
}

@Article{Costa2012,
  Title                    = {Silverâ€“gold nanotubes containing hot spots on their surface: facile synthesis and surface-enhanced Raman scattering investigations},
  Author                   = {Costa, Jean C. S. and Corio, Paola and Camargo, Pedro H. C.},
  Journal                  = {RSC Advances},
  Year                     = {2012},
  Number                   = {26},
  Pages                    = {9801},
  Volume                   = {2},

  Doi                      = {10.1039/c2ra21562d},
  ISSN                     = {2046-2069},
  Type                     = {Journal Article}
}

@Article{Cretu2014,
  Title                    = {Experimental Observation of Boron Nitride Chains},
  Author                   = {Cretu, Ovidiu and Komsa, Hannu-Pekka and Lehtinen, Ossi and Algara-Siller, Gerardo and Kaiser, Ute and Suenaga, Kazu and Krasheninnikov, Arkady V.},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {12},
  Pages                    = {11950-11957},
  Volume                   = {8},

  Abstract                 = {We report the formation and characterization of boron nitride atomic chains. The chains were made from hexagonal boron nitride sheets using the electron beam inside a transmission electron microscope. We find that the stability and lifetime of the chains are significantly improved when they are supported by another boron nitride layer. With the help of first-principles calculations, we prove the heteroatomic structure of the chains and determine their mechanical and electronic properties. Our study completes the analogy between various boron nitride and carbon polymorphs, in accordance with earlier theoretical predictions.},
  Doi                      = {10.1021/nn5046147},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn5046147}
}

@Article{Cui2013,
  Title                    = {Increased negatively charged nitrogen-vacancy centers in fluorinated diamond},
  Author                   = {Cui, Shanying and Hu, Evelyn L.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2013},
  Number                   = {5},
  Pages                    = {051603},
  Volume                   = {103},

  Doi                      = {10.1063/1.4817651},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Cui2014,
  Title                    = {Large scale thermal exfoliation and functionalization of boron nitride},
  Author                   = {Cui, Z. and Oyer, A. J. and Glover, A. J. and Schniepp, H. C. and Adamson, D. H.},
  Journal                  = {Small},
  Year                     = {2014},
  Number                   = {12},
  Pages                    = {2352-5},
  Volume                   = {10},

  Doi                      = {10.1002/smll.201303236},
  ISSN                     = {1613-6829 (Electronic)
1613-6810 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24578306}
}

@Article{Curto2010,
  Title                    = {Unidirectional emission of a quantum dot coupled to a nanoantenna},
  Author                   = {Curto, A. G. and Volpe, G. and Taminiau, T. H. and Kreuzer, M. P. and Quidant, R. and van Hulst, N. F.},
  Journal                  = {Science},
  Year                     = {2010},
  Number                   = {5994},
  Pages                    = {930-3},
  Volume                   = {329},

  Abstract                 = {Nanoscale quantum emitters are key elements in quantum optics and sensing. However, efficient optical excitation and detection of such emitters involves large solid angles because their interaction with freely propagating light is omnidirectional. Here, we present unidirectional emission of a single emitter by coupling to a nanofabricated Yagi-Uda antenna. A quantum dot is placed in the near field of the antenna so that it drives the resonant feed element of the antenna. The resulting quantum-dot luminescence is strongly polarized and highly directed into a narrow forward angular cone. The directionality of the quantum dot can be controlled by tuning the antenna dimensions. Our results show the potential of optical antennas to communicate energy to, from, and between nano-emitters.},
  Doi                      = {10.1126/science.1191922},
  ISSN                     = {1095-9203 (Electronic)
0036-8075 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20724630}
}

@Article{Dabbousi1995,
  Title                    = {Electroluminescence from CdSe quantum-dot/polymer composites},
  Author                   = {Dabbousi, B. O. and Bawendi, M. G.},
  Journal                  = {Applied Physics Letters},
  Year                     = {1995},
  Number                   = {11},
  Pages                    = {1316},
  Volume                   = {66},

  Abstract                 = {Reports the discovery of electroluminescence from CdSe quantum dots containing polymer composites. Effect of changed dot diameter on photoluminescence spectra; Size dependence to efficiency; Choice of lower work function cathode.},
  ISSN                     = {00036951},
  Keywords                 = {ELECTROLUMINESCENCE
CADMIUM compounds
QUANTUM dots
POLYMERS},
  Type                     = {Journal Article},
  Url                      = {https://www.lib.uts.edu.au/goto?url=http://search.ebscohost.com/login.aspx?direct=true&db=iih&AN=4203988&site=ehost-live}
}

@Article{Dai2010,
  Title                    = {Semiconductor-nanocrystals-based white light-emitting diodes},
  Author                   = {Dai, Q. and Duty, C. E. and Hu, M. Z.},
  Journal                  = {Small},
  Year                     = {2010},
  Number                   = {15},
  Pages                    = {1577-88},
  Volume                   = {6},

  Abstract                 = {In response to the demands for energy and the concerns of global warming and climate change, energy efficient and environmentally friendly solid-state lighting, such as white light-emitting diodes (WLEDs), is considered to be the most promising and suitable light source. Because of their small size, high efficiency, and long lifetime, WLEDs based on colloidal semiconductor nanocrystals (or quantum dots) are emerging as a completely new technology platform for the development of flat-panel displays and solid-state lighting, exhibiting the potential to replace the conventionally used incandescent and fluorescent lamps. This replacement can cut the ever-increasing level of energy consumption, solve the problem of rapidly depleting fossil fuel reserves, and improve the quality of the global environment. In this review, the recent progress in semiconductor-nanocrystals-based WLEDs is highlighted, the different approaches for generating white light are compared, and the benefits and challenges of the solid-state lighting technology are discussed.},
  Doi                      = {10.1002/smll.201000144},
  ISSN                     = {1613-6829 (Electronic)
1613-6810 (Linking)},
  Keywords                 = {*Light
*Nanotechnology
*Quantum Dots},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20602425}
}

@Article{Dai2014a,
  Title                    = {Tunable Phonon Polaritons in Atomically Thin van der Waals Crystals of Boron Nitride},
  Author                   = {Dai, S. and Fei, Z. and Ma, Q. and Rodin, A. S. and Wagner, M. and McLeod, A. S. and Liu, M. K. and Gannett, W. and Regan, W. and Watanabe, K. and Taniguchi, T. and Thiemens, M. and Dominguez, G. and Neto, A. H. Castro and Zettl, A. and Keilmann, F. and Jarillo-Herrero, P. and Fogler, M. M. and Basov, D. N.},
  Journal                  = {Science},
  Year                     = {2014},
  Number                   = {6175},
  Pages                    = {1125--1129},
  Volume                   = {343},

  Abstract                 = {van der Waals heterostructures assembled from atomically thin crystalline layers of diverse two-dimensional solids are emerging as a new paradigm in the physics of materials. We used infrared nanoimaging to study the properties of surface phonon polaritons in a representative van der Waals crystal, hexagonal boron nitride. We launched, detected, and imaged the polaritonic waves in real space and altered their wavelength by varying the number of crystal layers in our specimens. The measured dispersion of polaritonic waves was shown to be governed by the crystal thickness according to a scaling law that persists down to a few atomic layers. Our results are likely to hold true in other polar van der Waals crystals and may lead to new functionalities.},
  Comment                  = {10.1126/science.1246833},
  Owner                    = {Toan},
  Timestamp                = {2015.04.09},
  Url                      = {http://www.sciencemag.org/content/343/6175/1125.abstract}
}

@Article{Dai2014,
  Title                    = {Solution-processed, high-performance light-emitting diodes based on quantum dots},
  Author                   = {Dai, X. and Zhang, Z. and Jin, Y. and Niu, Y. and Cao, H. and Liang, X. and Chen, L. and Wang, J. and Peng, X.},
  Journal                  = {Nature},
  Year                     = {2014},
  Number                   = {7525},
  Pages                    = {96-9},
  Volume                   = {515},

  Abstract                 = {Solution-processed optoelectronic and electronic devices are attractive owing to the potential for low-cost fabrication of large-area devices and the compatibility with lightweight, flexible plastic substrates. Solution-processed light-emitting diodes (LEDs) using conjugated polymers or quantum dots as emitters have attracted great interest over the past two decades. However, the overall performance of solution-processed LEDs--including their efficiency, efficiency roll-off at high current densities, turn-on voltage and lifetime under operational conditions-remains inferior to that of the best vacuum-deposited organic LEDs. Here we report a solution-processed, multilayer quantum-dot-based LED with excellent performance and reproducibility. It exhibits colour-saturated deep-red emission, sub-bandgap turn-on at 1.7 volts, high external quantum efficiencies of up to 20.5 per cent, low efficiency roll-off (up to 15.1 per cent of the external quantum efficiency at 100 mA cm(-2)), and a long operational lifetime of more than 100,000 hours at 100 cd m(-2), making this device the best-performing solution-processed red LED so far, comparable to state-of-the-art vacuum-deposited organic LEDs. This optoelectronic performance is achieved by inserting an insulating layer between the quantum dot layer and the oxide electron-transport layer to optimize charge balance in the device and preserve the superior emissive properties of the quantum dots. We anticipate that our results will be a starting point for further research, leading to high-performance, all-solution-processed quantum-dot-based LEDs ideal for next-generation display and solid-state lighting technologies.},
  Doi                      = {10.1038/nature13829},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25363773}
}

@Article{Das2014,
  Title                    = {Synthesis, Properties, and Applications of 2-D Materials: A Comprehensive Review},
  Author                   = {Das, Santanu and Kim, Moonkyung and Lee, Jo-won and Choi, Wonbong},
  Journal                  = {Critical Reviews in Solid State and Materials Sciences},
  Year                     = {2014},
  Number                   = {4},
  Pages                    = {231-252},
  Volume                   = {39},

  Doi                      = {10.1080/10408436.2013.836075},
  ISSN                     = {1040-8436
1547-6561},
  Type                     = {Journal Article}
}

@Article{Datchi2004,
  Title                    = {Raman spectrum of cubic boron nitride at high pressure and temperature},
  Author                   = {Datchi, FrÃ©dÃ©ric and Canny, Bernard},
  Journal                  = {Physical Review B},
  Year                     = {2004},
  Number                   = {14},
  Pages                    = {144106},
  Volume                   = {69},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.69.144106}
}

@Article{David2012,
  Title                    = {Photonic crystal light-emitting sources},
  Author                   = {David, A. and Benisty, H. and Weisbuch, C.},
  Journal                  = {Rep Prog Phys},
  Year                     = {2012},
  Number                   = {12},
  Pages                    = {126501},
  Volume                   = {75},

  Abstract                 = {Photonic crystals (PhCs) are periodically structured optical media offering the opportunity for spontaneous emission (SpE) to be strongly controlled in spatial terms (directions) or in absolute terms (rates). We discuss the application of this concept for practical light-emitting sources, summarizing the principles and actual merits of various approaches based on two- and three-dimensional PhCs. We take into consideration the numerous constraints on real-world light-emitting structures and materials. The various mechanisms through which modified photonic bands and band gaps can be used are first revisited in view of their use in light sources. We then present an in-depth discussion of planar emitters and enhanced extraction of light thanks to grating diffraction. Applications to conventional III-V semiconductors and to III-nitrides are reviewed. Comparison with random surface roughening reveals some common physical limitations. Some advanced approaches with complex structures or etched active structures are also discussed. Finally, the most promising mechanism to enhance the SpE rate, the Purcell effect, is considered. Its implementation, including through plasmonic effects, is shown to be effective only for very specific sources. We conclude by outlining the mix of physics and material parameters needed to grasp the relevant issues.},
  Doi                      = {10.1088/0034-4885/75/12/126501},
  ISSN                     = {1361-6633 (Electronic)
0034-4885 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23099562}
}

@Article{Davies1976,
  Title                    = {Optical Studies of the 1.945 eV Vibronic Band in Diamond},
  Author                   = {Davies, G. and Hamer, M. F.},
  Journal                  = {Proceedings of the Royal Society of London. Series A, Mathematical and Physical Sciences},
  Year                     = {1976},
  Number                   = {1653},
  Pages                    = {285-298},
  Volume                   = {348},

  Abstract                 = {The 1.945 eV band is the dominant end product of annealing radiation damage in diamonds containing isolated substitutional nitrogen atoms. In this paper uniaxial stress experiments are described which show the band to be a transition between A1 (ground) and E (excited) electronic states of a trigonal centre, the E state being coupled predominantly to A1 modes of vibration. Annealing experiments suggest that the centre is either a substitutional nitrogen atom plus an interstitial nitrogen atom, or a substitutional nitrogen atom plus a vacancy. Small differences between the luminescence and absorption bands are shown to be consistent with the double minima vibrational potential of the nitrogen-vacancy model.},
  Doi                      = {10.2307/79142},
  ISSN                     = {00804630},
  Type                     = {Journal Article},
  Url                      = {http://www.jstor.org/stable/79142}
}

@Article{Davis2010,
  Title                    = {Simple Model for the Hybridization of Surface Plasmon Resonances in Metallic Nanoparticles},
  Author                   = {Davis, T. J. and GoÌ?mez, D. E. and Vernon, K. C.},
  Journal                  = {Nano Letters},
  Year                     = {2010},
  Number                   = {7},
  Pages                    = {2618-2625},
  Volume                   = {10},

  Doi                      = {10.1021/nl101335z},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl101335z}
}

@Article{Davoyan2014,
  Title                    = {Electrically controlled one-way photon flow in plasmonic nanostructures},
  Author                   = {Davoyan, A. and Engheta, N.},
  Journal                  = {Nat Commun},
  Year                     = {2014},
  Pages                    = {5250},
  Volume                   = {5},

  Abstract                 = {Photonics is frequently regarded as a potential pathway for substituting current solid-state electronics and as a promise for higher-speed all-optical computing. The fundamental challenges facing nanophotonics and electronics of the future are nanoscale on-chip integration of electronics and photonics with an efficient electric field tuning of light propagation, dynamic access to the light sources and material parameters of the system, as well as isolation of optical signals analogous to that in electronics. Here we suggest a paradigm for a monolithically integrated electronic control over the light propagation in nanoscale plasmonic waveguides. We theoretically demonstrate that magnetic field induced by the direct electric current flowing in metallic constituents of plasmonic nanostructures alters the material parameters and thus the optical signal flow. We use this principle for the design of an electrically controlled subwavelength optical isolator.},
  Doi                      = {10.1038/ncomms6250},
  ISSN                     = {2041-1723 (Electronic)
2041-1723 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25373887}
}

@Article{DeAngelis2010,
  Title                    = {Nanoscale chemical mapping using three-dimensional adiabatic compression of surface plasmon polaritons},
  Author                   = {De Angelis, F. and Das, G. and Candeloro, P. and Patrini, M. and Galli, M. and Bek, A. and Lazzarino, M. and Maksymov, I. and Liberale, C. and Andreani, L. C. and Di Fabrizio, E.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2010},
  Number                   = {1},
  Pages                    = {67-72},
  Volume                   = {5},

  Abstract                 = {The fields of plasmonics, Raman spectroscopy and atomic force microscopy have recently undergone considerable development, but independently of one another. By combining these techniques, a range of complementary information could be simultaneously obtained at a single molecule level. Here, we report the design, fabrication and application of a photonic-plasmonic device that is fully compatible with atomic force microscopy and Raman spectroscopy. Our approach relies on the generation and localization of surface plasmon polaritons by means of adiabatic compression through a metallic tapered waveguide to create strongly enhanced Raman excitation in a region just a few nanometres across. The tapered waveguide can also be used as an atomic force microscope tip. Using the device, topographic, chemical and structural information about silicon nanocrystals may be obtained with a spatial resolution of 7 nm.},
  Doi                      = {10.1038/nnano.2009.348},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/19935647}
}

@Article{Dean2010,
  Title                    = {Boron nitride substrates for high-quality graphene electronics},
  Author                   = {Dean, C. R. and Young, A. F. and Meric, I. and Lee, C. and Wang, L. and Sorgenfrei, S. and Watanabe, K. and Taniguchi, T. and Kim, P. and Shepard, K. L. and Hone, J.},
  Journal                  = {Nature Nanotechnology},
  Year                     = {2010},
  Number                   = {10},
  Pages                    = {722-6},
  Volume                   = {5},

  Abstract                 = {Graphene devices on standard SiO(2) substrates are highly disordered, exhibiting characteristics that are far inferior to the expected intrinsic properties of graphene. Although suspending the graphene above the substrate leads to a substantial improvement in device quality, this geometry imposes severe limitations on device architecture and functionality. There is a growing need, therefore, to identify dielectrics that allow a substrate-supported geometry while retaining the quality achieved with a suspended sample. Hexagonal boron nitride (h-BN) is an appealing substrate, because it has an atomically smooth surface that is relatively free of dangling bonds and charge traps. It also has a lattice constant similar to that of graphite, and has large optical phonon modes and a large electrical bandgap. Here we report the fabrication and characterization of high-quality exfoliated mono- and bilayer graphene devices on single-crystal h-BN substrates, by using a mechanical transfer process. Graphene devices on h-BN substrates have mobilities and carrier inhomogeneities that are almost an order of magnitude better than devices on SiO(2). These devices also show reduced roughness, intrinsic doping and chemical reactivity. The ability to assemble crystalline layered materials in a controlled way permits the fabrication of graphene devices on other promising dielectrics and allows for the realization of more complex graphene heterostructures.},
  Doi                      = {http://dx.doi.org/10.1038/nnano.2010.172},
  ISSN                     = {17483387},
  Keywords                 = {Physics},
  Type                     = {Journal Article},
  Url                      = {http://ezproxy.lib.uts.edu.au/login?url=http://search.proquest.com/docview/868393198?accountid=17095
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Journal_Search&Ntx=matchallpartial&Ntt=Nature+Nanotechnology
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Title_Search&Ntx=matchallpartial&Ntt=Boron+nitride+substrates+for+high-quality+graphene+electronics
http://sfx.lib.uts.edu.au/sfx_local?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:journal&genre=article&sid=ProQ:ProQ%3Ahealthcompleteshell&atitle=Boron+nitride+substrates+for+high-quality+graphene+electronics&title=Nature+Nanotechnology&issn=17483387&date=2010-10-01&volume=5&issue=10&spage=722&au=Dean%2C+C+R%3BYoung%2C+A+F%3BMeric%2C+I%3BLee%2C+C%3BWang%2C+L%3BSorgenfrei%2C+S%3BWatanabe%2C+K%3BTaniguchi%2C+T%3BKim%2C+P%3BShepard%2C+K+L%3BHone%2C+J&isbn=&jtitle=Nature+Nanotechnology&btitle=&rft_id=info:eric/&rft_id=info:doi/10.1038%2Fnnano.2010.172}
}

@Article{Demir2011,
  Title                    = {Quantum dot integrated LEDs using photonic and excitonic color conversion},
  Author                   = {Demir, Hilmi Volkan and Nizamoglu, Sedat and Erdem, Talha and Mutlugun, Evren and Gaponik, Nikolai and EychmÃ¼ller, Alexander},
  Journal                  = {Nano Today},
  Year                     = {2011},
  Number                   = {6},
  Pages                    = {632-647},
  Volume                   = {6},

  Doi                      = {10.1016/j.nantod.2011.10.006},
  ISSN                     = {17480132},
  Type                     = {Journal Article}
}

@Article{Denault2013,
  Title                    = {Improving color rendition in solid state white lighting through the use of quantum dots},
  Author                   = {Denault, Kristin A. and Mikhailovsky, Alexander A. and Brinkley, Stuart and DenBaars, Steven P. and Seshadri, Ram},
  Journal                  = {Journal of Materials Chemistry C},
  Year                     = {2013},
  Number                   = {7},
  Pages                    = {1461},
  Volume                   = {1},

  Doi                      = {10.1039/c2tc00420h},
  ISSN                     = {2050-7526
2050-7534},
  Type                     = {Journal Article}
}

@Article{Denk1990,
  Title                    = {Two-photon laser scanning fluorescence microscopy},
  Author                   = {Denk, W and Strickler, JH and Webb, WW},
  Journal                  = {Science},
  Year                     = {1990},
  Number                   = {4951},
  Pages                    = {73-76},
  Volume                   = {248},

  Abstract                 = {Molecular excitation by the simultaneous absorption of two photons provides intrinsic three-dimensional resolution in laser scanning fluorescence microscopy. The excitation of fluorophores having single-photon absorption in the ultraviolet with a stream of strongly focused subpicosecond pulses of red laser light has made possible fluorescence images of living cells and other microscopic objects. The fluorescence emission increased quadratically with the excitation intensity so that fluorescence and photo-bleaching were confined to the vicinity of the focal plane as expected for cooperative two-photon excitation. This technique also provides unprecedented capabilities for three-dimensional, spatially resolved photochemistry, particularly photolytic release of caged effector molecules.},
  Doi                      = {10.1126/science.2321027},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/248/4951/73.abstract}
}

@Article{DiMartino2012,
  Title                    = {Quantum Statistics of Surface Plasmon Polaritons in Metallic Stripe Waveguides},
  Author                   = {Di Martino, Giuliana and Sonnefraud, Yannick and KÃ©na-Cohen, StÃ©phane and Tame, Mark and Ã–zdemir, Åžahin K. and Kim, M. S. and Maier, Stefan A.},
  Journal                  = {Nano Letters},
  Year                     = {2012},
  Number                   = {5},
  Pages                    = {2504-2508},
  Volume                   = {12},

  Abstract                 = {Heralded single surface plasmon polaritons are excited using photons generated via spontaneous parametric down conversion. The mean excitation rates, intensity correlations, and Fock state populations are studied. The observed dependence of the second-order coherence in our experiment is consistent with a linear uncorrelated Markovian environment in the quantum regime. Our results provide important information about the effect of loss for assessing the potential of plasmonic waveguides for future nanophotonic circuitry in the quantum regime.},
  Doi                      = {10.1021/nl300671w},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl300671w}
}

@Article{Dickson2000,
  Title                    = {Unidirectional Plasmon Propagation in Metallic Nanowires},
  Author                   = {Dickson, Robert M. and Lyon, L. Andrew},
  Journal                  = {Journal of Physical Chemistry B},
  Year                     = {2000},
  Number                   = {26},
  Pages                    = {6095-6098},
  Volume                   = {104},

  Doi                      = {10.1021/jp001435b},
  ISSN                     = {1520-6106},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/jp001435b}
}

@Article{Dionne2013,
  Title                    = {Nanoplasmonics: Plasmons rock in metal bands},
  Author                   = {Dionne, J. A.},
  Journal                  = {Nat Mater},
  Year                     = {2013},
  Number                   = {5},
  Pages                    = {380-1},
  Volume                   = {12},

  Doi                      = {10.1038/nmat3607},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23503013}
}

@Article{Dionne2006,
  Title                    = {Plasmon slot waveguides: Towards chip-scale propagation with subwavelength-scale localization},
  Author                   = {Dionne, J. and Sweatlock, L. and Atwater, H. and Polman, A.},
  Journal                  = {Physical Review B},
  Year                     = {2006},
  Number                   = {3},
  Volume                   = {73},

  Doi                      = {10.1103/PhysRevB.73.035407},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Ditlbacher2005,
  Title                    = {Silver Nanowires as Surface Plasmon Resonators},
  Author                   = {Ditlbacher, Harald and Hohenau, Andreas and Wagner, Dieter and Kreibig, Uwe and Rogers, Michael and Hofer, Ferdinand and Aussenegg, Franz and Krenn, Joachim},
  Journal                  = {Physical Review Letters},
  Year                     = {2005},
  Number                   = {25},
  Volume                   = {95},

  Doi                      = {10.1103/PhysRevLett.95.257403},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Doherty2013,
  Title                    = {The nitrogen-vacancy colour centre in diamond},
  Author                   = {Doherty, Marcus W. and Manson, Neil B. and Delaney, Paul and Jelezko, Fedor and Wrachtrup, JÃ¶rg and Hollenberg, Lloyd C. L.},
  Journal                  = {Physics Reports},
  Year                     = {2013},
  Number                   = {1},
  Pages                    = {1-45},
  Volume                   = {528},

  Abstract                 = {The nitrogen-vacancy (NV) colour centre in diamond is an important physical system for emergent quantum technologies, including quantum metrology, information processing and communications, as well as for various nanotechnologies, such as biological and sub-diffraction limit imaging, and for tests of entanglement in quantum mechanics. Given this array of existing and potential applications and the almost 50Â years of NV research, one would expect that the physics of the centre is well understood, however, the study of the NV centre has proved challenging, with many early assertions now believed false and many remaining issues yet to be resolved. This review represents the first time that the key empirical and ab initio results have been extracted from the extensive NV literature and assembled into one consistent picture of the current understanding of the centre. As a result, the key unresolved issues concerning the NV centre are identified and the possible avenues for their resolution are examined.},
  Doi                      = {http://dx.doi.org/10.1016/j.physrep.2013.02.001},
  ISSN                     = {0370-1573},
  Keywords                 = {Diamond
Colour centre
Nitrogen-vacancy},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0370157313000562}
}

@Article{Dolan2014,
  Title                    = {Complete determination of the orientation of NV centers with radially polarized beams},
  Author                   = {Dolan, P. R. and Li, X. and Storteboom, J. and Gu, M.},
  Journal                  = {Opt Express},
  Year                     = {2014},
  Number                   = {4},
  Pages                    = {4379-87},
  Volume                   = {22},

  Abstract                 = {In this paper, we report on the precise determination of the orientation of NV centers by imaging with a radially polarized beam. Vectorial Debye theory is applied to the field in the focus of radially polarized beams to generate emission profiles of two orthogonal optical dipoles. By comparing features of the measured emission intensity patterns with simulated results, complete orientation determination of the NV axis is achieved. Results are corroborated by using established methods requiring the polarization rotation of a linearly polarized excitation source, and by analysis of optically detected magnetic resonance spectra. These results lay new ground for any application where the knowledge of the orientation of the NV centers is prerequisite.},
  Doi                      = {10.1364/OE.22.004379},
  ISSN                     = {1094-4087 (Electronic)
1094-4087 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24663761}
}

@Article{Dondapati2012,
  Title                    = {Voltage-induced adsorbate damping of single gold nanorod plasmons in aqueous solution},
  Author                   = {Dondapati, S. K. and Ludemann, M. and Muller, R. and Schwieger, S. and Schwemer, A. and Handel, B. and Kwiatkowski, D. and Djiango, M. and Runge, E. and Klar, T. A.},
  Journal                  = {Nano Lett},
  Year                     = {2012},
  Number                   = {3},
  Pages                    = {1247-52},
  Volume                   = {12},

  Abstract                 = {Unbiased gold nanoparticles are negatively charged in aqueous solution but not hydrated. Optical spectroscopy of voltage-clamped single gold nanoparticles reveals evidence that anion adsorption starts at positive potentials above the point of zero charge, causing severe but reversible plasmon damping in combination with a spectral red shift exceeding the linear double layer charging effect. Plasmon damping by adsorbate is relevant for the use of nanoparticles in catalysis, in biodiagnostics, and in surface enhanced Raman scattering.},
  Doi                      = {10.1021/nl203673g},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Adsorption/radiation effects
Electromagnetic Fields
Gold/*chemistry/radiation effects
Materials Testing
Nanostructures/*chemistry/*radiation effects
Solutions
Surface Plasmon Resonance/*methods
Surface Properties/radiation effects
Water/*chemistry},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22313237}
}

@Article{Drezet2015,
  Title                    = {Near-field microscopy with a scanning nitrogen-vacancy color center in a diamond nanocrystal: A brief review},
  Author                   = {Drezet, A. and Sonnefraud, Y. and Cuche, A. and Mollet, O. and Berthel, M. and Huant, S.},
  Journal                  = {Micron},
  Year                     = {2015},
  Number                   = {0},
  Pages                    = {55--63},
  Volume                   = {70},

  Abstract                 = {Abstract We review our recent developments of near-field scanning optical microscopy (NSOM) that uses an active tip made of a single fluorescent nanodiamond (ND) grafted onto the apex of a substrate fiber tip. The ND hosting a limited number of nitrogen-vacancy (NV) color centers, such a tip is a scanning quantum source of light. The method for preparing the ND-based tips and their basic properties are summarized. Then we discuss theoretically the concept of spatial resolution that is achievable in this special NSOM configuration and find it to be only limited by the scan height over the imaged system, in contrast with the standard aperture-tip NSOM whose resolution depends critically on both the scan height and aperture diameter. Finally, we describe a scheme we have introduced recently for high-resolution imaging of nanoplasmonic structures with ND-based tips that is capable of approaching the ultimate resolution anticipated by theory.},
  ISSN                     = {0968-4328},
  Keywords                 = {Near field optics, Near field microscopy, Nitrogen vacancy color center, Quantum optics, Plasmonics},
  Owner                    = {Toan},
  Timestamp                = {2015.04.10},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0968432814002194}
}

@Article{Du2014,
  Title                    = {One-step exfoliation and fluorination of boron nitride nanosheets and a study of their magnetic properties},
  Author                   = {Du, M. and Li, X. and Wang, A. and Wu, Y. and Hao, X. and Zhao, M.},
  Journal                  = {Angew Chem Int Ed Engl},
  Year                     = {2014},
  Number                   = {14},
  Pages                    = {3645-9},
  Volume                   = {53},

  Abstract                 = {A novel, simple, and efficient method for the preparation of the fluorinated hexagonal boron nitride nanosheets (F-BNNSs) and the corresponding magnetic properties is presented. A one-step route is used to exfoliate and fluorinate the BNNSs by ammonium fluoride (NH4F) from hexagonal boron nitride (h-BN) powder. Through related instrument characterizations and theoretical calculations, we confirm that large-area and few-layer F-BNNSs were successfully produced by this method, which can be attributed to a fluorination-assisted exfoliation mechanism from the bulk h-BN in NH4F. More intriguingly, we initially verified that the as-prepared F-BNNSs exhibit ferromagnetic characteristics, which would have good potential applications in spintronic devices.},
  Doi                      = {10.1002/anie.201308294},
  ISSN                     = {1521-3773 (Electronic)
1433-7851 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24591122}
}

@Article{Duan2001,
  Title                    = {Long-distance quantum communication with atomic ensembles and linear optics},
  Author                   = {Duan, L. M. and Lukin, M. D. and Cirac, J. I. and Zoller, P.},
  Journal                  = {Nature},
  Year                     = {2001},
  Number                   = {6862},
  Pages                    = {413-418},
  Volume                   = {414},

  Doi                      = {http://www.nature.com/nature/journal/v414/n6862/suppinfo/414413a0_S1.html},
  ISSN                     = {0028-0836},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/35106500}
}

@Article{Duan2003,
  Title                    = {Single-nanowire electrically driven lasers},
  Author                   = {Duan, Xiangfeng and Huang, Yu and Agarwal, Ritesh and Lieber, Charles M.},
  Journal                  = {Nature},
  Year                     = {2003},
  Number                   = {6920},
  Pages                    = {241-5},
  Volume                   = {421},

  Abstract                 = {Electrically driven semiconductor lasers are used in technologies ranging from telecommunications and information storage to medical diagnostics and therapeutics. The success of this class of lasers is due in part to well-developed planar semiconductor growth and processing, which enables reproducible fabrication of integrated, electrically driven devices. Yet this approach to device fabrication is also costly and difficult to integrate directly with other technologies such as silicon microelectronics. To overcome these issues for future applications, there has been considerable interest in using organic molecules, polymers, and inorganic nanostructures for lasers, because these materials can be fashioned into devices by chemical processing. Indeed, amplified stimulated emission and lasing have been reported for optically pumped organic systems and, more recently, inorganic nanocrystals and nanowires. However, electrically driven lasing, which is required in most applications, has met with several difficulties in organic systems, and has not been addressed for assembled nanocrystals or nanowires. Here Duan et al investigate the feasibility of achieving electrically driven lasing from individual nanowires. Optical and electrical measurements made on single-crystal cadmium sulphide nanowires show that these structures can function as Fabry and Perot optical cavities with mode spacing inversely related to the nanowire length. Investigations of optical and electrical pumping further indicate a threshold for lasing as characterized by optical modes with instrument-limited linewidths. Electrically driven nanowire lasers, which might be assembled in arrays capable of emitting a wide range of colours, could improve existing applications and suggest new opportunities.},
  ISSN                     = {00280836},
  Keywords                 = {Environmental Studies
Semiconductors
Lasers
Biology
Polymers},
  Type                     = {Journal Article},
  Url                      = {http://ezproxy.lib.uts.edu.au/login?url=http://search.proquest.com/docview/204555419?accountid=17095
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Journal_Search&Ntx=matchallpartial&Ntt=Nature
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Title_Search&Ntx=matchallpartial&Ntt=Single-nanowire+electrically+driven+lasers
http://sfx.lib.uts.edu.au/sfx_local?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:journal&genre=article&sid=ProQ:ProQ%3Ahealthcompleteshell&atitle=Single-nanowire+electrically+driven+lasers&title=Nature&issn=00280836&date=2003-01-16&volume=421&issue=6920&spage=241&au=Duan%2C+Xiangfeng%3BHuang%2C+Yu%3BAgarwal%2C+Ritesh%3BLieber%2C+Charles+M&isbn=&jtitle=Nature&btitle=&rft_id=info:eric/&rft_id=info:doi/}
}

@Article{Duan2014,
  Title                    = {Lateral epitaxial growth of two-dimensional layered semiconductor heterojunctions},
  Author                   = {Duan, X. and Wang, C. and Shaw, J. C. and Cheng, R. and Chen, Y. and Li, H. and Wu, X. and Tang, Y. and Zhang, Q. and Pan, A. and Jiang, J. and Yu, R. and Huang, Y. and Duan, X.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2014},
  Number                   = {12},
  Pages                    = {1024-30},
  Volume                   = {9},

  Abstract                 = {Two-dimensional layered semiconductors such as MoS2 and WSe2 have attracted considerable interest in recent times. Exploring the full potential of these layered materials requires precise spatial modulation of their chemical composition and electronic properties to create well-defined heterostructures. Here, we report the growth of compositionally modulated MoS2-MoSe2 and WS2-WSe2 lateral heterostructures by in situ modulation of the vapour-phase reactants during growth of these two-dimensional crystals. Raman and photoluminescence mapping studies demonstrate that the resulting heterostructure nanosheets exhibit clear structural and optical modulation. Transmission electron microscopy and elemental mapping studies reveal a single crystalline structure with opposite modulation of sulphur and selenium distributions across the heterostructure interface. Electrical transport studies demonstrate that the WSe2-WS2 heterojunctions form lateral p-n diodes and photodiodes, and can be used to create complementary inverters with high voltage gain. Our study is an important advance in the development of layered semiconductor heterostructures, an essential step towards achieving functional electronics and optoelectronics.},
  Doi                      = {10.1038/nnano.2014.222},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25262331}
}

@Article{Dzsotjan2010,
  Title                    = {Quantum emitters coupled to surface plasmons of a nanowire: A Greenâ€™s function approach},
  Author                   = {Dzsotjan, David and SÃ¸rensen, Anders S. and Fleischhauer, Michael},
  Journal                  = {Physical Review B},
  Year                     = {2010},
  Number                   = {7},
  Volume                   = {82},

  Doi                      = {10.1103/PhysRevB.82.075427},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Eichenfield2007,
  Title                    = {Actuation of micro-optomechanical systems via cavity-enhanced optical dipole forces},
  Author                   = {Eichenfield, Matt and Michael, Christopher P. and Perahia, Raviv and Painter, Oskar},
  Journal                  = {Nature Photonics},
  Year                     = {2007},
  Number                   = {7},
  Pages                    = {416-422},
  Volume                   = {1},

  Doi                      = {10.1038/nphoton.2007.96},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Elke2013,
  Title                    = {Low-temperature investigations of single silicon vacancy colour centres in diamond},
  Author                   = {Elke, Neu and Christian, Hepp and Michael, Hauschild and Stefan, Gsell and Martin, Fischer and Hadwig, Sternschulte and Doris, SteinmÃ¼ller-Nethl and Matthias, Schreck and Christoph, Becher},
  Journal                  = {New Journal of Physics},
  Year                     = {2013},
  Number                   = {4},
  Pages                    = {043005},
  Volume                   = {15},

  Abstract                 = {We study single silicon vacancy (SiV) centres in chemical vapour deposition (CVD) nanodiamonds on iridium as well as an ensemble of SiV centres in a high-quality, low-stress CVD diamond film by using temperature-dependent luminescence spectroscopy in the temperature range 5â€“295Â K. We investigate in detail the temperature-dependent fine structure of the zero-phonon line (ZPL) of the SiV centres. The ZPL transition is affected by inhomogeneous as well as temperature-dependent homogeneous broadening and blue shifts by about 20Â cm âˆ’1 upon cooling from room temperature to 5Â K. We employ excitation power-dependent g (2) measurements to explore the temperature-dependent internal population dynamics of single SiV centres and infer mostly temperature-independent dynamics.},
  ISSN                     = {1367-2630},
  Type                     = {Journal Article},
  Url                      = {http://stacks.iop.org/1367-2630/15/i=4/a=043005}
}

@Article{Elke2011,
  Title                    = {Single photon emission from silicon-vacancy colour centres in chemical vapour deposition nano-diamonds on iridium},
  Author                   = {Elke, Neu and David, Steinmetz and Janine, Riedrich-MÃ¶ller and Stefan, Gsell and Martin, Fischer and Matthias, Schreck and Christoph, Becher},
  Journal                  = {New J. Phys.},
  Year                     = {2011},
  Number                   = {2},
  Pages                    = {025012},
  Volume                   = {13},

  Abstract                 = {We introduce a process for the fabrication of high-quality, spatially isolated nano-diamonds on iridium via microwave-plasma-assisted chemical vapour deposition (CVD) growth. We perform spectroscopy of single silicon-vacancy (SiV) centres produced during the growth of the nano-diamonds. The colour centres exhibit extraordinary narrow zero-phonon-lines down to 0.7â€‰nm at room temperature. Single photon count rates up to 4.8â€‰Mcps at saturation make these SiV centres the brightest diamond-based single photon sources to date. We measure for the first time the fine structure of a single SiV centre, thus confirming the atomic composition of the investigated colour centres.},
  ISSN                     = {1367-2630},
  Type                     = {Journal Article},
  Url                      = {http://stacks.iop.org/1367-2630/13/i=2/a=025012}
}

@Article{Elson1974,
  Title                    = {Fluorescence correlation spectroscopy. I. Conceptual basis and theory},
  Author                   = {Elson, Elliot L. and Magde, Douglas},
  Journal                  = {Biopolymers},
  Year                     = {1974},
  Number                   = {1},
  Pages                    = {1-27},
  Volume                   = {13},

  Abstract                 = {We describe a method for determining chemical kinetic constants and diffusion coefficients by measuring the rates of decay of spontaneous concentration fluctuations. The equilibrium of the system is not disturbed during the measurement. We measure the number of molecules of a specified type in a defined open volume as a function of time and compute the time course of the deviations from the thermodynamic mean concentration. The method is based on the principle that the rates of decay of spontaneous microscopic fluctuations are determined by the same phenomenological rate coefficients as those of macroscopic departures from equilibrium which result from external perturbations. Hence, an analysis of fluctuations yields the same chemical rate constants and diffusion coefficients as are measured by conventional procedures. In practice the number of the specified molecules is measured by a property such as absorbance or fluorescence which is specific and sensitive to chemical change. The sample volume is defined by a light beam which traverses the cell. As the molecules appear in or disappear from the light beam, either due to diffusion or chemical reaction, their concentration fluctuations give rise to corresponding fluctuations of the intensity of absorbed or emitted light. This paper presents the theory needed to derive chemical rate constants and diffusion coefficients from these fluctuations in light intensity. The theory is applied to three examples of general interest: pure diffusion in the absence of chemical reaction; the binding of a small rapidly diffusing ligand to a larger slowly diffusing macromolecule; and a unimolecular isomerization. The method should be especially useful in studying highly cooperative systems, relatively noncooperative systems with intermediate states closely spaced in free energy, small systems, and systems not readily subject to perturbations of state.},
  Doi                      = {10.1002/bip.1974.360130102},
  ISSN                     = {1097-0282},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/bip.1974.360130102}
}

@Article{Engheta2011,
  Title                    = {Antenna-Guided Light},
  Author                   = {Engheta, Nader},
  Journal                  = {Science},
  Year                     = {2011},
  Number                   = {6054},
  Pages                    = {317-318},
  Volume                   = {334},

  Doi                      = {10.1126/science.1213278},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000296052500035}
}

@Article{Englund2007,
  Title                    = {Controlling cavity reflectivity with a single quantum dot},
  Author                   = {Englund, Dirk and Faraon, Andrei and Fushman, Ilya and Stoltz, Nick and Petroff, Pierre and Vuckovic, Jelena},
  Journal                  = {Nature},
  Year                     = {2007},
  Number                   = {7171},
  Pages                    = {857-861},
  Volume                   = {450},

  ISSN                     = {0028-0836},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nature06234}
}

@Article{Englund2010,
  Title                    = {Deterministic coupling of a single nitrogen vacancy center to a photonic crystal cavity},
  Author                   = {Englund, D. and Shields, B. and Rivoire, K. and Hatami, F. and Vuckovic, J. and Park, H. and Lukin, M. D.},
  Journal                  = {Nano Lett},
  Year                     = {2010},
  Number                   = {10},
  Pages                    = {3922-6},
  Volume                   = {10},

  Abstract                 = {We describe and experimentally demonstrate a technique for deterministic, large coupling between a photonic crystal (PC) nanocavity and single photon emitters. The technique is based on in situ scanning of a PC cavity over a sample and allows the precise positioning of the cavity over a desired emitter with nanoscale resolution. The power of the technique is demonstrated by coupling the PC nanocavity to a single nitrogen vacancy (NV) center in diamond, an emitter system that provides optically accessible electron and nuclear spin qubits.},
  Doi                      = {10.1021/nl101662v},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20825160}
}

@Article{Epstein2005,
  Title                    = {Anisotropic interactions of a single spin and dark-spin spectroscopy in diamond},
  Author                   = {Epstein, R. J. and Mendoza, F. M. and Kato, Y. K. and Awschalom, D. D.},
  Journal                  = {Nature Physics},
  Year                     = {2005},
  Number                   = {2},
  Pages                    = {94-98},
  Volume                   = {1},

  Doi                      = {10.1038/nphys141},
  ISSN                     = {1476-0000
1476-4636},
  Type                     = {Journal Article}
}

@Article{Eurenius2008,
  Title                    = {Grating formation by metal-nanoparticle-mediated coupling of light into waveguided modes},
  Author                   = {Eurenius, L. and HÃ¤gglund, C. and Olsson, E. and Kasemo, B. and Chakarov, D.},
  Journal                  = {Nature Photonics},
  Year                     = {2008},
  Number                   = {6},
  Pages                    = {360-364},
  Volume                   = {2},

  Doi                      = {10.1038/nphoton.2008.80},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Fairchild2008,
  Title                    = {Fabrication of Ultrathin Single-Crystal Diamond Membranes},
  Author                   = {Fairchild, Barbara A. and Olivero, Paolo and Rubanov, Sergey and Greentree, Andrew D. and Waldermann, Felix and Taylor, Robert A. and Walmsley, Ian and Smith, Jason M. and Huntington, Shane and Gibson, Brant C. and Jamieson, David N. and Prawer, Steven},
  Journal                  = {Advanced Materials},
  Year                     = {2008},
  Number                   = {24},
  Pages                    = {4793-4798},
  Volume                   = {20},

  Doi                      = {10.1002/adma.200801460},
  ISSN                     = {1521-4095},
  Keywords                 = {diamond
membranes
nano-electromechanical systems
nanostructure
photonics},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/adma.200801460}
}

@Article{Fakonas2014,
  Title                    = {Two-plasmon quantum interference},
  Author                   = {Fakonas, James S. and Lee, Hyunseok and Kelaita, Yousif A. and Atwater, Harry A.},
  Journal                  = {Nature Photonics},
  Year                     = {2014},
  Number                   = {4},
  Pages                    = {317-320},
  Volume                   = {8},

  Doi                      = {10.1038/nphoton.2014.40},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Falk2013,
  Title                    = {Polytype control of spin qubits in silicon carbide},
  Author                   = {Falk, Abram L. and Buckley, Bob B. and Calusine, Greg and Koehl, William F. and Dobrovitski, Viatcheslav V. and Politi, Alberto and Zorman, Christian A. and Feng, Philip X. L. and Awschalom, David D.},
  Journal                  = {Nat Commun},
  Year                     = {2013},
  Pages                    = {1819},
  Volume                   = {4},

  Doi                      = {10.1038/ncomms2854},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/ncomms2854}
}

@Article{Fan2010,
  Title                    = {Self-Assembled Plasmonic Nanoparticle Clusters},
  Author                   = {Fan, Jonathan A. and Wu, Chihhui and Bao, Kui and Bao, Jiming and Bardhan, Rizia and Halas, Naomi J. and Manoharan, Vinothan N. and Nordlander, Peter and Shvets, Gennady and Capasso, Federico},
  Journal                  = {Science},
  Year                     = {2010},
  Number                   = {5982},
  Pages                    = {1135-1138},
  Volume                   = {328},

  Abstract                 = {The self-assembly of colloids is an alternative to top-down processing that enables the fabrication of nanostructures. We show that self-assembled clusters of metal-dielectric spheres are the basis for nanophotonic structures. By tailoring the number and position of spheres in close-packed clusters, plasmon modes exhibiting strong magnetic and Fano-like resonances emerge. The use of identical spheres simplifies cluster assembly and facilitates the fabrication of highly symmetric structures. Dielectric spacers are used to tailor the interparticle spacing in these clusters to be approximately 2 nanometers. These types of chemically synthesized nanoparticle clusters can be generalized to other two- and three-dimensional structures and can serve as building blocks for new metamaterials.},
  Doi                      = {10.1126/science.1187949},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000278104700037}
}

@Article{Faraon2011,
  Title                    = {Resonant enhancement of the zero-phonon emission from a colour centre in a diamond cavity},
  Author                   = {Faraon, Andrei and Barclay, Paul E. and Santori, Charles and Fu, Kai-Mei C. and Beausoleil, Raymond G.},
  Journal                  = {Nature Photonics},
  Year                     = {2011},
  Number                   = {5},
  Pages                    = {301-305},
  Volume                   = {5},

  Doi                      = {10.1038/nphoton.2011.52},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Faraon2012,
  Title                    = {Coupling of Nitrogen-Vacancy Centers to Photonic Crystal Cavities in Monocrystalline Diamond},
  Author                   = {Faraon, Andrei and Santori, Charles and Huang, Zhihong and Acosta, Victor M. and Beausoleil, Raymond G.},
  Journal                  = {Physical Review Letters},
  Year                     = {2012},
  Number                   = {3},
  Volume                   = {109},

  Doi                      = {10.1103/PhysRevLett.109.033604},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Farrer1969,
  Title                    = {On the substitutional nitrogen donor in diamond},
  Author                   = {Farrer, R. G.},
  Journal                  = {Solid State Communications},
  Year                     = {1969},
  Number                   = {9},
  Pages                    = {685-688},
  Volume                   = {7},

  Abstract                 = {Measurements of photoconduction, optical absorption and resistance as a function of temperature in type Ib diamonds suggest that the level due to the substitutional nitrogen donor in diamond is situated 1.7 eV below the conduction band.},
  Doi                      = {http://dx.doi.org/10.1016/0038-1098(69)90593-6},
  ISSN                     = {0038-1098},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/0038109869905936}
}

@Article{Fedutik2007,
  Title                    = {Exciton-Plasmon-Photon Conversion in Plasmonic Nanostructures},
  Author                   = {Fedutik, Y. and Temnov, V. and SchÃ¶ps, O. and Woggon, U. and Artemyev, M.},
  Journal                  = {Physical Review Letters},
  Year                     = {2007},
  Number                   = {13},
  Volume                   = {99},

  Doi                      = {10.1103/PhysRevLett.99.136802},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Feigelson2015,
  Title                    = {Growth and spectroscopic characterization of monolayer and few-layer hexagonal boron nitride on metal substrates},
  Author                   = {Feigelson, B. N. and Bermudez, V. M. and Hite, J. K. and Robinson, Z. R. and Wheeler, V. D. and Sridhara, K. and Hernandez, S. C.},
  Journal                  = {Nanoscale},
  Year                     = {2015},
  Number                   = {8},
  Pages                    = {3694-702},
  Volume                   = {7},

  Abstract                 = {Atomically thin two dimensional hexagonal boron nitride (2D h-BN) is one of the key materials in the development of new van der Waals heterostructures due to its outstanding properties including an atomically smooth surface, high thermal conductivity, high mechanical strength, chemical inertness and high electrical resistance. The development of 2D h-BN growth is still in the early stages and largely depends on rapid and accurate characterization of the grown monolayer or few layers h-BN films. This paper demonstrates a new approach to characterizing monolayer h-BN films directly on metal substrates by grazing-incidence infrared reflection absorption spectroscopy (IRRAS). Using h-BN films grown by atmospheric-pressure chemical vapor deposition on Cu and Ni substrates, two new sub-bands are found for the A2u out-of-plane stretching mode. It is shown, using both experimental and computational methods, that the lower-energy sub-band is related to 2D h-BN coupled with substrate, while the higher energy sub-band is related to decoupled (or free-standing) 2D h-BN. It is further shown that this newly-observed fine structure in the A2u mode can be used to assess, quickly and easily, the homogeneity of the h-BN-metal interface and the effects of metal surface contamination on adhesion of the layer.},
  Doi                      = {10.1039/c4nr05557h},
  ISSN                     = {2040-3372 (Electronic)
2040-3364 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25640166}
}

@Article{Feng2014,
  Title                    = {Theoretical prediction of the mechanisms for defect healing or oxygen doping in a hexagonal boron nitride (h-BN) sheet with nitrogen vacancies by NO2 molecules},
  Author                   = {Feng, Jing-wen and Liu, Yue-Jie and Zhao, Jing-xiang},
  Journal                  = {Journal of Molecular Modeling},
  Year                     = {2014},
  Number                   = {6},
  Pages                    = {1-7},
  Volume                   = {20},

  Doi                      = {10.1007/s00894-014-2307-4},
  ISSN                     = {1610-2940},
  Keywords                 = {NO2
Healing
Defective hexagonal boron nitride sheet
DFT},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1007/s00894-014-2307-4}
}

@Article{Feng2013,
  Title                    = {Characteristics of plate-like and color-zoning cubic boron nitride crystals},
  Author                   = {Feng, Shuang and Hou, Lixin and Liu, Xiuhuan and Gao, Yanjun and Li, Xinlu and Wang, Qi and Chen, Zhanguo and Jia, Gang and Zheng, Jie},
  Journal                  = {Applied Surface Science},
  Year                     = {2013},
  Number                   = {0},
  Pages                    = {817-822},
  Volume                   = {285, Part B},

  Abstract                 = {The polarities of a kind of plate-like and color-zoning cubic boron nitride (cBN) crystal were extensively investigated by microscopy, chemical etching, XPS, Raman scattering, and currentâ€“voltage measurements. The {1 1 1}B faces and { 1 Â¯ â€‰ 1 Â¯ â€‰ 1 Â¯ } N faces of the cBN samples can be easily distinguished by optical microscope as there are a lot of defects incorporate in { 1 Â¯ â€‰ 1 Â¯ â€‰ 1 Â¯ } N sectors serving as the color centers, while the {1 1 1}B sectors have less defects and are nearly colorless. Both XPS and Raman spectra also revealed the uneven distributions of N vacancies and substitutional impurities in cBN crystals. The determination of {1 1 1}B faces and { 1 Â¯ â€‰ 1 Â¯ â€‰ 1 Â¯ } N faces can also be verified by the results of the chemical etching because the { 1 Â¯ â€‰ 1 Â¯ â€‰ 1 Â¯ } N faces have much faster etch rates than the {1 1 1}B faces. According to XPS, the {1 1 1}B faces have more C and O contaminations than the { 1 Â¯ â€‰ 1 Â¯ â€‰ 1 Â¯ } N faces, however the { 1 Â¯ â€‰ 1 Â¯ â€‰ 1 Â¯ } N faces have larger atomic ratio of B:N after surface cleaning by Ar+ sputtering. In the Raman spectra of the { 1 Â¯ â€‰ 1 Â¯ â€‰ 1 Â¯ } N sectors of cBN, several small broad infrared-active phonon bands emerge nearby TO and LO modes because of the disorder-activated Raman scattering. As for the {1 1 1}B sectors, this phenomenon disappears. In addition, the {1 1 1}B faces have much smaller leakage current than the { 1 Â¯ â€‰ 1 Â¯ â€‰ 1 Â¯ } N faces, which indicates that the {1 1 1}B sectors have higher crystalline quality.},
  Doi                      = {http://dx.doi.org/10.1016/j.apsusc.2013.08.134},
  ISSN                     = {0169-4332},
  Keywords                 = {Wide bandgap semiconductors
IIIâ€“V compounds
Cubic boron nitride
Surface polarity},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0169433213016255}
}

@Article{Fevrier2012,
  Title                    = {Giant coupling effect between metal nanoparticle chain and optical waveguide},
  Author                   = {Fevrier, M. and Gogol, P. and Aassime, A. and Megy, R. and Delacour, C. and Chelnokov, A. and Apuzzo, A. and Blaize, S. and Lourtioz, J. M. and Dagens, B.},
  Journal                  = {Nano Lett},
  Year                     = {2012},
  Number                   = {2},
  Pages                    = {1032-7},
  Volume                   = {12},

  Abstract                 = {We demonstrate that the optical energy carried by a TE dielectric waveguide mode can be totally transferred into a transverse plasmon mode of a coupled metal nanoparticle chain. Experiments are performed at 1.5 mum. Mode coupling occurs through the evanescent field of the dielectric waveguide mode. Giant coupling effects are evidenced from record coupling lengths as short as ~560 nm. This result opens the way to nanometer scale devices based on localized plasmons in photonic integrated circuits.},
  Doi                      = {10.1021/nl204265f},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Gold/*chemistry
Metal Nanoparticles/*chemistry
*Optical Devices
Silicon/chemistry
Surface Plasmon Resonance},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22251002}
}

@Article{Fleury2000,
  Title                    = {Nonclassical Photon Statistics in Single-Molecule Fluorescence at Room Temperature},
  Author                   = {Fleury, L. and Segura, J. M. and Zumofen, G. and Hecht, B. and Wild, U. P.},
  Journal                  = {Physical Review Letters},
  Year                     = {2000},
  Number                   = {6},
  Pages                    = {1148-1151},
  Volume                   = {84},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.84.1148}
}

@Article{Frederich2014,
  Title                    = {Determination of the Surface Plasmon Polariton Extraction Efficiency from a Self-Assembled Plasmonic Crystal},
  Author                   = {Frederich, Hugo and Wen, Fangfang and Laverdant, Julien and de Marcillac, Willy Daney and Schwob, Catherine and Coolen, Laurent and MaÃ®tre, AgnÃ¨s},
  Journal                  = {Plasmonics},
  Year                     = {2014},
  Number                   = {4},
  Pages                    = {917-924},
  Volume                   = {9},

  Doi                      = {10.1007/s11468-014-9697-0},
  ISSN                     = {1557-1955
1557-1963},
  Type                     = {Journal Article}
}

@Article{Fu2007,
  Title                    = {Characterization and application of single fluorescent nanodiamonds as cellular biomarkers},
  Author                   = {Fu, C. C. and Lee, H. Y. and Chen, K. and Lim, T. S. and Wu, H. Y. and Lin, P. K. and Wei, P. K. and Tsao, P. H. and Chang, H. C. and Fann, W.},
  Journal                  = {Proc Natl Acad Sci U S A},
  Year                     = {2007},
  Number                   = {3},
  Pages                    = {727-32},
  Volume                   = {104},

  Abstract                 = {Type Ib diamonds emit bright fluorescence at 550-800 nm from nitrogen-vacancy point defects, (N-V)(0) and (N-V)(-), produced by high-energy ion beam irradiation and subsequent thermal annealing. The emission, together with noncytotoxicity and easiness of surface functionalization, makes nano-sized diamonds a promising fluorescent probe for single-particle tracking in heterogeneous environments. We present the result of our characterization and application of single fluorescent nanodiamonds as cellular biomarkers. We found that, under the same excitation conditions, the fluorescence of a single 35-nm diamond is significantly brighter than that of a single dye molecule such as Alexa Fluor 546. The latter photobleached in the range of 10 s at a laser power density of 10(4) W/cm(2), whereas the nanodiamond particle showed no sign of photobleaching even after 5 min of continuous excitation. Furthermore, no fluorescence blinking was detected within a time resolution of 1 ms. The photophysical properties of the particles do not deteriorate even after surface functionalization with carboxyl groups, which form covalent bonding with polyL-lysines that interact with DNA molecules through electrostatic forces. The feasibility of using surface-functionalized fluorescent nanodiamonds as single-particle biomarkers is demonstrated with both fixed and live HeLa cells.},
  Doi                      = {10.1073/pnas.0605409104},
  ISSN                     = {0027-8424 (Print)
0027-8424 (Linking)},
  Keywords                 = {Biological Markers/analysis/chemistry
DNA/chemistry
Diamond/*analysis/*chemistry
Fluorescence
HeLa Cells
Humans
*Molecular Probe Techniques
Molecular Probes/*analysis/*chemistry
Nanostructures/*analysis/*chemistry
Polylysine/chemistry
Static Electricity},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/17213326}
}

@Article{Fu2010,
  Title                    = {Conversion of neutral nitrogen-vacancy centers to negatively charged nitrogen-vacancy centers through selective oxidation},
  Author                   = {Fu, K. M. C. and Santori, C. and Barclay, P. E. and Beausoleil, R. G.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2010},
  Number                   = {12},
  Pages                    = {121907},
  Volume                   = {96},

  Doi                      = {10.1063/1.3364135},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Fu2014,
  Title                    = {Efficient adiabatic silicon-on-insulator waveguide taper},
  Author                   = {Fu, Yunfei and Ye, Tong and Tang, Weijie and Chu, Tao},
  Journal                  = {Photonics Research},
  Year                     = {2014},
  Number                   = {3},
  Pages                    = {A41},
  Volume                   = {2},

  Doi                      = {10.1364/prj.2.000a41},
  ISSN                     = {2327-9125},
  Type                     = {Journal Article}
}

@Article{Fuchs2013,
  Title                    = {Silicon carbide light-emitting diode as a prospective room temperature source for single photons},
  Author                   = {Fuchs, F. and Soltamov, V. A. and Vath, S. and Baranov, P. G. and Mokhov, E. N. and Astakhov, G. V. and Dyakonov, V.},
  Journal                  = {Sci Rep},
  Year                     = {2013},
  Pages                    = {1637},
  Volume                   = {3},

  Abstract                 = {Generation of single photons has been demonstrated in several systems. However, none of them satisfies all the conditions, e.g. room temperature functionality, telecom wavelength operation, high efficiency, as required for practical applications. Here, we report the fabrication of light-emitting diodes (LEDs) based on intrinsic defects in silicon carbide (SiC). To fabricate our devices we used a standard semiconductor manufacturing technology in combination with high-energy electron irradiation. The room temperature electroluminescence (EL) of our LEDs reveals two strong emission bands in the visible and near infrared (NIR) spectral ranges, associated with two different intrinsic defects. As these defects can potentially be generated at a low or even single defect level, our approach can be used to realize electrically driven single photon source for quantum telecommunication and information processing.},
  Doi                      = {10.1038/srep01637},
  ISSN                     = {2045-2322 (Electronic)
2045-2322 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23572127}
}

@Article{Fuchs2011,
  Title                    = {A quantum memory intrinsic to single nitrogenâ€“vacancy centres in diamond},
  Author                   = {Fuchs, G. D. and Burkard, G. and Klimov, P. V. and Awschalom, D. D.},
  Journal                  = {Nature Physics},
  Year                     = {2011},
  Number                   = {10},
  Pages                    = {789-793},
  Volume                   = {7},

  Doi                      = {10.1038/nphys2026},
  ISSN                     = {1745-2473
1745-2481},
  Type                     = {Journal Article}
}

@Article{Fuchs2010,
  Title                    = {Excited-state spin coherence of a single nitrogenâ€“vacancy centre in diamond},
  Author                   = {Fuchs, G. D. and Dobrovitski, V. V. and Toyli, D. M. and Heremans, F. J. and Weis, C. D. and Schenkel, T. and Awschalom, D. D.},
  Journal                  = {Nature Physics},
  Year                     = {2010},
  Number                   = {9},
  Pages                    = {668-672},
  Volume                   = {6},

  Doi                      = {10.1038/nphys1716},
  ISSN                     = {1745-2473
1745-2481},
  Type                     = {Journal Article}
}

@Article{Gaebel2012,
  Title                    = {Size-reduction of nanodiamonds via air oxidation},
  Author                   = {Gaebel, T. and Bradac, C. and Chen, J. and Say, J. M. and Brown, L. and Hemmer, P. and Rabeau, J. R.},
  Journal                  = {Diamond and Related Materials},
  Year                     = {2012},
  Pages                    = {28-32},
  Volume                   = {21},

  Doi                      = {10.1016/j.diamond.2011.09.002},
  ISSN                     = {09259635},
  Type                     = {Journal Article}
}

@Article{Gaebel2004,
  Title                    = {Stable single-photon source in the near infrared},
  Author                   = {Gaebel, T. and Popa, I. and Gruber, A. and Domhan, M. and Jelezko, F. and Wrachtrup, J.},
  Journal                  = {New Journal of Physics},
  Year                     = {2004},
  Pages                    = {98-98},
  Volume                   = {6},

  Doi                      = {10.1088/1367-2630/6/1/098},
  ISSN                     = {1367-2630},
  Type                     = {Journal Article}
}

@Article{Gao2014,
  Title                    = {Large-scale nanoshaping of ultrasmooth 3D crystalline metallic structures},
  Author                   = {Gao, Huang and Hu, Yaowu and Xuan, Yi and Li, Ji and Yang, Yingling and Martinez, Ramses V. and Li, Chunyu and Luo, Jian and Qi, Minghao and Cheng, Gary J.},
  Journal                  = {Science},
  Year                     = {2014},
  Number                   = {6215},
  Pages                    = {1352-1356},
  Volume                   = {346},

  Abstract                 = {We report a low-cost, high-throughput benchtop method that enables thin layers of metal to be shaped with nanoscale precision by generating ultrahigh-strain-rate deformations. Laser shock imprinting can create three-dimensional crystalline metallic structures as small as 10 nanometers with ultrasmooth surfaces at ambient conditions. This technique enables the successful fabrications of large-area, uniform nanopatterns with aspect ratios as high as 5 for plasmonic and sensing applications, as well as mechanically strengthened nanostructures and metal-graphene hybrid nanodevices.},
  Doi                      = {10.1126/science.1260139},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/346/6215/1352.abstract}
}

@Article{GarcA­a-Vidal2002,
  Title                    = {Transmission and focusing of light in one-dimensional periodically nanostructured metals},
  Author                   = {GarcÃ­a-Vidal, F. and MartÃ­n-Moreno, L.},
  Journal                  = {Physical Review B},
  Year                     = {2002},
  Number                   = {15},
  Volume                   = {66},

  Doi                      = {10.1103/PhysRevB.66.155412},
  ISSN                     = {0163-1829
1095-3795},
  Type                     = {Journal Article}
}

@Article{Gather2010,
  Title                    = {Net optical gain in a plasmonic waveguide embedded in a fluorescent polymer},
  Author                   = {Gather, Malte C. and Meerholz, Klaus and Danz, Norbert and Leosson, Kristjan},
  Journal                  = {Nature Photonics},
  Year                     = {2010},
  Number                   = {7},
  Pages                    = {457-461},
  Volume                   = {4},

  Doi                      = {10.1038/nphoton.2010.121},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Geim2013,
  Title                    = {Van der Waals heterostructures},
  Author                   = {Geim, A. K. and Grigorieva, I. V.},
  Journal                  = {Nature},
  Year                     = {2013},

  Month                    = {Jul 25},
  Number                   = {7459},
  Pages                    = {419-425},
  Volume                   = {499},

  Doi                      = {{10.1038/nature12385}},
  ISSN                     = {{0028-0836}},
  Orcid-numbers            = {{Geim, Andre/0000-0003-2861-8331}},
  Owner                    = {Toan},
  Researcherid-numbers     = {{Geim, Andre/J-7888-2012}},
  Timestamp                = {2015.04.08},
  Unique-id                = {{ISI:000322157900029}}
}

@Article{Geiselmann2014,
  Title                    = {Deterministic optical-near-field-assisted positioning of nitrogen-vacancy centers},
  Author                   = {Geiselmann, M. and Marty, R. and Renger, J. and Garcia de Abajo, F. J. and Quidant, R.},
  Journal                  = {Nano Lett},
  Year                     = {2014},
  Number                   = {3},
  Pages                    = {1520-5},
  Volume                   = {14},

  Abstract                 = {Nanopositioning of single quantum emitters to control their coupling to integrated photonic structures is a crucial step in the fabrication of solid-state quantum optics devices. We use the optical near-field enhancement produced by nanofabricated gold antennas subject to near-infrared illumination to deterministically trap and position single nanodiamonds (NDs) hosting nitrogen-vacancy (NV) centers. The positioning of the NDs at the antenna regions of maximum field intensity is first characterized using both fluorescence and electron microscopy imaging. We further study the interaction between the nanoantenna and the delivered NV center by analyzing its change in fluorescence lifetime, which is driven by the increase in the local density of optical states at the trapping positions. Additionally, the plasmonic enhancement of the near-field intensity allows us to optically control the NV excited lifetime using relatively low NIR illumination intensities, some 20 times lower than in the absence of the antennas.},
  Doi                      = {10.1021/nl4047587},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24571659}
}

@Article{Gengxu2013,
  Title                    = {Photoluminescence Enhancement Dependent on the Orientations of Single NV Centers in Nanodiamonds on a Gold Film},
  Author                   = {Gengxu, Chen and Yan, Liu and Min, Song and Botao, Wu and Wu, E. and Heping, Zeng},
  Journal                  = {Selected Topics in Quantum Electronics, IEEE Journal of},
  Year                     = {2013},
  Number                   = {3},
  Pages                    = {4602404-4602404},
  Volume                   = {19},

  Abstract                 = {We studied the orientations of single Nitrogen-Vacancy (NV) color centers in nanodiamonds on a gold film by defocused imaging with a scanning confocal microscopy system and an electron-multiplying charge-coupled device. It was demonstrated that the perpendicular oriented dipole of single NV color center showed shorter fluorescence lifetime and higher fluorescence intensity than any other oriented ones on account of higher coupling efficiency of local electronic field induced by the surface plasmon resonance on the gold film for a vertical transition dipole.},
  Doi                      = {10.1109/JSTQE.2013.2247977},
  ISSN                     = {1077-260X},
  Keywords                 = {gold
nanophotonics
nanostructured materials
photoluminescence
surface plasmon resonance
electron-multiplying charge-coupled device
electronic field
gold film
nanodiamonds
photoluminescence enhancement
scanning confocal microscopy system
shorter fluorescence lifetime
single nitrogen-vacancy color centers
vertical transition dipole
Films
Fluorescence
Image color analysis
Photonics
Plasmons
Diamond
image orientation analysis},
  Type                     = {Journal Article}
}

@Article{Gisin2002,
  Title                    = {Quantum cryptography},
  Author                   = {Gisin, Nicolas and Ribordy, GrÃ©goire and Tittel, Wolfgang and Zbinden, Hugo},
  Journal                  = {Reviews of Modern Physics},
  Year                     = {2002},
  Number                   = {1},
  Pages                    = {145-195},
  Volume                   = {74},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/RevModPhys.74.145}
}

@Article{Gisin2002a,
  Title                    = {Quantum cryptography},
  Author                   = {Gisin, Nicolas and Ribordy, GrÃ©goire and Tittel, Wolfgang and Zbinden, Hugo},
  Journal                  = {Reviews of Modern Physics},
  Year                     = {2002},
  Number                   = {1},
  Pages                    = {145-195},
  Volume                   = {74},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/RevModPhys.74.145}
}

@Article{Gisin2007,
  Title                    = {Quantum communication},
  Author                   = {Gisin, Nicolas and Thew, Rob},
  Journal                  = {Nature Photonics},
  Year                     = {2007},
  Number                   = {3},
  Pages                    = {165-171},
  Volume                   = {1},

  Abstract                 = {Quantum communication, and indeed quantum information in general, has changed the way we think about quantum physics. In 1984 and 1991, the first protocol for quantum cryptography and the first application of quantum non-locality, respectively, attracted interest from a diverse field of researchers in theoretical and experimental physics, mathematics and computer science. Since then we have seen a fundamental shift in how we understand information when it is encoded in quantum systems. We review the current state of research and future directions in this field of science with special emphasis on quantum key distribution and quantum networks. [ABSTRACT FROM AUTHOR]
Copyright of Nature Photonics is the property of Nature Publishing Group and its content may not be copied or emailed to multiple sites or posted to a listserv without the copyright holder's express written permission. However, users may print, download, or email articles for individual use. This abstract may be abridged. No warranty is given about the accuracy of the copy. Users should refer to the original published version of the material for the full abstract. (Copyright applies to all Abstracts.)},
  Doi                      = {10.1038/nphoton.2007.22},
  ISSN                     = {17494885},
  Keywords                 = {QUANTUM communication
OPTICAL communications
CRYPTOGRAPHY
PHOTONICS
OPTICS},
  Type                     = {Journal Article},
  Url                      = {https://www.lib.uts.edu.au/goto?url=http://search.ebscohost.com/login.aspx?direct=true&db=a9h&AN=24220693&site=ehost-live}
}

@Article{Golberg2010,
  Title                    = {Boron Nitride Nanotubes and Nanosheets},
  Author                   = {Golberg, Dmitri and Bando, Yoshio and Huang, Yang and Terao, Takeshi and Mitome, Masanori and Tang, Chengchun and Zhi, Chunyi},
  Journal                  = {ACS Nano},
  Year                     = {2010},
  Number                   = {6},
  Pages                    = {2979-2993},
  Volume                   = {4},

  Abstract                 = {Hexagonal boron nitride (h-BN) is a layered material with a graphite-like structure in which planar networks of BN hexagons are regularly stacked. As the structural analogue of a carbon nanotube (CNT), a BN nanotube (BNNT) was first predicted in 1994; since then, it has become one of the most intriguing non-carbon nanotubes. Compared with metallic or semiconducting CNTs, a BNNT is an electrical insulator with a band gap of ca. 5 eV, basically independent of tube geometry. In addition, BNNTs possess a high chemical stability, excellent mechanical properties, and high thermal conductivity. The same advantages are likely applicable to a graphene analogue?a monatomic layer of a hexagonal BN. Such unique properties make BN nanotubes and nanosheets a promising nanomaterial in a variety of potential fields such as optoelectronic nanodevices, functional composites, hydrogen accumulators, electrically insulating substrates perfectly matching the CNT, and graphene lattices. This review gives an introduction to the rich BN nanotube/nanosheet field, including the latest achievements in the synthesis, structural analyses, and property evaluations, and presents the purpose and significance of this direction in the light of the general nanotube/nanosheet developments.},
  Doi                      = {10.1021/nn1006495},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn1006495}
}

@Article{Gong2014,
  Title                    = {Vertical and in-plane heterostructures from WS2/MoS2 monolayers},
  Author                   = {Gong, Y. and Lin, J. and Wang, X. and Shi, G. and Lei, S. and Lin, Z. and Zou, X. and Ye, G. and Vajtai, R. and Yakobson, B. I. and Terrones, H. and Terrones, M. and Tay, B. K. and Lou, J. and Pantelides, S. T. and Liu, Z. and Zhou, W. and Ajayan, P. M.},
  Journal                  = {Nat Mater},
  Year                     = {2014},
  Number                   = {12},
  Pages                    = {1135-42},
  Volume                   = {13},

  Abstract                 = {Layer-by-layer stacking or lateral interfacing of atomic monolayers has opened up unprecedented opportunities to engineer two-dimensional heteromaterials. Fabrication of such artificial heterostructures with atomically clean and sharp interfaces, however, is challenging. Here, we report a one-step growth strategy for the creation of high-quality vertically stacked as well as in-plane interconnected heterostructures of WS2/MoS2 via control of the growth temperature. Vertically stacked bilayers with WS2 epitaxially grown on top of the MoS2 monolayer are formed with preferred stacking order at high temperature. A strong interlayer excitonic transition is observed due to the type II band alignment and to the clean interface of these bilayers. Vapour growth at low temperature, on the other hand, leads to lateral epitaxy of WS2 on MoS2 edges, creating seamless and atomically sharp in-plane heterostructures that generate strong localized photoluminescence enhancement and intrinsic p-n junctions. The fabrication of heterostructures from monolayers, using simple and scalable growth, paves the way for the creation of unprecedented two-dimensional materials with exciting properties.},
  Doi                      = {10.1038/nmat4091},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25262094}
}

@Article{Gonzalez-Tudela2011,
  Title                    = {Entanglement of Two Qubits Mediated by One-Dimensional Plasmonic Waveguides},
  Author                   = {Gonzalez-Tudela, A. and Martin-Cano, D. and Moreno, E. and Martin-Moreno, L. and Tejedor, C. and Garcia-Vidal, F. J.},
  Journal                  = {Physical Review Letters},
  Year                     = {2011},
  Number                   = {2},
  Volume                   = {106},

  Doi                      = {10.1103/PhysRevLett.106.020501},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Gorbachev2011,
  Title                    = {Hunting for Monolayer Boron Nitride: Optical and Raman Signatures},
  Author                   = {Gorbachev, Roman V. and Riaz, Ibtsam and Nair, Rahul R. and Jalil, Rashid and Britnell, Liam and Belle, Branson D. and Hill, Ernie W. and Novoselov, Kostya S. and Watanabe, Kenji and Taniguchi, Takashi and Geim, Andre K. and Blake, Peter},
  Journal                  = {Small},
  Year                     = {2011},
  Number                   = {4},
  Pages                    = {465--468},
  Volume                   = {7},

  Doi                      = {10.1002/smll.201001628},
  ISSN                     = {1613-6829},
  Keywords                 = {boron nitride, two-dimensional crystals, graphene, Raman spectra, optical properties},
  Owner                    = {Toan},
  Publisher                = {WILEY-VCH Verlag},
  Timestamp                = {2015.04.01},
  Url                      = {http://dx.doi.org/10.1002/smll.201001628}
}

@Article{Gramotnev2010,
  Title                    = {Plasmonics beyond the diffraction limit},
  Author                   = {Gramotnev, Dmitri K. and Bozhevolnyi, Sergey I.},
  Journal                  = {Nature Photonics},
  Year                     = {2010},
  Number                   = {2},
  Pages                    = {83-91},
  Volume                   = {4},

  Doi                      = {10.1038/nphoton.2009.282},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Grandidier2009,
  Title                    = {Gain-Assisted Propagation in a Plasmonic Waveguide at Telecom Wavelength},
  Author                   = {Grandidier, Jonathan and des Francs, GÃ©rard Colas and Massenot, SÃ©bastien and Bouhelier, Alexandre and Markey, Laurent and Weeber, Jean-Claude and Finot, Christophe and Dereux, Alain},
  Journal                  = {Nano Letters},
  Year                     = {2009},
  Number                   = {8},
  Pages                    = {2935-2939},
  Volume                   = {9},

  Doi                      = {10.1021/nl901314u},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl901314u}
}

@Article{Grigorenko2012,
  Title                    = {Graphene plasmonics},
  Author                   = {Grigorenko, A. N. and Polini, M. and Novoselov, K. S.},
  Journal                  = {Nature Photonics},
  Year                     = {2012},
  Number                   = {11},
  Pages                    = {749-758},
  Volume                   = {6},

  Doi                      = {10.1038/nphoton.2012.262},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Grosse2014,
  Title                    = {Dynamic control of plasmon generation by an individual quantum system},
  Author                   = {Grosse, C. and Kabakchiev, A. and Lutz, T. and Froidevaux, R. and Schramm, F. and Ruben, M. and Etzkorn, M. and Schlickum, U. and Kuhnke, K. and Kern, K.},
  Journal                  = {Nano Lett},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {5693-7},
  Volume                   = {14},

  Abstract                 = {Controlling light on the nanoscale in a similar way as electric currents has the potential to revolutionize the exchange and processing of information. Although light can be guided on this scale by coupling it to plasmons, that is, collective electron oscillations in metals, their local electronic control remains a challenge. Here, we demonstrate that an individual quantum system is able to dynamically gate the electrical plasmon generation. Using a single molecule in a double tunnel barrier between two electrodes we show that this gating can be exploited to monitor fast changes of the quantum system itself and to realize a single-molecule plasmon-generating field-effect transistor operable in the gigahertz range. This opens new avenues toward atomic scale quantum interfaces bridging nanoelectronics and nanophotonics.},
  Doi                      = {10.1021/nl502413k},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25181332}
}

@Article{Gruber1997,
  Title                    = {Scanning Confocal Optical Microscopy and Magnetic Resonance on Single Defect Centers},
  Author                   = {Gruber, A. and DrÃ¤benstedt, A. and Tietz, C. and Fleury, L. and Wrachtrup, J. and Borczyskowski, C. von},
  Journal                  = {Science},
  Year                     = {1997},
  Number                   = {5321},
  Pages                    = {2012-2014},
  Volume                   = {276},

  Abstract                 = {The fluorescence of individual nitrogen-vacancy defect centers in diamond was observed with room-temperature scanning confocal optical microscopy. The centers were photostable, showing no detectable change in their fluorescence emission spectrum as a function of time. Magnetic resonance on single centers at room temperature was shown to be feasible. The magnetic resonance spectra revealed marked changes in zero-field splitting parameters among different centers. These changes were attributed to strain-induced differences in the symmetry of the centers.},
  Doi                      = {10.1126/science.276.5321.2012},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/276/5321/2012.abstract}
}

@Article{Gu2013,
  Title                    = {Super-resolving single nitrogen vacancy centers within single nanodiamonds using a localization microscope},
  Author                   = {Gu, M. and Cao, Y. and Castelletto, S. and Kouskousis, B. and Li, X.},
  Journal                  = {Opt Express},
  Year                     = {2013},
  Number                   = {15},
  Pages                    = {17639-46},
  Volume                   = {21},

  Abstract                 = {In this paper, we show super-resolving single nitrogen vacancy (NV) centers with a sub-20 nanometer resolution in a wide-field localization microscope based on the discovery of photoluminescence blinking in high-pressure high-temperature nanodiamonds (NDs). The photon statistics reveals that NDs containing not only single but also multiple NV centers show photoluminescence blinking. The combination of an atomic force microscope and an optical localization microscope built on the blinking feature enables the optically resolved two NV centers within single NDs for the first time. Our method establishes new avenues for studying nanoscale photon dynamics associated with single NV centers within NDs together with ND-based ultra-sensitive bioimaging devices.},
  Doi                      = {10.1364/OE.21.017639},
  ISSN                     = {1094-4087 (Electronic)
1094-4087 (Linking)},
  Keywords                 = {Image Enhancement/*methods
Luminescent Measurements/*methods
Microscopy/*methods
Nanoparticles/*chemistry/*ultrastructure
Nitrogen/*chemistry},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23938636}
}

@Article{Guler2014,
  Title                    = {Refractory Plasmonics},
  Author                   = {Guler, Urcan and Boltasseva, Alexandra and Shalaev, Vladimir M.},
  Journal                  = {Science},
  Year                     = {2014},
  Number                   = {6181},
  Pages                    = {263-264},
  Volume                   = {344},

  Doi                      = {10.1126/science.1252722},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000334474500023}
}

@Article{Guo2015,
  Title                    = {Magnetism in Oxygen-Functionalized Hexagonal Boron Nitride Nanosheet on Copper Substrate},
  Author                   = {Guo, Yufeng and Guo, Wanlin},
  Journal                  = {The Journal of Physical Chemistry C},
  Year                     = {2015},
  Number                   = {1},
  Pages                    = {873-878},
  Volume                   = {119},

  Doi                      = {10.1021/jp5122799},
  ISSN                     = {1932-7447
1932-7455},
  Type                     = {Journal Article}
}

@Article{Guo2014,
  Title                    = {Insulating to metallic transition of an oxidized boron nitride nanosheet coating by tuning surface oxygen adsorption},
  Author                   = {Guo, Y. and Guo, W.},
  Journal                  = {Nanoscale},
  Year                     = {2014},
  Number                   = {7},
  Pages                    = {3731-6},
  Volume                   = {6},

  Abstract                 = {Surface modification and functionalization are of fundamental importance in actual application of insulating coating, such as hexagon boron nitride (h-BN) nanosheet. Our first-principles calculations reveal that an oxidized h-BN monolayer supported by a Cu substrate exhibits metallic properties when O adatom vertically bonds with the B atom. This is mainly due to the hybridization of the p orbital of the BN layer and O adatom around the Fermi level. Charge transfer from the Cu substrate to the O atom stabilizes the formation of the vertical O-B bond. Injecting negative charges could trigger the migration of the O adatom from the B-N bond to B atom for metal or insulator-supported h-BN monolayer, which will lead to a metallic transition in the oxidized h-BN nanosheet. Our results provide a viable way to tune the electronic properties of surface h-BN coating through charge injection mediated O adsorption.},
  Doi                      = {10.1039/c3nr06227a},
  ISSN                     = {2040-3372 (Electronic)
2040-3364 (Linking)},
  Keywords                 = {Adsorption
Boron Compounds/*chemistry
Copper/chemistry
Graphite/chemistry
Nanostructures/*chemistry
Oxidation-Reduction
Oxygen/*chemistry
Surface Properties},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24569839}
}

@Article{Ha1996,
  Title                    = {Single Molecule Dynamics Studied by Polarization Modulation},
  Author                   = {Ha, T. and Enderle, Th. and Chemla, D. S. and Selvin, P. R. and Weiss, S.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {1996},
  Number                   = {19},
  Pages                    = {3979-3982},
  Volume                   = {77},

  Owner                    = {Toan},
  Publisher                = {American Physical Society},
  Refid                    = {10.1103/PhysRevLett.77.3979},
  Timestamp                = {2015.04.10},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.77.3979}
}

@Article{Ha1999,
  Title                    = {Polarization Spectroscopy of Single Fluorescent Molecules},
  Author                   = {Ha, Taekjip and Laurence, Ted A. and Chemla, Daniel S. and Weiss, Shimon},
  Journal                  = {J. Phys. Chem. B},
  Year                     = {1999},
  Number                   = {33},
  Pages                    = {6839-6850},
  Volume                   = {103},

  Booktitle                = {The Journal of Physical Chemistry B},
  Comment                  = {doi: 10.1021/jp990948j},
  Doi                      = {10.1021/jp990948j},
  ISSN                     = {1520-6106},
  Owner                    = {Toan},
  Publisher                = {American Chemical Society},
  Timestamp                = {2015.04.10},
  Url                      = {http://dx.doi.org/10.1021/jp990948j}
}

@Article{Haes2003,
  Title                    = {A Nanoscale Optical Biosensor:â€‰ The Long Range Distance Dependence of the Localized Surface Plasmon Resonance of Noble Metal Nanoparticles},
  Author                   = {Haes, Amanda J. and Zou, Shengli and Schatz, George C. and Van Duyne, Richard P.},
  Journal                  = {Journal of Physical Chemistry B},
  Year                     = {2003},
  Number                   = {1},
  Pages                    = {109-116},
  Volume                   = {108},

  Doi                      = {10.1021/jp0361327},
  ISSN                     = {1520-6106},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/jp0361327}
}

@Article{Halas2011,
  Title                    = {Plasmons in strongly coupled metallic nanostructures},
  Author                   = {Halas, N. J. and Lal, S. and Chang, W. S. and Link, S. and Nordlander, P.},
  Journal                  = {Chem Rev},
  Year                     = {2011},
  Number                   = {6},
  Pages                    = {3913-61},
  Volume                   = {111},

  Doi                      = {10.1021/cr200061k},
  ISSN                     = {1520-6890 (Electronic)
0009-2665 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/21542636}
}

@Article{Hamon2014,
  Title                    = {Hierarchical Self-Assembly of Gold Nanoparticles into Patterned Plasmonic Nanostructures},
  Author                   = {Hamon, Cyrille and Novikov, Sergey and Scarabelli, Leonardo and Basabe-Desmonts, Lourdes and Liz-MarzÃ¡n, Luis M.},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {10694-10703},
  Volume                   = {8},

  Doi                      = {10.1021/nn504407z},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn504407z}
}

@Article{HanburyBrown1956,
  Title                    = {A Test of a New Type of Stellar Interferometer on Sirius},
  Author                   = {Hanbury Brown, R. and Twiss, R. Q.},
  Journal                  = {Nature},
  Year                     = {1956},
  Number                   = {4541},
  Pages                    = {1046-1048},
  Volume                   = {178},

  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/1781046a0}
}

@Article{Hanson2006,
  Title                    = {Polarization and Readout of Coupled Single Spins in Diamond},
  Author                   = {Hanson, R. and Mendoza, F. and Epstein, R. and Awschalom, D.},
  Journal                  = {Physical Review Letters},
  Year                     = {2006},
  Number                   = {8},
  Volume                   = {97},

  Doi                      = {10.1103/PhysRevLett.97.087601},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Hao2004,
  Title                    = {Electromagnetic fields around silver nanoparticles and dimers},
  Author                   = {Hao, E. and Schatz, G. C.},
  Journal                  = {J Chem Phys},
  Year                     = {2004},
  Number                   = {1},
  Pages                    = {357-66},
  Volume                   = {120},

  Abstract                 = {We use the discrete dipole approximation to investigate the electromagnetic fields induced by optical excitation of localized surface plasmon resonances of silver nanoparticles, including monomers and dimers, with emphasis on what size, shape, and arrangement leads to the largest local electric field (E-field) enhancement near the particle surfaces. The results are used to determine what conditions are most favorable for producing enhancements large enough to observe single molecule surface enhanced Raman spectroscopy. Most of the calculations refer to triangular prisms, which exhibit distinct dipole and quadrupole resonances that can easily be controlled by varying particle size. In addition, for the dimer calculations we study the influence of dimer separation and orientation, especially for dimers that are separated by a few nanometers. We find that the largest /E/2 values for dimers are about a factor of 10 larger than those for all the monomers examined. For all particles and particle orientations, the plasmon resonances which lead to the largest E-fields are those with the longest wavelength dipolar excitation. The spacing of the particles in the dimer plays a crucial role, and we find that the spacing needed to achieve a given /E/2 is proportional to nanoparticle size for particles below 100 nm in size. Particle shape and curvature are of lesser importance, with a head to tail configuration of two triangles giving enhanced fields comparable to head to head, or rounded head to tail. The largest /E/2 values we have calculated for spacings of 2 nm or more is approximately 10(5).},
  Doi                      = {10.1063/1.1629280},
  ISSN                     = {0021-9606 (Print)
0021-9606 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/15267296}
}

@Article{Harats2014,
  Title                    = {Full spectral and angular characterization of highly directional emission from nanocrystal quantum dots positioned on circular plasmonic lenses},
  Author                   = {Harats, M. G. and Livneh, N. and Zaiats, G. and Yochelis, S. and Paltiel, Y. and Lifshitz, E. and Rapaport, R.},
  Journal                  = {Nano Lett},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {5766-71},
  Volume                   = {14},

  Abstract                 = {We design a circular plasmonic lens for collimation of light emission from nanocrystal quantum dots at room temperature in the near IR spectral range. We implement a two-dimensional k-space imaging technique to obtain the full spectral-angular response of the surface plasmon resonance modes of the bare plasmonic lens. This method is also used to map the full spectral-angular emission from nanocrystal quantum dots positioned at the center of the circular plasmonic lens. A narrow directional emitting beam with a divergence angle of only approximately 4.5 degrees full width at half-maximum is achieved with a spectrally broad bandwidth of 30 nm. The spectrally resolved k-space imaging method allows us to get a direct comparison between the spectral-angular response of the resonant surface plasmon modes of the lens and the emission pattern of the quantum dots. This comparison gives a clear and detailed picture of the direct role of these resonant surface waves in directing the emission. The directional emission effect agrees well with calculations based on the coupled mode method. These results are a step toward fabricating an efficient room-temperature single photon source based on nanocrystal quantum dots.},
  Doi                      = {10.1021/nl502652k},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25153365}
}

@Article{Harrison2004,
  Title                    = {Optical spin polarisation of the N-V centre in diamond},
  Author                   = {Harrison, J. and Sellars, M. J. and Manson, N. B.},
  Journal                  = {Journal of Luminescence},
  Year                     = {2004},
  Number                   = {1â€“4},
  Pages                    = {245-248},
  Volume                   = {107},

  Abstract                 = {Low-temperature electron paramagnetic resonance (EPR) spectroscopy has been used to establish the ordering of the ground state spin levels of the nitrogen-vacancy colour centre in diamond. EPR spectroscopy with laser illumination of the sample is used to show that the optically induced spin polarisation observed in the ground state arises due to preferential population of the Sz=0 state.},
  Doi                      = {http://dx.doi.org/10.1016/j.jlumin.2003.12.020},
  ISSN                     = {0022-2313},
  Keywords                 = {EPR
Nitrogen-vacancy centre
Diamond},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0022231303001972}
}

@Article{Hattori2015,
  Title                    = {Layer-by-Layer Dielectric Breakdown of Hexagonal Boron Nitride},
  Author                   = {Hattori, Yoshiaki and Taniguchi, Takashi and Watanabe, Kenji and Nagashio, Kosuke},
  Journal                  = {ACS Nano},
  Year                     = {2015},
  Number                   = {1},
  Pages                    = {916-921},
  Volume                   = {9},

  Abstract                 = {Hexagonal boron nitride (BN) is widely used as a substrate and gate insulator for two-dimensional (2D) electronic devices. The studies on insulating properties and electrical reliability of BN itself, however, are quite limited. Here, we report a systematic investigation of the dielectric breakdown characteristics of BN using conductive atomic force microscopy. The electric field strength was found to be ?12 MV/cm, which is comparable to that of conventional SiO2 oxides because of the covalent bonding nature of BN. After the hard dielectric breakdown, the BN fractured like a flower into equilateral triangle fragments. However, when the applied voltage was terminated precisely in the middle of the dielectric breakdown, the formation of a hole that did not penetrate to the bottom metal electrode was clearly observed. Subsequent I?V measurements of the hole indicated that the BN layer remaining in the hole was still electrically inactive. On the basis of these observations, layer-by-layer breakdown was confirmed for BN with regard to both physical fracture and electrical breakdown. Moreover, statistical analysis of the breakdown voltages using a Weibull plot suggested the anisotropic formation of defects. These results are unique to layered materials and unlike the behavior observed for conventional 3D amorphous oxides.},
  Doi                      = {10.1021/nn506645q},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn506645q}
}

@Article{Hauf2011,
  Title                    = {Chemical control of the charge state of nitrogen-vacancy centers in diamond},
  Author                   = {Hauf, M. V. and Grotz, B. and Naydenov, B. and Dankerl, M. and Pezzagna, S. and Meijer, J. and Jelezko, F. and Wrachtrup, J. and Stutzmann, M. and Reinhard, F. and Garrido, J. A.},
  Journal                  = {Physical Review B},
  Year                     = {2011},
  Number                   = {8},
  Volume                   = {83},

  Doi                      = {10.1103/PhysRevB.83.081304},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Hausmann2014,
  Title                    = {Diamond nonlinear photonics},
  Author                   = {Hausmann, B. J. M. and Bulu, I. and Venkataraman, V. and Deotare, P. and LonÄ?ar, M.},
  Journal                  = {Nature Photonics},
  Year                     = {2014},
  Number                   = {5},
  Pages                    = {369-374},
  Volume                   = {8},

  Doi                      = {10.1038/nphoton.2014.72},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Hausmann2012,
  Title                    = {Diamond nanophotonics and applications in quantum science and technology},
  Author                   = {Hausmann, B. J. M. and Choy, J. T. and Babinec, T. M. and Shields, B. J. and Bulu, I. and Lukin, M. D. and Loncar, Marko},
  Journal                  = {Physica Status Solidi a-Applications and Materials Science},
  Year                     = {2012},
  Number                   = {9},
  Pages                    = {1619-1630},
  Volume                   = {209},

  Abstract                 = {Diamond nanophotonics have evolved tremendously from the study of color centers in bulk single crystals and nanocrystals to their characterization in nanostructured environments. This development was facilitated by the ability to generate monolithic, sophisticated nanodevices in high quality single crystal diamond. Here, we present some recent contributions to the field of diamond nanophotonics: increase in single photon collection from nitrogen vacancy (NV) centers embedded in diamond nanowires, broadband spontaneous emission enhancement of single NV centers in plasmonic resonators, and coupling of single NV centers to planar resonators on-chip.},
  Doi                      = {10.1002/pssa.201200576},
  ISSN                     = {1862-6300},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000308942100003}
}

@Article{He2014,
  Title                    = {Tightly Bound Excitons in Monolayer WSe2},
  Author                   = {He, Keliang and Kumar, Nardeep and Zhao, Liang and Wang, Zefang and Mak, Kin Fai and Zhao, Hui and Shan, Jie},
  Journal                  = {Physical Review Letters},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {026803},
  Volume                   = {113},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.113.026803}
}

@Article{He1993,
  Title                    = {Paramagnetic resonance of photoexcited N-V defects in diamond. I. Level anticrossing in the 3A ground state},
  Author                   = {He, Xing-Fei and Manson, Neil and Fisk, Peter},
  Journal                  = {Physical Review B},
  Year                     = {1993},
  Number                   = {14},
  Pages                    = {8809-8815},
  Volume                   = {47},

  Doi                      = {10.1103/PhysRevB.47.8809},
  ISSN                     = {0163-1829
1095-3795},
  Type                     = {Journal Article}
}

@Article{Hell2007,
  Title                    = {Far-Field Optical Nanoscopy},
  Author                   = {Hell, Stefan W.},
  Journal                  = {Science},
  Year                     = {2007},
  Number                   = {5828},
  Pages                    = {1153-1158},
  Volume                   = {316},

  Abstract                 = {In 1873, Ernst Abbe discovered what was to become a well-known paradigm: the inability of a lens-based optical microscope to discern details that are closer together than half of the wavelength of light. However, for its most popular imaging mode, fluorescence microscopy, the diffraction barrier is crumbling. Here, I discuss the physical concepts that have pushed fluorescence microscopy to the nanoscale, once the prerogative of electron and scanning probe microscopes. Initial applications indicate that emergent far-field optical nanoscopy will have a strong impact in the life sciences and in other areas benefiting from nanoscale visualization.},
  Doi                      = {10.1126/science.1137395},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/316/5828/1153.abstract}
}

@Article{Hess2012,
  Title                    = {Active nanoplasmonic metamaterials},
  Author                   = {Hess, O. and Pendry, J. B. and Maier, S. A. and Oulton, R. F. and Hamm, J. M. and Tsakmakidis, K. L.},
  Journal                  = {Nat Mater},
  Year                     = {2012},
  Number                   = {7},
  Pages                    = {573-84},
  Volume                   = {11},

  Abstract                 = {Optical metamaterials and nanoplasmonics bridge the gap between conventional optics and the nanoworld. Exciting and technologically important capabilities range from subwavelength focusing and stopped light to invisibility cloaking, with applications across science and engineering from biophotonics to nanocircuitry. A problem that has hampered practical implementations have been dissipative metal losses, but the efficient use of optical gain has been shown to compensate these and to allow for loss-free operation, amplification and nanoscopic lasing. Here, we review recent and ongoing progress in the realm of active, gain-enhanced nanoplasmonic metamaterials. On introducing and expounding the underlying theoretical concepts of the complex interaction between plasmons and gain media, we examine the experimental efforts in areas such as nanoplasmonic and metamaterial lasers. We underscore important current trends that may lead to improved active imaging, ultrafast nonlinearities on the nanoscale or cavity-free lasing in the stopped-light regime.},
  Doi                      = {10.1038/nmat3356},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22717488}
}

@Article{Hikmet2005,
  Title                    = {Polarized-Light-Emitting Quantum-Rod Diodes},
  Author                   = {Hikmet, R. â€‰A â€‰M and Chin, P. â€‰T â€‰K and Talapin, D. â€‰V and Weller, H.},
  Journal                  = {Advanced Materials},
  Year                     = {2005},
  Number                   = {11},
  Pages                    = {1436-1439},
  Volume                   = {17},

  Doi                      = {10.1002/adma.200401763},
  ISSN                     = {1521-4095},
  Keywords                 = {Coreâ€“shell particles
Light-emitting diodes, inorganic
Quantum rods},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/adma.200401763}
}

@Article{Hiroshi1996,
  Title                    = {Linear and Nonlinear Optical Properties of CdS and CdSe Nanoparticles Stabilized with Poly(N-vinyl-2-pyrrolidone)},
  Author                   = {Hiroshi, Yao and Shigeru, Takahara and Hirokazu, Mizuma and Takashi, Kozeki and Toyoharu, Hayashi},
  Journal                  = {Japanese Journal of Applied Physics},
  Year                     = {1996},
  Number                   = {9R},
  Pages                    = {4633},
  Volume                   = {35},

  Abstract                 = {CdS and CdSe nanoparticles were prepared in organic solvents in the presence of poly(N-vinyl-2-pyrrolidone) (PVP). PVP plays an essential role in preventing the flocculation of concentrated nanoparticles (stabilizing effect), and in controlling the particle size under the influence of the solvent used. FT-IR measurements were performed to study the effect of the functional groups of PVP on particle size control at molecular levels. The PVP-coated CdS and CdSe nanoparticles obtained were dispersed in acrylonitrile-styrene (AS) copolymer or poly(2-hydroxyethyl methacrylate) (PHEMA) organic films, and third-order nonlinear optical susceptibilities |Ï‡ (3) | of these films were measured using a degenerate four-wave mixing (DFWM) technique. The largest |Ï‡ (3) value of 1.1Ã—10 -7 esu was obtained by excitonic resonant excitation for about 4.0 vol% CdS-doped PHEMA film.},
  ISSN                     = {1347-4065},
  Type                     = {Journal Article},
  Url                      = {http://stacks.iop.org/1347-4065/35/i=9R/a=4633}
}

@Article{Holzmeister2014,
  Title                    = {Quantum yield and excitation rate of single molecules close to metallic nanostructures},
  Author                   = {Holzmeister, Phil and Pibiri, Enrico and Schmied, JÃ¼rgen J. and Sen, Tapasi and Acuna, Guillermo P. and Tinnefeld, Philip},
  Journal                  = {Nat Commun},
  Year                     = {2014},
  Volume                   = {5},

  Abstract                 = {The interaction of dyes and metallic nanostructures strongly affects the fluorescence and can lead to significant fluorescence enhancement at plasmonic hot spots, but also to quenching. Here we present a method to distinguish the individual contributions to the changes of the excitation, radiative and non-radiative rate and use this information to determine the quantum yields for single molecules. The method is validated by precisely placing single fluorescent dyes with respect to gold nanoparticles as well as with respect to the excitation polarization using DNA origami nanostructures. Following validation, measurements in zeromode waveguides reveal that suppression of the radiative rate and enhancement of the non-radiative rate lead to a reduced quantum yield. Because the method exploits the intrinsic blinking of dyes, it can generally be applied to fluorescence measurements in arbitrary nanophotonic environments.},
  Doi                      = {10.1038/ncomms6356},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/ncomms6356}
}

@Article{Hong2014,
  Title                    = {Ultrafast charge transfer in atomically thin MoS(2)/WS(2) heterostructures},
  Author                   = {Hong, X. and Kim, J. and Shi, S. F. and Zhang, Y. and Jin, C. and Sun, Y. and Tongay, S. and Wu, J. and Zhang, Y. and Wang, F.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2014},
  Number                   = {9},
  Pages                    = {682-6},
  Volume                   = {9},

  Abstract                 = {Van der Waals heterostructures have recently emerged as a new class of materials, where quantum coupling between stacked atomically thin two-dimensional layers, including graphene, hexagonal-boron nitride and transition-metal dichalcogenides (MX2), give rise to fascinating new phenomena. MX2 heterostructures are particularly exciting for novel optoelectronic and photovoltaic applications, because two-dimensional MX2 monolayers can have an optical bandgap in the near-infrared to visible spectral range and exhibit extremely strong light-matter interactions. Theory predicts that many stacked MX2 heterostructures form type II semiconductor heterojunctions that facilitate efficient electron-hole separation for light detection and harvesting. Here, we report the first experimental observation of ultrafast charge transfer in photoexcited MoS2/WS2 heterostructures using both photoluminescence mapping and femtosecond pump-probe spectroscopy. We show that hole transfer from the MoS2 layer to the WS2 layer takes place within 50 fs after optical excitation, a remarkable rate for van der Waals coupled two-dimensional layers. Such ultrafast charge transfer in van der Waals heterostructures can enable novel two-dimensional devices for optoelectronics and light harvesting.},
  Doi                      = {10.1038/nnano.2014.167},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25150718}
}

@Article{Hongwei2014,
  Title                    = {Fluorinated graphene and hexagonal boron nitride as ALD seed layers for graphene-based van der Waals heterostructures},
  Author                   = {Hongwei, Guo and Yunlong, Liu and Yang, Xu and Nan, Meng and Hongtao, Wang and Tawfique, Hasan and Xinran, Wang and Jikui, Luo and Bin, Yu},
  Journal                  = {Nanotechnology},
  Year                     = {2014},
  Number                   = {35},
  Pages                    = {355202},
  Volume                   = {25},

  Abstract                 = {Ultrathin dielectric materials prepared by atomic-layer-deposition (ALD) technology are commonly used in graphene electronics. Using the first-principles density functional theory calculations with van der Waals (vdW) interactions included, we demonstrate that single-side fluorinated graphene (SFG) and hexagonal boron nitride ( h -BN) exhibit large physical adsorption energy and strong electrostatic interactions with H 2 O-based ALD precursors, indicating their potential as the ALD seed layer for dielectric growth on graphene. In graphene-SFG vdW heterostructures, graphene is n -doped after ALD precursor adsorption on the SFG surface caused by vertical intrinsic polarization of SFG. However, graphene- h -BN vdW heterostructures help preserving the intrinsic characteristics of the underlying graphene due to in-plane intrinsic polarization of h -BN. By choosing SFG or BN as the ALD seed layer on the basis of actual device design needs, the graphene vdW heterostructures may find applications in low-dimensional electronics.},
  ISSN                     = {0957-4484},
  Type                     = {Journal Article},
  Url                      = {http://stacks.iop.org/0957-4484/25/i=35/a=355202}
}

@Article{Hu2014,
  Title                    = {Designable luminescence with quantum dot-silver plasmon coupler},
  Author                   = {Hu, L. and Wu, H. and Zhang, B. and Du, L. and Xu, T. and Chen, Y. and Zhang, Y.},
  Journal                  = {Small},
  Year                     = {2014},
  Number                   = {15},
  Pages                    = {3099-109},
  Volume                   = {10},

  Abstract                 = {We explore a strongly interacting QDs/Ag plasmonic coupling structure that enables multiple approaches to manipulate light emission from QDs. Group II-VI semiconductor QDs with unique surface states (SSs) impressively modify the plasmonic character of the contiguous Ag nanostructures whereby the localized plasmons (LPs) in the Ag nanostructures can effectively extract the non-radiative SSs of the QDs to radiatively emit via SS-LP resonance. The SS-LP coupling is demonstrated to be readily tunable through surface-state engineering both during QD synthesis and in the post-synthesis stage. The combination of surface-state engineering and band-tailoring engineering allows us to precisely control the luminescence color of the QDs and enables the realization of white-light emission with single-size QDs. Being a versatile metal, the Ag in our optical device functions in multiple ways: as a support for the LPs, for optical reflection, and for electrical conduction. Two application examples of the QDs/Ag plasmon coupler for optical devices are given, an Ag microcavity + plasmon-coupling structure and a new QD light-emitting diode. The new QDs/Ag plasmon coupler opens exciting possibilities in developing novel light sources and biomarker detectors.},
  Doi                      = {10.1002/smll.201400094},
  ISSN                     = {1613-6829 (Electronic)
1613-6810 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24711344}
}

@Article{Hu2014a,
  Title                    = {Proton transport through one-atom-thick crystals},
  Author                   = {Hu, S. and Lozada-Hidalgo, M. and Wang, F. C. and Mishchenko, A. and Schedin, F. and Nair, R. R. and Hill, E. W. and Boukhvalov, D. W. and Katsnelson, M. I. and Dryfe, R. A. W. and Grigorieva, I. V. and Wu, H. A. and Geim, A. K.},
  Journal                  = {Nature},
  Year                     = {2014},
  Number                   = {7530},
  Pages                    = {227},
  Volume                   = {516},

  Doi                      = {10.1038/nature14015},
  Owner                    = {Toan},
  Pm                       = {25470058},
  Ri                       = {Katsnelson, Mikhail/D-4359-2012; Wu, Hengan/A-3646-2009; Wang, Feng-Chao/G-1708-2012},
  Sn                       = {0028-0836},
  Tc                       = {3},
  Timestamp                = {2015.04.09},
  Ut                       = {WOS:000346383500040},
  Z8                       = {0},
  Z9                       = {3},
  Zb                       = {1},
  Zs                       = {0}
}

@Article{Hu2009,
  Title                    = {Synthesis and luminescence of nanodiamonds from carbon black},
  Author                   = {Hu, Shengliang and Tian, Fei and Bai, Peikang and Cao, Shirui and Sun, Jing and Yang, Jing},
  Journal                  = {Materials Science and Engineering: B},
  Year                     = {2009},
  Number                   = {1-3},
  Pages                    = {11-14},
  Volume                   = {157},

  Doi                      = {10.1016/j.mseb.2008.12.001},
  ISSN                     = {09215107},
  Type                     = {Journal Article}
}

@Article{Huang2014,
  Title                    = {Lateral heterojunctions within monolayer MoSe2-WSe2 semiconductors},
  Author                   = {Huang, C. and Wu, S. and Sanchez, A. M. and Peters, J. J. and Beanland, R. and Ross, J. S. and Rivera, P. and Yao, W. and Cobden, D. H. and Xu, X.},
  Journal                  = {Nat Mater},
  Year                     = {2014},
  Number                   = {12},
  Pages                    = {1096-101},
  Volume                   = {13},

  Abstract                 = {Heterojunctions between three-dimensional (3D) semiconductors with different bandgaps are the basis of modern light-emitting diodes, diode lasers and high-speed transistors. Creating analogous heterojunctions between different 2D semiconductors would enable band engineering within the 2D plane and open up new realms in materials science, device physics and engineering. Here we demonstrate that seamless high-quality in-plane heterojunctions can be grown between the 2D monolayer semiconductors MoSe2 and WSe2. The junctions, grown by lateral heteroepitaxy using physical vapour transport, are visible in an optical microscope and show enhanced photoluminescence. Atomically resolved transmission electron microscopy reveals that their structure is an undistorted honeycomb lattice in which substitution of one transition metal by another occurs across the interface. The growth of such lateral junctions will allow new device functionalities, such as in-plane transistors and diodes, to be integrated within a single atomically thin layer.},
  Doi                      = {10.1038/nmat4064},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25150560}
}

@Article{Huang2014a,
  Title                    = {Nanotwinned diamond with unprecedented hardness and stability},
  Author                   = {Huang, Q. and Yu, D. and Xu, B. and Hu, W. and Ma, Y. and Wang, Y. and Zhao, Z. and Wen, B. and He, J. and Liu, Z. and Tian, Y.},
  Journal                  = {Nature},
  Year                     = {2014},
  Number                   = {7504},
  Pages                    = {250-3},
  Volume                   = {510},

  Abstract                 = {Although diamond is the hardest material for cutting tools, poor thermal stability has limited its applications, especially at high temperatures. Simultaneous improvement of the hardness and thermal stability of diamond has long been desirable. According to the Hall-Petch effect, the hardness of diamond can be enhanced by nanostructuring (by means of nanograined and nanotwinned microstructures), as shown in previous studies. However, for well-sintered nanograined diamonds, the grain sizes are technically limited to 10-30 nm (ref. 3), with degraded thermal stability compared with that of natural diamond. Recent success in synthesizing nanotwinned cubic boron nitride (nt-cBN) with a twin thickness down to approximately 3.8 nm makes it feasible to simultaneously achieve smaller nanosize, ultrahardness and superior thermal stability. At present, nanotwinned diamond (nt-diamond) has not been fabricated successfully through direct conversions of various carbon precursors (such as graphite, amorphous carbon, glassy carbon and C60). Here we report the direct synthesis of nt-diamond with an average twin thickness of approximately 5 nm, using a precursor of onion carbon nanoparticles at high pressure and high temperature, and the observation of a new monoclinic crystalline form of diamond coexisting with nt-diamond. The pure synthetic bulk nt-diamond material shows unprecedented hardness and thermal stability, with Vickers hardness up to approximately 200 GPa and an in-air oxidization temperature more than 200 degrees C higher than that of natural diamond. The creation of nanotwinned microstructures offers a general pathway for manufacturing new advanced carbon-based materials with exceptional thermal stability and mechanical properties.},
  Doi                      = {10.1038/nature13381},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24919919}
}

@Article{Huang2014b,
  Title                    = {Tin Disulfideâ€”An Emerging Layered Metal Dichalcogenide Semiconductor: Materials Properties and Device Characteristics},
  Author                   = {Huang, Yuan and Sutter, Eli and Sadowski, Jerzy T. and Cotlet, Mircea and Monti, Oliver L. A. and Racke, David A. and Neupane, Mahesh R. and Wickramaratne, Darshana and Lake, Roger K. and Parkinson, Bruce A. and Sutter, Peter},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {10743-10755},
  Volume                   = {8},

  Abstract                 = {Layered metal dichalcogenides have attracted significant interest as a family of single- and few-layer materials that show new physics and are of interest for device applications. Here, we report a comprehensive characterization of the properties of tin disulfide (SnS2), an emerging semiconducting metal dichalcogenide, down to the monolayer limit. Using flakes exfoliated from layered bulk crystals, we establish the characteristics of single- and few-layer SnS2 in optical and atomic force microscopy, Raman spectroscopy and transmission electron microscopy. Band structure measurements in conjunction with ab initio calculations and photoluminescence spectroscopy show that SnS2 is an indirect bandgap semiconductor over the entire thickness range from bulk to single-layer. Field effect transport in SnS2 supported by SiO2/Si suggests predominant scattering by centers at the support interface. Ultrathin transistors show on?off current ratios >106, as well as carrier mobilities up to 230 cm2/(V s), minimal hysteresis, and near-ideal subthreshold swing for devices screened by a high-k (deionized water) top gate. SnS2 transistors are efficient photodetectors but, similar to other metal dichalcogenides, show a relatively slow response to pulsed irradiation, likely due to adsorbate-induced long-lived extrinsic trap states.},
  Doi                      = {10.1021/nn504481r},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn504481r}
}

@Article{Huck2011,
  Title                    = {Controlled Coupling of a Single Nitrogen-Vacancy Center to a Silver Nanowire},
  Author                   = {Huck, Alexander and Kumar, Shailesh and Shakoor, Abdul and Andersen, Ulrik L.},
  Journal                  = {Physical Review Letters},
  Year                     = {2011},
  Number                   = {9},
  Pages                    = {096801},
  Volume                   = {106},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.106.096801}
}

@Article{Hutter2004,
  Title                    = {Exploitation of localized surface plasmon resonance},
  Author                   = {Hutter, E. and Fendler, J. H.},
  Journal                  = {Advanced Materials},
  Year                     = {2004},
  Number                   = {19},
  Pages                    = {1685-1706},
  Volume                   = {16},

  Abstract                 = {Recent advances in the exploitation of localized surface plasmons (charge density oscillations confined to metallic nanoparticles and nanostructures) in nanoscale optics and photonics, as well as in the construction of sensors and biosensors, are reviewed here. In particular, subsequent to brief surveys of the most-commonly used methods of preparation and arraying of materials with localized surface plasmon resonance (LSPR), and of the optical manifestations of LSPR, attention will be focused on the exploitation of metallic nanostructures as waveguides; as optical transmission, information storage, and nanophotonic devices; as switches; as resonant light scatterers (employed in the different near-field scanning optical microscopies); and finally as sensors and biosensors.},
  Doi                      = {10.1002/adma.200400271},
  ISSN                     = {0935-9648},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000224948300001}
}

@Article{Hwang2003,
  Title                    = {Quantum Key Distribution with High Loss: Toward Global Secure Communication},
  Author                   = {Hwang, Won-Young},
  Journal                  = {Physical Review Letters},
  Year                     = {2003},
  Number                   = {5},
  Volume                   = {91},

  Doi                      = {10.1103/PhysRevLett.91.057901},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Iakoubovskii2000,
  Title                    = {Optical Study of Some Interstitial-Related Centres in CVD Diamond},
  Author                   = {Iakoubovskii, K. and Adriaenssens, G.J.},
  Journal                  = {Phys. Stat. Sol. (a)},
  Year                     = {2000},
  Number                   = {1},
  Pages                    = {59--64},
  Volume                   = {181},

  ISSN                     = {1521-396X},
  Owner                    = {Toan},
  Timestamp                = {2015.04.09},
  Url                      = {http://dx.doi.org/10.1002/1521-396X(200009)181:1<59::AID-PSSA59>3.0.CO;2-D}
}

@Article{Inam2013,
  Title                    = {Emission and Nonradiative Decay of Nanodiamond NV Centers in a Low Refractive Index Environment},
  Author                   = {Inam, Faraz A. and Grogan, Michael D. W. and Rollings, Mathew and Gaebel, Torsten and Say, Jana M. and Bradac, Carlo and Birks, Tim A. and Wadsworth, William J. and Castelletto, Stefania and Rabeau, James R. and Steel, Michael J.},
  Journal                  = {ACS Nano},
  Year                     = {2013},
  Number                   = {5},
  Pages                    = {3833-3843},
  Volume                   = {7},

  Doi                      = {10.1021/nn304202g},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn304202g}
}

@Article{Ismach2012,
  Title                    = {Toward the Controlled Synthesis of Hexagonal Boron Nitride Films},
  Author                   = {Ismach, Ariel and Chou, Harry and Ferrer, Domingo A. and Wu, Yaping and McDonnell, Stephen and Floresca, Herman C. and Covacevich, Alan and Pope, Cody and Piner, Richard and Kim, Moon J. and Wallace, Robert M. and Colombo, Luigi and Ruoff, Rodney S.},
  Journal                  = {ACS Nano},
  Year                     = {2012},
  Number                   = {7},
  Pages                    = {6378-6385},
  Volume                   = {6},

  Abstract                 = {Atomically smooth hexagonal boron nitride (h-BN) layers have very useful properties and thus potential applications for protective coatings, deep ultraviolet (DUV) emitters, and as a dielectric for nanoelectronics devices. In this paper, we report on the growth of h-BN by a low-pressure chemical vapor deposition (LPCVD) process using diborane and ammonia as the gas precursors. The use of LPCVD allows synthesis of h-BN with a controlled number of layers defined by the growth conditions, temperature, time, and gas partial pressure. Furthermore, few-layer h-BN was also grown by a sequential growth method, and insights into the growth mechanism are described, thus forming the basis of future growth of h-BN by atomic layer epitaxy.},
  Doi                      = {10.1021/nn301940k},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn301940k}
}

@Article{Jelezko2004,
  Title                    = {Observation of Coherent Oscillation of a Single Nuclear Spin and Realization of a Two-Qubit Conditional Quantum Gate},
  Author                   = {Jelezko, F. and Gaebel, T. and Popa, I. and Domhan, M. and Gruber, A. and Wrachtrup, J.},
  Journal                  = {Physical Review Letters},
  Year                     = {2004},
  Number                   = {13},
  Volume                   = {93},

  Doi                      = {10.1103/PhysRevLett.93.130501},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Jelezko2004a,
  Title                    = {Observation of Coherent Oscillations in a Single Electron Spin},
  Author                   = {Jelezko, F. and Gaebel, T. and Popa, I. and Gruber, A. and Wrachtrup, J.},
  Journal                  = {Physical Review Letters},
  Year                     = {2004},
  Number                   = {7},
  Volume                   = {92},

  Doi                      = {10.1103/PhysRevLett.92.076401},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Jelezko2002,
  Title                    = {Single spin states in a defect center resolved by optical spectroscopy},
  Author                   = {Jelezko, F. and Popa, I. and Gruber, A. and Tietz, C. and Wrachtrup, J. and Nizovtsev, A. and Kilin, S.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2002},
  Number                   = {12},
  Pages                    = {2160},
  Volume                   = {81},

  Doi                      = {10.1063/1.1507838},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Jelezko2001,
  Title                    = {Spectroscopy of Single N-V Centers in Diamond},
  Author                   = {Jelezko, F. and Tietz, C. and Gruber, A. and Popa, I. and Nizovtsev, A. and Kilin, S. and Wrachtrup, J.},
  Journal                  = {Single Molecules},
  Year                     = {2001},
  Number                   = {4},
  Pages                    = {255-260},
  Volume                   = {2},

  Abstract                 = {Over the past few years, the detection of single N-V centers in diamond has attracted much interest, since it is expected to lead to innovative applications in various domains of quantum information. The N-V center in diamond is a defectconsisting of a substitutional nitrogen atom adjacent to a carbon-atom vacancy. The optical transition between the 3A ground state and the 3E excited state has a very high quantum efficiency allowing single defect spectroscopy. Because of the paramagnetic nature of the ground electronic state, single N-V defects are believed to be promising candidates for solid state quantum computation. To date, however, the photophysics of the defect is not entirely understood. The existence of a singlet metastable state 1A was challenged in a series of papers reporting hole-burning, optically detected magnetic resonance and single molecule experiments. We present here an overview of recent low and room temperature data, indicating the important role of a metastable state of the defect in single center experiments.},
  Doi                      = {10.1002/1438-5171(200112)2:4<255::AID-SIMO255>3.0.CO;2-D},
  ISSN                     = {1438-5171},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/1438-5171(200112)2:4<255::AID-SIMO255>3.0.CO;2-D}
}

@Article{Jelezko2006,
  Title                    = {Single defect centres in diamond: A review},
  Author                   = {Jelezko, F. and Wrachtrup, J.},
  Journal                  = {physica status solidi (a)},
  Year                     = {2006},
  Number                   = {13},
  Pages                    = {3207-3225},
  Volume                   = {203},

  Doi                      = {10.1002/pssa.200671403},
  ISSN                     = {18626300
18626319},
  Type                     = {Journal Article}
}

@Article{Jelezko2004b,
  Title                    = {Read-out of single spins by optical spectroscopy},
  Author                   = {Jelezko, F and Wrachtrup, J},
  Journal                  = {Journal of Physics: Condensed Matter},
  Year                     = {2004},
  Number                   = {30},
  Pages                    = {R1089-},
  Volume                   = {16},

  Abstract                 = {We review recent experiments on optical detection and manipulation of spin states of impurity centres in a solid. This research topic is of particular interest because of possible applications of the single-spin read-out technique in solid state quantum computing. The experimental background of optical detection of single quantum systems in solids is introduced. The interaction of an impurity centre with an excitation field is analysed in terms of optical Bloch equations. Recent experiments on the electron spin resonance of single organic molecules and paramagnetic defect centres in diamonds are presented. We show how the spin state of the nitrogenâ€“vacancy paramagnetic defect in diamond can be read out optically. Pulsed electron spin resonance of the single paramagnetic defect centre in diamond is discussed.},
  ISSN                     = {0953-8984},
  Owner                    = {Toan},
  Timestamp                = {2015.04.10},
  Url                      = {http://stacks.iop.org/0953-8984/16/i=30/a=R03}
}

@Article{Jin2009,
  Title                    = {Fabrication of a Freestanding Boron Nitride Single Layer and Its Defect Assignments},
  Author                   = {Jin, Chuanhong and Lin, Fang and Suenaga, Kazu and Iijima, Sumio},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2009},

  Month                    = may,
  Number                   = {19},
  Pages                    = {195505--},
  Volume                   = {102},

  Owner                    = {Toan},
  Publisher                = {American Physical Society},
  Refid                    = {10.1103/PhysRevLett.102.195505},
  Timestamp                = {2015.04.15},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.102.195505}
}

@Article{Johnson2002,
  Title                    = {Single gallium nitride nanowire lasers},
  Author                   = {Johnson, J. C. and Choi, H. J. and Knutsen, K. P. and Schaller, R. D. and Yang, P. and Saykally, R. J.},
  Journal                  = {Nat Mater},
  Year                     = {2002},
  Number                   = {2},
  Pages                    = {106-10},
  Volume                   = {1},

  Abstract                 = {There is much current interest in the optical properties of semiconductor nanowires, because the cylindrical geometry and strong two-dimensional confinement of electrons, holes and photons make them particularly attractive as potential building blocks for nanoscale electronics and optoelectronic devices, including lasersand nonlinear optical frequency converters. Gallium nitride (GaN) is a wide-bandgap semiconductor of much practical interest, because it is widely used in electrically pumped ultraviolet-blue light-emitting diodes, lasers and photodetectors. Recent progress in microfabrication techniques has allowed stimulated emission to be observed from a variety of GaN microstructures and films. Here we report the observation of ultraviolet-blue laser action in single monocrystalline GaN nanowires, using both near-field and far-field optical microscopy to characterize the waveguide mode structure and spectral properties of the radiation at room temperature. The optical microscope images reveal radiation patterns that correlate with axial Fabry-Perot modes (Q approximately 10(3)) observed in the laser spectrum, which result from the cylindrical cavity geometry of the monocrystalline nanowires. A redshift that is strongly dependent on pump power (45 meV microJ x cm(-2)) supports the idea that the electron-hole plasma mechanism is primarily responsible for the gain at room temperature. This study is a considerable advance towards the realization of electron-injected, nanowire-based ultraviolet-blue coherent light sources.},
  Doi                      = {10.1038/nmat728},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Keywords                 = {Crystallization
Electrons
Equipment Design
Equipment Failure Analysis/methods
Gallium/*chemistry
*Lasers
Materials Testing/methods
Microchemistry/methods
Miniaturization/methods
Nanotechnology/*instrumentation/methods
Nitrogen/*chemistry
Photochemistry/instrumentation/methods
Semiconductors
Sensitivity and Specificity
Ultraviolet Rays},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/12618824}
}

@Article{Joshi1990,
  Title                    = {Oxidation kinetics of diamond, graphite, and chemical vapor deposited diamond films by thermal gravimetry},
  Author                   = {Joshi, A.},
  Journal                  = {Journal of Vacuum Science \& Technology A: Vacuum, Surfaces, and Films},
  Year                     = {1990},
  Number                   = {3},
  Pages                    = {2137},
  Volume                   = {8},

  Doi                      = {10.1116/1.577028},
  ISSN                     = {07342101},
  Type                     = {Journal Article}
}

@Article{Jung2014,
  Title                    = {Chemically Synthesized Heterostructures of Two-Dimensional Molybdenum/Tungsten-Based Dichalcogenides with Vertically Aligned Layers},
  Author                   = {Jung, Yeonwoong and Shen, Jie and Sun, Yong and Cha, Judy J.},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {9},
  Pages                    = {9550-9557},
  Volume                   = {8},

  Abstract                 = {We demonstrate a one-step, facile chemical synthesis of heterostructures based on two-dimensional (2D) transition metal dichalcogenides (TMDCs) with vertically aligned 2D layers. Specifically, by using a chemical vapor transport method, we synthesize molybdenum (Mo)/tungsten (W)-based disulfide and diselenide heterostructures, such as MoS2/WS2 and MoSe2/WSe2. Detailed structural characterizations reveal that the 2D layers of two different TMDCs are vertically standing/aligned exposing the edge sites of the layers. The TMDC heterostructure materials exhibit a high uniformity of structural/chemical heterogeneity over a large area (>1 cm2) and show anisotropic carrier transport properties. These materials with unique heterostructures have great implications for both technological applications and fundamental sciences.},
  Doi                      = {10.1021/nn503853a},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn503853a}
}

@Article{Kaiser1959,
  Title                    = {Nitrogen, A Major Impurity in Common Type I Diamond},
  Author                   = {Kaiser, W. and Bond, W.},
  Journal                  = {Physical Review},
  Year                     = {1959},
  Number                   = {4},
  Pages                    = {857-863},
  Volume                   = {115},

  Doi                      = {10.1103/PhysRev.115.857},
  ISSN                     = {0031-899X
1536-6065},
  Type                     = {Journal Article}
}

@Article{Kauranen2012,
  Title                    = {Nonlinear plasmonics},
  Author                   = {Kauranen, Martti and Zayats, Anatoly V.},
  Journal                  = {Nature Photonics},
  Year                     = {2012},
  Number                   = {11},
  Pages                    = {737-748},
  Volume                   = {6},

  Doi                      = {10.1038/nphoton.2012.244},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Kennedy2003,
  Title                    = {Long coherence times at 300 K for nitrogen-vacancy center spins in diamond grown by chemical vapor deposition},
  Author                   = {Kennedy, T. A. and Colton, J. S. and Butler, J. E. and Linares, R. C. and Doering, P. J.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2003},
  Number                   = {20},
  Pages                    = {4190},
  Volume                   = {83},

  Doi                      = {10.1063/1.1626791},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Khan2015,
  Title                    = {Synthesis of Large and Few Atomic Layers of Hexagonal Boron Nitride on Melted Copper},
  Author                   = {Khan, Majharul Haque and Huang, Zhenguo and Xiao, Feng and Casillas, Gilberto and Chen, Zhixin and Molino, Paul J. and Liu, Hua Kun},
  Journal                  = {Sci. Rep.},
  Year                     = {2015},
  Pages                    = {1-8},
  Volume                   = {5},

  Type                     = {Journal Article}
}

@Article{Khanal2012,
  Title                    = {Generalized Synthesis of Hybrid Metalâ€“Semiconductor Nanostructures Tunable from the Visible to the Infrared},
  Author                   = {Khanal, Bishnu P. and Pandey, Anshu and Li, Liang and Lin, Qianglu and Bae, Wan Ki and Luo, Hongmei and Klimov, Victor I. and Pietryga, Jeffrey M.},
  Journal                  = {ACS Nano},
  Year                     = {2012},
  Number                   = {5},
  Pages                    = {3832-3840},
  Volume                   = {6},

  Doi                      = {10.1021/nn204932m},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn204932m}
}

@Article{Kharintsev2014,
  Title                    = {Experimental Evidence for Axial Anisotropy beyond the Diffraction Limit Induced with a Bias Voltage Plasmonic Nanoantenna and Longitudinal Optical Near-Fields in Photoreactive Polymer Thin Films},
  Author                   = {Kharintsev, Sergey S. and Fishman, Alexander I. and Kazarian, Sergei G. and Gabitov, Ildar R. and Salakhov, Myakzyum Kh},
  Journal                  = {ACS Photonics},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {1025-1032},
  Volume                   = {1},

  Doi                      = {10.1021/ph5002318},
  ISSN                     = {2330-4022
2330-4022},
  Type                     = {Journal Article}
}

@Article{Khon2011,
  Title                    = {Suppression of the plasmon resonance in Au/CdS colloidal nanocomposites},
  Author                   = {Khon, E. and Mereshchenko, A. and Tarnovsky, A. N. and Acharya, K. and Klinkova, A. and Hewa-Kasakarage, N. N. and Nemitz, I. and Zamkov, M.},
  Journal                  = {Nano Lett},
  Year                     = {2011},
  Number                   = {4},
  Pages                    = {1792-9},
  Volume                   = {11},

  Abstract                 = {The nature of exciton-plasmon interactions in Au-tipped CdS nanorods has been investigated using femtosecond transient absorption spectroscopy. The study demonstrates that the key optoelectronic properties of composite heterostructures comprising electrically coupled metal and semiconductor domains are substantially different from those observed in systems with weak interdomain coupling. In particular, strongly coupled nanocomposites promote mixing of electronic states at semiconductor-metal domain interfaces, which causes a significant suppression of both plasmon and exciton excitations of carriers.},
  Doi                      = {10.1021/nl200409x},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Cadmium Compounds/*chemistry
Gold/*chemistry
Light
Materials Testing
Nanostructures/*chemistry/*ultrastructure
Particle Size
Scattering, Radiation
Selenium Compounds/*chemistry
Surface Plasmon Resonance/*methods},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/21417253}
}

@Article{Kildishev2013,
  Title                    = {Planar Photonics with Metasurfaces},
  Author                   = {Kildishev, Alexander V. and Boltasseva, Alexandra and Shalaev, Vladimir M.},
  Journal                  = {Science},
  Year                     = {2013},
  Number                   = {6125},
  Volume                   = {339},

  Abstract                 = {Metamaterials, or engineered materials with rationally designed, subwavelength-scale building blocks, allow us to control the behavior of physical fields in optical, microwave, radio, acoustic, heat transfer, and other applications with flexibility and performance that are unattainable with naturally available materials. In turn, metasurfacesâ€”planar, ultrathin metamaterialsâ€”extend these capabilities even further. Optical metasurfaces offer the fascinating possibility of controlling light with surface-confined, flat components. In the planar photonics concept, it is the reduced dimensionality of the optical metasurfaces that enables new physics and, therefore, leads to functionalities and applications that are distinctly different from those achievable with bulk, multilayer metamaterials. Here, we review the progress in developing optical metasurfaces that has occurred over the past few years with an eye toward the promising future directions in the field.},
  Doi                      = {10.1126/science.1232009},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/339/6125/1232009.abstract}
}

@Article{Kim2012,
  Title                    = {Synthesis and Characterization of Hexagonal Boron Nitride Film as a Dielectric Layer for Graphene Devices},
  Author                   = {Kim, Ki Kang and Hsu, Allen and Jia, Xiaoting and Kim, Soo Min and Shi, Yumeng and Dresselhaus, Mildred and Palacios, Tomas and Kong, Jing},
  Journal                  = {ACS Nano},
  Year                     = {2012},
  Number                   = {10},
  Pages                    = {8583-8590},
  Volume                   = {6},

  Abstract                 = {Hexagonal boron nitride (h-BN) is a promising material as a dielectric layer or substrate for two-dimensional electronic devices. In this work, we report the synthesis of large-area h-BN film using atmospheric pressure chemical vapor deposition on a copper foil, followed by Cu etching and transfer to a target substrate. The growth rate of h-BN film at a constant temperature is strongly affected by the concentration of borazine as a precursor and the ambient gas condition such as the ratio of hydrogen and nitrogen. h-BN films with different thicknesses can be achieved by controlling the growth time or tuning the growth conditions. Transmission electron microscope characterization reveals that these h-BN films are polycrystalline, and the c-axis of the crystallites points to different directions. The stoichiometry ratio of boron and nitrogen is close to 1:1, obtained by electron energy loss spectroscopy. The dielectric constant of h-BN film obtained by parallel capacitance measurements (25 ?m2 large areas) is 2?4. These CVD-grown h-BN films were integrated as a dielectric layer in top-gated CVD graphene devices, and the mobility of the CVD graphene device (in the few thousands cm2/(VÂ·s) range) remains the same before and after device integration.},
  Doi                      = {10.1021/nn301675f},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn301675f}
}

@Article{Kim2012a,
  Title                    = {Synthesis of Monolayer Hexagonal Boron Nitride on Cu Foil Using Chemical Vapor Deposition},
  Author                   = {Kim, Ki Kang and Hsu, Allen and Jia, Xiaoting and Kim, Soo Min and Shi, Yumeng and Hofmann, Mario and Nezich, Daniel and Rodriguez-Nieva, Joaquin F. and Dresselhaus, Mildred and Palacios, Tomas and Kong, Jing},
  Journal                  = {Nano Lett.},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {161-166},
  Volume                   = {12},

  Abstract                 = {Hexagonal boron nitride (h-BN) is very attractive for many applications, particularly, as protective coating, dielectric layer/substrate, transparent membrane, or deep ultraviolet emitter. In this work, we carried out a detailed investigation of h-BN synthesis on Cu substrate using chemical vapor deposition (CVD) with two heating zones under low pressure (LP). Previous atmospheric pressure (AP) CVD syntheses were only able to obtain few layer h-BN without a good control on the number of layers. In contrast, under LPCVD growth, monolayer h-BN was synthesized and time-dependent growth was investigated. It was also observed that the morphology of the Cu surface affects the location and density of the h-BN nucleation. Ammonia borane is used as a BN precursor, which is easily accessible and more stable under ambient conditions than borazine. The h-BN films are characterized by atomic force microscopy, transmission electron microscopy, and electron energy loss spectroscopy analyses. Our results suggest that the growth here occurs via surface-mediated growth, which is similar to graphene growth on Cu under low pressure. These atomically thin layers are particularly attractive for use as atomic membranes or dielectric layers/substrates for graphene devices.},
  Doi                      = {10.1021/nl203249a},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl203249a}
}

@Article{Kim2014,
  Title                    = {Effect of oxygen plasma and thermal oxidation on shallow nitrogen-vacancy centers in diamond},
  Author                   = {Kim, M. and Mamin, H. J. and Sherwood, M. H. and Rettner, C. T. and Frommer, J. and Rugar, D.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2014},
  Number                   = {4},
  Pages                    = {042406},
  Volume                   = {105},

  Doi                      = {10.1063/1.4891839},
  ISSN                     = {0003-6951
1077-3118},
  Type                     = {Journal Article}
}

@Article{Kim2013,
  Title                    = {Synthesis of patched or stacked graphene and hBN flakes: a route to hybrid structure discovery},
  Author                   = {Kim, S. M. and Hsu, A. and Araujo, P. T. and Lee, Y. H. and Palacios, T. and Dresselhaus, M. and Idrobo, J. C. and Kim, K. K. and Kong, J.},
  Journal                  = {Nano Lett},
  Year                     = {2013},
  Number                   = {3},
  Pages                    = {933-41},
  Volume                   = {13},

  Abstract                 = {Two-dimensional (2D) materials such as graphene and hexagonal boron nitride (hBN) have attracted significant attention due to their remarkable properties. Numerous interesting graphene/hBN hybrid structures have been proposed but their implementation has been very limited. In this work, the synthesis of patched structures through consecutive chemical vapor deposition (CVD) on the same substrate was investigated. Both in-plane junctions and stacked layers were obtained. For stacked layers, depending on the synthesis sequence, in one case turbostratic stacking with random rotations were obtained. In another, "AA-like", slightly twisted stacking between graphene and hBN was observed with lattice orientation misalignment consistently to be <1 degrees . Raman characterizations not only confirmed that hBN is a superior substrate but also revealed for the first time that a graphene edge with hBN passivation displays reduced D band intensity compared to an open edge. These studies pave the way for the proposed well-ordered graphene/hBN structures and outline exciting future directions for hybrid 2D materials.},
  Doi                      = {10.1021/nl303760m},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23414526}
}

@Article{Kim2011,
  Title                    = {Full-colour quantum dot displays fabricated by transfer printing},
  Author                   = {Kim, Tae-Ho and Cho, Kyung-Sang and Lee, Eun Kyung and Lee, Sang Jin and Chae, Jungseok and Kim, Jung Woo and Kim, Do Hwan and Kwon, Jang-Yeon and Amaratunga, Gehan and Lee, Sang Yoon and Choi, Byoung Lyong and Kuk, Young and Kim, Jong Min and Kim, Kinam},
  Journal                  = {Nature Photonics},
  Year                     = {2011},
  Number                   = {3},
  Pages                    = {176-182},
  Volume                   = {5},

  Doi                      = {10.1038/nphoton.2011.12},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Klinkova2014,
  Title                    = {Self-assembled plasmonic nanostructures},
  Author                   = {Klinkova, A. and Choueiri, R. M. and Kumacheva, E.},
  Journal                  = {Chem Soc Rev},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {3976-91},
  Volume                   = {43},

  Abstract                 = {Self-assembly of plasmonic nanoparticles offers a labour- and cost-efficient strategy for the expansion of the library of plasmonic nanostructures with highly tunable, coupled optical properties. This review covers recent advances in solution-based self-assembly of plasmonic nanoparticles, modelling of the self-assembly process and of the optical properties of the resulting nanostructures, and potential applications of self-assembled plasmonic nanostructures.},
  Doi                      = {10.1039/c3cs60341e},
  ISSN                     = {1460-4744 (Electronic)
0306-0012 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24599020}
}

@Article{Knill2001,
  Title                    = {A scheme for efficient quantum computation with linear optics},
  Author                   = {Knill, E. and Laflamme, R. and Milburn, G. J.},
  Journal                  = {Nature},
  Year                     = {2001},
  Number                   = {6816},
  Pages                    = {46-52},
  Volume                   = {409},

  Abstract                 = {Quantum computers promise to increase greatly the efficiency of solving problems such as factoring large integers, combinatorial optimization, and quantum physics simulation. One of the greatest challenges now is to implement the basic quantum-computational elements in a physical system and to demonstrate that they can be reliably and scalably controlled. One of the earliest proposals for quantum computation is based on implementing a quantum bit with two optical modes containing one photon. The proposal is appealing because of the ease with which photon interference can be observed. Until now, it suffered from the requirement for nonlinear couplings between optical modes containing few photons. In this work we show that efficient quantum computation is possible using only beam splitters, phase shifters, single photon sources, and photodetectors. Our methods exploit feedback from photodetectors and are robust against errors from photon loss and detector inefficiency. The basic elements are accessible to experimental investigation with current technology. (Author)},
  ISSN                     = {0028-0836, 0028-0836},
  Keywords                 = {Aerospace & High Technology (AH)
ERROR ANALYSIS
PHASE SHIFT
PHOTODETECTORS
OPTICAL DATA PROCESSING
PHOTONS
LINEAR EQUATIONS
BEAM SPLITTERS
QUANTUM COMPUTERS
QUANTUM COMPUTING
Article
74: OPTICS (AH)},
  Type                     = {Journal Article},
  Url                      = {http://ezproxy.lib.uts.edu.au/login?url=http://search.proquest.com/docview/26938564?accountid=17095
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Journal_Search&Ntx=matchallpartial&Ntt=Nature
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Title_Search&Ntx=matchallpartial&Ntt=A+scheme+for+efficient+quantum+computation+with+linear+optics
http://sfx.lib.uts.edu.au/sfx_local?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:journal&genre=article&sid=ProQ:ProQ%3Aaerospace&atitle=A+scheme+for+efficient+quantum+computation+with+linear+optics&title=Nature&issn=00280836&date=2001-01-04&volume=409&issue=6816&spage=46&au=Knill%2C+E%3BLaflamme%2C+R%3BMilburn%2C+G+J&isbn=&jtitle=Nature&btitle=&rft_id=info:eric/&rft_id=info:doi/}
}

@Article{Kociak2014,
  Title                    = {Mapping plasmons at the nanometer scale in an electron microscope},
  Author                   = {Kociak, Mathieu and Stephan, Odile},
  Journal                  = {Chemical Society Reviews},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {3865-3883},
  Volume                   = {43},

  Abstract                 = {In this tutorial review, we present the use of electron energy loss spectroscopy (EELS) and cathodoluminescence (CL) spectroscopy for surface plasmon mapping within metallic nanoparticles. We put a special emphasis on particles that are much smaller than the wavelength of visible light. We start by introducing the concept of surface plasmons, keeping the formalism as simple as possible by focusing on the quasi-static approximation. We then make a link between optical cross-sections, EELS and CL probabilities, and the surface plasmons' physical properties. A short survey of simulation tools is given. We then present typical experimental set-ups and describe some problems frequently encountered with spectrometers. Experimental conditions for improved signal to noise ratio are discussed. Analysis techniques are discussed, especially those related to the spectral imaging mode, which is extremely useful in EELS and CL experiments. Finally, the specific range of applications of EELS and CL with respect to other nano-optic techniques is discussed, as well as the strengths and weaknesses of EELS as compared with CL.},
  Doi                      = {10.1039/C3CS60478K},
  ISSN                     = {0306-0012},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1039/C3CS60478K}
}

@Article{Kolchin2014,
  Title                    = {High Purcell Factor Due To Coupling of a Single Emitter to a Dielectric Slot Waveguide},
  Author                   = {Kolchin, P. and Pholchai, N. and Mikkelsen, M. H. and Oh, J. and Ota, S. and Islam, M. S. and Yin, X. and Zhang, X.},
  Journal                  = {Nano Lett},
  Year                     = {2014},

  Abstract                 = {We demonstrate an all-dielectric quantum electrodynamical nanowire-slab system with a single emitter that concentrates the extremely intense light at the scale of 10 x 75 nm2. The quantum dot exhibits a record high 31-fold spontaneous decay rate enhancement, its optical saturation and blinking are strongly suppressed, and 80% of emission couples into a waveguide mode.},
  Doi                      = {10.1021/nl5037808},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25432015}
}

@Article{Kolesov2009,
  Title                    = {Waveâ€“particle duality of single surface plasmonÂ polaritons},
  Author                   = {Kolesov, Roman and Grotz, Bernhard and Balasubramanian, Gopalakrishnan and StÃ¶hr, Rainer J. and Nicolet, AurÃ©lien A. L. and Hemmer, Philip R. and Jelezko, Fedor and Wrachtrup, JÃ¶rg},
  Journal                  = {Nature Physics},
  Year                     = {2009},
  Number                   = {7},
  Pages                    = {470-474},
  Volume                   = {5},

  Doi                      = {10.1038/nphys1278},
  ISSN                     = {1745-2473
1745-2481},
  Type                     = {Journal Article}
}

@Article{Kolesov2012,
  Title                    = {Optical detection of a single rare-earth ion in a crystal},
  Author                   = {Kolesov, R. and Xia, K. and Reuter, R. and Stohr, R. and Zappe, A. and Meijer, J. and Hemmer, P. R. and Wrachtrup, J.},
  Journal                  = {Nat Commun},
  Year                     = {2012},
  Pages                    = {1029},
  Volume                   = {3},

  Abstract                 = {Rare-earth-doped laser materials show strong prospects for quantum information storage and processing, as well as for biological imaging, due to their high-Q 4f<-->4f optical transitions. However, the inability to optically detect single rare-earth dopants has prevented these materials from reaching their full potential. Here we detect a single photostable Pr(3+) ion in yttrium aluminium garnet nanocrystals with high contrast photon antibunching by using optical upconversion of the excited state population of the 4f<-->4f optical transition into ultraviolet fluorescence. We also demonstrate on-demand creation of Pr(3+) ions in a bulk yttrium aluminium garnet crystal by patterned ion implantation. Finally, we show generation of local nanophotonic structures and cell death due to photochemical effects caused by upconverted ultraviolet fluorescence of praseodymium-doped yttrium aluminium garnet in the surrounding environment. Our study demonstrates versatile use of rare-earth atomic-size ultraviolet emitters for nanoengineering and biotechnological applications.},
  Doi                      = {10.1038/ncomms2034},
  ISSN                     = {2041-1723 (Electronic)
2041-1723 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22929786}
}

@Article{Kottmann2001,
  Title                    = {Plasmon resonant coupling in metallic nanowires},
  Author                   = {Kottmann, Joerg and Martin, Olivier},
  Journal                  = {Optics Express},
  Year                     = {2001},
  Number                   = {12},
  Pages                    = {655-663},
  Volume                   = {8},

  Abstract                 = {We investigate the plasmon resonances of interacting silver nanowires with a 50 nm diameter. Both non-touching and intersecting configurations are investigated. While individual cylinders exhibit a single plasmon resonance, weobserve much more complex spectra of resonances for interacting structures. The number and magnitude of the different resonances depend on the illumination direction and on the distance between the particles. For very small separations, we observe a dramatic field enhancement between the particles, where the electric field amplitude reaches a hundredfold of the illumination. A similar enhancement is observed in the grooves created in slightly intersecting particles. The topology of these different resonances is related to the induced polarization charges. The implication of these results to surface enhanced Raman scattering (SERS) are discussed.},
  Doi                      = {10.1364/OE.8.000655},
  Keywords                 = {Metals
Polaritons
Metal optics
Resonance
Scattering
Scattering, Raman
Micro-optics
Particles},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-8-12-655}
}

@Article{Krasheninnikov2007,
  Title                    = {Engineering of nanostructured carbon materials with electron or ion beams},
  Author                   = {Krasheninnikov, A. V. and Banhart, F.},
  Journal                  = {Nat Mater},
  Year                     = {2007},
  Number                   = {10},
  Pages                    = {723-733},
  Volume                   = {6},

  Comment                  = {10.1038/nmat1996},
  ISSN                     = {1476-1122},
  Owner                    = {Toan},
  Publisher                = {Nature Publishing Group},
  Timestamp                = {2015.04.10},
  Url                      = {http://dx.doi.org/10.1038/nmat1996}
}

@Article{Kresse1996,
  Title                    = {Efficiency of ab-initio total energy calculations for metals and semiconductors using a plane-wave basis set},
  Author                   = {Kresse, G. and Furthmüller, J.},
  Journal                  = {Comput. Mater. Sci.},
  Year                     = {1996},
  Number                   = {1},
  Pages                    = {15--50},
  Volume                   = {6},

  Abstract                 = {We present a detailed description and comparison of algorithms for performing ab-initio quantum-mechanical calculations using pseudopotentials and a plane-wave basis set. We will discuss: (a) partial occupancies within the framework of the linear tetrahedron method and the finite temperature density-functional theory, (b) iterative methods for the diagonalization of the Kohn-Sham Hamiltonian and a discussion of an efficient iterative method based on the ideas of Pulay's residual minimization, which is close to an order Natoms2 scaling even for relatively large systems, (c) efficient Broyden-like and Pulay-like mixing methods for the charge density including a new special â€˜preconditioningâ€™ optimized for a plane-wave basis set, (d) conjugate gradient methods for minimizing the electronic free energy with respect to all degrees of freedom simultaneously. We have implemented these algorithms within a powerful package called VAMP (Vienna ab-initio molecular-dynamics package). The program and the techniques have been used successfully for a large number of different systems (liquid and amorphous semiconductors, liquid simple and transition metals, metallic and semi-conducting surfaces, phonons in simple metals, transition metals and semiconductors) and turned out to be very reliable.},
  ISSN                     = {0927-0256},
  Owner                    = {Toan},
  Timestamp                = {2015.04.14},
  Url                      = {http://www.sciencedirect.com/science/article/pii/0927025696000080}
}

@Article{Kresse1996a,
  Title                    = {Efficient iterative schemes for \textit{ab initio} total-energy calculations using a plane-wave basis set},
  Author                   = {Kresse, G. and Furthmüller, J.},
  Journal                  = {Phys. Rev. B},
  Year                     = {1996},
  Number                   = {16},
  Pages                    = {11169--11186},
  Volume                   = {54},

  Owner                    = {Toan},
  Publisher                = {American Physical Society},
  Refid                    = {10.1103/PhysRevB.54.11169},
  Timestamp                = {2015.04.14},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.54.11169}
}

@Article{Kresse1994,
  Title                    = {\textit{Ab initio} molecular-dynamics simulation of the liquid-metal amorphous-semiconductor transition in germanium},
  Author                   = {Kresse, G. and Hafner, J.},
  Journal                  = {Phys. Rev. B},
  Year                     = {1994},
  Number                   = {20},
  Pages                    = {14251--14269},
  Volume                   = {49},

  Owner                    = {Toan},
  Publisher                = {American Physical Society},
  Refid                    = {10.1103/PhysRevB.49.14251},
  Timestamp                = {2015.04.14},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.49.14251}
}

@Article{Kubota2007,
  Title                    = {Deep Ultraviolet Light-Emitting Hexagonal Boron Nitride Synthesized at Atmospheric Pressure},
  Author                   = {Kubota, Yoichi and Watanabe, Kenji and Tsuda, Osamu and Taniguchi, Takashi},
  Journal                  = {Science},
  Year                     = {2007},
  Number                   = {5840},
  Pages                    = {932-934},
  Volume                   = {317},

  Abstract                 = {Materials emitting light in the deep ultraviolet region around 200 nanometers are essential in a wide-range of applications, such as information storage technology, environmental protection, and medical treatment. Hexagonal boron nitride (hBN), which was recently found to be a promising deep ultraviolet light emitter, has traditionally been synthesized under high pressure and at high temperature. We successfully synthesized high-purity hBN crystals at atmospheric pressure by using a nickel-molybdenum solvent. The obtained hBN crystals emitted intense 215-nanometer luminescence at room temperature. This study demonstrates an easier way to grow high-quality hBN crystals, through their liquid-phase deposition on a substrate at atmospheric pressure.},
  Doi                      = {10.1126/science.1144216},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/317/5840/932.abstract}
}

@Article{Kuhlicke2013,
  Title                    = {In situ observation of plasmon tuning in a single gold nanoparticle during controlled melting},
  Author                   = {Kuhlicke, A. and Schietinger, S. and Matyssek, C. and Busch, K. and Benson, O.},
  Journal                  = {Nano Lett},
  Year                     = {2013},
  Number                   = {5},
  Pages                    = {2041-6},
  Volume                   = {13},

  Abstract                 = {In this Letter we study the relations among shape, symmetry, and plasmon resonance shift in a single gold nanoparticle during laser melting. A beam of an argon ion laser is focused on a selected particle, while its optical and shape properties can be observed with the help of a combined dark-field/photoluminescence microscope and an atomic force microscope, respectively. Starting from a spherical shape, radiation pressure forms the melting gold particle into an upright standing rod on a glass substrate, showing a characteristic dipole scattering pattern. A red-shift of the photoluminescence signal and the scattering spectrum is observed. The melting process can be controlled allowing the formation of different particle heights and plasmon resonance shifts. In situ tuning of the plasmon resonance of individual particles is possible with this reversible melting process.},
  Doi                      = {10.1021/nl400232r},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23627496}
}

@Article{Kulakovich2002,
  Title                    = {Enhanced Luminescence of CdSe Quantum Dots on Gold Colloids},
  Author                   = {Kulakovich, Olga and Strekal, Natalya and Yaroshevich, Alexandr and Maskevich, Sergey and Gaponenko, Sergey and Nabiev, Igor and Woggon, Ulrike and Artemyev, Mikhail},
  Journal                  = {Nano Letters},
  Year                     = {2002},
  Number                   = {12},
  Pages                    = {1449-1452},
  Volume                   = {2},

  Doi                      = {10.1021/nl025819k},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl025819k}
}

@Article{Kumar2013,
  Title                    = {Efficient coupling of a single diamond color center to propagating plasmonic gap modes},
  Author                   = {Kumar, S. and Huck, A. and Andersen, U. L.},
  Journal                  = {Nano Lett},
  Year                     = {2013},
  Number                   = {3},
  Pages                    = {1221-5},
  Volume                   = {13},

  Abstract                 = {We report on coupling of a single nitrogen-vacancy (NV) center in a nanodiamond to the propagating gap mode of two parallel placed chemically grown silver nanowires. The coupled NV-center nanowire system is made by manipulating nanodiamonds and nanowires with the tip of an atomic force microscope cantilever. An efficient coupling of an NV-center to an easily accessible gap plasmon mode is demonstrated and we measure an enhancement of the spontaneous emission decay rate by a factor of 8.3.},
  Doi                      = {10.1021/nl304682r},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23414581}
}

@Article{Kumar2013a,
  Title                    = {Coupling of a single quantum emitter to end-to-end aligned silver nanowires},
  Author                   = {Kumar, Shailesh and Huck, Alexander and Chen, Yuntian and Andersen, Ulrik L.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2013},
  Number                   = {10},
  Pages                    = {103106},
  Volume                   = {102},

  Doi                      = {10.1063/1.4795015},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Kurtsiefer2000,
  Title                    = {Stable solid-state source of single photons},
  Author                   = {Kurtsiefer, C. and Mayer, S. and Zarda, P. and Weinfurter, H.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2000},
  Number                   = {2},
  Pages                    = {290-293},
  Volume                   = {85},

  Abstract                 = {Fluorescence light observed from a single nitrogen-vacancy center in diamond exhibits strong photon antibunching: The measured pair correlation function g((2))(0) shows that only one photon is emitted at a time. Nitrogen-vacancy centers an well localized, stable against photobleaching even at room temperature. and can be addressed in simple experimental configurations.},
  Doi                      = {10.1103/PhysRevLett.85.290},
  ISSN                     = {0031-9007},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000088048700016}
}

@Article{Kutsay2010,
  Title                    = {Studying cubic boron nitride by Raman and infrared spectroscopies},
  Author                   = {Kutsay, O. and Yan, C. and Chong, Y. M. and Ye, Q. and Bello, I. and Zhang, W. J. and Zapien, J. A. and Zhou, Z. F. and Li, Y. K. and Garashchenko, V. and Gontar, A. G. and Novikov, N. V. and Lee, S. T.},
  Journal                  = {Diamond and Related Materials},
  Year                     = {2010},
  Number                   = {7â€“9},
  Pages                    = {968-971},
  Volume                   = {19},

  Abstract                 = {In this paper, optical properties of cubic boron nitride (cBN) in forms of films, powders and monocrystals are studied in vibrational spectral regions. For cBN single crystals, the reststrahlen peak reflectivity of about 95% has been obtained. The second-order Raman scattering spectra induced by visible light excitation is also presented. The infrared two-phonon absorption bands are suggested as additional fingerprints for identification of the cBN nature.},
  Doi                      = {http://dx.doi.org/10.1016/j.diamond.2010.02.033},
  ISSN                     = {0925-9635},
  Keywords                 = {III-Nitrides
Cubic boron nitride
Optical characterization
Raman spectroscopy},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0925963510001147}
}

@Article{Kwak2012,
  Title                    = {Bright and efficient full-color colloidal quantum dot light-emitting diodes using an inverted device structure},
  Author                   = {Kwak, J. and Bae, W. K. and Lee, D. and Park, I. and Lim, J. and Park, M. and Cho, H. and Woo, H. and Yoon do, Y. and Char, K. and Lee, S. and Lee, C.},
  Journal                  = {Nano Lett},
  Year                     = {2012},
  Number                   = {5},
  Pages                    = {2362-6},
  Volume                   = {12},

  Abstract                 = {We report highly bright and efficient inverted structure quantum dot (QD) based light-emitting diodes (QLEDs) by using solution-processed ZnO nanoparticles as the electron injection/transport layer and by optimizing energy levels with the organic hole transport layer. We have successfully demonstrated highly bright red, green, and blue QLEDs showing maximum luminances up to 23,040, 218,800, and 2250 cd/m(2), and external quantum efficiencies of 7.3, 5.8, and 1.7%, respectively. It is also noticeable that they showed turn-on voltages as low as the bandgap energy of each QD and long operational lifetime, mainly attributed to the direct exciton recombination within QDs through the inverted device structure. These results signify a remarkable progress in QLEDs and offer a practicable platform for the realization of QD-based full-color displays and lightings.},
  Doi                      = {10.1021/nl3003254},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22468609}
}

@Article{LA¤nger2009,
  Title                    = {Standardization of quantum key distribution and the ETSI standardization initiative ISG-QKD},
  Author                   = {LÃ¤nger, Thomas and Lenhart, Gaby},
  Journal                  = {New Journal of Physics},
  Year                     = {2009},
  Number                   = {5},
  Pages                    = {055051},
  Volume                   = {11},

  Doi                      = {10.1088/1367-2630/11/5/055051},
  ISSN                     = {1367-2630},
  Type                     = {Journal Article}
}

@Article{Lai2006,
  Title                    = {Structural and Electronic Properties of Fluorinated Boron Nitride Nanotubes},
  Author                   = {Lai, Lin and Song, Wei and Lu, Jing and Gao, Zhengxiang and Nagase, Shigeru and Ni, Ming and Mei, W. N. and Liu, Jianjun and Yu, Dapeng and Ye, Hengqiang},
  Journal                  = {The Journal of Physical Chemistry B},
  Year                     = {2006},
  Number                   = {29},
  Pages                    = {14092-14097},
  Volume                   = {110},

  Abstract                 = {The effects of F doping on the structural and electronic properties of the (5, 5) single-walled boron nitride nanotube (BNNT) are investigated by using the density functional theory method. The chemiadsorption of F maintains the hexagonal BN network, increases the lattice constant, and introduces acceptor impurity states. On the other hand, substitutional doping of F destroys the hexagonal BN network, decreases the lattice constant, but does not alter the insulating feature of the BNNT. The observed insulator-to-semiconducting transition, a lattice contraction, and a highly disordered atom arrangement in the sidewall of BNNTs upon F doping appear to be most reasonably attributed to a codoping of dominating substitutional F over chemiabsorbed F, which can induce deep donor impurity states, a lattice contraction, and a destruction of the hexagonal BN network simultaneously.},
  Doi                      = {10.1021/jp061203y},
  ISSN                     = {1520-6106},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/jp061203y}
}

@Article{Langille2012,
  Title                    = {Stepwise Evolution of Spherical Seeds into 20-Fold Twinned Icosahedra},
  Author                   = {Langille, Mark R. and Zhang, Jian and Personick, Michelle L. and Li, Shuyou and Mirkin, Chad A.},
  Journal                  = {Science},
  Year                     = {2012},
  Number                   = {6097},
  Pages                    = {954-957},
  Volume                   = {337},

  Abstract                 = {Understanding the factors that influence the growth and final shape of noble metal nanostructures is important for controlling their properties. However, relative to their single-crystalline counterparts, the growth of nanoparticles that contain twin defects can be difficult to control because multiple competitive growth pathways can yield such structures. We used spherical, cubic, and octahedral single-crystalline gold nanoparticles as dual electron microscopy labels and plasmonic seeds to track the growth of multiply twinned silver nanostructures. As the bimetallic nanostructures grew, they successively developed twin planes to ultimately form multiply twinned nanoparticles from single-crystalline seeds. Collectively, these data demonstrate how a series of nanoparticles of different shapes and internal crystal structures are interrelated and develop from one another.},
  Doi                      = {10.1126/science.1225653},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/337/6097/954.abstract}
}

@Article{Larson2003,
  Title                    = {Water-Soluble Quantum Dots for Multiphoton Fluorescence Imaging in Vivo},
  Author                   = {Larson, Daniel R. and Zipfel, Warren R. and Williams, Rebecca M. and Clark, Stephen W. and Bruchez, Marcel P. and Wise, Frank W. and Webb, Watt W.},
  Journal                  = {Science},
  Year                     = {2003},
  Number                   = {5624},
  Pages                    = {1434-1436},
  Volume                   = {300},

  Abstract                 = {The use of semiconductor nanocrystals (quantum dots) as fluorescent labels for multiphoton microscopy enables multicolor imaging in demanding biological environments such as living tissue. We characterized water-soluble cadmium selenideâ€“zinc sulfide quantum dots for multiphoton imaging in live animals. These fluorescent probes have two-photon action cross sections as high as 47,000 Goeppert-Mayer units, by far the largest of any label used in multiphoton microscopy. We visualized quantum dots dynamically through the skin of living mice, in capillaries hundreds of micrometers deep. We found no evidence of blinking (fluorescence intermittency) in solution on nanosecond to millisecond time scales.},
  Doi                      = {10.1126/science.1083780},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/300/5624/1434.abstract}
}

@Article{Lassiter2013,
  Title                    = {Plasmonic waveguide modes of film-coupled metallic nanocubes},
  Author                   = {Lassiter, J. B. and McGuire, F. and Mock, J. J. and Ciraci, C. and Hill, R. T. and Wiley, B. J. and Chilkoti, A. and Smith, D. R.},
  Journal                  = {Nano Lett},
  Year                     = {2013},
  Number                   = {12},
  Pages                    = {5866-72},
  Volume                   = {13},

  Abstract                 = {A metallic nanoparticle positioned over a metal film offers great advantages as a highly controllable system relevant for probing field-enhancement and other plasmonic effects. Because the size and shape of the gap between the nanoparticle and film can be controlled to subnanometer precision using relatively simple, bottom-up fabrication approaches, the film-coupled nanoparticle geometry has recently been applied to enhancing optical fields, accessing the quantum regime of plasmonics, and the design of surfaces with controlled reflectance. In the present work, we examine the plasmon modes associated with a silver nanocube positioned above a silver or gold film, separated by an organic, dielectric spacer layer. The film-coupled nanocube is of particular interest due to the formation of waveguide cavity-like modes between the nanocube and film. These modes impart distinctive scattering characteristics to the system that can be used in the creation of controlled reflectance surfaces and other applications. We perform both experimental spectroscopy and numerical simulations of individual nanocubes positioned over a metal film, finding excellent agreement between experiment and simulation. The waveguide mode description serves as a starting point to explain the optical properties observed.},
  Doi                      = {10.1021/nl402660s},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Gold/*chemistry
Light
Metal Nanoparticles/*chemistry
*Optics and Photonics
Silver/chemistry
Surface Plasmon Resonance},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24199752}
}

@Article{LeBlanc2013,
  Title                    = {Enhancement of multiphoton emission from single CdSe quantum dots coupled to gold films},
  Author                   = {LeBlanc, S. J. and McClanahan, M. R. and Jones, M. and Moyer, P. J.},
  Journal                  = {Nano Lett},
  Year                     = {2013},
  Number                   = {4},
  Pages                    = {1662-9},
  Volume                   = {13},

  Abstract                 = {Single molecule time-resolved fluorescence spectroscopy of CdSe/ZnS core-shell quantum dots (QDs) localized near a rough gold thin film demonstrates significant enhancement of multiphoton emission while at the same time showing a decrease in single photon emission. A rigorous analysis of time-resolved photon correlation spectroscopy and fluorescence lifetime data on single quantum dots at room temperature reveals an increase in radiative recombination rate of multiexcitons that is much higher than expected and, perhaps more significantly, is not correlated with concomitant increases in single exciton recombination rates. We believe that these results confirm a stronger coupling of multiexcitons to plasmon modes via a coupling to plasmon multipole modes.},
  Doi                      = {10.1021/nl400117h},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Cadmium Compounds/*chemistry
Gold/*chemistry
Photons
Quantum Dots/*chemistry
Selenium Compounds/*chemistry
Spectrometry, Fluorescence
Sulfides/chemistry
Surface Plasmon Resonance},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23510412}
}

@Article{LefA¨vre2009,
  Title                    = {Thermal stability of irradiation-induced point defects in cubic silicon carbide},
  Author                   = {LefÃ¨vre, JÃ©rÃ©mie and Costantini, Jean-Marc and Esnouf, StÃ©phane and Petite, Guillaume},
  Journal                  = {Journal of Applied Physics},
  Year                     = {2009},
  Number                   = {8},
  Pages                    = {-},
  Volume                   = {106},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.3245397},
  Keywords                 = {thermal stability
photoluminescence
antisite defects
wide band gap semiconductors
interstitials
electron beam effects
silicon compounds
annealing},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/jap/106/8/10.1063/1.3245397}
}

@Article{Lenef1996,
  Title                    = {Electronic structure of the N-V center in diamond: Experiments},
  Author                   = {Lenef, A. and Brown, S. and Redman, D. and Rand, S. and Shigley, J. and Fritsch, E.},
  Journal                  = {Physical Review B},
  Year                     = {1996},
  Number                   = {20},
  Pages                    = {13427-13440},
  Volume                   = {53},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.53.13427}
}

@Article{Leon2012,
  Title                    = {Tailoring Light-Matter Interaction with a Nanoscale Plasmon Resonator},
  Author                   = {de Leon, Nathalie P. and Shields, Brendan J. and Yu, Chun L. and Englund, Dirk E. and Akimov, Alexey V. and Lukin, Mikhail D. and Park, Hongkun},
  Journal                  = {Physical Review Letters},
  Year                     = {2012},
  Number                   = {22},
  Volume                   = {108},

  Doi                      = {10.1103/PhysRevLett.108.226803},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Leung2006,
  Title                    = {Structural analysis of cubic boron nitride films by ultraviolet Raman spectroscopy},
  Author                   = {Leung, K. M. and Li, H. Q. and Zou, Y. S. and Ma, K. L. and Chong, Y. M. and Ye, Q. and Zhang, W. J. and Lee, S. T. and Bello, I.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2006},
  Number                   = {24},
  Pages                    = {241922},
  Volume                   = {88},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.2207994},
  Keywords                 = {boron compounds
Raman spectra
sputter deposition
wide band gap semiconductors
ultraviolet spectra
infrared spectra
Fourier transform spectra
inclusions
semiconductor thin films
semiconductor growth},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/apl/88/24/10.1063/1.2207994}
}

@Article{Lezec2007,
  Title                    = {Negative Refraction at Visible Frequencies},
  Author                   = {Lezec, Henri J. and Dionne, Jennifer A. and Atwater, Harry A.},
  Journal                  = {Science},
  Year                     = {2007},
  Number                   = {5823},
  Pages                    = {430-432},
  Volume                   = {316},

  Abstract                 = {Nanofabricated photonic materials offer opportunities for crafting the propagation and dispersion of light in matter. We demonstrate an experimental realization of a two-dimensional negative-index material in the blue-green region of the visible spectrum, substantiated by direct geometric visualization of negative refraction. Negative indices were achieved with the use of an ultrathin Au-Si3N4-Ag waveguide sustaining a surface plasmon polariton mode with antiparallel group and phase velocities. All-angle negative refraction was observed at the interface between this bimetal waveguide and a conventional Ag-Si3N4-Ag slot waveguide. The results may enable the development of practical negative-index optical designs in the visible regime.},
  Doi                      = {10.1126/science.1139266},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/316/5823/430.abstract}
}

@Article{Li2014,
  Title                    = {Recent Advances of Light Propagation in Surface Plasmon Enhanced Quantum Dot Devices},
  Author                   = {Li, Jin-Jin and Zhu, Ka-Di},
  Journal                  = {Critical Reviews in Solid State and Materials Sciences},
  Year                     = {2014},
  Number                   = {1},
  Pages                    = {25-45},
  Volume                   = {39},

  Doi                      = {10.1080/10408436.2012.668862},
  ISSN                     = {1040-8436
1547-6561},
  Type                     = {Journal Article}
}

@Article{Li2015,
  Title                    = {Efficient Photon Collection from a Nitrogen Vacancy Center in a Circular Bullseye Grating},
  Author                   = {Li, Luozhou and Chen, Edward H. and Zheng, Jiabao and Mouradian, Sara L. and Dolde, Florian and SchrÃ¶der, Tim and Karaveli, Sinan and Markham, Matthew L. and Twitchen, Daniel J. and Englund, Dirk},
  Journal                  = {Nano Letters},
  Year                     = {2015},
  Number                   = {3},
  Pages                    = {1493-1497},
  Volume                   = {15},

  Doi                      = {10.1021/nl503451j},
  Eprint                   = { 
 http://dx.doi.org/10.1021/nl503451j
 
},
  Owner                    = {Toan},
  Timestamp                = {2015.04.08},
  Url                      = { 
 http://dx.doi.org/10.1021/nl503451j
 
}
}

@Article{Li2013,
  Title                    = {High-quality boron nitride nanoribbons: unzipping during nanotube synthesis},
  Author                   = {Li, L. and Li, L. H. and Chen, Y. and Dai, X. J. and Lamb, P. R. and Cheng, B. M. and Lin, M. Y. and Liu, X.},
  Journal                  = {Angew Chem Int Ed Engl},
  Year                     = {2013},
  Number                   = {15},
  Pages                    = {4212-6},
  Volume                   = {52},

  Doi                      = {10.1002/anie.201209597},
  ISSN                     = {1521-3773 (Electronic)
1433-7851 (Linking)},
  Keywords                 = {Boron Compounds/*chemistry
Nanostructures/*chemistry
Particle Size
Surface Properties},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23460119}
}

@Article{Li2014a,
  Title                    = {Resolving Single Plasmons Generated by Multiquantum-Emitters on a Silver Nanowire},
  Author                   = {Li, Qiang and Wei, Hong and Xu, Hongxing},
  Journal                  = {Nano Letters},
  Year                     = {2014},
  Number                   = {6},
  Pages                    = {3358-3363},
  Volume                   = {14},

  Abstract                 = {Surface plasmons, the collective oscillations of electrons at metal surface, provide the ability to enhance the weak interaction between individual quantum emitters and photons for quantum information applications. The generation of single plasmons by coupling silver nanowire with single quantum emitters opens the prospects of using quantum optical techniques to control single surface plasmons and designing novel quantum plasmonic devices. However, the real applications will deal with multiple plasmons generated from multiple quantum emitters. Here we report the first experimental demonstration of resolving single plasmons generated by a pair of quantum dots (QDs) on a silver nanowire waveguide. The accurate positions of the two QDs with separation ranging from micrometers to 200 nm within the diffraction limit are determined by using super-resolution imaging method. The efficiency of plasmon generation due to the exciton?plasmon coupling is obtained for each QD. Our research takes a crucial step toward the experimental study of coupled systems of multiple quantum emitters and plasmonic waveguides and would shed new light on the study of light-matter interactions for potential quantum optics and quantum information applications.},
  Doi                      = {10.1021/nl500838q},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl500838q}
}

@Article{Li2014b,
  Title                    = {Silicon carbide-derived carbon nanocomposite as a substitute for mercury in the catalytic hydrochlorination of acetylene},
  Author                   = {Li, X. and Pan, X. and Yu, L. and Ren, P. and Wu, X. and Sun, L. and Jiao, F. and Bao, X.},
  Journal                  = {Nat Commun},
  Year                     = {2014},
  Pages                    = {3688},
  Volume                   = {5},

  Abstract                 = {Acetylene hydrochlorination is an important coal-based technology for the industrial production of vinyl chloride, however it is plagued by the toxicity of the mercury chloride catalyst. Therefore extensive efforts have been made to explore alternative catalysts with various metals. Here we report that a nanocomposite of nitrogen-doped carbon derived from silicon carbide activates acetylene directly for hydrochlorination in the absence of additional metal species. The catalyst delivers stable performance during a 150 hour test with acetylene conversion reaching 80% and vinyl chloride selectivity over 98% at 200 degrees C. Experimental studies and theoretical simulations reveal that the carbon atoms bonded with pyrrolic nitrogen atoms are the active sites. This proof-of-concept study demonstrates that such a nanocomposite is a potential substitute for mercury while further work is still necessary to bring this to the industrial stage. Furthermore, the finding also provides guidance for design of carbon-based catalysts for activation of other alkynes.},
  Doi                      = {10.1038/ncomms4688},
  ISSN                     = {2041-1723 (Electronic)
2041-1723 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24751500}
}

@Article{Li2012,
  Title                    = {Band-Gap Engineering via Tailored Line Defects in Boron-Nitride Nanoribbons, Sheets, and Nanotubes},
  Author                   = {Li, Xiuling and Wu, Xiaojun and Zeng, Xiao Cheng and Yang, Jinlong},
  Journal                  = {ACS Nano},
  Year                     = {2012},
  Number                   = {5},
  Pages                    = {4104-4112},
  Volume                   = {6},

  Abstract                 = {We perform a comprehensive study of the effects of line defects on electronic and magnetic properties of monolayer boron-nitride (BN) sheets, nanoribbons, and single-walled BN nanotubes using first-principles calculations and Born?Oppenheimer quantum molecular dynamic simulation. Although line defects divide the BN sheet (or nanotube) into domains, we show that certain line defects can lead to tailor-made edges on BN sheets (or imperfect nanotube) that can significantly reduce the band gap of the BN sheet or nanotube. In particular, we find that the line-defect-embedded zigzag BN nanoribbons (LD-zBNNRs) with chemically homogeneous edges such as B- or N-terminated edges can be realized by introducing a B2, N2, or C2 pentagon?octagon?pentagon (5?8?5) line defect or through the creation of the antisite line defect. The LD-zBNNRs with only B-terminated edges are predicted to be antiferromagnetic semiconductors at the ground state, whereas the LD-zBNNRs with only N-terminated edges are metallic with degenerated antiferromagnetic and ferromagnetic states. In addition, we find that the hydrogen-passivated LD-zBNNRs as well as line-defect-embedded BN sheets (and nanotubes) are nonmagnetic semiconductors with markedly reduced band gap. The band gap reduction is attributed to the line-defect-induced impurity states. Potential applications of line-defect-embedded BN nanomaterials include nanoelectronic and spintronic devices.},
  Doi                      = {10.1021/nn300495t},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn300495t}
}

@Article{Li2010,
  Title                    = {Correlation between incident and emission polarization in nanowire surface plasmon waveguides},
  Author                   = {Li, Z. and Bao, K. and Fang, Y. and Huang, Y. and Nordlander, P. and Xu, H.},
  Journal                  = {Nano Lett},
  Year                     = {2010},
  Number                   = {5},
  Pages                    = {1831-5},
  Volume                   = {10},

  Abstract                 = {Nanowire plasmons can be launched by illumination at one terminus of the nanowire and emission can be detected at the other end of the wire. Using polarization dependent dark-field scattering spectroscopy, we measure how the polarization of the emitted light depends on the polarization of the incident light. We observe that the shape of the nanowire termination plays an important role in determining this polarization change. Depending on termination shape, a nanowire can serve as either a polarization-maintaining waveguide, or as a polarization-rotating, nanoscale half-wave plate. The understanding of how plasmonic waveguiding influence the polarization of the guided light is important for optimizing the structure of integrated plasmonic devices.},
  Doi                      = {10.1021/nl100528c},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Computer Simulation
Equipment Design
Equipment Failure Analysis
Light
Materials Testing
*Models, Chemical
Nanostructures/*chemistry/ultrastructure
Nanotechnology/*instrumentation
Particle Size
Refractometry/*instrumentation
Scattering, Radiation
Surface Plasmon Resonance/*instrumentation},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20369891}
}

@Article{Lim2005,
  Title                    = {Repeat-Until-Success Linear Optics Distributed Quantum Computing},
  Author                   = {Lim, Yuan and Beige, Almut and Kwek, Leong},
  Journal                  = {Physical Review Letters},
  Year                     = {2005},
  Number                   = {3},
  Volume                   = {95},

  Doi                      = {10.1103/PhysRevLett.95.030505},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Lin2014,
  Title                    = {Trapping particles using waveguide-coupled gold bowtie plasmonic tweezers},
  Author                   = {Lin, P. T. and Chu, H. Y. and Lu, T. W. and Lee, P. T.},
  Journal                  = {Lab Chip},
  Year                     = {2014},
  Number                   = {24},
  Pages                    = {4647-52},
  Volume                   = {14},

  Abstract                 = {We propose and demonstrate a trapping configuration integrating coupled waveguides and gold bowtie structures to form near-field plasmonic tweezers. Compared with excitation from the top, waves coupled through the waveguide can excite specific bowties on the waveguide and trap particles precisely. Thus this scheme is more efficient and compact, and will assist the circuit design on a chip. With lightning rod and gap effects, the gold bowtie structures can generate highly concentrated resonant fields and induce trapping forces as strong as 652 pN W(-1) on particles with diameters as small as 20 nm. This trapping capability is investigated numerically and verified experimentally with observations of the transport, trapping, and release of particles in the system.},
  Doi                      = {10.1039/c4lc00731j},
  ISSN                     = {1473-0189 (Electronic)
1473-0189 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25288366}
}

@Article{Lin2012,
  Title                    = {Advances in 2D boron nitride nanostructures: nanosheets, nanoribbons, nanomeshes, and hybrids with graphene},
  Author                   = {Lin, Y. and Connell, J. W.},
  Journal                  = {Nanoscale},
  Year                     = {2012},
  Number                   = {22},
  Pages                    = {6908-39},
  Volume                   = {4},

  Abstract                 = {The recent surge in graphene research has stimulated interest in the investigation of various 2-dimensional (2D) nanomaterials. Among these materials, the 2D boron nitride (BN) nanostructures are in a unique position. This is because they are the isoelectric analogs to graphene structures and share very similar structural characteristics and many physical properties except for the large band gap. The main forms of the 2D BN nanostructures include nanosheets (BNNSs), nanoribbons (BNNRs), and nanomeshes (BNNMs). BNNRs are essentially BNNSs with narrow widths in which the edge effects become significant; BNNMs are also variations of BNNSs, which are supported on certain metal substrates where strong interactions and the lattice mismatch between the substrate and the nanosheet result in periodic shallow regions on the nanosheet surface. Recently, the hybrids of 2D BN nanostructures with graphene, in the form of either in-plane hybrids or inter-plane heterolayers, have also drawn much attention. In particular, the BNNS-graphene heterolayer architectures are finding important electronic applications as BNNSs may serve as excellent dielectric substrates or separation layers for graphene electronic devices. In this article, we first discuss the structural basics, spectroscopic signatures, and physical properties of the 2D BN nanostructures. Then, various top-down and bottom-up preparation methodologies are reviewed in detail. Several sections are dedicated to the preparation of BNNRs, BNNMs, and BNNS-graphene hybrids, respectively. Following some more discussions on the applications of these unique materials, the article is concluded with a summary and perspectives of this exciting new field.},
  Doi                      = {10.1039/c2nr32201c},
  ISSN                     = {2040-3372 (Electronic)
2040-3364 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23023445}
}

@Article{Lingner2001,
  Title                    = {Structure of the silicon vacancy in 6H-SiC after annealing identified as the carbon vacancy\char21{}carbon antisite pair},
  Author                   = {Lingner, Th and Greulich-Weber, S. and Spaeth, J. M. and Gerstmann, U. and Rauls, E. and Hajnal, Z. and Frauenheim, Th and Overhof, H.},
  Journal                  = {Physical Review B},
  Year                     = {2001},
  Number                   = {24},
  Pages                    = {245212},
  Volume                   = {64},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.64.245212}
}

@Article{Linic2011,
  Title                    = {Plasmonic-metal nanostructures for efficient conversion of solar to chemical energy},
  Author                   = {Linic, S. and Christopher, P. and Ingram, D. B.},
  Journal                  = {Nat Mater},
  Year                     = {2011},
  Number                   = {12},
  Pages                    = {911-21},
  Volume                   = {10},

  Abstract                 = {Recent years have seen a renewed interest in the harvesting and conversion of solar energy. Among various technologies, the direct conversion of solar to chemical energy using photocatalysts has received significant attention. Although heterogeneous photocatalysts are almost exclusively semiconductors, it has been demonstrated recently that plasmonic nanostructures of noble metals (mainly silver and gold) also show significant promise. Here we review recent progress in using plasmonic metallic nanostructures in the field of photocatalysis. We focus on plasmon-enhanced water splitting on composite photocatalysts containing semiconductor and plasmonic-metal building blocks, and recently reported plasmon-mediated photocatalytic reactions on plasmonic nanostructures of noble metals. We also discuss the areas where major advancements are needed to move the field of plasmon-mediated photocatalysis forward.},
  Doi                      = {10.1038/nmat3151},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22109608}
}

@Article{Liu2005,
  Title                    = {Novel surface plasmon waveguide for high integration},
  Author                   = {Liu, Liu and Han, Zhanghua and He, Sailing},
  Journal                  = {Optics Express},
  Year                     = {2005},
  Number                   = {17},
  Pages                    = {6645-6650},
  Volume                   = {13},

  Abstract                 = {A novel surface plasmon waveguide structure is proposed for highly integrated planar lightwave circuits. By etching a small trench through a metallic thin film on a silica substrate, a guided mode with highly confined light fields is realized. The mode properties of the proposed structure are studied. The necessity of using a polymer upper-cladding is discussed. The coupling between two closely positioned waveguides and a 90o bending are also studied numerically. Sharp bending and high integration can be realized with the present surface plasmon waveguide. The proposed structure is easy to fabricate as compared with some other types of surface plasmon waveguides for high integration.},
  Doi                      = {10.1364/OPEX.13.006645},
  Keywords                 = {Guided waves
Surface plasmons
Photonic integrated circuits},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-13-17-6645}
}

@Article{Liu2010,
  Title                    = {Light-driven nanoscale plasmonic motors},
  Author                   = {Liu, M. and Zentgraf, T. and Liu, Y. and Bartal, G. and Zhang, X.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2010},
  Number                   = {8},
  Pages                    = {570-3},
  Volume                   = {5},

  Abstract                 = {When Sir William Crookes developed a four-vaned radiometer, also known as the light-mill, in 1873, it was believed that this device confirmed the existence of linear momentum carried by photons, as predicted by Maxwell's equations. Although Reynolds later proved that the torque on the radiometer was caused by thermal transpiration, researchers continued to search for ways to take advantage of the momentum of photons and to use it for generating rotational forces. The ability to provide rotational force at the nanoscale could open up a range of applications in physics, biology and chemistry, including DNA unfolding and sequencing and nanoelectromechanical systems. Here, we demonstrate a nanoscale plasmonic structure that can, when illuminated with linearly polarized light, generate a rotational force that is capable of rotating a silica microdisk that is 4,000 times larger in volume. Furthermore, we can control the rotation velocity and direction by varying the wavelength of the incident light to excite different plasmonic modes.},
  Doi                      = {10.1038/nnano.2010.128},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {Crystallization/methods
Energy Transfer/radiation effects
Equipment Design
Equipment Failure Analysis
Gold/*chemistry/radiation effects
Light
Materials Testing
Molecular Conformation/radiation effects
Motion
Nanostructures/*chemistry/radiation effects/*ultrastructure
Nanotechnology/*instrumentation
Particle Size
Photons
Surface Plasmon Resonance/*instrumentation},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20601945}
}

@Article{Liu2011,
  Title                    = {Three-Dimensional Plasmon Rulers},
  Author                   = {Liu, Na and Hentschel, Mario and Weiss, Thomas and Alivisatos, A. Paul and Giessen, Harald},
  Journal                  = {Science},
  Year                     = {2011},
  Number                   = {6036},
  Pages                    = {1407-1410},
  Volume                   = {332},

  Abstract                 = {Plasmon rulers can be used to determine nanoscale distances within chemical or biological species. They are based on the spectral shift of the scattering spectrum when two plasmonic nanoparticles approach one another. However, the one-dimensionality of current plasmon rulers hampers the comprehensive understanding of many intriguing processes in soft matter, which take place in three dimensions. We demonstrated a three-dimensional plasmon ruler that is based on coupled plasmonic oligomers in combination with high-resolution plasmon spectroscopy. This enables retrieval of the complete spatial configuration of complex macromolecular and biological processes as well as their dynamic evolution.},
  Doi                      = {10.1126/science.1199958},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000291689000035}
}

@Article{Liu2008,
  Title                    = {Surface plasmon propagation in a pair of metal nanowires coupled to a nanosized optical emitter},
  Author                   = {Liu, Shao-Ding and Cheng, Mu-Tian and Yang, Zhong-Jian and Wang, Qu-Quan},
  Journal                  = {Optics Letters},
  Year                     = {2008},
  Number                   = {8},
  Pages                    = {851-853},
  Volume                   = {33},

  Abstract                 = {The coupling, propagations, and far-field emissions of surface plasmons in a pair of Au nanowires with a dipole emitter have been investigated using the finite-difference time domain method. The surface plasmon wavelength is tunable from 650 to 380 nm by adjusting the distance between the two wires, which leads to an enhancement of coupling constant and density of states of the surface plasmon. The converted energy from the dipole emitter to the propagating surface plasmon as well as the far-field emission intensity of a pair of Au nanowires increase to approximately four times as large as those of a single nanowire. (C) 2008 Optical Society of America.},
  Doi                      = {10.1364/ol.33.000851},
  ISSN                     = {0146-9592},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000255769100031}
}

@Article{Liu2014,
  Title                    = {Heavily-doped colloidal semiconductor and metal oxide nanocrystals: an emerging new class of plasmonic nanomaterials},
  Author                   = {Liu, X. and Swihart, M. T.},
  Journal                  = {Chem Soc Rev},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {3908-20},
  Volume                   = {43},

  Abstract                 = {The creation and study of non-metallic nanomaterials that exhibit localized surface plasmon resonance (LSPR) interactions with light is a rapidly growing field of research. These doped nanocrystals, mainly self-doped semiconductor nanocrystals (NCs) and extrinsically-doped metal oxide NCs, have extremely high concentrations of free charge carriers, which allows them to exhibit LSPR at near infrared (NIR) wavelengths. In this tutorial review, we discuss recent progress in developing and synthesizing doped semiconductor and metal oxide nanocrystals with LSPR, and in studying the optical properties of these plasmonic nanocrystals. We go on to discuss their growing potential for advancing biomedical and optoelectronic applications.},
  Doi                      = {10.1039/c3cs60417a},
  ISSN                     = {1460-4744 (Electronic)
0306-0012 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24566528}
}

@Article{Liu2011a,
  Title                    = {Plasmon-enhanced photoluminescence from bioconjugated gold nanoparticle and nanodiamond assembly},
  Author                   = {Liu, Y. L. and Sun, K. W.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2011},
  Number                   = {15},
  Pages                    = {153702},
  Volume                   = {98},

  Doi                      = {10.1063/1.3576852},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Liz-Marzan2014,
  Title                    = {Nanoplasmonics},
  Author                   = {Liz-Marzan, L. M. and Murphy, C. J. and Wang, J.},
  Journal                  = {Chem Soc Rev},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {3820-2},
  Volume                   = {43},

  Doi                      = {10.1039/c4cs90026j},
  ISSN                     = {1460-4744 (Electronic)
0306-0012 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24728184}
}

@Article{Loncar2013,
  Title                    = {Quantum photonic networks in diamond},
  Author                   = {Loncar, Marko and Faraon, Andrei},
  Journal                  = {Mrs Bulletin},
  Year                     = {2013},
  Number                   = {2},
  Pages                    = {144-148},
  Volume                   = {38},

  Abstract                 = {Advances in nanotechnology have enabled the opportunity to fabricate nanoscale optical devices and chip-scale systems in diamond that can generate, manipulate, and store optical signals at the single-photon level. In particular, nanophotonics has emerged as a powerful interface between optical elements such as optical fibers and lenses, and solid-state quantum objects such as luminescent color centers in diamond that can be used effectively to manipulate quantum information. While quantum science and technology has been the main driving force behind recent interest in diamond nanophotonics, such a platform would have many applications that go well beyond the quantum realm. For example, diamond's transparency over a wide wavelength range, large third-order nonlinearity, and excellent thermal properties are of great interest for the implementation of frequency combs and integrated Raman lasers. Diamond is also an inert material that makes it well suited for biological applications and for devices that must operate in harsh environments.},
  Doi                      = {10.1557/mrs.2013.19},
  ISSN                     = {0883-7694},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000317549500011}
}

@Article{Loubser1978,
  Title                    = {Electron spin resonance in the study of diamond},
  Author                   = {Loubser, J. H. N. and Wyk, J. A. van},
  Journal                  = {Reports on Progress in Physics},
  Year                     = {1978},
  Number                   = {8},
  Pages                    = {1201},
  Volume                   = {41},

  Abstract                 = {The role of electron spin resonance in the study of both natural and synthetic diamond is reviewed. A brief survey of the physical significance of the constants in the spin Hamiltonian, as well as experimental technique, is given. The various nitrogen centres are discussed treating exchange-interaction, Jahn-Teller and relaxation effects associated with these centres. The spin Hamiltonian parameters of these centres are tabled and the results are discussed within the framework of the defect molecule approach. In conclusion, the correlation between optical effects and the ESR measurements in the case of four defect centres are discussed in some detail as this seems to be a powerful method of testing the various models suggested for the observed defects.},
  ISSN                     = {0034-4885},
  Type                     = {Journal Article},
  Url                      = {http://stacks.iop.org/0034-4885/41/i=8/a=002}
}

@Article{Lounis2000,
  Title                    = {Photon antibunching in single CdSe/ZnS quantum dot fluorescence},
  Author                   = {Lounis, B. and Bechtel, H. A. and Gerion, D. and Alivisatos, P. and Moerner, W. E.},
  Journal                  = {Chemical Physics Letters},
  Year                     = {2000},
  Number                   = {5-6},
  Pages                    = {399-404},
  Volume                   = {329},

  Abstract                 = {We investigate the fluorescence intensity correlation function of a single CdSe quantum dot (QD) using a start-stop experiment. We observe strong photon antibunching, a signature of non-classical light emission, over a large range of intensities (0.1-100 kW/cm(2)). The lack of coincidence at zero time delay indicates a highly efficient Auger ionization process, which suppresses multi-photon emission in these colloidal QDs. Using careful analysis of the saturation behavior of the coincidence histograms, the absorption cross-section of a single QD has also been derived. (C) 2000 Elsevier Science B.V. All rights reserved.},
  Doi                      = {10.1016/s0009-2614(00)01042-3},
  ISSN                     = {0009-2614},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000165164000012}
}

@Article{Lounis2005,
  Title                    = {Single-photon sources},
  Author                   = {Lounis, Brahim and Orrit, Michel},
  Journal                  = {Rep. Prog. Phys.},
  Year                     = {2005},
  Number                   = {5},
  Pages                    = {1129-1179},
  Volume                   = {68},

  Doi                      = {10.1088/0034-4885/68/5/r04},
  ISSN                     = {0034-4885
1361-6633},
  Type                     = {Journal Article}
}

@Article{Lu2015,
  Title                    = {Synthesis of large single-crystal hexagonal boron nitride grains on Cu-Ni alloy},
  Author                   = {Lu, G. and Wu, T. and Yuan, Q. and Wang, H. and Wang, H. and Ding, F. and Xie, X. and Jiang, M.},
  Journal                  = {Nat Commun},
  Year                     = {2015},
  Pages                    = {6160},
  Volume                   = {6},

  Abstract                 = {Hexagonal boron nitride (h-BN) has attracted significant attention because of its superior properties as well as its potential as an ideal dielectric layer for graphene-based devices. The h-BN films obtained via chemical vapour deposition in earlier reports are always polycrystalline with small grains because of high nucleation density on substrates. Here we report the successful synthesis of large single-crystal h-BN grains on rational designed Cu-Ni alloy foils. It is found that the nucleation density can be greatly reduced to 60 per mm(2) by optimizing Ni ratio in substrates. The strategy enables the growth of single-crystal h-BN grains up to 7,500 mum(2), approximately two orders larger than that in previous reports. This work not only provides valuable information for understanding h-BN nucleation and growth mechanisms, but also gives an effective alternative to exfoliated h-BN as a high-quality dielectric layer for large-scale nanoelectronic applications.},
  Doi                      = {10.1038/ncomms7160},
  ISSN                     = {2041-1723 (Electronic)
2041-1723 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25606802}
}

@Article{Lu2014,
  Title                    = {Selective Growth and Integration of Silver Nanoparticles on Silver Nanowires at Room Conditions for Transparent Nano-Network Electrode},
  Author                   = {Lu, Haifei and Zhang, Di and Ren, Xingang and Liu, Jian and Choy, Wallace C. H.},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {10980-10987},
  Volume                   = {8},

  Doi                      = {10.1021/nn504969z},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn504969z}
}

@Article{Lu2012,
  Title                    = {Plasmonic Nanolaser Using Epitaxially Grown Silver Film},
  Author                   = {Lu, Yu-Jung and Kim, Jisun and Chen, Hung-Ying and Wu, Chihhui and Dabidian, Nima and Sanders, Charlotte E. and Wang, Chun-Yuan and Lu, Ming-Yen and Li, Bo-Hong and Qiu, Xianggang and Chang, Wen-Hao and Chen, Lih-Juann and Shvets, Gennady and Shih, Chih-Kang and Gwo, Shangjr},
  Journal                  = {Science},
  Year                     = {2012},
  Number                   = {6093},
  Pages                    = {450-453},
  Volume                   = {337},

  Abstract                 = {A nanolaser is a key component for on-chip optical communications and computing systems. Here, we report on the low-threshold, continuous-wave operation of a subdiffraction nanolaser based on surface plasmon amplification by stimulated emission of radiation. The plasmonic nanocavity is formed between an atomically smooth epitaxial silver film and a single optically pumped nanorod consisting of an epitaxial gallium nitride shell and an indium gallium nitride core acting as gain medium. The atomic smoothness of the metallic film is crucial for reducing the modal volume and plasmonic losses. Bimodal lasing with similar pumping thresholds was experimentally observed, and polarization properties of the two modes were used to unambiguously identify them with theoretically predicted modes. The all-epitaxial approach opens a scalable platform for low-loss, active nanoplasmonics.},
  Doi                      = {10.1126/science.1223504},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000306802300038}
}

@Article{Lukyanchuk2010,
  Title                    = {The Fano resonance in plasmonic nanostructures and metamaterials},
  Author                   = {Luk'yanchuk, B. and Zheludev, N. I. and Maier, S. A. and Halas, N. J. and Nordlander, P. and Giessen, H. and Chong, C. T.},
  Journal                  = {Nat Mater},
  Year                     = {2010},
  Number                   = {9},
  Pages                    = {707-15},
  Volume                   = {9},

  Abstract                 = {Since its discovery, the asymmetric Fano resonance has been a characteristic feature of interacting quantum systems. The shape of this resonance is distinctively different from that of conventional symmetric resonance curves. Recently, the Fano resonance has been found in plasmonic nanoparticles, photonic crystals, and electromagnetic metamaterials. The steep dispersion of the Fano resonance profile promises applications in sensors, lasing, switching, and nonlinear and slow-light devices.},
  Doi                      = {10.1038/nmat2810},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20733610}
}

@Article{MA¥rlid1999,
  Title                    = {Hydrogen and Fluorine Adsorption on the h-BN (001) Plane},
  Author                   = {MÃ¥rlid, B. and Larsson, K. and Carlsson, J. O.},
  Journal                  = {The Journal of Physical Chemistry B},
  Year                     = {1999},
  Number                   = {36},
  Pages                    = {7637-7642},
  Volume                   = {103},

  Doi                      = {10.1021/jp984797g},
  ISSN                     = {1520-6106},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/jp984797g}
}

@Article{MacDonald2008,
  Title                    = {Ultrafast active plasmonics},
  Author                   = {MacDonald, Kevin F. and SÃ¡mson, Zsolt L. and Stockman, Mark I. and Zheludev, Nikolay I.},
  Journal                  = {Nature Photonics},
  Year                     = {2008},
  Number                   = {1},
  Pages                    = {55-58},
  Volume                   = {3},

  Doi                      = {10.1038/nphoton.2008.249},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Machaka2010,
  Title                    = {Formation of cBN nanocrystals by He+ implantation into hBN},
  Author                   = {Machaka, Ronald and Erasmus, Rudolph M. and Derry, Trevor E.},
  Journal                  = {Diamond and Related Materials},
  Year                     = {2010},
  Number                   = {10},
  Pages                    = {1131-1134},
  Volume                   = {19},

  Abstract                 = {The structural modifications of polycrystalline hexagonal boron nitride implanted with He+ beams at energies between 200 keV and 1.2 MeV to fluences of 1.0 Ã— 1017 ions cmâˆ’ 2 were investigated using micro-Raman spectroscopy. The measured Raman spectra show evidence of implantation-induced structural transformations from the hexagonal phase to nanocrystalline cubic boron nitride, rhombohedral boron nitride and amorphous boron nitride phases. The first-order Longitudinal-Optical cubic boron nitride phonon was observed to be downshifted and asymmetrically broadened and this was explained using the spatial correlation model coupled with the high ion implantation-induced defect density.},
  Doi                      = {http://dx.doi.org/10.1016/j.diamond.2010.04.001},
  ISSN                     = {0925-9635},
  Keywords                 = {Ion implantation
Implantation-induced phase transformations
Boron nitride
Raman spectroscopy
cBN nanocrystals
Spatial correlation model},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0925963510001731}
}

@Article{Magde1972,
  Title                    = {Thermodynamic Fluctuations in a Reacting System Measurement by Fluorescence Correlation Spectroscopy},
  Author                   = {Magde, Douglas and Elson, Elliot and Webb, W. W.},
  Journal                  = {Physical Review Letters},
  Year                     = {1972},
  Number                   = {11},
  Pages                    = {705-708},
  Volume                   = {29},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.29.705}
}

@Article{Mahmoud2009,
  Title                    = {Synthesis and characterization of PVP-capped CdSe nanoparticles embedded in PVA matrix for photovoltaic application},
  Author                   = {Mahmoud, Waleed E. and El-Mallah, H. M.},
  Journal                  = {Journal of Physics D: Applied Physics},
  Year                     = {2009},
  Number                   = {3},
  Pages                    = {035502},
  Volume                   = {42},

  Doi                      = {10.1088/0022-3727/42/3/035502},
  ISSN                     = {0022-3727
1361-6463},
  Type                     = {Journal Article}
}

@Article{Maier2005,
  Title                    = {Experimental demonstration of fiber-accessible metal nanoparticle plasmon waveguides for planar energy guiding and sensing},
  Author                   = {Maier, Stefan A. and Friedman, Michelle D. and Barclay, Paul E. and Painter, Oskar},
  Journal                  = {Applied Physics Letters},
  Year                     = {2005},
  Number                   = {7},
  Pages                    = {071103},
  Volume                   = {86},

  Doi                      = {10.1063/1.1862340},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Maier2002,
  Title                    = {Observation of coupled plasmon-polariton modes in Au nanoparticle chain waveguides of different lengths: Estimation of waveguide loss},
  Author                   = {Maier, Stefan A. and Kik, Pieter G. and Atwater, Harry A.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2002},
  Number                   = {9},
  Pages                    = {1714},
  Volume                   = {81},

  Doi                      = {10.1063/1.1503870},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Majety2012,
  Title                    = {Band-edge transitions in hexagonal boron nitride epilayers},
  Author                   = {Majety, S. and Cao, X. K. and Li, J. and Dahal, R. and Lin, J. Y. and Jiang, H. X.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2012},
  Number                   = {5},
  Pages                    = {051110},
  Volume                   = {101},

  Doi                      = {10.1063/1.4742194},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Mak2012,
  Title                    = {Control of valley polarization in monolayer MoS2 by optical helicity},
  Author                   = {Mak, Kin Fai and He, Keliang and Shan, Jie and Heinz, Tony F.},
  Journal                  = {Nat. Nanotechnol.},
  Year                     = {2012},
  Number                   = {8},
  Pages                    = {494-498},
  Volume                   = {7},

  Doi                      = {http://www.nature.com/nnano/journal/v7/n8/abs/nnano.2012.96.html},
  ISSN                     = {1748-3387},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nnano.2012.96}
}

@Article{Mak2010,
  Title                    = {Atomically Thin MoS2: A New Direct-Gap Semiconductor},
  Author                   = {Mak, Kin Fai and Lee, Changgu and Hone, James and Shan, Jie and Heinz, Tony F.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2010},

  Month                    = {Sep},
  Pages                    = {136805},
  Volume                   = {105},

  Doi                      = {10.1103/PhysRevLett.105.136805},
  Issue                    = {13},
  Numpages                 = {4},
  Owner                    = {Toan},
  Publisher                = {American Physical Society},
  Timestamp                = {2015.04.09},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.105.136805}
}

@Article{Maldovan2004,
  Title                    = {Diamond-structured photonic crystals},
  Author                   = {Maldovan, Martin and Thomas, Edwin L.},
  Journal                  = {Nat Mater},
  Year                     = {2004},
  Number                   = {9},
  Pages                    = {593-600},
  Volume                   = {3},

  ISSN                     = {1476-1122},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nmat1201}
}

@Article{Maletinsky2012,
  Title                    = {A robust scanning diamond sensor for nanoscale imaging with single nitrogen-vacancy centres},
  Author                   = {Maletinsky, P. and Hong, S. and Grinolds, M. S. and Hausmann, B. and Lukin, M. D. and Walsworth, R. L. and Loncar, M. and Yacoby, A.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2012},
  Number                   = {5},
  Pages                    = {320-4},
  Volume                   = {7},

  Abstract                 = {The nitrogen-vacancy defect centre in diamond has potential applications in nanoscale electric and magnetic-field sensing, single-photon microscopy, quantum information processing and bioimaging. These applications rely on the ability to position a single nitrogen-vacancy centre within a few nanometres of a sample, and then scan it across the sample surface, while preserving the centre's spin coherence and readout fidelity. However, existing scanning techniques, which use a single diamond nanocrystal grafted onto the tip of a scanning probe microscope, suffer from short spin coherence times due to poor crystal quality, and from inefficient far-field collection of the fluorescence from the nitrogen-vacancy centre. Here, we demonstrate a robust method for scanning a single nitrogen-vacancy centre within tens of nanometres from a sample surface that addresses both of these concerns. This is achieved by positioning a single nitrogen-vacancy centre at the end of a high-purity diamond nanopillar, which we use as the tip of an atomic force microscope. Our approach ensures long nitrogen-vacancy spin coherence times ( approximately 75 micros), enhanced nitrogen-vacancy collection efficiencies due to waveguiding, and mechanical robustness of the device (several weeks of scanning time). We are able to image magnetic domains with widths of 25 nm, and demonstrate a magnetic field sensitivity of 56 nT Hz(-1/2) at a frequency of 33 kHz, which is unprecedented for scanning nitrogen-vacancy centres.},
  Doi                      = {10.1038/nnano.2012.50},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {Diamond/*chemistry
Equipment Design
Molecular Imaging/*instrumentation/*methods
Nanotechnology/*instrumentation/*methods
Nitrogen/*chemistry},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22504708}
}

@Article{Mamin2013,
  Title                    = {Nanoscale Nuclear Magnetic Resonance with a Nitrogen-Vacancy Spin Sensor},
  Author                   = {Mamin, H. J. and Kim, M. and Sherwood, M. H. and Rettner, C. T. and Ohno, K. and Awschalom, D. D. and Rugar, D.},
  Journal                  = {Science},
  Year                     = {2013},
  Number                   = {6119},
  Pages                    = {557-560},
  Volume                   = {339},

  Abstract                 = {Extension of nuclear magnetic resonance (NMR) to nanoscale samples has been a longstanding challenge because of the insensitivity of conventional detection methods. We demonstrated the use of an individual, near-surface nitrogen-vacancy (NV) center in diamond as a sensor to detect proton NMR in an organic sample located external to the diamond. Using a combination of electron spin echoes and proton spin manipulation, we showed that the NV center senses the nanotesla field fluctuations from the protons, enabling both time-domain and spectroscopic NMR measurements on the nanometer scale.},
  Doi                      = {10.1126/science.1231540},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/339/6119/557.abstract}
}

@Article{Manfredotti2006,
  Title                    = {Vibronic spectrum of c-BN measured with cathodoluminescence},
  Author                   = {Manfredotti, C. and Cossio, R. and Giudice, A. Lo and Vittone, E. and Fizzotti, F.},
  Journal                  = {Physical Review B},
  Year                     = {2006},
  Number                   = {15},
  Pages                    = {155204},
  Volume                   = {74},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.74.155204}
}

@Article{Manjavacas2008,
  Title                    = {Robust Plasmon Waveguides in Strongly Interacting Nanowire Arrays},
  Author                   = {Manjavacas, A. and GarcÃ­a de Abajo, F. J.},
  Journal                  = {Nano Letters},
  Year                     = {2008},
  Number                   = {4},
  Pages                    = {1285-1289},
  Volume                   = {9},

  Doi                      = {10.1021/nl802044t},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl802044t}
}

@Article{Manson1994,
  Title                    = {Transient hole burning in N-V centre in diamond},
  Author                   = {Manson, N. B. and Wei, C.},
  Journal                  = {Journal of Luminescence},
  Year                     = {1994},
  Number                   = {1â€“6},
  Pages                    = {158-160},
  Volume                   = {58},

  Abstract                 = {The hole-burning spectrum associated with the 637 nm zero-phonon line in diamond is obtained using two CW lasers of equal intensity. Antiholes are observed at 2.88 and 0.8 GHz when burning on the low energy side of the zero-phonon line and at 2.88, 2.05 and 0.46 GHz when burning on the high energy side of the line. One sidehole is detected but only when the fastest sweep rates are used. The frequencies of the holes and antiholes are compared with frequencies obtained by other measurements and excited state energy levels are proposed.},
  Doi                      = {http://dx.doi.org/10.1016/0022-2313(94)90385-9},
  ISSN                     = {0022-2313},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/0022231394903859}
}

@Article{Marago2013,
  Title                    = {Optical trapping and manipulation of nanostructures},
  Author                   = {Marago, O. M. and Jones, P. H. and Gucciardi, P. G. and Volpe, G. and Ferrari, A. C.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2013},
  Number                   = {11},
  Pages                    = {807-19},
  Volume                   = {8},

  Abstract                 = {Optical trapping and manipulation of micrometre-sized particles was first reported in 1970. Since then, it has been successfully implemented in two size ranges: the subnanometre scale, where light-matter mechanical coupling enables cooling of atoms, ions and molecules, and the micrometre scale, where the momentum transfer resulting from light scattering allows manipulation of microscopic objects such as cells. But it has been difficult to apply these techniques to the intermediate - nanoscale - range that includes structures such as quantum dots, nanowires, nanotubes, graphene and two-dimensional crystals, all of crucial importance for nanomaterials-based applications. Recently, however, several new approaches have been developed and demonstrated for trapping plasmonic nanoparticles, semiconductor nanowires and carbon nanostructures. Here we review the state-of-the-art in optical trapping at the nanoscale, with an emphasis on some of the most promising advances, such as controlled manipulation and assembly of individual and multiple nanostructures, force measurement with femtonewton resolution, and biosensors.},
  Doi                      = {10.1038/nnano.2013.208},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {Biosensing Techniques
Graphite
Light
Nanostructures/*chemistry
Nanotechnology/*methods
*Optical Tweezers
Particle Size
Quantum Dots
Semiconductors
Spectrum Analysis},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24202536}
}

@Article{Martin1999,
  Title                    = {Fine structure of excited 3E state in nitrogen-vacancy centre of diamond},
  Author                   = {Martin, J. P. D.},
  Journal                  = {Journal of Luminescence},
  Year                     = {1999},
  Number                   = {4},
  Pages                    = {237-247},
  Volume                   = {81},

  Abstract                 = {New analysis of hole burning and magnetic circular dichroism observations on the fine structure of the excited 3E state in the nitrogen-vacancy centre of diamond finds that the effective spinâ€“orbit contribution is much smaller than previously estimated. This situation means that the spinâ€“spin interaction determines the fine structure in centres with strain splittings &gt;0.5 cmâˆ’1. It is discussed that this result is more consistent with the observed weak strain dependence of hole-burning features than earlier calculations and supports the six electron model of the centre.},
  Doi                      = {http://dx.doi.org/10.1016/S0022-2313(99)00013-7},
  ISSN                     = {0022-2313},
  Keywords                 = {Hole burning
Diamond
Excited state
Zero phonon line
Spinâ€“orbit interaction
Spinâ€“spin interaction},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0022231399000137}
}

@Article{Martin2000,
  Title                    = {Spectral hole burning and Raman heterodyne signals associated with an avoided crossing in the NV centre in diamond},
  Author                   = {Martin, J. P. D. and Manson, N. B. and Doetschman, D. C. and Sellars, M. J. and Neuhaus, R. and Wilson, E.},
  Journal                  = {Journal of Luminescence},
  Year                     = {2000},
  Number                   = {3â€“4},
  Pages                    = {355-362},
  Volume                   = {86},

  Abstract                 = {The nitrogen-vacancy centre in diamond exhibits an avoided crossing of ground state electron spin levels in a magnetic field of âˆ¼1028 G applied along the ã€ˆ1 1 1ã€‰ direction. In this paper, the magnetic field dependence of Raman heterodyne signals and the optical transmission at 638 nm in the vicinity of the avoided crossing are reported. It is discussed that the optically induced spin polarization of ground state populations produces anomalous fine structure hole-burning behaviour.},
  Doi                      = {http://dx.doi.org/10.1016/S0022-2313(00)00179-4},
  ISSN                     = {0022-2313},
  Keywords                 = {Hole burning
Diamond
Spin polarization
Raman heterodyne},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0022231300001794}
}

@Article{Matsui2014,
  Title                    = {Coupling of Er light emissions to plasmon modes on In2O3: Sn nanoparticle sheets in the near-infrared range},
  Author                   = {Matsui, Hiroaki and Badalawa, Wasanthamala and Hasebe, Takayuki and Furuta, Shinya and Nomura, Wataru and Yatsui, Takashi and Ohtsu, Motoichi and Tabata, Hitoshi},
  Journal                  = {Applied Physics Letters},
  Year                     = {2014},
  Number                   = {4},
  Pages                    = {041903},
  Volume                   = {105},

  Doi                      = {10.1063/1.4892004},
  ISSN                     = {0003-6951
1077-3118},
  Type                     = {Journal Article}
}

@Article{Matte2010,
  Title                    = {MoS2 and WS2 Analogues of Graphene},
  Author                   = {Matte, H. S. S. Ramakrishna and Gomathi, A. and Manna, Arun K. and Late, Dattatray J. and Datta, Ranjan and Pati, Swapan K. and Rao, C. N. R.},
  Journal                  = {Angew. Chem. Int. Ed.},
  Year                     = {2010},
  Number                   = {24},
  Pages                    = {4059--4062},
  Volume                   = {49},

  Doi                      = {10.1002/anie.201000009},
  Oi                       = {Matte, Krishna/0000-0001-8279-8447; Ahirwal, AshishEOLEOL/0000-0002-9127-6541; Ahirwal, Ashish/0000-0002-8247-9793},
  Owner                    = {Toan},
  Pm                       = {20425874},
  Ri                       = {Matte, Krishna/F-1790-2011; Ahirwal, Ashish /F-2532-2013; Ahirwal, Ashish/B-8886-2015},
  Sn                       = {1433-7851},
  Tc                       = {307},
  Timestamp                = {2015.04.09},
  Ut                       = {WOS:000278796400010},
  Z8                       = {5},
  Z9                       = {309},
  Zb                       = {18},
  Zs                       = {0}
}

@Article{Mattoussi1998,
  Title                    = {Electroluminescence from heterostructures of poly(phenylene vinylene) and inorganic CdSe nanocrystals},
  Author                   = {Mattoussi, Hedi and Radzilowski, Leonard H. and Dabbousi, Bashir O. and Thomas, Edwin L. and Bawendi, Moungi G. and Rubner, Michael F.},
  Journal                  = {Journal of Applied Physics},
  Year                     = {1998},
  Number                   = {12},
  Pages                    = {7965-7974},
  Volume                   = {83},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.367978},
  Keywords                 = {adsorption
wide band gap semiconductors
nanostructured materials
cadmium compounds
electroluminescence
optical polymers
polymer films
photoluminescence
II-VI semiconductors},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/jap/83/12/10.1063/1.367978}
}

@Article{Maze2011,
  Title                    = {Properties of nitrogen-vacancy centers in diamond: the group theoretic approach},
  Author                   = {Maze, J. R. and Gali, A. and Togan, E. and Chu, Y. and Trifonov, A. and Kaxiras, E. and Lukin, M. D.},
  Journal                  = {New Journal of Physics},
  Year                     = {2011},
  Number                   = {2},
  Pages                    = {025025},
  Volume                   = {13},

  Doi                      = {10.1088/1367-2630/13/2/025025},
  ISSN                     = {1367-2630},
  Type                     = {Journal Article}
}

@Article{Maze2008,
  Title                    = {Nanoscale magnetic sensing with an individual electronic spin in diamond},
  Author                   = {Maze, J. R. and Stanwix, P. L. and Hodges, J. S. and Hong, S. and Taylor, J. M. and Cappellaro, P. and Jiang, L. and Dutt, M. V. and Togan, E. and Zibrov, A. S. and Yacoby, A. and Walsworth, R. L. and Lukin, M. D.},
  Journal                  = {Nature},
  Year                     = {2008},
  Number                   = {7213},
  Pages                    = {644-7},
  Volume                   = {455},

  Abstract                 = {Detection of weak magnetic fields with nanoscale spatial resolution is an outstanding problem in the biological and physical sciences. For example, at a distance of 10 nm, the spin of a single electron produces a magnetic field of about 1 muT, and the corresponding field from a single proton is a few nanoteslas. A sensor able to detect such magnetic fields with nanometre spatial resolution would enable powerful applications, ranging from the detection of magnetic resonance signals from individual electron or nuclear spins in complex biological molecules to readout of classical or quantum bits of information encoded in an electron or nuclear spin memory. Here we experimentally demonstrate an approach to such nanoscale magnetic sensing, using coherent manipulation of an individual electronic spin qubit associated with a nitrogen-vacancy impurity in diamond at room temperature. Using an ultra-pure diamond sample, we achieve detection of 3 nT magnetic fields at kilohertz frequencies after 100 s of averaging. In addition, we demonstrate a sensitivity of 0.5 muT Hz(-1/2) for a diamond nanocrystal with a diameter of 30 nm.},
  Doi                      = {10.1038/nature07279},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/18833275}
}

@Article{McCreary2014,
  Title                    = {Large-Area Synthesis of Continuous and Uniform MoS2 Monolayer Films on Graphene},
  Author                   = {McCreary, Kathleen M. and Hanbicki, Aubrey T. and Robinson, Jeremy T. and Cobas, Enrique and Culbertson, James C. and Friedman, Adam L. and Jernigan, Glenn G. and Jonker, Berend T.},
  Journal                  = {Advanced Functional Materials},
  Year                     = {2014},
  Number                   = {41},
  Pages                    = {6449-6454},
  Volume                   = {24},

  Abstract                 = {Heterostructures composed of multiple layers of different atomically thin materials are of interest due to their unique properties and potential for new device functionality. MoS2-graphene heterostructures have shown promise as photodetectors and vertical tunnel transistors. However, progress is limited by the typically micrometer-scale devices and by the multiple alignments required for fabrication when utilizing mechanically exfoliated material. Here, the synthesis of large-area, continuous, and uniform MoS2 monolayers directly on graphene by chemical vapor deposition is reported, resulting in heterostructure samples on the centimeter scale with the possibility for even larger lateral dimensions. Atomic force microscopy, photoluminescence, X-ray photoelectron, and Raman spectroscopies demonstrate uniform single-layer growth of stoichiometric MoS2. The ability to reproducibly generate large-area heterostructures is highly advantageous for both fundamental investigations and technological applications.},
  Doi                      = {10.1002/adfm.201401511},
  ISSN                     = {1616-3028},
  Keywords                 = {graphene
MoS2
2D heterostructures
synthesis},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/adfm.201401511}
}

@Article{Medintz2005,
  Title                    = {Quantum dot bioconjugates for imaging, labelling and sensing},
  Author                   = {Medintz, Igor L. and Uyeda, H. Tetsuo and Goldman, Ellen R. and Mattoussi, Hedi},
  Journal                  = {Nat Mater},
  Year                     = {2005},
  Number                   = {6},
  Pages                    = {435-446},
  Volume                   = {4},

  ISSN                     = {1476-1122},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nmat1390}
}

@InProceedings{Meuret,
  Title                    = {Quantum nano optics of defect centers in diamond and h-BN with nano-cathodoluminescence},
  Author                   = {Meuret, S. and Tizei, L. H. G. and Bourrellier, R. and Blazit, J. D. and Tence, M. and Zobelli, A. and Kociak, M.},
  Booktitle                = {Lasers and Electro-Optics (CLEO), 2014 Conference on},
  Pages                    = {1-2},

  Keywords                 = {III-V semiconductors
boron compounds
cathodoluminescence
diamond
vacancies (crystal)
wide band gap semiconductors
BN
C
NV<sup>0</sup> center
cathodoluminescence-based single emitter detection
deep subwavelength resolution
defect center
hexagonal boron nitride
nanocathodoluminescence
quantum nano-optics
Boron
Correlation
Diamonds
Heterojunction bipolar transistors
Photonics
Stimulated emission},
  Type                     = {Conference Proceedings}
}

@Article{Michalet2005,
  Title                    = {Quantum Dots for Live Cells, in Vivo Imaging, and Diagnostics},
  Author                   = {Michalet, X. and Pinaud, F. F. and Bentolila, L. A. and Tsay, J. M. and Doose, S. and Li, J. J. and Sundaresan, G. and Wu, A. M. and Gambhir, S. S. and Weiss, S.},
  Journal                  = {Science},
  Year                     = {2005},
  Number                   = {5709},
  Pages                    = {538-544},
  Volume                   = {307},

  Abstract                 = {Research on fluorescent semiconductor nanocrystals (also known as quantum dots or qdots) has evolved over the past two decades from electronic materials science to biological applications. We review current approaches to the synthesis, solubilization, and functionalization of qdots and their applications to cell and animal biology. Recent examples of their experimental use include the observation of diffusion of individual glycine receptors in living neurons and the identification of lymph nodes in live animals by near-infrared emission during surgery. The new generations of qdots have far-reaching potential for the study of intracellular processes at the single-molecule level, high-resolution cellular imaging, long-term in vivo observation of cell trafficking, tumor targeting, and diagnostics.},
  Doi                      = {10.1126/science.1104274},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/307/5709/538.abstract}
}

@Article{Michler2000,
  Title                    = {Quantum correlation among photons from a single quantum dot at room temperature},
  Author                   = {Michler, P. and Imamoglu, A. and Mason, M. D. and Carson, P. J. and Strouse, G. F. and Buratto, S. K.},
  Journal                  = {Nature},
  Year                     = {2000},
  Number                   = {6799},
  Pages                    = {968-70},
  Volume                   = {406},

  Abstract                 = {Maxwell's equations successfully describe the statistical properties of fluorescence from an ensemble of atoms or semiconductors in one or more dimensions. But quantization of the radiation field is required to explain the correlations of light generated by a single two-level quantum emitter, such as an atom, ion or single molecule. The observation of photon antibunching in resonance fluorescence from a single atom unequivocally demonstrated the non-classical nature of radiation. Here we report the experimental observation of photon antibunching from an artificial system--a single cadmium selenide quantum dot at room temperature. Apart from providing direct evidence for a solid-state non-classical light source, this result proves that a single quantum dot acts like an artificial atom, with a discrete anharmonic spectrum. In contrast, we find the photon-emission events from a cluster of several dots to be uncorrelated.},
  Doi                      = {10.1038/35023100},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/10984045}
}

@Article{Michler2000a,
  Title                    = {A quantum dot single-photon turnstile device},
  Author                   = {Michler, P. and Kiraz, A. and Becher, C. and Schoenfeld, W. V. and et al.},
  Journal                  = {Science},
  Year                     = {2000},
  Number                   = {5500},
  Pages                    = {2282-5},
  Volume                   = {290},

  Abstract                 = {Quantum communication relies on the availability of light pulses with strong quantum correlations among photons. An example of such an optical source is a single-photon pulse with a vanishing probability for detecting two or more photons.},
  ISSN                     = {00368075},
  Keywords                 = {Technology: Comprehensive Works
Atoms & subatomic particles
Quantum theory
Light
Electrical engineering},
  Type                     = {Journal Article},
  Url                      = {http://ezproxy.lib.uts.edu.au/login?url=http://search.proquest.com/docview/213577642?accountid=17095
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Journal_Search&Ntx=matchallpartial&Ntt=Science
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Title_Search&Ntx=matchallpartial&Ntt=A+quantum+dot+single-photon+turnstile+device
http://sfx.lib.uts.edu.au/sfx_local?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:journal&genre=article&sid=ProQ:ProQ%3Ahealthcompleteshell&atitle=A+quantum+dot+single-photon+turnstile+device&title=Science&issn=00368075&date=2000-12-22&volume=290&issue=5500&spage=2282&au=Michler%2C+P%3BKiraz%2C+A%3BBecher%2C+C%3BSchoenfeld%2C+W+V%3Bet+al&isbn=&jtitle=Science&btitle=&rft_id=info:eric/&rft_id=info:doi/}
}

@Article{Min2009,
  Title                    = {High-Q surface-plasmon-polariton whispering-gallery microcavity},
  Author                   = {Min, B. and Ostby, E. and Sorger, V. and Ulin-Avila, E. and Yang, L. and Zhang, X. and Vahala, K.},
  Journal                  = {Nature},
  Year                     = {2009},
  Number                   = {7228},
  Pages                    = {455-8},
  Volume                   = {457},

  Abstract                 = {Surface plasmon polaritons (SPPs) are electron density waves excited at the interfaces between metals and dielectric materials. Owing to their highly localized electromagnetic fields, they may be used for the transport and manipulation of photons on subwavelength scales. In particular, plasmonic resonant cavities represent an application that could exploit this field compression to create ultrasmall-mode-volume devices. A key figure of merit in this regard is the ratio of cavity quality factor, Q (related to the dissipation rate of photons confined to the cavity), to cavity mode volume, V (refs 10, 11). However, plasmonic cavity Q factors have so far been limited to values less than 100 both for visible and near-infrared wavelengths. Significantly, such values are far below the theoretically achievable Q factors for plasmonic resonant structures. Here we demonstrate a high-Q SPP whispering-gallery microcavity that is made by coating the surface of a high-Q silica microresonator with a thin layer of a noble metal. Using this structure, Q factors of 1,376 +/- 65 can be achieved in the near infrared for surface-plasmonic whispering-gallery modes at room temperature. This nearly ideal value, which is close to the theoretical metal-loss-limited Q factor, is attributed to the suppression and minimization of radiation and scattering losses that are made possible by the geometrical structure and the fabrication method. The SPP eigenmodes, as well as the dielectric eigenmodes, are confined within the whispering-gallery microcavity and accessed evanescently using a single strand of low-loss, tapered optical waveguide. This coupling scheme provides a convenient way of selectively exciting and probing confined SPP eigenmodes. Up to 49.7 per cent of input power is coupled by phase-matching control between the microcavity SPP and the tapered fibre eigenmodes.},
  Doi                      = {10.1038/nature07627},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/19158793}
}

@Article{Miro2014,
  Title                    = {Two Dimensional Materials Beyond MoS2 : Noble-Transition-Metal Dichalcogenides},
  Author                   = {Miro, Pere and Ghorbani-Asl, Mahdi and Heine, Thomas},
  Journal                  = {Angew. Chem. Int. Ed.},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {3015--3018},
  Volume                   = {53},

  Doi                      = {10.1002/anie.201309280},
  Oi                       = {Heine, Thomas/0000-0003-2379-6251},
  Owner                    = {Toan},
  Pm                       = {24554594},
  Ri                       = {Heine, Thomas/H-5446-2011},
  Sn                       = {1433-7851},
  Tc                       = {5},
  Timestamp                = {2015.04.09},
  Ut                       = {WOS:000336846300021},
  Z8                       = {0},
  Z9                       = {5},
  Zb                       = {0},
  Zs                       = {0}
}

@Article{Miroshnichenko2010,
  Title                    = {Fano resonances in nanoscale structures},
  Author                   = {Miroshnichenko, Andrey E. and Flach, Sergej and Kivshar, Yuri S.},
  Journal                  = {Reviews of Modern Physics},
  Year                     = {2010},
  Number                   = {3},
  Pages                    = {2257-2298},
  Volume                   = {82},

  Doi                      = {10.1103/RevModPhys.82.2257},
  ISSN                     = {0034-6861
1539-0756},
  Type                     = {Journal Article}
}

@Article{Mishima1987,
  Title                    = {Crystal growth of cubic boron nitride by temperature difference method at âˆ¼55 kbar and âˆ¼1800â€‰Â°C},
  Author                   = {Mishima, O. and Yamaoka, S. and Fukunaga, O.},
  Journal                  = {Journal of Applied Physics},
  Year                     = {1987},
  Number                   = {8},
  Pages                    = {2822-2825},
  Volume                   = {61},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.337874},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/jap/61/8/10.1063/1.337874}
}

@Article{Mizuochi2012,
  Title                    = {Electrically driven single-photon source at room temperature in diamond},
  Author                   = {Mizuochi, N. and Makino, T. and Kato, H. and Takeuchi, D. and Ogura, M. and Okushi, H. and Nothaft, M. and Neumann, P. and Gali, A. and Jelezko, F. and Wrachtrup, J. and Yamasaki, S.},
  Journal                  = {Nature Photonics},
  Year                     = {2012},
  Number                   = {5},
  Pages                    = {299-303},
  Volume                   = {6},

  Doi                      = {10.1038/nphoton.2012.75},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Mochalin2012,
  Title                    = {The properties and applications of nanodiamonds},
  Author                   = {Mochalin, V. N. and Shenderova, O. and Ho, D. and Gogotsi, Y.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {11-23},
  Volume                   = {7},

  Abstract                 = {Nanodiamonds have excellent mechanical and optical properties, high surface areas and tunable surface structures. They are also non-toxic, which makes them well suited to biomedical applications. Here we review the synthesis, structure, properties, surface chemistry and phase transformations of individual nanodiamonds and clusters of nanodiamonds. In particular we discuss the rational control of the mechanical, chemical, electronic and optical properties of nanodiamonds through surface doping, interior doping and the introduction of functional groups. These little gems have a wide range of potential applications in tribology, drug delivery, bioimaging and tissue engineering, and also as protein mimics and a filler material for nanocomposites.},
  Doi                      = {10.1038/nnano.2011.209},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {Animals
Drug Delivery Systems
Humans
Lubricants
Nanodiamonds/*chemistry
Nanomedicine/*methods
Nanotechnology/*methods
Tissue Scaffolds},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22179567}
}

@Article{Moerner2003,
  Title                    = {Methods of single-molecule fluorescence spectroscopy and microscopy},
  Author                   = {Moerner, W. E. and Fromm, David P.},
  Journal                  = {Review of Scientific Instruments},
  Year                     = {2003},
  Number                   = {8},
  Pages                    = {3597-3619},
  Volume                   = {74},

  Doi                      = {http://dx.doi.org/10.1063/1.1589587},
  Owner                    = {Toan},
  Timestamp                = {2015.04.10},
  Url                      = {http://scitation.aip.org/content/aip/journal/rsi/74/8/10.1063/1.1589587}
}

@Article{Moerner1999,
  Title                    = {Illuminating Single Molecules in Condensed Matter},
  Author                   = {Moerner, W. E. and Orrit, Michel},
  Journal                  = {Science},
  Year                     = {1999},
  Number                   = {5408},
  Pages                    = {1670--1676},
  Volume                   = {283},

  Abstract                 = {Efficient collection and detection of fluorescence coupled with careful minimization of background from impurities and Raman scattering now enable routine optical microscopy and study of single molecules in complex condensed matter environments. This ultimate method for unraveling ensemble averages leads to the observation of new effects and to direct measurements of stochastic fluctuations. Experiments at cryogenic temperatures open new directions in molecular spectroscopy, quantum optics, and solid-state dynamics. Room-temperature investigations apply several techniques (polarization microscopy, single-molecule imaging, emission time dependence, energy transfer, lifetime studies, and the like) to a growing array of biophysical problems where new insight may be gained from direct observations of hidden static and dynamic inhomogeneity.},
  Comment                  = {10.1126/science.283.5408.1670},
  Owner                    = {Toan},
  Timestamp                = {2015.04.10},
  Url                      = {http://www.sciencemag.org/content/283/5408/1670.abstract}
}

@Article{Mohan2010,
  Title                    = {Sub-20-nm fluorescent nanodiamonds as photostable biolabels and fluorescence resonance energy transfer donors},
  Author                   = {Mohan, N. and Tzeng, Y. K. and Yang, L. and Chen, Y. Y. and Hui, Y. Y. and Fang, C. Y. and Chang, H. C.},
  Journal                  = {Adv Mater},
  Year                     = {2010},
  Number                   = {7},
  Pages                    = {843-7},
  Volume                   = {22},

  Doi                      = {10.1002/adma.200901596},
  ISSN                     = {1521-4095 (Electronic)
0935-9648 (Linking)},
  Keywords                 = {Diamond/*chemistry
Fluorescence Resonance Energy Transfer
Fluorescent Dyes/*chemistry
Helium/chemistry
Microscopy, Fluorescence
Nanostructures/*chemistry
Particle Size
Proteins/chemistry
Spectrometry, Fluorescence},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20217795}
}

@Article{Moradi2008,
  Title                    = {Plasmon hybridization in metallic nanotubes},
  Author                   = {Moradi, Afshin},
  Journal                  = {Journal of Physics and Chemistry of Solids},
  Year                     = {2008},
  Number                   = {11},
  Pages                    = {2936-2938},
  Volume                   = {69},

  Doi                      = {10.1016/j.jpcs.2008.08.004},
  ISSN                     = {00223697},
  Type                     = {Journal Article}
}

@Article{Mortensen2010,
  Title                    = {Optimized localization analysis for single-molecule tracking and super-resolution microscopy},
  Author                   = {Mortensen, K. I. and Churchman, L. S. and Spudich, J. A. and Flyvbjerg, H.},
  Journal                  = {Nat Methods},
  Year                     = {2010},
  Number                   = {5},
  Pages                    = {377-81},
  Volume                   = {7},

  Abstract                 = {We optimally localized isolated fluorescent beads and molecules imaged as diffraction-limited spots, determined the orientation of molecules and present reliable formulas for the precision of various localization methods. Both theory and experimental data showed that unweighted least-squares fitting of a Gaussian squanders one-third of the available information, a popular formula for its precision exaggerates beyond Fisher's information limit, and weighted least-squares may do worse, whereas maximum-likelihood fitting is practically optimal.},
  Doi                      = {10.1038/nmeth.1447},
  ISSN                     = {1548-7105 (Electronic)
1548-7091 (Linking)},
  Keywords                 = {Image Interpretation, Computer-Assisted/*methods
Likelihood Functions
Microscopy, Fluorescence/*methods
Nanotechnology
Photons},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20364147}
}

@Article{Muller2014,
  Title                    = {Optical signatures of silicon-vacancy spins in diamond},
  Author                   = {Muller, T. and Hepp, C. and Pingault, B. and Neu, E. and Gsell, S. and Schreck, M. and Sternschulte, H. and Steinmuller-Nethl, D. and Becher, C. and Atature, M.},
  Journal                  = {Nat Commun},
  Year                     = {2014},
  Pages                    = {3328},
  Volume                   = {5},

  Abstract                 = {Colour centres in diamond have emerged as versatile tools for solid-state quantum technologies ranging from quantum information to metrology, where the nitrogen-vacancy centre is the most studied to date. Recently, this toolbox has expanded to include novel colour centres to realize more efficient spin-photon quantum interfaces. Of these, the silicon-vacancy centre stands out with highly desirable photonic properties. The challenge for utilizing this centre is to realize the hitherto elusive optical access to its electronic spin. Here we report spin-tagged resonance fluorescence from the negatively charged silicon-vacancy centre. Our measurements reveal a spin-state purity approaching unity in the excited state, highlighting the potential of the centre as an efficient spin-photon quantum interface.},
  Doi                      = {10.1038/ncomms4328},
  ISSN                     = {2041-1723 (Electronic)
2041-1723 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24534908}
}

@Article{Museur2007,
  Title                    = {Photoluminescence of hexagonal boron nitride: Effect of surface oxidation under UV-laser irradiation},
  Author                   = {Museur, Luc and Anglos, Demetrios and Petitet, Jean-Pierre and Michel, Jean-Pierre and Kanaev, Andrei V.},
  Journal                  = {Journal of Luminescence},
  Year                     = {2007},
  Number                   = {2},
  Pages                    = {595-600},
  Volume                   = {127},

  Abstract                 = {We report on the UV laser-induced fluorescence of hexagonal boron nitride (h-BN) following nanosecond laser irradiation under vacuum and in different environments of nitrogen gas and ambient air. The observed fluorescence bands are tentatively ascribed to impurity and mono (VN) or multiple (m-VN with m=2 or 3) nitrogen vacancies. A structured fluorescence band between 300 and 350 nm is assigned to impurity-band transition and its complex lineshape is attributed to phonon replicas. An additional band at 340 nm, assigned to VN vacancies on surface, is observed under vacuum and quenched by adsorbed molecular oxygen. UV-irradiation of h-BN under vacuum results in a broad asymmetric fluorescence at âˆ¼400 nm assigned to m-VN vacancies; further irradiation breaks more Bâ€“N bonds enriching the surface with elemental boron. However, no boron deposit appears under irradiation of samples in ambient atmosphere. This effect is explained by oxygen healing of radiation-induced surface defects. Formation of the oxide layer prevents Bâ€“N dissociation and preserves the bulk sample stoichiometry.},
  Doi                      = {http://dx.doi.org/10.1016/j.jlumin.2007.01.024},
  ISSN                     = {0022-2313},
  Keywords                 = {Hexagonal boron nitride
Photoluminescence
Surface oxidation
UV-laser irradiation},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0022231307001172}
}

@Article{Museur2008,
  Title                    = {Defect-related photoluminescence of hexagonal boron nitride},
  Author                   = {Museur, Luc and Feldbach, Eduard and Kanaev, Andrei},
  Journal                  = {Physical Review B},
  Year                     = {2008},
  Number                   = {15},
  Pages                    = {155204},
  Volume                   = {78},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.78.155204}
}

@Article{Muzha2014,
  Title                    = {Room-temperature near-infrared silicon carbide nanocrystalline emitters based on optically aligned spin defects},
  Author                   = {Muzha, A. and Fuchs, F. and Tarakina, N. V. and Simin, D. and Trupke, M. and Soltamov, V. A. and Mokhov, E. N. and Baranov, P. G. and Dyakonov, V. and Krueger, A. and Astakhov, G. V.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2014},
  Number                   = {24},
  Pages                    = {-},
  Volume                   = {105},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.4904807},
  Keywords                 = {nanostructured materials
amorphisation
nanofabrication
wide band gap semiconductors
neutron effects
silicon compounds
semiconductor growth
vacancies (crystal)
photoluminescence},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/apl/105/24/10.1063/1.4904807}
}

@Article{Myers2014,
  Title                    = {Probing Surface Noise with Depth-Calibrated Spins in Diamond},
  Author                   = {Myers, B. â€‰A and Das, A. and Dartiailh, M. â€‰C and Ohno, K. and Awschalom, D. â€‰D and Bleszynski Jayich, A. â€‰C},
  Journal                  = {Physical Review Letters},
  Year                     = {2014},
  Number                   = {2},
  Volume                   = {113},

  Doi                      = {10.1103/PhysRevLett.113.027602},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Nagpal2009,
  Title                    = {Ultrasmooth Patterned Metals for Plasmonics and Metamaterials},
  Author                   = {Nagpal, Prashant and Lindquist, Nathan C. and Oh, Sang-Hyun and Norris, David J.},
  Journal                  = {Science},
  Year                     = {2009},
  Number                   = {5940},
  Pages                    = {594-597},
  Volume                   = {325},

  Abstract                 = {Surface plasmons are electromagnetic waves that can exist at metal interfaces because of coupling between light and free electrons. Restricted to travel along the interface, these waves can be channeled, concentrated, or otherwise manipulated by surface patterning. However, because surface roughness and other inhomogeneities have so far limited surface-plasmon propagation in real plasmonic devices, simple high-throughput methods are needed to fabricate high-quality patterned metals. We combined template stripping with precisely patterned silicon substrates to obtain ultrasmooth pure metal films with grooves, bumps, pyramids, ridges, and holes. Measured surface-plasmonâ€“propagation lengths on the resulting surfaces approach theoretical values for perfectly flat films. With the use of our method, we demonstrated structures that exhibit Raman scattering enhancements above 107 for sensing applications and multilayer films for optical metamaterials.},
  Doi                      = {10.1126/science.1174655},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/325/5940/594.abstract}
}

@Article{Naguib2011,
  Title                    = {Two-Dimensional Nanocrystals Produced by Exfoliation of Ti3AlC2},
  Author                   = {Naguib, Michael and Kurtoglu, Murat and Presser, Volker and Lu, Jun and Niu, Junjie and Heon, Min and Hultman, Lars and Gogotsi, Yury and Barsoum, Michel W.},
  Journal                  = {Advanced Materials},
  Year                     = {2011},
  Number                   = {37},
  Pages                    = {4248-4253},
  Volume                   = {23},

  Doi                      = {10.1002/adma.201102306},
  ISSN                     = {1521-4095},
  Keywords                 = {nanosheets
exfoliation
carbides
two-dimensional materials},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/adma.201102306}
}

@Article{Naik2013,
  Title                    = {Alternative plasmonic materials: beyond gold and silver},
  Author                   = {Naik, G. V. and Shalaev, V. M. and Boltasseva, A.},
  Journal                  = {Adv Mater},
  Year                     = {2013},
  Number                   = {24},
  Pages                    = {3264-94},
  Volume                   = {25},

  Abstract                 = {Materials research plays a vital role in transforming breakthrough scientific ideas into next-generation technology. Similar to the way silicon revolutionized the microelectronics industry, the proper materials can greatly impact the field of plasmonics and metamaterials. Currently, research in plasmonics and metamaterials lacks good material building blocks in order to realize useful devices. Such devices suffer from many drawbacks arising from the undesirable properties of their material building blocks, especially metals. There are many materials, other than conventional metallic components such as gold and silver, that exhibit metallic properties and provide advantages in device performance, design flexibility, fabrication, integration, and tunability. This review explores different material classes for plasmonic and metamaterial applications, such as conventional semiconductors, transparent conducting oxides, perovskite oxides, metal nitrides, silicides, germanides, and 2D materials such as graphene. This review provides a summary of the recent developments in the search for better plasmonic materials and an outlook of further research directions.},
  Doi                      = {10.1002/adma.201205076},
  ISSN                     = {1521-4095 (Electronic)
0935-9648 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23674224}
}

@Article{Nakanishi2009,
  Title                    = {Photoconductance and inverse photoconductance in films of functionalized metal nanoparticles},
  Author                   = {Nakanishi, H. and Bishop, K. J. and Kowalczyk, B. and Nitzan, A. and Weiss, E. A. and Tretiakov, K. V. and Apodaca, M. M. and Klajn, R. and Stoddart, J. F. and Grzybowski, B. A.},
  Journal                  = {Nature},
  Year                     = {2009},
  Number                   = {7253},
  Pages                    = {371-5},
  Volume                   = {460},

  Abstract                 = {In traditional photoconductors, the impinging light generates mobile charge carriers in the valence and/or conduction bands, causing the material's conductivity to increase. Such positive photoconductance is observed in both bulk and nanostructured photoconductors. Here we describe a class of nanoparticle-based materials whose conductivity can either increase or decrease on irradiation with visible light of wavelengths close to the particles' surface plasmon resonance. The remarkable feature of these plasmonic materials is that the sign of the conductivity change and the nature of the electron transport between the nanoparticles depend on the molecules comprising the self-assembled monolayers (SAMs) stabilizing the nanoparticles. For SAMs made of electrically neutral (polar and non-polar) molecules, conductivity increases on irradiation. If, however, the SAMs contain electrically charged (either negatively or positively) groups, conductivity decreases. The optical and electrical characteristics of these previously undescribed inverse photoconductors can be engineered flexibly by adjusting the material properties of the nanoparticles and of the coating SAMs. In particular, in films comprising mixtures of different nanoparticles or nanoparticles coated with mixed SAMs, the overall photoconductance is a weighted average of the changes induced by the individual components. These and other observations can be rationalized in terms of light-induced creation of mobile charge carriers whose transport through the charged SAMs is inhibited by carrier trapping in transient polaron-like states. The nanoparticle-based photoconductors we describe could have uses in chemical sensors and/or in conjunction with flexible substrates.},
  Doi                      = {10.1038/nature08131},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Keywords                 = {Electric Conductivity
Gold/chemistry
*Light
Metal Nanoparticles/*chemistry/*radiation effects
Models, Chemical
Photochemistry/*instrumentation
Silver/chemistry
Surface Plasmon Resonance
Temperature},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/19606145}
}

@Article{Nelayah2007,
  Title                    = {Mapping surface plasmons on a single metallic nanoparticle},
  Author                   = {Nelayah, Jaysen and Kociak, Mathieu and StÃ©phan, Odile and GarcÃ­a de Abajo, F. Javier and TencÃ©, Marcel and Henrard, Luc and Taverna, Dario and Pastoriza-Santos, Isabel and Liz-MarzÃ¡n, Luis M. and Colliex, Christian},
  Journal                  = {Nature Physics},
  Year                     = {2007},
  Number                   = {5},
  Pages                    = {348-353},
  Volume                   = {3},

  Doi                      = {10.1038/nphys575},
  ISSN                     = {1745-2473
1745-2481},
  Type                     = {Journal Article}
}

@Article{Neu2012a,
  Title                    = {Photophysics of single silicon vacancy centers in diamond: implications for single photon emission},
  Author                   = {Neu, Elke and Agio, Mario and Becher, Christoph},
  Journal                  = {Opt. Express},
  Year                     = {2012},
  Number                   = {18},
  Pages                    = {19956-19971},
  Volume                   = {20},

  Abstract                 = {Single silicon vacancy (SiV) color centers in diamond have recently shown the ability for high brightness, narrow bandwidth, room temperature single photon emission. This work develops a model describing the three level population dynamics of single SiV centers in diamond nanocrystals on iridium surfaces including an intensity dependent de-shelving process. Furthermore, we investigate the brightness and photostability of single centers and find maximum single photon rates of 6.2 Mcps under continuous excitation. We investigate the collection efficiency of the fluorescence and estimate quantum efficiencies of the SiV centers.},
  Doi                      = {10.1364/OE.20.019956},
  Keywords                 = {Quantum optics
Photon statistics
Spectroscopy, condensed matter},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-20-18-19956}
}

@Article{Neu2012,
  Title                    = {Electronic transitions of single silicon vacancy centers in the near-infrared spectral region},
  Author                   = {Neu, Elke and Albrecht, Roland and Fischer, Martin and Gsell, Stefan and Schreck, Matthias and Becher, Christoph},
  Journal                  = {Physical Review B},
  Year                     = {2012},
  Number                   = {24},
  Pages                    = {245207},
  Volume                   = {85},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.85.245207}
}

@Article{Neu2011,
  Title                    = {Narrowband fluorescent nanodiamonds produced from chemical vapor deposition films},
  Author                   = {Neu, E. and Arend, C. and Gross, E. and Guldner, F. and Hepp, C. and Steinmetz, D. and Zscherpel, E. and Ghodbane, S. and Sternschulte, H. and SteinmÃ¼ller-Nethl, D. and Liang, Y. and Krueger, A. and Becher, C.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2011},
  Number                   = {24},
  Pages                    = {243107},
  Volume                   = {98},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.3599608},
  Keywords                 = {fluorescence
nanostructured materials
chemical vapour deposition
nanofabrication
photoluminescence
diamond
infrared spectra},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/apl/98/24/10.1063/1.3599608}
}

@Article{Neu2011a,
  Title                    = {Fluorescence and polarization spectroscopy of single silicon vacancy centers in heteroepitaxial nanodiamonds on iridium},
  Author                   = {Neu, Elke and Fischer, Martin and Gsell, Stefan and Schreck, Matthias and Becher, Christoph},
  Journal                  = {Physical Review B},
  Year                     = {2011},
  Number                   = {20},
  Pages                    = {205211},
  Volume                   = {84},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.84.205211}
}

@Article{Neu2013,
  Title                    = {Low temperature investigations and surface treatments of colloidal narrowband fluorescent nanodiamonds},
  Author                   = {Neu, E. and Guldner, F. and Arend, C. and Liang, Y. and Ghodbane, S. and Sternschulte, H. and SteinmÃ¼ller-Nethl, D. and Krueger, A. and Becher, C.},
  Journal                  = {Journal of Applied Physics},
  Year                     = {2013},
  Number                   = {20},
  Pages                    = {203507},
  Volume                   = {113},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.4807398},
  Keywords                 = {colloidal crystals
oxidation
chemical vapour deposition
diamond
phonons
surface treatment
fluorescence
nanofabrication
nanostructured materials
thin films
Raman spectra
vacancies (crystal)},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/jap/113/20/10.1063/1.4807398}
}

@Article{Neutens2010,
  Title                    = {Electrical excitation of confined surface plasmon polaritons in metallic slot waveguides},
  Author                   = {Neutens, P. and Lagae, L. and Borghs, G. and Van Dorpe, P.},
  Journal                  = {Nano Lett},
  Year                     = {2010},
  Number                   = {4},
  Pages                    = {1429-32},
  Volume                   = {10},

  Abstract                 = {We present the realization of an integrated electrical source of confined surface plasmon polaritons (SPPs) in metal-insulator-metal waveguides. Using an integrated light-emitting diode (LED) and subwavelength slits, we can couple light emitted by the LED directly into waveguided plasmon modes. Polarization-dependent measurements, decay length measurements, and spectral measurements are performed to confirm the electrical excitation of SPPs and characterize the properties of the plasmonic waveguide.},
  Doi                      = {10.1021/nl1003416},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {*Electrons
Equipment Design
Metal Nanoparticles/*chemistry
Nanotechnology/instrumentation/*methods
Quantum Theory
Surface Plasmon Resonance/instrumentation/*methods},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20334350}
}

@Article{Neutens2009,
  Title                    = {Electrical detection of confined gap plasmons in metalâ€“insulatorâ€“metal waveguides},
  Author                   = {Neutens, Pieter and Van Dorpe, Pol and De Vlaminck, Iwijn and Lagae, Liesbet and Borghs, Gustaaf},
  Journal                  = {Nature Photonics},
  Year                     = {2009},
  Number                   = {5},
  Pages                    = {283-286},
  Volume                   = {3},

  Doi                      = {10.1038/nphoton.2009.47},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Nguyen2010,
  Title                    = {Isotope effect in spin response of [pi]-conjugated polymer films and devices},
  Author                   = {Nguyen, Tho D. and Hukic-markosian, Golda and Wang, Fujian and Wojcik, Leonard and Li, Xiao-guang and Ehrenfreund, Eitan and Vardeny, Z. Valy},
  Journal                  = {Nature Materials},
  Year                     = {2010},
  Number                   = {4},
  Pages                    = {345-52},
  Volume                   = {9},

  Abstract                 = {Recent advances in organic spin response include long polaron spin-coherence times measured by optically detected magnetic resonance (ODMR), substantive room-temperature magnetoelectroluminescence and magnetoconductance obtained in organic light-emitting diodes (OLEDs) and spin-polarized carrier injection from ferromagnetic electrodes in organic spin valves (OSVs). Although the hyperfine interaction (HFI) has been foreseen to have an important role in organic spin response, no clear experimental evidence has been reported so far. Using the chemical versatility advantage of the organics, we studied and compared spin responses in films, OLED and OSV devices based on pi-conjugated polymers made of protonated, H-, and deuterated, D-hydrogen having a weaker HFI strength. We demonstrate that the HFI does indeed have a crucial role in all three spin responses. OLED films based on the D-polymers show substantially narrower magneto-electroluminescence and ODMR responses, and as a result of the longer spin diffusion obtained, OSV devices based on D-polymers show a substantially larger magnetoresistance. [PUBLICATION ABSTRACT]},
  Doi                      = {http://dx.doi.org/10.1038/nmat2633},
  ISSN                     = {14761122},
  Keywords                 = {Engineering--Engineering Mechanics And Materials
Materials science
Polymers
Magnetism
Organic light emitting diodes
Comparative studies},
  Type                     = {Journal Article},
  Url                      = {http://ezproxy.lib.uts.edu.au/login?url=http://search.proquest.com/docview/222749369?accountid=17095
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Journal_Search&Ntx=matchallpartial&Ntt=Nature+Materials
http://find.lib.uts.edu.au/search.do?N=0&Ntk=Title_Search&Ntx=matchallpartial&Ntt=Isotope+effect+in+spin+response+of+-conjugated+polymer+films+and+devices
http://sfx.lib.uts.edu.au/sfx_local?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:journal&genre=article&sid=ProQ:ProQ%3Ahealthcompleteshell&atitle=Isotope+effect+in+spin+response+of+%5Bpi%5D-conjugated+polymer+films+and+devices&title=Nature+Materials&issn=14761122&date=2010-04-01&volume=9&issue=4&spage=345&au=Nguyen%2C+Tho+D%3BHukic-markosian%2C+Golda%3BWang%2C+Fujian%3BWojcik%2C+Leonard%3BLi%2C+Xiao-guang%3BEhrenfreund%2C+Eitan%3BVardeny%2C+Z+Valy&isbn=&jtitle=Nature+Materials&btitle=&rft_id=info:eric/&rft_id=info:doi/10.1038%2Fnmat2633}
}

@Article{Ni2012,
  Title                    = {Broadband Light Bending with Plasmonic Nanoantennas},
  Author                   = {Ni, Xingjie and Emani, Naresh K. and Kildishev, Alexander V. and Boltasseva, Alexandra and Shalaev, Vladimir M.},
  Journal                  = {Science},
  Year                     = {2012},
  Number                   = {6067},
  Pages                    = {427-427},
  Volume                   = {335},

  Doi                      = {10.1126/science.1214686},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000299466800038}
}

@Article{Nirmal1996,
  Title                    = {Fluorescence intermittency in single cadmium selenide nanocrystals},
  Author                   = {Nirmal, M. and Dabbousi, B. O. and Bawendi, M. G. and Macklin, J. J. and Trautman, J. K. and Harris, T. D. and Brus, L. E.},
  Journal                  = {Nature},
  Year                     = {1996},
  Number                   = {6603},
  Pages                    = {802-804},
  Volume                   = {383},

  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/383802a0}
}

@Article{Nizovtsev2003,
  Title                    = {NV centers in diamond: spin-selective photokinetics, optical ground-state spin alignment and hole burning},
  Author                   = {Nizovtsev, A. P. and Kilin, S. Ya and Jelezko, F. and Popa, I. and Gruber, A. and Wrachtrup, J.},
  Journal                  = {Physica B: Condensed Matter},
  Year                     = {2003},
  Number                   = {0},
  Pages                    = {106-110},
  Volume                   = {340â€“342},

  Abstract                 = {It is shown that the spin-selective photokinetics of the substitutional nitrogen atom and a vacancy (NV) defect center in diamond, which have been elucidated recently by low-temperature, fine-structure-resolved experiments on an individual NV center in diamond nanocrystals, underlies the optical alignment of the electron spin of the center in the ground 3A state and allows to interpret the complicated hole/antihole burning spectra for NV ensemble in diamond samples with a high NV content.},
  Doi                      = {http://dx.doi.org/10.1016/j.physb.2003.09.014},
  ISSN                     = {0921-4526},
  Keywords                 = {Single defect
Quantum optics
NV center
Diamond},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0921452603006513}
}

@Article{Noda2000,
  Title                    = {Trapping and emission of photons by a single defect in a photonic bandgap structure},
  Author                   = {Noda, S. and Chutinan, A. and Imada, M.},
  Journal                  = {Nature},
  Year                     = {2000},
  Number                   = {6804},
  Pages                    = {608-10},
  Volume                   = {407},

  Abstract                 = {By introducing artificial defects and/or light-emitters into photonic bandgap structures, it should be possible to manipulate photons. For example, it has been predicted that strong localization (or trapping) of photons should occur in structures with single defects, and that the propagation of photons should be controllable using arrays of defects. But there has been little experimental progress in this regard, with the exception of a laser based on a single-defect photonic crystal. Here we demonstrate photon trapping by a single defect that has been created artificially inside a two-dimensional photonic bandgap structure. Photons propagating through a linear waveguide are trapped by the defect, which then emits them to free space. We envisage that this phenomenon may be used in ultra-small optical devices whose function is to selectively drop (or add) photons with various energies from (or to) optical communication traffic. More generally, our work should facilitate the development of all-optical circuits incorporating photonic bandgap waveguides and resonators.},
  Doi                      = {10.1038/35036532},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/11034204}
}

@Article{Noginova2011,
  Title                    = {Light-to-current and current-to-light coupling in plasmonic systems},
  Author                   = {Noginova, N. and Yakim, A. V. and Soimo, J. and Gu, L. and Noginov, M. A.},
  Journal                  = {Physical Review B},
  Year                     = {2011},
  Number                   = {3},
  Volume                   = {84},

  Doi                      = {10.1103/PhysRevB.84.035447},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Novo2009,
  Title                    = {Electrochemical Charging of Single Gold Nanorods},
  Author                   = {Novo, Carolina and Funston, Alison M. and Gooding, Ann K. and Mulvaney, Paul},
  Journal                  = {Journal of the American Chemical Society},
  Year                     = {2009},
  Number                   = {41},
  Pages                    = {14664-14666},
  Volume                   = {131},

  Doi                      = {10.1021/ja905216h},
  ISSN                     = {0002-7863},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/ja905216h}
}

@Article{Novoselov2005,
  Title                    = {Two-dimensional atomic crystals},
  Author                   = {Novoselov, K. S. and Jiang, D. and Schedin, F. and Booth, T. J. and Khotkevich, V. V. and Morozov, S. V. and Geim, A. K.},
  Journal                  = {Proc. Natl. Acad. Sci.},
  Year                     = {2005},
  Number                   = {30},
  Pages                    = {10451-10453},
  Volume                   = {102},

  Abstract                 = {We report free-standing atomic crystals that are strictly 2D and can be viewed as individual atomic planes pulled out of bulk crystals or as unrolled single-wall nanotubes. By using micromechanical cleavage, we have prepared and studied a variety of 2D crystals including single layers of boron nitride, graphite, several dichalcogenides, and complex oxides. These atomically thin sheets (essentially gigantic 2D molecules unprotected from the immediate environment) are stable under ambient conditions, exhibit high crystal quality, and are continuous on a macroscopic scale.},
  Doi                      = {10.1073/pnas.0502848102},
  Type                     = {Journal Article},
  Url                      = {http://www.pnas.org/content/102/30/10451.abstract}
}

@Article{Novotny2011,
  Title                    = {Antennas for light},
  Author                   = {Novotny, Lukas and van Hulst, Niek},
  Journal                  = {Nature Photonics},
  Year                     = {2011},
  Number                   = {2},
  Pages                    = {83-90},
  Volume                   = {5},

  Doi                      = {10.1038/nphoton.2010.237},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Ohno2012,
  Title                    = {Engineering shallow spins in diamond with nitrogen delta-doping},
  Author                   = {Ohno, Kenichi and Joseph Heremans, F. and Bassett, Lee C. and Myers, Bryan A. and Toyli, David M. and Bleszynski Jayich, Ania C. and PalmstroÌ¸m, Christopher J. and Awschalom, David D.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2012},
  Number                   = {8},
  Pages                    = {082413},
  Volume                   = {101},

  Doi                      = {10.1063/1.4748280},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Ohtsu2002,
  Title                    = {Nanophotonics: design, fabrication, and operation of nanometric devices using optical near fields},
  Author                   = {Ohtsu, Motoichi and Kobayashi, K. and Kawazoe, T. and Sangu, S. and Yatsui, Takashi},
  Journal                  = {Selected Topics in Quantum Electronics, IEEE Journal of},
  Year                     = {2002},
  Number                   = {4},
  Pages                    = {839-862},
  Volume                   = {8},

  Abstract                 = {This paper reviews progress in nanophotonics, a novel optical nanotechnology, utilizing local electromagnetic interactions between a few nanometric elements and an optical near field. A prototype of a nanophotonic integrated circuit (IC) is presented, in which the optical near field is used as a carrier to transmit a signal from one nanometric dot to another. Each section of this paper reviews theoretical and experimental studies carried out to assess the possibility of designing, fabricating, and operating each nanophotonic IC device. A key device, the nanophotonic switch, is proposed based on optical near-field energy transfer between quantum dots (QDs). The optical near-field interaction is expressed as the sum of the Yukawa function, and the oscillation period of the nutation of cubic CuCl QDs is estimated to be less than 100 ps. To guarantee one-directional (i.e., irreversible) energy transfer between two resonant levels of QDs, intrasublevel transitions due to phonon coupling are examined by considering a simple two-QD plus phonon heat bath system. As a result, the state-filling time is estimated as 22 ps for CuCl QDs. This time is almost independent of the temperature in the Born-Markov approximation. Using cubic CuCl QDs in a NaCl matrix as a test sample, the optical near-field energy transfer was experimentally verified by near-field optical spectroscopy with a spatial resolution smaller than 50 nm in the near-UV region at 15 K. This transfer occurs from the lowest state of excitons in 4.6-nm QDs to the first dipole-forbidden excited state of excitons in 6.3-nm QDs. To fabricate nanophotonic devices and ICs, chemical vapor deposition using an optical near field is proposed; this is sufficiently precise in controlling the size and position of the deposited material. A novel deposition scheme under nonresonant conditions is also demonstrated and its origin is discussed. In order to confirm the possibility of using a nanometric ZnO dot as a light emitter in a nanophotonic IC, spatially and spectrally resolved photoluminescence imaging of individual ZnO nanocrystallites was carried out with a spatial resolution as high as 55 nm, using a UV fiber probe, and the spectral shift due to the quantum size effect was found. To connect the nanophotonic IC- to external photonic devices, a nanometer-scale waveguide was developed using a metal-coated silicon wedge structure. Illumination (wavelength: 830 nm) of the metal-coated silicon wedge (width: 150 nm) excites a TM plasmon mode with a beam width of 150 nm and propagation length of 2.5 &mu;m. A key device for nanophotonics, an optical near-field probe with an extremely high throughput, was developed by introducing a pyramidal silicon structure with localized surface plasmon resonance at the metallized probe tip. A throughput as high as 2.3% was achieved. Finally, as an application of nanophotonics to, a high-density, high-speed optical memory system, a novel contact slider with a pyramidal silicon probe array was developed. This slider was used for phase-change recording and reading, and a mark length as short as 110 nm was demonstrated.},
  Doi                      = {10.1109/JSTQE.2002.801738},
  ISSN                     = {1077-260X},
  Keywords                 = {II-VI semiconductors
excitons
integrated optoelectronics
nanotechnology
near-field scanning optical microscopy
optical design techniques
optical fabrication
optical storage
phonons
photoluminescence
plasmons
semiconductor quantum dots
zinc compounds
100 ps
15 K
150 nm
2.5 micron
22 ps
4.6 nm
6.3 nm
830 nm
Born-Markov approximation
CuCl
TM plasmon mode
UV fiber probe
Yukawa function
ZnO nanocrystallites
chemical vapor deposition
dipole-forbidden excited state
external photonic devices
high-speed optical memory
local electromagnetic interactions
localized surface plasmon resonance
metal-coated silicon wedge
nanometric devices
nanometric dot
nanometric elements
nanophotonic IC
nanophotonic IC device
nanophotonic integrated circuit
nanophotonics design
nanophotonics fabrication
optical nanotechnology
optical near fields
optical near-field energy transfer
oscillation period
phase-change recording
phonon coupling
phonon heat bath system
pyramidal silicon structure
quantum size effect
resonant levels
spectral shift
spectrally resolved photoluminescence imaging
Energy exchange
High speed optical techniques
Nanophotonics
Nanoscale devices
Optical design
Optical device fabrication
Optical devices
Photonic integrated circuits
Probes
Silicon},
  Type                     = {Journal Article}
}

@Article{Okada2014,
  Title                    = {Direct Chemical Vapor Deposition Growth of WS2 Atomic Layers on Hexagonal Boron Nitride},
  Author                   = {Okada, Mitsuhiro and Sawazaki, Takumi and Watanabe, Kenji and Taniguch, Takashi and Hibino, Hiroki and Shinohara, Hisanori and Kitaura, Ryo},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {8},
  Pages                    = {8273-8277},
  Volume                   = {8},

  Abstract                 = {Atomically thin transition metal dichalcogenides (TMDCs) have attracted considerable interest owing to the spin-valley coupled electronic structure and possibility in next-generation devices. Substrates are one of the most important factors to limit physical properties of atomic-layer materials, and among various substrates so far investigated, hexagonal boron nitride (hBN) is the best substrate to explore the intrinsic properties of atomic layers. Here we report direct chemical vapor deposition (CVD) growth of WS2 onto high-quality hBN using a 3-furnace CVD setup. Triangular-shaped WS2 grown on hBN have shown limited crystallographic orientation that is related to that of the underlying hBN. Photoluminescence spectra of the WS2 show an intense emission peak at 2.01 eV with a quite small fwhm of 26 meV. The sharp emission peak indicates the high quality of the present WS2 atomic layers with high crystallinity and clean interface.},
  Doi                      = {10.1021/nn503093k},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn503093k}
}

@Article{Oort1990,
  Title                    = {Low-field optically detected magnetic resonance of a coupled triplet-doublet defect pair in diamond},
  Author                   = {van Oort, Eric and Stroomer, Paul and Glasbeek, Max},
  Journal                  = {Physical Review B},
  Year                     = {1990},
  Number                   = {13},
  Pages                    = {8605-8608},
  Volume                   = {42},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.42.8605}
}

@Article{Orellana2001,
  Title                    = {Stability of native defects in hexagonal and cubic boron nitride},
  Author                   = {Orellana, Walter and Chacham, H.},
  Journal                  = {Phys. Rev. B},
  Year                     = {2001},
  Number                   = {12},
  Volume                   = {63},

  Type                     = {Journal Article}
}

@Article{Orlinski2003,
  Title                    = {Silicon and carbon vacancies in neutron-irradiated SiC:\quad{}A high-field electron paramagnetic resonance study},
  Author                   = {Orlinski, S. B. and Schmidt, J. and Mokhov, E. N. and Baranov, P. G.},
  Journal                  = {Physical Review B},
  Year                     = {2003},
  Number                   = {12},
  Pages                    = {125207},
  Volume                   = {67},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.67.125207}
}

@Article{Osipov2006,
  Title                    = {Magnetic and high resolution TEM studies of nanographite derived from nanodiamond},
  Author                   = {Osipov, V. Yu and Enoki, T. and Takai, K. and Takahara, K. and Endo, M. and Hayashi, T. and Hishiyama, Y. and Kaburagi, Y. and Vulâ€™, A. Ya},
  Journal                  = {Carbon},
  Year                     = {2006},
  Number                   = {7},
  Pages                    = {1225-1234},
  Volume                   = {44},

  Doi                      = {10.1016/j.carbon.2005.10.047},
  ISSN                     = {00086223},
  Type                     = {Journal Article}
}

@Article{Osswald2008,
  Title                    = {Increase of nanodiamond crystal size by selective oxidation},
  Author                   = {Osswald, S. and Havel, M. and Mochalin, V. and Yushin, G. and Gogotsi, Y.},
  Journal                  = {Diamond and Related Materials},
  Year                     = {2008},
  Number                   = {7-10},
  Pages                    = {1122-1126},
  Volume                   = {17},

  Doi                      = {10.1016/j.diamond.2008.01.102},
  ISSN                     = {09259635},
  Type                     = {Journal Article}
}

@Article{Osterkamp2013,
  Title                    = {Increasing the creation yield of shallow single defects in diamond by surface plasma treatment},
  Author                   = {Osterkamp, Christian and Scharpf, Jochen and Pezzagna, Sebastien and Meijer, Jan and Diemant, Thomas and JuÌˆrgen Behm, Rolf and Naydenov, Boris and Jelezko, Fedor},
  Journal                  = {Applied Physics Letters},
  Year                     = {2013},
  Number                   = {19},
  Pages                    = {193118},
  Volume                   = {103},

  Doi                      = {10.1063/1.4829875},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Oulton2008,
  Title                    = {A hybrid plasmonic waveguide for subwavelength confinement and long-range propagation},
  Author                   = {Oulton, R. F. and Sorger, V. J. and Genov, D. A. and Pile, D. F. P. and Zhang, X.},
  Journal                  = {Nature Photonics},
  Year                     = {2008},
  Number                   = {8},
  Pages                    = {496-500},
  Volume                   = {2},

  Doi                      = {10.1038/nphoton.2008.131},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Oulton2009,
  Title                    = {Plasmon lasers at deep subwavelength scale},
  Author                   = {Oulton, R. F. and Sorger, V. J. and Zentgraf, T. and Ma, R. M. and Gladden, C. and Dai, L. and Bartal, G. and Zhang, X.},
  Journal                  = {Nature},
  Year                     = {2009},
  Number                   = {7264},
  Pages                    = {629-32},
  Volume                   = {461},

  Abstract                 = {Laser science has been successful in producing increasingly high-powered, faster and smaller coherent light sources. Examples of recent advances are microscopic lasers that can reach the diffraction limit, based on photonic crystals, metal-clad cavities and nanowires. However, such lasers are restricted, both in optical mode size and physical device dimension, to being larger than half the wavelength of the optical field, and it remains a key fundamental challenge to realize ultracompact lasers that can directly generate coherent optical fields at the nanometre scale, far beyond the diffraction limit. A way of addressing this issue is to make use of surface plasmons, which are capable of tightly localizing light, but so far ohmic losses at optical frequencies have inhibited the realization of truly nanometre-scale lasers based on such approaches. A recent theoretical work predicted that such losses could be significantly reduced while maintaining ultrasmall modes in a hybrid plasmonic waveguide. Here we report the experimental demonstration of nanometre-scale plasmonic lasers, generating optical modes a hundred times smaller than the diffraction limit. We realize such lasers using a hybrid plasmonic waveguide consisting of a high-gain cadmium sulphide semiconductor nanowire, separated from a silver surface by a 5-nm-thick insulating gap. Direct measurements of the emission lifetime reveal a broad-band enhancement of the nanowire's exciton spontaneous emission rate by up to six times owing to the strong mode confinement and the signature of apparently threshold-less lasing. Because plasmonic modes have no cutoff, we are able to demonstrate downscaling of the lateral dimensions of both the device and the optical mode. Plasmonic lasers thus offer the possibility of exploring extreme interactions between light and matter, opening up new avenues in the fields of active photonic circuits, bio-sensing and quantum information technology.},
  Doi                      = {10.1038/nature08364},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/19718019}
}

@Article{Ozbay2006,
  Title                    = {Plasmonics: Merging photonics and electronics at nanoscale dimensions},
  Author                   = {Ozbay, E.},
  Journal                  = {Science},
  Year                     = {2006},
  Number                   = {5758},
  Pages                    = {189-193},
  Volume                   = {311},

  Doi                      = {10.1126/science.1114849},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000234722200030}
}

@Article{PacilA©2008,
  Title                    = {The two-dimensional phase of boron nitride: Few-atomic-layer sheets and suspended membranes},
  Author                   = {PacilÃ©, D. and Meyer, J. C. and Girit, Ã‡. Ã–. and Zettl, A.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2008},
  Number                   = {13},
  Pages                    = {133107},
  Volume                   = {92},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.2903702},
  Keywords                 = {membranes
optical microscopy
atomic force microscopy
semiconductor growth
vacuum deposition
transmission electron microscopy
III-V semiconductors
boron compounds
wide band gap semiconductors
semiconductor thin films},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/apl/92/13/10.1063/1.2903702}
}

@Article{Pan2012,
  Title                    = {Biaxial compressive strain engineering in graphene/boron nitride heterostructures},
  Author                   = {Pan, W. and Xiao, J. and Zhu, J. and Yu, C. and Zhang, G. and Ni, Z. and Watanabe, K. and Taniguchi, T. and Shi, Y. and Wang, X.},
  Journal                  = {Sci Rep},
  Year                     = {2012},
  Pages                    = {893},
  Volume                   = {2},

  Abstract                 = {Strain engineered graphene has been predicted to show many interesting physics and device applications. Here we study biaxial compressive strain in graphene/hexagonal boron nitride heterostructures after thermal cycling to high temperatures likely due to their thermal expansion coefficient mismatch. The appearance of sub-micron self-supporting bubbles indicates that the strain is spatially inhomogeneous. Finite element modeling suggests that the strain is concentrated on the edges with regular nano-scale wrinkles, which could be a playground for strain engineering in graphene. Raman spectroscopy and mapping is employed to quantitatively probe the magnitude and distribution of strain. From the temperature-dependent shifts of Raman G and 2D peaks, we estimate the TEC of graphene from room temperature to above 1000K for the first time.},
  Doi                      = {10.1038/srep00893},
  ISSN                     = {2045-2322 (Electronic)
2045-2322 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23189242}
}

@Article{Park2014,
  Title                    = {Large-Area Monolayer Hexagonal Boron Nitride on Pt Foil},
  Author                   = {Park, Ji-Hoon and Park, Jin Cheol and Yun, Seok Joon and Kim, Hyun and Luong, Dinh Hoa and Kim, Soo Min and Choi, Soo Ho and Yang, Woochul and Kong, Jing and Kim, Ki Kang and Lee, Young Hee},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {8},
  Pages                    = {8520-8528},
  Volume                   = {8},

  Abstract                 = {Hexagonal boron nitride (h-BN) has recently been in the spotlight due to its numerous applications including its being an ideal substrate for two-dimensional electronics, a tunneling material for vertical tunneling devices, and a growth template for heterostructures. However, to obtain a large area of h-BN film while maintaining uniform thickness is still challenging and has not been realized. Here, we report the systematical study of h-BN growth on Pt foil by using low pressure chemical vapor deposition with a borazine source. The monolayer h-BN film was obtained over the whole Pt foil (2 ? 5 cm2) under <100 mTorr, where the size is limited only by the Pt foil size. A borazine source was catalytically decomposed on the Pt surface, leading to the self-limiting growth of the monolayer without the associating precipitation, which is very similar to the growth of graphene on Cu. The orientation of the h-BN domains was largely confined by the Pt domain, which is confirmed by polarizing optical microscopy (POM) assisted by the nematic liquid crystal (LC) film. The total pressure and orientation of the Pt lattice plane are crucial parameters for thickness control. At high pressure (?0.5 Torr), thick film was grown on Pt (111), and in contrast, thin film was grown on Pt (001). Our advances in monolayer h-BN growth will play an important role to further develop a high quality h-BN film that can be used for vertical tunneling, optoelectronic devices and growth templates for a variety of heterostructures.},
  Doi                      = {10.1021/nn503140y},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn503140y}
}

@Article{Park2015,
  Title                    = {Formation of Hexagonal Boron Nitride by Metal Atomic Vacancy-Assisted Bâ€“N Molecular Diffusion},
  Author                   = {Park, Seongjun and Lee, Jinyeong and Kim, Han Sol and Park, Jong-Bong and Lee, Kang Hyuck and Han, Sang A. and Hwang, Sungwoo and Kim, Sang-Woo and Shin, Hyeon-Jin},
  Journal                  = {ACS Nano},
  Year                     = {2015},
  Number                   = {1},
  Pages                    = {633-638},
  Volume                   = {9},

  Abstract                 = {Because of the low solubility of N atoms in metals, hexagonal boron nitride (h-BN) growth has explained by surface reaction on metal rather than by penetration/precipitation of B and N atoms in metal. Here, we present an impressive pathway of h-BN formation at the interface between Ni and oxide substrate based on B?N molecular diffusion into Ni through individual atomic vacancies. First-principles calculations confirmed the formation energies of the h-BN layers on and under the metal and the probability of B?N molecular diffusion in metal. The interface growth behavior depends on the species of metal catalysts, and these simulation results well support experimental results.},
  Doi                      = {10.1021/nn505960b},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn505960b}
}

@Article{Park2014a,
  Title                    = {Interlayer coupling enhancement in graphene/hexagonal boron nitride heterostructures by intercalated defects or vacancies},
  Author                   = {Park, S. and Park, C. and Kim, G.},
  Journal                  = {J Chem Phys},
  Year                     = {2014},
  Number                   = {13},
  Pages                    = {134706},
  Volume                   = {140},

  Abstract                 = {Hexagonal boron nitride (hBN), a remarkable material with a two-dimensional atomic crystal structure, has the potential to fabricate heterostructures with unusual properties. We perform first-principles calculations to determine whether intercalated metal atoms and vacancies can mediate interfacial coupling and influence the structural and electronic properties of the graphene/hBN heterostructure. Metal impurity atoms (Li, K, Cr, Mn, Co, and Cu), acting as extrinsic defects between the graphene and hBN sheets, produce n-doped graphene. We also consider intrinsic vacancy defects and find that a boron monovacancy in hBN acts as a magnetic dopant for graphene, whereas a nitrogen monovacancy in hBN serves as a nonmagnetic dopant for graphene. In contrast, the smallest triangular vacancy defects in hBN are unlikely to result in significant changes in the electronic transport of graphene. Our findings reveal that a hBN layer with some vacancies or metal impurities enhances the interlayer coupling in the graphene/hBN heterostructure with respect to charge doping and electron scattering.},
  Doi                      = {10.1063/1.4870097},
  ISSN                     = {1089-7690 (Electronic)
0021-9606 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24712807}
}

@Article{Pawlak2013,
  Title                    = {Local detection of nitrogen-vacancy centers in a nanodiamond monolayer},
  Author                   = {Pawlak, R. and Glatzel, T. and Pichot, V. and Schmidlin, L. and Kawai, S. and Fremy, S. and Spitzer, D. and Meyer, E.},
  Journal                  = {Nano Lett},
  Year                     = {2013},
  Number                   = {12},
  Pages                    = {5803-7},
  Volume                   = {13},

  Abstract                 = {Nitrogen-vacancy defect centers (NV) contained in nanodiamonds (NDs) are a promising candidate in quantum information processing and single photon sources due to the capability of controlling their assembly on various surfaces. However, their detection with traditional optical techniques becomes challenging when probing high NV densities at the nanometer scale. Here, we combine scanning probe techniques to characterize in a monolayer the structural and electronic properties of bucky-diamonds with sizes below 10 nm. We further observe by light-assisted Kelvin- and scanning tunneling spectroscopy a clear signature of negatively charged subsurface NV centers in NDs at the nanoscale where conventional techniques are limited.},
  Doi                      = {10.1021/nl402243s},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Light
Nanodiamonds/*chemistry
Nitrogen/*chemistry
*Optics and Photonics
Photons
Surface Properties},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24144018}
}

@Article{Pease1950,
  Title                    = {Crystal Structure of Boron Nitride},
  Author                   = {Pease, R. S.},
  Journal                  = {Nature},
  Year                     = {1950},

  Month                    = may,
  Number                   = {4201},
  Pages                    = {722--723},
  Volume                   = {165},

  Comment                  = {10.1038/165722b0},
  Owner                    = {Toan},
  Timestamp                = {2015.04.22},
  Url                      = {http://dx.doi.org/10.1038/165722b0}
}

@Article{Pelton2002,
  Title                    = {Efficient Source of Single Photons: A Single Quantum Dot in a Micropost Microcavity},
  Author                   = {Pelton, Matthew and Santori, Charles and VucÌ†koviÄ‡, Jelena and Zhang, Bingyang and Solomon, Glenn and Plant, Jocelyn and Yamamoto, Yoshihisa},
  Journal                  = {Physical Review Letters},
  Year                     = {2002},
  Number                   = {23},
  Volume                   = {89},

  Doi                      = {10.1103/PhysRevLett.89.233602},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Pendry2012,
  Title                    = {Transformation Optics and Subwavelength Control of Light},
  Author                   = {Pendry, J. B. and Aubry, A. and Smith, D. R. and Maier, S. A.},
  Journal                  = {Science},
  Year                     = {2012},
  Number                   = {6094},
  Pages                    = {549-552},
  Volume                   = {337},

  Abstract                 = {Our intuitive understanding of light has its foundation in the ray approximation and is intimately connected with our vision. As far as our eyes are concerned, light behaves like a stream of particles. We look inside the wavelength and study the properties of plasmonic structures with dimensions of just a few nanometers, where at a tenth or even a hundredth of the wavelength of visible light the ray picture fails. We review the concept of transformation optics that manipulates electric and magnetic field lines, rather than rays; can provide an equally intuitive understanding of subwavelength phenomena; and at the same time can be an exact description at the level of Maxwell's equations.},
  Doi                      = {10.1126/science.1220600},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000307058700035}
}

@Article{Perdew1996,
  Title                    = {Generalized Gradient Approximation Made Simple},
  Author                   = {Perdew, John P. and Burke, Kieron and Ernzerhof, Matthias},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {1996},
  Number                   = {18},
  Pages                    = {3865--3868},
  Volume                   = {77},

  Owner                    = {Toan},
  Publisher                = {American Physical Society},
  Refid                    = {10.1103/PhysRevLett.77.3865},
  Timestamp                = {2015.04.14},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.77.3865}
}

@Article{Pfaff2013,
  Title                    = {Top-down fabrication of plasmonic nanostructures for deterministic coupling to single quantum emitters},
  Author                   = {Pfaff, Wolfgang and Vos, Arthur and Hanson, Ronald},
  Journal                  = {Journal of Applied Physics},
  Year                     = {2013},
  Number                   = {2},
  Pages                    = {024310},
  Volume                   = {113},

  Doi                      = {10.1063/1.4774240},
  ISSN                     = {00218979},
  Type                     = {Journal Article}
}

@Article{Piccione2014,
  Title                    = {Tailoring light-matter coupling in semiconductor and hybrid-plasmonic nanowires},
  Author                   = {Piccione, B. and Aspetti, C. O. and Cho, C. H. and Agarwal, R.},
  Journal                  = {Rep Prog Phys},
  Year                     = {2014},
  Number                   = {8},
  Pages                    = {086401},
  Volume                   = {77},

  Abstract                 = {Understanding interactions between light and matter is central to many fields, providing invaluable insights into the nature of matter. In its own right, a greater understanding of light-matter coupling has allowed for the creation of tailored applications, resulting in a variety of devices such as lasers, switches, sensors, modulators, and detectors. Reduction of optical mode volume is crucial to enhancing light-matter coupling strength, and among solid-state systems, self-assembled semiconductor and hybrid-plasmonic nanowires are amenable to creation of highly-confined optical modes. Following development of unique spectroscopic techniques designed for the nanowire morphology, carefully engineered semiconductor nanowire cavities have recently been tailored to enhance light-matter coupling strength in a manner previously seen in optical microcavities. Much smaller mode volumes in tailored hybrid-plasmonic nanowires have recently allowed for similar breakthroughs, resulting in sub-picosecond excited-state lifetimes and exceptionally high radiative rate enhancement. Here, we review literature on light-matter interactions in semiconductor and hybrid-plasmonic monolithic nanowire optical cavities to highlight recent progress made in tailoring light-matter coupling strengths. Beginning with a discussion of relevant concepts from optical physics, we will discuss how our knowledge of light-matter coupling has evolved with our ability to produce ever-shrinking optical mode volumes, shifting focus from bulk materials to optical microcavities, before moving on to recent results obtained from semiconducting nanowires.},
  Doi                      = {10.1088/0034-4885/77/8/086401},
  ISSN                     = {1361-6633 (Electronic)
0034-4885 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25093385}
}

@Article{Plakhotnik1996,
  Title                    = {Nonlinear Spectroscopy on a Single Quantum System: Two-Photon Absorption of a Single Molecule},
  Author                   = {Plakhotnik, Taras and Walser, Daniel and Pirotta, Marco and Renn, Alois and Wild, Urs P.},
  Journal                  = {Science},
  Year                     = {1996},
  Number                   = {5256},
  Pages                    = {1703--1705},
  Volume                   = {271},

  Abstract                 = {Two-photon fluorescence excitation spectra of single diphenyloctatetraene molecules trapped in an n-tetradecane matrix were measured at cryogenic temperatures. The purely electronic zero-phonon line (transition at 444 nanometers) of these single molecules with a width of about 60 megahertz was excited by a continuous-wave, single-mode laser at 888 nanometers. Even though the two-photon absorption cross section is extremely small, a high photon count rate and low background allowed nonlinear spectroscopy to be extended to the single-molecule level. This experiment also suggests the possibility of two-photon single-molecule scanning microscopy.},
  Comment                  = {10.1126/science.271.5256.1703},
  Owner                    = {Toan},
  Timestamp                = {2015.04.10},
  Url                      = {http://www.sciencemag.org/content/271/5256/1703.abstract}
}

@Article{Pompa2006,
  Title                    = {Metal-enhanced fluorescence of colloidal nanocrystals with nanoscale control},
  Author                   = {Pompa, P. P. and Martiradonna, L. and Torre, A. D. and Sala, F. D. and Manna, L. and De Vittorio, M. and Calabi, F. and Cingolani, R. and Rinaldi, R.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2006},
  Number                   = {2},
  Pages                    = {126-30},
  Volume                   = {1},

  Abstract                 = {Engineering the spectral properties of fluorophores, such as the enhancement of luminescence intensity, can be achieved through coupling with surface plasmons in metallic nanostructures. This process, referred to as metal-enhanced fluorescence, offers promise for a range of applications, including LEDs, sensor technology, microarrays and single-molecule studies. It becomes even more appealing when applied to colloidal semiconductor nanocrystals, which exhibit size-dependent optical properties, have high photochemical stability, and are characterized by broad excitation spectra and narrow emission bands. Other approaches have relied upon the coupling of fluorophores (typically organic dyes) to random distributions of metallic nanoparticles or nanoscale roughness in metallic films. Here, we develop a new strategy based on the highly reproducible fabrication of ordered arrays of gold nanostructures coupled to CdSe/ZnS nanocrystals dispersed in a polymer blend. We demonstrate the possibility of obtaining precise control and a high spatial selectivity of the fluorescence enhancement process.},
  Doi                      = {10.1038/nnano.2006.93},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {Cadmium Compounds/*chemistry
Crystallization/*methods
Gold Colloid/*chemistry
Nanostructures/*chemistry
Selenium Compounds/*chemistry
Spectrometry, Fluorescence/*methods
Surface Plasmon Resonance/*methods
Zinc Compounds/*chemistry},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/18654164}
}

@Article{Press2007,
  Title                    = {Photon Antibunching from a Single Quantum-Dot-Microcavity System in the Strong Coupling Regime},
  Author                   = {Press, David and GÃ¶tzinger, Stephan and Reitzenstein, Stephan and Hofmann, Carolin and LÃ¶ffler, Andreas and Kamp, Martin and Forchel, Alfred and Yamamoto, Yoshihisa},
  Journal                  = {Physical Review Letters},
  Year                     = {2007},
  Number                   = {11},
  Volume                   = {98},

  Doi                      = {10.1103/PhysRevLett.98.117402},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Pryce1950,
  Title                    = {A Modified Perturbation Procedure for a Problem in Paramagnetism},
  Author                   = {Pryce, M. H. L.},
  Journal                  = {Proceedings of the Physical Society. Section A},
  Year                     = {1950},
  Number                   = {1},
  Pages                    = {25},
  Volume                   = {63},

  Abstract                 = {A modified perturbation technique is described for problems in which second-order effects are comparable in magnitude with first-order effects, where orthodox methods break down. It is applied to the energy levels of paramagnetic ions in a crystal, giving an effective Hamiltonian in which the Stark splitting, the anomalous g -value and the temperature-independent paramagnetism are clearly exhibited.},
  ISSN                     = {0370-1298},
  Type                     = {Journal Article},
  Url                      = {http://stacks.iop.org/0370-1298/63/i=1/a=304}
}

@Article{Punj2013,
  Title                    = {A plasmonic antenna-in-box platform for enhanced single-molecule analysis at micromolar concentrations},
  Author                   = {Punj, Deep and Mivelle, Mathieu and Moparthi, Satish Babu and van Zanten, Thomas S. and Rigneault, Herve and van Hulst, Niek F. and Garcia-Parajo, Maria F. and Wenger, Jerome},
  Journal                  = {Nat Nano},
  Year                     = {2013},
  Number                   = {7},
  Pages                    = {512-516},
  Volume                   = {8},

  Doi                      = {10.1038/nnano.2013.98
http://www.nature.com/nnano/journal/v8/n7/abs/nnano.2013.98.html},
  ISSN                     = {1748-3387},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nnano.2013.98}
}

@Article{Purcell1946,
  Title                    = {Resonance Absorption by Nuclear Magnetic Moments in a Solid},
  Author                   = {Purcell, E. M. and Torrey, H. C. and Pound, R. V.},
  Journal                  = {Physical Review},
  Year                     = {1946},
  Number                   = {1-2},
  Pages                    = {37-38},
  Volume                   = {69},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRev.69.37}
}

@Article{Qian2014,
  Title                    = {Electrical Tuning of Surface Plasmon Polariton Propagation in Grapheneâ€“Nanowire Hybrid Structure},
  Author                   = {Qian, Haoliang and Ma, Yaoguang and Yang, Qing and Chen, Bigeng and Liu, Ying and Guo, Xin and Lin, Shisheng and Ruan, Jili and Liu, Xu and Tong, Limin and Wang, Zhong Lin},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {3},
  Pages                    = {2584-2589},
  Volume                   = {8},

  Doi                      = {10.1021/nn406221s},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn406221s}
}

@Article{Qin1998,
  Title                    = {Tem characterization of nanodiamond thin films},
  Author                   = {Qin, L. C. and Zhou, D. and Krauss, A. R. and Gruen, D. M.},
  Journal                  = {Nanostructured Materials},
  Year                     = {1998},
  Number                   = {4},
  Pages                    = {649-660},
  Volume                   = {10},

  Abstract                 = {The microstructure of thin films grown by microwave plasma-enhanced chemical vapor deposition (MPCVD) from fullerene C60 precursors has been characterized by scanning electron microscopy (SEM), selected-area electron diffraction (SAED), bright-field electron microscopy, high-resolution electron microscopy (HREM), and parallel electron energyloss spectroscopy (PEELS). The films are composed of nanosize crystallites of diamond, and no graphitic or amorphous phases were observed. The diamond crystallite size measured from lattice images shows that most grains range between 3â€“5 nm, reflecting a gamma distribution. SAED gave no evidence of either sp2-bonded glassy carbon or sp3-bonded diamondlike amorphous carbon. The sp2-bonded configuration found in PEELS was attributed to grain boundary carbon atoms, which constitute 5â€“10% of the total. Occasionally observed larger diamond grains tend to be highly faulted.},
  Doi                      = {http://dx.doi.org/10.1016/S0965-9773(98)00092-0},
  ISSN                     = {0965-9773},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0965977398000920}
}

@Article{Rabeau2007,
  Title                    = {Single Nitrogen Vacancy Centers in Chemical Vapor Deposited Diamond Nanocrystals},
  Author                   = {Rabeau, J. R. and Stacey, A. and Rabeau, A. and Prawer, S. and Jelezko, F. and Mirza, I. and Wrachtrup, J.},
  Journal                  = {Nano Letters},
  Year                     = {2007},
  Number                   = {11},
  Pages                    = {3433-3437},
  Volume                   = {7},

  Doi                      = {10.1021/nl0719271},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl0719271}
}

@Article{Radisavljevic2011,
  Title                    = {Single-layer MoS2 transistors},
  Author                   = {Radisavljevic, B and Radenovic, A and Brivio, J and Giacometti, V and Kis, A},
  Journal                  = {Nature Nanotechnology},
  Year                     = {2011},
  Number                   = {3},
  Pages                    = {147--50},
  Volume                   = {6},

  Abstract                 = {Two-dimensional materials are attractive for use in next-generation nanoelectronic devices because, compared to one-dimensional materials, it is relatively easy to fabricate complex structures from them. The most widely studied two-dimensional material is graphene, both because of its rich physics and its high mobility. However, pristine graphene does not have a bandgap, a property that is essential for many applications, including transistors. Engineering a graphene bandgap increases fabrication complexity and either reduces mobilities to the level of strained silicon films or requires high voltages. Although single layers of MoS(2) have a large intrinsic bandgap of 1.8 eV (ref. 16), previously reported mobilities in the 0.5-3 cm(2) V(-1) s(-1) range are too low for practical devices. Here, we use a halfnium oxide gate dielectric to demonstrate a room-temperature single-layer MoS(2) mobility of at least 200 cm(2) V(-1) s(-1), similar to that of graphene nanoribbons, and demonstrate transistors with room-temperature current on/off ratios of 1 Ã-- 10(8) and ultralow standby power dissipation. Because monolayer MoS(2) has a direct bandgap, it can be used to construct interband tunnel FETs, which offer lower power consumption than classical transistors. Monolayer MoS(2) could also complement graphene in applications that require thin transparent semiconductors, such as optoelectronics and energy harvesting.},
  Address                  = {London},
  Comment                  = {Copyright - Copyright Nature Publishing Group Mar 2011
Last updated - 2014-04-02},
  ISSN                     = {17483387},
  Keywords                 = {Physics, Disulfides, Nanotubes, Carbon, Silicon Dioxide, Graphite, Molybdenum, Silicon, molybdenum disulfide, Silicon -- chemistry, Equipment Design, Nanotubes, Carbon -- chemistry, Temperature, Microscopy, Atomic Force -- methods, Nanotechnology -- methods, Graphite -- chemistry, Silicon Dioxide -- chemistry, Surface Properties, Disulfides -- chemistry, Nanostructures -- chemistry, Nanotechnology -- instrumentation, Molybdenum -- chemistry, Semiconductors -- instrumentation, Transistors, Electronic},
  Owner                    = {Toan},
  Publisher                = {Nature Publishing Group},
  Timestamp                = {2015.04.09},
  Url                      = {http://ezproxy.lib.uts.edu.au/login?url=http://search.proquest.com/docview/868398470?accountid=17095}
}

@Article{Radulaski2015,
  Title                    = {Visible Photoluminescence from Cubic (3C) Silicon Carbide Microdisks Coupled to High Quality Whispering Gallery Modes},
  Author                   = {Radulaski, Marina and Babinec, Thomas M. and MÃ¼ller, Kai and Lagoudakis, Konstantinos G. and Zhang, Jingyuan Linda and Buckley, Sonia and Kelaita, Yousif A. and Alassaad, Kassem and Ferro, Gabriel and VuÄ?koviÄ‡, Jelena},
  Journal                  = {ACS Photonics},
  Year                     = {2015},
  Number                   = {1},
  Pages                    = {14-19},
  Volume                   = {2},

  Doi                      = {10.1021/ph500384p},
  ISSN                     = {2330-4022
2330-4022},
  Type                     = {Journal Article}
}

@Article{Rakovich2015,
  Title                    = {Plasmonic Control of Radiative Properties of Semiconductor Quantum Dots Coupled to Plasmonic Ring Cavities},
  Author                   = {Rakovich, Aliaksandra and Albella, Pablo and Maier, Stefan A.},
  Journal                  = {ACS Nano},
  Year                     = {2015},

  Abstract                 = {In recent years, a lot of effort has been made to achieve controlled delivery of target particles to the hotspots of plasmonic nanoantennas, in order to probe and/or exploit the extremely large field enhancements produced by such structures. While in many cases such high fields are advantageous, there are instances where they should be avoided. In this work, we consider the implications of using the standard nanoantenna geometries when colloidal quantum dots are employed as target entities. We show that in this case, and for various reasons, dimer antennas are not the optimum choice. Plasmonic ring cavities are a better option despite low field enhancements, as they allow collective coupling of many quantum dots in a reproducible and predictable manner. In cases where larger field enhancements are required, or for larger quantum dots, nonconcentric ring-disk cavities can be employed instead.},
  Doi                      = {10.1021/nn506433e},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn506433e}
}

@Article{Rakovich2015a,
  Title                    = {Plasmonic Control of Radiative Properties of Semiconductor Quantum Dots Coupled to Plasmonic Ring Cavities},
  Author                   = {Rakovich, Aliaksandra and Albella, Pablo and Maier, Stefan A.},
  Journal                  = {ACS Nano},
  Year                     = {2015},

  Abstract                 = {In recent years, a lot of effort has been made to achieve controlled delivery of target particles to the hotspots of plasmonic nanoantennas, in order to probe and/or exploit the extremely large field enhancements produced by such structures. While in many cases such high fields are advantageous, there are instances where they should be avoided. In this work, we consider the implications of using the standard nanoantenna geometries when colloidal quantum dots are employed as target entities. We show that in this case, and for various reasons, dimer antennas are not the optimum choice. Plasmonic ring cavities are a better option despite low field enhancements, as they allow collective coupling of many quantum dots in a reproducible and predictable manner. In cases where larger field enhancements are required, or for larger quantum dots, nonconcentric ring-disk cavities can be employed instead.},
  Doi                      = {10.1021/nn506433e},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn506433e}
}

@Article{Raty2003,
  Title                    = {Quantum Confinement and Fullerenelike Surface Reconstructions in Nanodiamonds},
  Author                   = {Raty, Jean-Yves and Galli, Giulia and Bostedt, C. and van Buuren, Tony and Terminello, Louis},
  Journal                  = {Physical Review Letters},
  Year                     = {2003},
  Number                   = {3},
  Volume                   = {90},

  Doi                      = {10.1103/PhysRevLett.90.037401},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Reddy1987,
  Title                    = {Two-laser spectral hole burning in a colour centre in diamond},
  Author                   = {Reddy, N. R. S. and Manson, N. B. and Krausz, E. R.},
  Journal                  = {Journal of Luminescence},
  Year                     = {1987},
  Number                   = {1â€“6},
  Pages                    = {46-47},
  Volume                   = {38},

  Abstract                 = {Using two high-resolution lasers a short lived (âˆ¼1 ms) hole burning spectrum has been observed in the 637 nm zero-phonon transition associated with the nitrogen-vacancy centre in diamond. Amongst the prominent antiholes the ones at Â±2.88 GHz coincide in frequency with that obtained in EPR for a spin-doublet-singlet splitting of a metastable 3A state. In this work it is claimed that 3A is the ground state and this is supported by the observation of temperature-dependent magnetic circular dichroism signals. Details in the hole burning spectrum are then interpreted in terms of a strain split 3Aâ†’3E transition.},
  Doi                      = {http://dx.doi.org/10.1016/0022-2313(87)90057-3},
  ISSN                     = {0022-2313},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/0022231387900573}
}

@Article{Redman1991,
  Title                    = {Spin dynamics and electronic states of N-V centers in diamond by EPR and four-wave-mixing spectroscopy},
  Author                   = {Redman, D. and Brown, S. and Sands, R. and Rand, S.},
  Journal                  = {Physical Review Letters},
  Year                     = {1991},
  Number                   = {24},
  Pages                    = {3420-3423},
  Volume                   = {67},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.67.3420}
}

@Article{Reich2005,
  Title                    = {Resonant Raman scattering in cubic and hexagonal boron nitride},
  Author                   = {Reich, S. and Ferrari, A. C. and Arenal, R. and Loiseau, A. and Bello, I. and Robertson, J.},
  Journal                  = {Physical Review B},
  Year                     = {2005},
  Number                   = {20},
  Pages                    = {205201},
  Volume                   = {71},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.71.205201}
}

@Article{Reich2004,
  Title                    = {Raman spectroscopy of graphite},
  Author                   = {Reich, S. and Thomsen, C.},
  Journal                  = {Philosophical Transactions of the Royal Society a-Mathematical Physical and Engineering Sciences},
  Year                     = {2004},
  Number                   = {1824},
  Pages                    = {2271-2288},
  Volume                   = {362},

  Abstract                 = {We present a review of the Raman spectra of graphite from an experimental and theoretical point of view. The disorder-induced Raman bands in this material have been a puzzling Raman problem for almost 30 years. Double-resonant Raman scattering explains their origin as well as the excitation-energy dependence, the overtone spectrum and the difference between Stokes and anti-Stokes scattering. We develop the symmetry-imposed selection rules for double-resonant Raman scattering in graphite and point out misassignments in previously published works. An excellent agreement is found between the graphite phonon dispersion from double-resonant Raman scattering and other experimental methods.},
  Doi                      = {10.1098/rsta.2004.1454},
  ISSN                     = {1364-503X},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000224919400002}
}

@Article{Reithmaier2004,
  Title                    = {Strong coupling in a single quantum dot-semiconductor microcavity system},
  Author                   = {Reithmaier, J. P. and Sek, G. and Loffler, A. and Hofmann, C. and Kuhn, S. and Reitzenstein, S. and Keldysh, L. V. and Kulakovskii, V. D. and Reinecke, T. L. and Forchel, A.},
  Journal                  = {Nature},
  Year                     = {2004},
  Number                   = {7014},
  Pages                    = {197-200},
  Volume                   = {432},

  Abstract                 = {Cavity quantum electrodynamics, a central research field in optics and solid-state physics, addresses properties of atom-like emitters in cavities and can be divided into a weak and a strong coupling regime. For weak coupling, the spontaneous emission can be enhanced or reduced compared with its vacuum level by tuning discrete cavity modes in and out of resonance with the emitter. However, the most striking change of emission properties occurs when the conditions for strong coupling are fulfilled. In this case there is a change from the usual irreversible spontaneous emission to a reversible exchange of energy between the emitter and the cavity mode. This coherent coupling may provide a basis for future applications in quantum information processing or schemes for coherent control. Until now, strong coupling of individual two-level systems has been observed only for atoms in large cavities. Here we report the observation of strong coupling of a single two-level solid-state system with a photon, as realized by a single quantum dot in a semiconductor microcavity. The strong coupling is manifest in photoluminescence data that display anti-crossings between the quantum dot exciton and cavity-mode dispersion relations, characterized by a vacuum Rabi splitting of about 140 microeV.},
  Doi                      = {10.1038/nature02969},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/15538362}
}

@Article{Riedrich-Moller2012,
  Title                    = {One- and two-dimensional photonic crystal microcavities in single crystal diamond},
  Author                   = {Riedrich-Moller, J. and Kipfstuhl, L. and Hepp, C. and Neu, E. and Pauly, C. and Mucklich, F. and Baur, A. and Wandt, M. and Wolff, S. and Fischer, M. and Gsell, S. and Schreck, M. and Becher, C.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {69-74},
  Volume                   = {7},

  Abstract                 = {Diamond is an attractive material for photonic quantum technologies because its colour centres have a number of outstanding properties, including bright single photon emission and long spin coherence times. To take advantage of these properties it is favourable to directly fabricate optical microcavities in high-quality diamond samples. Such microcavities could be used to control the photons emitted by the colour centres or to couple widely separated spins. Here, we present a method for the fabrication of one- and two-dimensional photonic crystal microcavities with quality factors of up to 700 in single crystal diamond. Using a post-processing etching technique, we tune the cavity modes into resonance with the zero phonon line of an ensemble of silicon-vacancy colour centres, and we measure an intensity enhancement factor of 2.8. The controlled coupling of colour centres to photonic crystal microcavities could pave the way to larger-scale photonic quantum devices based on single crystal diamond.},
  Doi                      = {10.1038/nnano.2011.190},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22081214}
}

@Article{Robertson2002,
  Title                    = {Diamond-like amorphous carbon},
  Author                   = {Robertson, J.},
  Journal                  = {Materials Science and Engineering: R: Reports},
  Year                     = {2002},
  Number                   = {4â€“6},
  Pages                    = {129--281},
  Volume                   = {37},

  Abstract                 = {Diamond-like carbon (DLC) is a metastable form of amorphous carbon with significant sp3 bonding. DLC is a semiconductor with a high mechanical hardness, chemical inertness, and optical transparency. This review will describe the deposition methods, deposition mechanisms, characterisation methods, electronic structure, gap states, defects, doping, luminescence, field emission, mechanical properties and some applications of DLCs. The films have widespread applications as protective coatings in areas, such as magnetic storage disks, optical windows and micro-electromechanical devices (MEMs).},
  ISSN                     = {0927-796X},
  Keywords                 = {Diamond-like carbon, Properties, Applications},
  Owner                    = {Toan},
  Timestamp                = {2015.04.10},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0927796X02000050}
}

@Article{Robledo2011,
  Title                    = {Spin dynamics in the optical cycle of single nitrogen-vacancy centres in diamond},
  Author                   = {Robledo, Lucio and Bernien, Hannes and Sar, Toeno van der and Hanson, Ronald},
  Journal                  = {New Journal of Physics},
  Year                     = {2011},
  Number                   = {2},
  Pages                    = {025013},
  Volume                   = {13},

  Doi                      = {10.1088/1367-2630/13/2/025013},
  ISSN                     = {1367-2630},
  Type                     = {Journal Article}
}

@Article{Roelkens2006,
  Title                    = {Laser emission and photodetection in an InP/InGaAsP layer integrated on and coupled to a Silicon-on-Insulator waveguide circuit},
  Author                   = {Roelkens, G. and Van Thourhout, D. and Baets, R. and NÃ¶tzel, R. and Smit, M.},
  Journal                  = {Optics Express},
  Year                     = {2006},
  Number                   = {18},
  Pages                    = {8154-8159},
  Volume                   = {14},

  Abstract                 = {Laser emission from an InP/InGaAsP thin film epitaxial layer bonded to a Silicon-on-Insulator waveguide circuit was observed. Adhesive bonding using divinyl-tetramethyldisiloxane-benzocyclobutene (DVS-BCB) was used to integrate the InP/InGaAsP epitaxial layers onto the waveguide circuit. Light is coupled from the laser diode into an underlying waveguide using an adiabatic inverted taper approach. 0.9mW optical power was coupled into the SOI waveguide using a 500?m long laser. Besides for use as a laser diode, the same type of devices can be used as a photodetector.50?m long devices obtained a responsivity of 0.23A/W.},
  Doi                      = {10.1364/OE.14.008154},
  Keywords                 = {Integrated optics
Optical fabrication},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-14-18-8154}
}

@Article{Rogach2008,
  Title                    = {Light-emitting diodes with semiconductor nanocrystals},
  Author                   = {Rogach, A. L. and Gaponik, N. and Lupton, J. M. and Bertoni, C. and Gallardo, D. E. and Dunn, S. and Li Pira, N. and Paderi, M. and Repetto, P. and Romanov, S. G. and O'Dwyer, C. and Sotomayor Torres, C. M. and Eychmuller, A.},
  Journal                  = {Angew Chem Int Ed Engl},
  Year                     = {2008},
  Number                   = {35},
  Pages                    = {6538-49},
  Volume                   = {47},

  Abstract                 = {Colloidal semiconductor nanocrystals are promising luminophores for creating a new generation of electroluminescence devices. Research on semiconductor nanocrystal based light-emitting diodes (LEDs) has made remarkable advances in just one decade: the external quantum efficiency has improved by over two orders of magnitude and highly saturated color emission is now the norm. Although the device efficiencies are still more than an order of magnitude lower than those of the purely organic LEDs there are potential advantages associated with nanocrystal-based devices, such as a spectrally pure emission color, which will certainly merit future research. Further developments of nanocrystal-based LEDs will be improving material stability, understanding and controlling chemical and physical phenomena at the interfaces, and optimizing charge injection and charge transport.},
  Doi                      = {10.1002/anie.200705109},
  ISSN                     = {1521-3773 (Electronic)
1433-7851 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/18666276}
}

@Article{Rondin2010,
  Title                    = {Surface-induced charge state conversion of nitrogen-vacancy defects in nanodiamonds},
  Author                   = {Rondin, L. and Dantelle, G. and Slablab, A. and Grosshans, F. and Treussart, F. and Bergonzo, P. and Perruchas, S. and Gacoin, T. and Chaigneau, M. and Chang, H. C. and Jacques, V. and Roch, J. F.},
  Journal                  = {Physical Review B},
  Year                     = {2010},
  Number                   = {11},
  Volume                   = {82},

  Doi                      = {10.1103/PhysRevB.82.115449},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Rosskopf2014,
  Title                    = {Investigation of Surface Magnetic Noise by Shallow Spins in Diamond},
  Author                   = {Rosskopf, T. and Dussaux, A. and Ohashi, K. and Loretz, M. and Schirhagl, R. and Watanabe, H. and Shikata, S. and Itoh, K. â€‰M and Degen, C. â€‰L},
  Journal                  = {Physical Review Letters},
  Year                     = {2014},
  Number                   = {14},
  Volume                   = {112},

  Doi                      = {10.1103/PhysRevLett.112.147602},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Ruan2006,
  Title                    = {Enhanced Transmission through Periodic Arrays of Subwavelength Holes: The Role of Localized Waveguide Resonances},
  Author                   = {Ruan, Zhichao and Qiu, Min},
  Journal                  = {Physical Review Letters},
  Year                     = {2006},
  Number                   = {23},
  Volume                   = {96},

  Doi                      = {10.1103/PhysRevLett.96.233901},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Rugar1994,
  Title                    = {Force Detection of Nuclear Magnetic Resonance},
  Author                   = {Rugar, D. and ZÃ¼ger, O. and Hoen, S. and Yannoni, C. S. and Vieth, H.-M. and Kendrick, R. D.},
  Journal                  = {Science},
  Year                     = {1994},
  Number                   = {5165},
  Pages                    = {1560-1563},
  Volume                   = {264},

  Abstract                 = {Micromechanical sensing of magnetic force was used to detect nuclear magnetic resonance with exceptional sensitivity and spatial resolution. With a 900 angstrom thick silicon nitride cantilever capable of detecting subfemtonewton forces, a single shot sensitivity of 1.6 x 1013 protons was achieved for an ammonium nitrate sample mounted on the cantilever. A nearby millimeter-size iron particle produced a 600 tesla per meter magnetic field gradient, resulting in a spatial resolution of 2.6 micrometers in one dimension. These results suggest that magnetic force sensing is a viable approach for enhancing the sensitivity and spatial resolution of nuclear magnetic resonance microimaging.},
  Doi                      = {10.1126/science.264.5165.1560},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/264/5165/1560.abstract}
}

@Article{Rybczynski2007,
  Title                    = {Subwavelength waveguide for visible light},
  Author                   = {Rybczynski, J. and Kempa, K. and Herczynski, A. and Wang, Y. and Naughton, M. J. and Ren, Z. F. and Huang, Z. P. and Cai, D. and Giersig, M.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2007},
  Number                   = {2},
  Pages                    = {021104},
  Volume                   = {90},

  Doi                      = {10.1063/1.2430400},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Sainsbury2014,
  Title                    = {Dibromocarbene Functionalization of Boron Nitride Nanosheets: Toward Band Gap Manipulation and Nanocomposite Applications},
  Author                   = {Sainsbury, Toby and Oâ€™Neill, Arlene and Passarelli, Melissa K. and Seraffon, Maud and Gohil, Dipak and Gnaniah, Sam and Spencer, Steve J. and Rae, Alasdair and Coleman, Jonathan N.},
  Journal                  = {Chemistry of Materials},
  Year                     = {2014},
  Number                   = {24},
  Pages                    = {7039-7050},
  Volume                   = {26},

  Doi                      = {10.1021/cm503475t},
  ISSN                     = {0897-4756
1520-5002},
  Type                     = {Journal Article}
}

@Article{Sainsbury2012,
  Title                    = {Oxygen Radical Functionalization of Boron Nitride Nanosheets},
  Author                   = {Sainsbury, Toby and Satti, Amro and May, Peter and Wang, Zhiming and McGovern, Ignatius and Gunâ€™ko, Yurii K. and Coleman, Jonathan},
  Journal                  = {Journal of the American Chemical Society},
  Year                     = {2012},
  Number                   = {45},
  Pages                    = {18758-18771},
  Volume                   = {134},

  Abstract                 = {The covalent chemical functionalization of exfoliated hexagonal boron?nitride nanosheets (BNNSs) is achieved by the solution-phase oxygen radical functionalization of boron atoms in the h-BN lattice. This involves a two-step procedure to initially covalently graft alkoxy groups to boron atoms and the subsequent hydrolytic defunctionalization of the groups to yield hydroxyl-functionalized BNNSs (OH-BNNSs). Characterization of the functionalized-BNNSs using HR-TEM, Raman, UV?vis, FTIR, NMR, and TGA was performed to investigate both the structure of the BNNSs and the covalent functionalization methodology. OH-BNNSs were used to prepare polymer nanocomposites and their mechanical properties analyzed. The influence of the functional groups grafted to the surface of the BNNSs is investigated by demonstrating the impact on mechanical properties of both noncovalent and covalent bonding at the interface between the nanofiller and polymer matrixes.},
  Doi                      = {10.1021/ja3080665},
  ISSN                     = {0002-7863},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/ja3080665}
}

@Article{Sajjad2011,
  Title                    = {Low temperature synthesis of c-BN films},
  Author                   = {Sajjad, M. and Feng, P. X.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2011},
  Number                   = {25},
  Pages                    = {253109},
  Volume                   = {99},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.3671170},
  Keywords                 = {semiconductor growth
Raman spectra
boron compounds
X-ray diffraction
phonons
crystal structure
III-V semiconductors
scanning electron microscopy
transmission electron microscopy
X-ray chemical analysis
wide band gap semiconductors
semiconductor thin films
pulsed laser deposition},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/apl/99/25/10.1063/1.3671170}
}

@Article{Sajjad2014,
  Title                    = {Nanoscale structure study of boron nitride nanosheets and development of a deep-UV photo-detector},
  Author                   = {Sajjad, M. and Jadwisienczak, W. M. and Feng, P.},
  Journal                  = {Nanoscale},
  Year                     = {2014},
  Number                   = {9},
  Pages                    = {4577-82},
  Volume                   = {6},

  Abstract                 = {In this communication, we report on the synthesis of few atomic-layer boron nitride nanosheets (BNNSs) and their application for deep ultraviolet photo-detection. Synthesis of BNNSs is carried out by using the short-pulse plasma beam deposition technique. High-resolution tunneling electron microscopy, cathodoluminescence spectroscopy and photo-stimulated measurements are conducted and linked to characterize the BNNS morphology. The obtained BNNSs are flat with a typical size of 50 x 50 mum(2) and are optically transparent down to 210 nm. Nanoscale studies by transmission electron microscopy revealed that these nanosheets are composed of a densely packed honeycomb crystal lattice structure of covalently bonded boron and nitrogen atoms. Cathodoluminescence spectroscopy of these nanosheets revealed a single sharp excitonic peak centered at 233 nm at 300 K. The synthesized BNNSs are used to demonstrate applicability of BNNSs for detecting ultraviolet photons. The initial experimental tests of the developed prototype BNNSs based deep-ultraviolet photo-detector show that it is blind to photons with an energy less than 4 eV. The calculated output power of the detector is approximately 2 muW and the ratio between the output electrical power and the input optical power is approximately 1%.},
  Doi                      = {10.1039/c3nr05817d},
  ISSN                     = {2040-3372 (Electronic)
2040-3364 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24686984}
}

@Article{Sandstrom2014,
  Title                    = {Study of narrowband single photon emitters in polycrystalline diamond films},
  Author                   = {Sandstrom, Russell G. and Shimoni, Olga and Martin, Aiden A. and Aharonovich, Igor},
  Journal                  = {Applied Physics Letters},
  Year                     = {2014},
  Number                   = {18},
  Volume                   = {105},

  Doi                      = {http://dx.doi.org/10.1063/1.4901083},
  Eid                      = {181104},
  Owner                    = {Toan},
  Timestamp                = {2015.04.07},
  Url                      = {http://scitation.aip.org/content/aip/journal/apl/105/18/10.1063/1.4901083}
}

@Article{Santori2006,
  Title                    = {Coherent population trapping in diamond N-V centers at zero magneticfield},
  Author                   = {Santori, Charles and Fattal, David and Spillane, Sean M. and Fiorentino, Marco and Beausoleil, Raymond G. and Greentree, Andrew D. and Olivero, Paolo and Draganski, Martin and Rabeau, James R. and Reichart, Patrick and Gibson, Brant C. and Rubanov, Sergey and Jamieson, David N. and Prawer, Steven},
  Journal                  = {Optics Express},
  Year                     = {2006},
  Number                   = {17},
  Pages                    = {7986-7993},
  Volume                   = {14},

  Abstract                 = {Coherent population trapping at zero magnetic field was observed for nitrogen-vacancy centers in diamond under optical excitation. This was measured as a reduction in photoluminescence when the detuningbetween two excitation lasers matched the 2.88 GHz crystal-field splittingof the color center ground states. This behavior is highly sensitive to strain,which modifies the excited states, and was unexpected following recentexperiments demonstrating optical readout of single nitrogen-vacancyelectron spins based on cycling transitions. These results demonstrate forthe first time that three-level Lambda configurations suitable for proposedquantum information applications can be realized simultaneously for allfour orientations of nitrogen-vacancy centers at zero magnetic field.},
  Doi                      = {10.1364/OE.14.007986},
  Keywords                 = {Coherent optical effects
Spectroscopy, condensed matter
Spectroscopy, nonlinear},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-14-17-7986}
}

@Article{Santori2006a,
  Title                    = {Coherent population trapping in diamond N-V centers at zero magneticfield},
  Author                   = {Santori, Charles and Fattal, David and Spillane, Sean M. and Fiorentino, Marco and Beausoleil, Raymond G. and Greentree, Andrew D. and Olivero, Paolo and Draganski, Martin and Rabeau, James R. and Reichart, Patrick and Gibson, Brant C. and Rubanov, Sergey and Jamieson, David N. and Prawer, Steven},
  Journal                  = {Optics Express},
  Year                     = {2006},
  Number                   = {17},
  Pages                    = {7986-7993},
  Volume                   = {14},

  Abstract                 = {Coherent population trapping at zero magnetic field was observed for nitrogen-vacancy centers in diamond under optical excitation. This was measured as a reduction in photoluminescence when the detuningbetween two excitation lasers matched the 2.88 GHz crystal-field splittingof the color center ground states. This behavior is highly sensitive to strain,which modifies the excited states, and was unexpected following recentexperiments demonstrating optical readout of single nitrogen-vacancyelectron spins based on cycling transitions. These results demonstrate forthe first time that three-level Lambda configurations suitable for proposedquantum information applications can be realized simultaneously for allfour orientations of nitrogen-vacancy centers at zero magnetic field.},
  Doi                      = {10.1364/OE.14.007986},
  Keywords                 = {Coherent optical effects
Spectroscopy, condensed matter
Spectroscopy, nonlinear},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-14-17-7986}
}

@Article{Santori2006b,
  Title                    = {Coherent Population Trapping of Single Spins in Diamond under Optical Excitation},
  Author                   = {Santori, Charles and Tamarat, Philippe and Neumann, Philipp and Wrachtrup, JÃ¶rg and Fattal, David and Beausoleil, Raymond and Rabeau, James and Olivero, Paolo and Greentree, Andrew and Prawer, Steven and Jelezko, Fedor and Hemmer, Philip},
  Journal                  = {Physical Review Letters},
  Year                     = {2006},
  Number                   = {24},
  Pages                    = {247401},
  Volume                   = {97},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.97.247401}
}

@Article{Schietinger2009,
  Title                    = {Plasmon-Enhanced Single Photon Emission from a Nanoassembled Metalâˆ’Diamond Hybrid Structure at Room Temperature},
  Author                   = {Schietinger, Stefan and Barth, Michael and Aichele, Thomas and Benson, Oliver},
  Journal                  = {Nano Lett.},
  Year                     = {2009},
  Number                   = {4},
  Pages                    = {1694-1698},
  Volume                   = {9},

  Doi                      = {10.1021/nl900384c},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl900384c}
}

@Article{Schietinger2008,
  Title                    = {One-by-One Coupling of Single Defect Centers in Nanodiamonds to High-Q Modes of an Optical Microresonator},
  Author                   = {Schietinger, Stefan and SchrÃ¶der, Tim and Benson, Oliver},
  Journal                  = {Nano Letters},
  Year                     = {2008},
  Number                   = {11},
  Pages                    = {3911-3915},
  Volume                   = {8},

  Doi                      = {10.1021/nl8023627},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl8023627}
}

@Article{Schirhagl2014,
  Title                    = {Nitrogen-vacancy centers in diamond: nanoscale sensors for physics and biology},
  Author                   = {Schirhagl, R. and Chang, K. and Loretz, M. and Degen, C. L.},
  Journal                  = {Annu Rev Phys Chem},
  Year                     = {2014},
  Pages                    = {83-105},
  Volume                   = {65},

  Abstract                 = {Crystal defects in diamond have emerged as unique objects for a variety of applications, both because they are very stable and because they have interesting optical properties. Embedded in nanocrystals, they can serve, for example, as robust single-photon sources or as fluorescent biomarkers of unlimited photostability and low cytotoxicity. The most fascinating aspect, however, is the ability of some crystal defects, most prominently the nitrogen-vacancy (NV) center, to locally detect and measure a number of physical quantities, such as magnetic and electric fields. This metrology capacity is based on the quantum mechanical interactions of the defect's spin state. In this review, we introduce the new and rapidly evolving field of nanoscale sensing based on single NV centers in diamond. We give a concise overview of the basic properties of diamond, from synthesis to electronic and magnetic properties of embedded NV centers. We describe in detail how single NV centers can be harnessed for nanoscale sensing, including the physical quantities that may be detected, expected sensitivities, and the most common measurement protocols. We conclude by highlighting a number of the diverse and exciting applications that may be enabled by these novel sensors, ranging from measurements of ion concentrations and membrane potentials to nanoscale thermometry and single-spin nuclear magnetic resonance.},
  Doi                      = {10.1146/annurev-physchem-040513-103659},
  ISSN                     = {1545-1593 (Electronic)
0066-426X (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24274702}
}

@Article{Schlamp1997,
  Title                    = {Improved efficiencies in light emitting diodes made with CdSe(CdS) core/shell type nanocrystals and a semiconducting polymer},
  Author                   = {Schlamp, M. C. and Peng, Xiaogang and Alivisatos, A. P.},
  Journal                  = {Journal of Applied Physics},
  Year                     = {1997},
  Number                   = {11},
  Pages                    = {5837-5842},
  Volume                   = {82},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.366452},
  Keywords                 = {hole traps
nanostructured materials
organic semiconductors
cadmium compounds
electron traps
II-VI semiconductors},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/jap/82/11/10.1063/1.366452}
}

@Article{Scholl2012,
  Title                    = {Quantum plasmon resonances of individual metallic nanoparticles},
  Author                   = {Scholl, J. A. and Koh, A. L. and Dionne, J. A.},
  Journal                  = {Nature},
  Year                     = {2012},
  Number                   = {7390},
  Pages                    = {421-7},
  Volume                   = {483},

  Abstract                 = {The plasmon resonances of metallic nanoparticles have received considerable attention for their applications in nanophotonics, biology, sensing, spectroscopy and solar energy harvesting. Although thoroughly characterized for spheres larger than ten nanometres in diameter, the plasmonic properties of particles in the quantum size regime have been historically difficult to describe owing to weak optical scattering, metal-ligand interactions, and inhomogeneity in ensemble measurements. Such difficulties have precluded probing and controlling the plasmonic properties of quantum-sized particles in many natural and engineered processes, notably catalysis. Here we investigate the plasmon resonances of individual ligand-free silver nanoparticles using aberration-corrected transmission electron microscope (TEM) imaging and monochromated scanning TEM electron energy-loss spectroscopy (EELS). This technique allows direct correlation between a particle's geometry and its plasmon resonance. As the nanoparticle diameter decreases from 20 nanometres to less than two nanometres, the plasmon resonance shifts to higher energy by 0.5 electronvolts, a substantial deviation from classical predictions. We present an analytical quantum mechanical model that describes this shift due to a change in particle permittivity. Our results highlight the quantum plasmonic properties of small metallic nanospheres, with direct application to understanding and exploiting catalytically active and biologically relevant nanoparticles.},
  Doi                      = {10.1038/nature10904},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22437611}
}

@Article{Schraml2014,
  Title                    = {Optical properties and interparticle coupling of plasmonic bowtie nanoantennas on a semiconducting substrate},
  Author                   = {Schraml, K. and Spiegl, M. and Kammerlocher, M. and Bracher, G. and Bartl, J. and Campbell, T. and Finley, J. J. and Kaniber, M.},
  Journal                  = {Physical Review B},
  Year                     = {2014},
  Number                   = {3},
  Volume                   = {90},

  Doi                      = {10.1103/PhysRevB.90.035435},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Schrand2009,
  Title                    = {Nanodiamond Particles: Properties and Perspectives for Bioapplications},
  Author                   = {Schrand, Amanda M. and Hens, Suzanne A. Ciftan and Shenderova, Olga A.},
  Journal                  = {Critical Reviews in Solid State and Materials Sciences},
  Year                     = {2009},
  Number                   = {1-2},
  Pages                    = {18-74},
  Volume                   = {34},

  Doi                      = {10.1080/10408430902831987},
  ISSN                     = {1040-8436},
  Type                     = {Journal Article},
  Url                      = {http://www.tandfonline.com/doi/abs/10.1080/10408430902831987}
}

@Article{Schuck2005,
  Title                    = {Improving the Mismatch between Light and Nanoscale Objects with Gold Bowtie Nanoantennas},
  Author                   = {Schuck, P. J. and Fromm, D. P. and Sundaramurthy, A. and Kino, G. S. and Moerner, W. E.},
  Journal                  = {Physical Review Letters},
  Year                     = {2005},
  Number                   = {1},
  Volume                   = {94},

  Doi                      = {10.1103/PhysRevLett.94.017402},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Schuller2010,
  Title                    = {Plasmonics for extreme light concentration and manipulation},
  Author                   = {Schuller, J. A. and Barnard, E. S. and Cai, W. and Jun, Y. C. and White, J. S. and Brongersma, M. L.},
  Journal                  = {Nat Mater},
  Year                     = {2010},
  Number                   = {3},
  Pages                    = {193-204},
  Volume                   = {9},

  Abstract                 = {The unprecedented ability of nanometallic (that is, plasmonic) structures to concentrate light into deep-subwavelength volumes has propelled their use in a vast array of nanophotonics technologies and research endeavours. Plasmonic light concentrators can elegantly interface diffraction-limited dielectric optical components with nanophotonic structures. Passive and active plasmonic devices provide new pathways to generate, guide, modulate and detect light with structures that are similar in size to state-of-the-art electronic devices. With the ability to produce highly confined optical fields, the conventional rules for light-matter interactions need to be re-examined, and researchers are venturing into new regimes of optical physics. In this review we will discuss the basic concepts behind plasmonics-enabled light concentration and manipulation, make an attempt to capture the wide range of activities and excitement in this area, and speculate on possible future directions.},
  Doi                      = {10.1038/nmat2630},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20168343}
}

@Article{Seker2013,
  Title                    = {Bio-nanohybrids of quantum dots and photoproteins facilitating strong nonradiative energy transfer},
  Author                   = {Seker, U. O. and Mutlugun, E. and Hernandez-Martinez, P. L. and Sharma, V. K. and Lesnyak, V. and Gaponik, N. and Eychmuller, A. and Demir, H. V.},
  Journal                  = {Nanoscale},
  Year                     = {2013},
  Number                   = {15},
  Pages                    = {7034-40},
  Volume                   = {5},

  Abstract                 = {Utilization of light is crucial for the life cycle of many organisms. Also, many organisms can create light by utilizing chemical energy emerged from biochemical reactions. Being the most important structural units of the organisms, proteins play a vital role in the formation of light in the form of bioluminescence. Such photoproteins have been isolated and identified for a long time; the exact mechanism of their bioluminescence is well established. Here we show a biomimetic approach to build a photoprotein based excitonic nanoassembly model system using colloidal quantum dots (QDs) for a new bioluminescent couple to be utilized in biotechnological and photonic applications. We concentrated on the formation mechanism of nanohybrids using a kinetic and thermodynamic approach. Finally we propose a biosensing scheme with an ON/OFF switch using the QD-GFP hybrid. The QD-GFP hybrid system promises strong exciton-exciton coupling between the protein and the quantum dot at a high efficiency level, possessing enhanced capabilities of light harvesting, which may bring new technological opportunities to mimic biophotonic events.},
  Doi                      = {10.1039/c3nr01417g},
  ISSN                     = {2040-3372 (Electronic)
2040-3364 (Linking)},
  Keywords                 = {Biomimetics/methods
*Biosensing Techniques
Green Fluorescent Proteins/*chemistry
Kinetics
*Models, Chemical
Optics and Photonics/methods
Quantum Dots/*chemistry
Thermodynamics},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23803876}
}

@Article{Seo2012,
  Title                    = {Plasmonic monitoring of catalytic hydrogen generation by a single nanoparticle probe},
  Author                   = {Seo, D. and Park, G. and Song, H.},
  Journal                  = {Journal of the American Chemical Society},
  Year                     = {2012},
  Number                   = {2},
  Pages                    = {1221-7},
  Volume                   = {134},

  Abstract                 = {Plasmonic nanostructures such as gold nanoparticles are very useful for monitoring chemical reactions because their optical properties are highly dependent upon the environment surrounding the particle surface. Here, we designed the catalytic structure composed of platinized cadmium sulfide with gold domains as a sensitive probe, and we monitored the photocatalytic decomposition of lactic acid to generate hydrogen gas in situ by single-particle dark-field spectroscopy. The plasmon band shift of the gold probe throughout the reaction exhibits significant particle-to-particle variation, and by simulating the reaction kinetics, the rate constant and structural information (including the diffusion coefficient through the shell and the relative arrangement of the active sites) can be estimated for individual catalyst particles. This approach is versatile for the monitoring of various heterogeneous reactions with distinct components at a single-particle level.},
  Doi                      = {10.1021/ja2093663},
  ISSN                     = {1520-5126 (Electronic)
0002-7863 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22176153}
}

@Article{Shan2013,
  Title                    = {Single photon sources with single semiconductor quantum dots},
  Author                   = {Shan, Guang-Cun and Yin, Zhang-Qi and Shek, Chan Hung and Huang, Wei},
  Journal                  = {Frontiers of Physics},
  Year                     = {2013},
  Number                   = {2},
  Pages                    = {170-193},
  Volume                   = {9},

  Doi                      = {10.1007/s11467-013-0360-6},
  ISSN                     = {2095-0462
2095-0470},
  Type                     = {Journal Article}
}

@Article{Sheldon2014,
  Title                    = {Plasmoelectric potentials in metal nanostructures},
  Author                   = {Sheldon, Matthew T. and van de Groep, Jorik and Brown, Ana M. and Polman, Albert and Atwater, Harry A.},
  Journal                  = {Science},
  Year                     = {2014},
  Number                   = {6211},
  Pages                    = {828-831},
  Volume                   = {346},

  Abstract                 = {The conversion of optical power to an electric potential is of general interest for energy applications and is typically obtained via optical excitation of semiconductor materials. We developed a method for achieving electric potential that uses an all-metal geometry based on the plasmon resonance in metal nanostructures. In arrays of gold nanoparticles on an indium tin oxide substrate and arrays of 100-nanometer-diameter holes in 20-nanometer-thick gold films on a glass substrate, we detected negative and positive surface potentials during monochromatic irradiation at wavelengths below or above the plasmon resonance, respectively. We observed plasmoelectric surface potentials as large as 100 millivolts under illumination of 100 milliwatts per square centimeter. Plasmoelectric devices may enable the development of all-metal optoelectronic devices that can convert light into electrical energy.},
  Doi                      = {10.1126/science.1258405},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/346/6211/828.abstract}
}

@Article{Shen2013,
  Title                    = {Efficient and bright colloidal quantum dot light-emitting diodes via controlling the shell thickness of quantum dots},
  Author                   = {Shen, H. and Lin, Q. and Wang, H. and Qian, L. and Yang, Y. and Titov, A. and Hyvonen, J. and Zheng, Y. and Li, L. S.},
  Journal                  = {ACS Appl Mater Interfaces},
  Year                     = {2013},
  Number                   = {22},
  Pages                    = {12011-6},
  Volume                   = {5},

  Abstract                 = {In this paper, we use a simple device architecture based on solution-processed ZnO nanoparticles (NPs) as the electron injection/transport layer and bilayer structure of poly(ethylenedioxythiophene):polystyrene sulfonate (PEDOT:PSS)/poly[9,9-dioctylfluorene-co-N-[4-(3-methylpropyl)]-diphenylamine] (TFB) as the hole injection/transport layer to assess the effect of shell thickness on the properties of quantum-dot-based light emitting diodes (QD-LEDs), comprising CdSe/CdS/ZnS core-shell QDs as the emitting layer. QDs with varying shell thickness were assessed to determine the best option of shell thickness, and the best improvement in device performance was observed when the shell thickness was 2.1 nm. Thereafter, different emissions of QDs, but with optimized same shell thickness ( approximately 2.1 nm), were selected as emitters to be fabricated into same structured QD-LEDs. Highly bright orange-red and green QD-LEDs with peak luminances up to approximately 30 000 and approximately 52 000 cd m(-2), and power efficiencies of 16 and 19.7 lm W(-1), respectively, were demonstrated successfully. These results may demonstrate a striking basic prototype for the commercialization of QD-based displays and solid-state lightings.},
  Doi                      = {10.1021/am4038068},
  ISSN                     = {1944-8252 (Electronic)
1944-8244 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24191742}
}

@Article{Shevchenko2008,
  Title                    = {Self-Assembled Binary Superlattices of CdSe and Au Nanocrystals and Their Fluorescence Properties},
  Author                   = {Shevchenko, Elena V. and Ringler, Moritz and Schwemer, Alexander and Talapin, Dmitri V. and Klar, Thomas A. and Rogach, Andrey L. and Feldmann, Jochen and Alivisatos, A. Paul},
  Journal                  = {Journal of the American Chemical Society},
  Year                     = {2008},
  Number                   = {11},
  Pages                    = {3274-3275},
  Volume                   = {130},

  Doi                      = {10.1021/ja710619s},
  ISSN                     = {0002-7863},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/ja710619s}
}

@Article{Shevlin2007,
  Title                    = {Hydrogen sorption in defective hexagonal BN sheets and BN nanotubes},
  Author                   = {Shevlin, S. A. and Guo, Z. X.},
  Journal                  = {Physical Review B},
  Year                     = {2007},
  Number                   = {2},
  Pages                    = {024104},
  Volume                   = {76},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.76.024104}
}

@Article{Shi2010,
  Title                    = {Synthesis of few-layer hexagonal boron nitride thin film by chemical vapor deposition},
  Author                   = {Shi, Y. and Hamsen, C. and Jia, X. and Kim, K. K. and Reina, A. and Hofmann, M. and Hsu, A. L. and Zhang, K. and Li, H. and Juang, Z. Y. and Dresselhaus, M. S. and Li, L. J. and Kong, J.},
  Journal                  = {Nano Lett.},
  Year                     = {2010},
  Number                   = {10},
  Pages                    = {4134-9},
  Volume                   = {10},

  Abstract                 = {In this contribution we demonstrate a method of synthesizing a hexagonal boron nitride (h-BN) thin film by ambient pressure chemical vapor deposition on polycrystalline Ni films. Depending on the growth conditions, the thickness of the obtained h-BN film is between approximately 5 and 50 nm. The h-BN grows continuously on the entire Ni surface and the region with uniform thickness can be up to 20 mum in lateral size which is only limited by the size of the Ni single crystal grains. The hexagonal structure was confirmed by both electron and X-ray diffraction. X-ray photoelectron spectroscopy shows the B/N atomic ratio to be 1:1.12. A large optical band gap (5.92 eV) was obtained from the photoabsorption spectra which suggest the potential usage of this h-BN film in optoelectronic devices.},
  Doi                      = {10.1021/nl1023707},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20812716}
}

@Article{Si2014,
  Title                    = {Intrinsic ferromagnetism in hexagonal boron nitride nanosheets},
  Author                   = {Si, M. S. and Gao, D. and Yang, D. and Peng, Y. and Zhang, Z. Y. and Xue, D. and Liu, Y. and Deng, X. and Zhang, G. P.},
  Journal                  = {J Chem Phys},
  Year                     = {2014},
  Number                   = {20},
  Pages                    = {204701},
  Volume                   = {140},

  Abstract                 = {Understanding the mechanism of ferromagnetism in hexagonal boron nitride nanosheets, which possess only s and p electrons in comparison with normal ferromagnets based on localized d or f electrons, is a current challenge. In this work, we report an experimental finding that the ferromagnetic coupling is an intrinsic property of hexagonal boron nitride nanosheets, which has never been reported before. Moreover, we further confirm it from ab initio calculations. We show that the measured ferromagnetism should be attributed to the localized pi states at edges, where the electron-electron interaction plays the role in this ferromagnetic ordering. More importantly, we demonstrate such edge-induced ferromagnetism causes a high Curie temperature well above room temperature. Our systematical work, including experimental measurements and theoretical confirmation, proves that such unusual room temperature ferromagnetism in hexagonal boron nitride nanosheets is edge-dependent, similar to widely reported graphene-based materials. It is believed that this work will open new perspectives for hexagonal boron nitride spintronic devices.},
  Doi                      = {10.1063/1.4879055},
  ISSN                     = {1089-7690 (Electronic)
0021-9606 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24880305}
}

@Article{Silly2007,
  Title                    = {Luminescence properties of hexagonal boron nitride: Cathodoluminescence and photoluminescence spectroscopy measurements},
  Author                   = {Silly, M. G. and Jaffrennou, P. and Barjon, J. and Lauret, J. S. and Ducastelle, F. and Loiseau, A. and Obraztsova, E. and Attal-Tretout, B. and Rosencher, E.},
  Journal                  = {Physical Review B},
  Year                     = {2007},
  Number                   = {8},
  Pages                    = {085205},
  Volume                   = {75},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.75.085205}
}

@Article{Sipahigil2014,
  Title                    = {Indistinguishable Photons from Separated Silicon-Vacancy Centers in Diamond},
  Author                   = {Sipahigil, A. and Jahnke, K. â€‰D and Rogers, L. â€‰J and Teraji, T. and Isoya, J. and Zibrov, A. â€‰S and Jelezko, F. and Lukin, M. â€‰D},
  Journal                  = {Physical Review Letters},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {113602},
  Volume                   = {113},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.113.113602}
}

@Article{Smith2010,
  Title                    = {The effects of surface oxidation on luminescence of nano diamonds},
  Author                   = {Smith, Bradley R. and Gruber, Daniel and Plakhotnik, Taras},
  Journal                  = {Diamond and Related Materials},
  Year                     = {2010},
  Number                   = {4},
  Pages                    = {314-318},
  Volume                   = {19},

  Doi                      = {10.1016/j.diamond.2009.12.009},
  ISSN                     = {09259635},
  Type                     = {Journal Article}
}

@Article{Smith2010a,
  Title                    = {Fast, single-molecule localization that achieves theoretically minimum uncertainty},
  Author                   = {Smith, C. S. and Joseph, N. and Rieger, B. and Lidke, K. A.},
  Journal                  = {Nat Methods},
  Year                     = {2010},
  Number                   = {5},
  Pages                    = {373-5},
  Volume                   = {7},

  Abstract                 = {We describe an iterative algorithm that converges to the maximum likelihood estimate of the position and intensity of a single fluorophore. Our technique efficiently computes and achieves the Cramer-Rao lower bound, an essential tool for parameter estimation. An implementation of the algorithm on graphics processing unit hardware achieved more than 10(5) combined fits and Cramer-Rao lower bound calculations per second, enabling real-time data analysis for super-resolution imaging and other applications.},
  Doi                      = {10.1038/nmeth.1449},
  ISSN                     = {1548-7105 (Electronic)
1548-7091 (Linking)},
  Keywords                 = {Algorithms
*Likelihood Functions
Microscopy, Fluorescence/*methods
Reproducibility of Results
Software
Uncertainty},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20364146}
}

@Article{Smith1959,
  Title                    = {Electron-Spin Resonance of Nitrogen Donors in Diamond},
  Author                   = {Smith, W. and Sorokin, P. and Gelles, I. and Lasher, G.},
  Journal                  = {Physical Review},
  Year                     = {1959},
  Number                   = {6},
  Pages                    = {1546-1552},
  Volume                   = {115},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRev.115.1546}
}

@Article{Smyder2014,
  Title                    = {The influence of continuous vs. pulsed laser excitation on single quantum dot photophysics},
  Author                   = {Smyder, Julie A. and Amori, Amanda R. and Odoi, Michael Y. and Stern, Harry A. and Peterson, Jeffrey J. and Krauss, Todd D.},
  Journal                  = {Physical Chemistry Chemical Physics},
  Year                     = {2014},
  Number                   = {47},
  Pages                    = {25723-25728},
  Volume                   = {16},

  Abstract                 = {The impact of pulsed versus continuous wave (cw) laser excitation on the photophysical properties of single quantum dots (QDs) has been investigated in an experiment in which all macroscopic variables are identical except the nature of laser excitation. Pulsed excitation exaggerates the effects of photobleaching, results in a lower probability of long ON fluorescence blinking events, and leads to shorter fluorescence lifetimes with respect to cw excitation at the same wavelength and average intensity. Spectral wandering, biexciton quantum yields, and power law exponents that describe fluorescence blinking are largely insensitive to the nature of laser excitation. These results explicitly illustrate important similarities and differences in fluorescence dynamics between pulsed and cw excitation, enabling more meaningful comparisons between literature reports and aiding in the design of new experiments to mitigate possible influences of high photon flux on QDs.},
  Doi                      = {10.1039/C4CP01395F},
  ISSN                     = {1463-9076},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1039/C4CP01395F}
}

@Article{Solomon1996,
  Title                    = {Electroluminescence in vertically aligned quantum dot multilayer light-emitting diodes fabricating by growth-induced islanding},
  Author                   = {Solomon, G. S. and Larson, M. C. and Harris, J. S.},
  Journal                  = {Applied Physics Letters},
  Year                     = {1996},
  Number                   = {13},
  Pages                    = {1897},
  Volume                   = {69},

  Abstract                 = {A molecular beam epitaxy (MBE) growth-induced islanding process has been used to form self-organized multiple quantum dot layers, in which quantum dots from different layers are vertically aligned in columns and are electronically coupled. These structures are used as the active region in light-emitting diodes operating at room temperature. Light-emitting diodes are investigated using quantum dot columns containing single, 5 and 10 InAs quantum dots. These diodes emit light over a broad band with typical spectral linewidths of 120 nm, peaked between 1000 and 1100 nm. In addition to the quantum dot spectral feature, a spectral feature from a thin quantum well region, integral to the quantum dot formation process, is seen in the single quantum dot diode, but is eliminated in diodes with active regions containing columns of multiple quantum dots. Â© 1996 American Institute of Physics. [ABSTRACT FROM AUTHOR]
Copyright of Applied Physics Letters is the property of American Institute of Physics and its content may not be copied or emailed to multiple sites or posted to a listserv without the copyright holder's express written permission. However, users may print, download, or email articles for individual use. This abstract may be abridged. No warranty is given about the accuracy of the copy. Users should refer to the original published version of the material for the full abstract. (Copyright applies to all Abstracts.)},
  ISSN                     = {00036951},
  Keywords                 = {QUANTUM dots
MOLECULAR beam epitaxy},
  Type                     = {Journal Article},
  Url                      = {https://www.lib.uts.edu.au/goto?url=http://search.ebscohost.com/login.aspx?direct=true&db=iih&AN=6290174&site=ehost-live}
}

@Article{Son2003,
  Title                    = {Silicon vacancy related Tv2a center in 4H-SiC},
  Author                   = {Son, N. T. and Zolnai, Z. and JanzÃ©n, E.},
  Journal                  = {Physical Review B},
  Year                     = {2003},
  Number                   = {20},
  Pages                    = {205211},
  Volume                   = {68},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevB.68.205211}
}

@Article{Song2012,
  Title                    = {Nonblinking plasmonic quantum dot assemblies for multiplex biological detection},
  Author                   = {Song, F. and Tang, P. S. and Durst, H. and Cramb, D. T. and Chan, W. C.},
  Journal                  = {Angew Chem Int Ed Engl},
  Year                     = {2012},
  Number                   = {35},
  Pages                    = {8773-7},
  Volume                   = {51},

  Doi                      = {10.1002/anie.201201872},
  ISSN                     = {1521-3773 (Electronic)
1433-7851 (Linking)},
  Keywords                 = {Acrylates/chemistry
Electrolytes/chemistry
Gold/chemistry
Metal Nanoparticles/chemistry
Microscopy, Fluorescence
Polystyrenes/chemistry
*Quantum Dots
Ultraviolet Rays},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22847993}
}

@Article{Song2014,
  Title                    = {Plasmon-enhanced photoluminescence of Si-V centers in diamond from a nanoassembled metal-diamond hybrid structure},
  Author                   = {Song, Jie and Li, Hongdong and Lin, Feng and Wang, Liying and Wu, Honglin and Yang, Yanqiang},
  Journal                  = {CrystEngComm},
  Year                     = {2014},
  Number                   = {36},
  Pages                    = {8356-8362},
  Volume                   = {16},

  Abstract                 = {Using a facile top-down etching approach, a subwavelength-sized diamond pit structure infilled with semi-ellipsoidal gold nanoparticles was fabricated. The three-dimensional finite-difference time-domain simulations reveal strong localized surface plasmon resonance (LSPR) scattering and enhanced electric field exhibited by this hybrid nanoassembled metal-diamond-pit. Experimentally, with excitation at 633 and 830 nm close to the calculated LSPR wavelength, the photoluminescence (PL) intensities of the peak at 738 nm originating from the single photon source of silicon-vacancy centers in diamond were significantly enhanced by factors of ~100 and ~50, respectively, with respect to that from normal Si-doped diamond without the hybrid structure. By means of time-resolved PL measurements, the decay kinetic mechanisms of the plasmon-related PL enhancement were investigated and are discussed.},
  Doi                      = {10.1039/C4CE01140F},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1039/C4CE01140F}
}

@Article{Song2010,
  Title                    = {Large Scale Growth and Characterization of Atomic Hexagonal Boron Nitride Layers},
  Author                   = {Song, Li and Ci, Lijie and Lu, Hao and Sorokin, Pavel B. and Jin, Chuanhong and Ni, Jie and Kvashnin, Alexander G. and Kvashnin, Dmitry G. and Lou, Jun and Yakobson, Boris I. and Ajayan, Pulickel M.},
  Journal                  = {Nano Lett.},
  Year                     = {2010},
  Number                   = {8},
  Pages                    = {3209-3215},
  Volume                   = {10},

  Abstract                 = {Hexagonal boron nitride (h-BN), a layered material similar to graphite, is a promising dielectric. Monolayer h-BN, so-called ?white graphene?, has been isolated from bulk BN and could be useful as a complementary two-dimensional dielectric substrate for graphene electronics. Here we report the large area synthesis of h-BN films consisting of two to five atomic layers, using chemical vapor deposition. These atomic films show a large optical energy band gap of 5.5 eV and are highly transparent over a broad wavelength range. The mechanical properties of the h-BN films, measured by nanoindentation, show 2D elastic modulus in the range of 200?500 N/m, which is corroborated by corresponding theoretical calculations.},
  Doi                      = {10.1021/nl1022139},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl1022139}
}

@Article{Song2010a,
  Title                    = {Broadband coupler between silicon waveguide and hybrid plasmonic waveguide},
  Author                   = {Song, Yi and Wang, Jing and Li, Qiang and Yan, Min and Qiu, Min},
  Journal                  = {Optics Express},
  Year                     = {2010},
  Number                   = {12},
  Pages                    = {13173-13179},
  Volume                   = {18},

  Abstract                 = {Efficient broadband coupling of light between a dielectric waveguide and a hybrid plasmonic waveguide is investigated theoretically. A plasmonic linear taper is used as a coupler which connects the two types of waveguides. Broadband coupling is realized by such a compact plasmonic taper with a length of only 0.4&#x03BC;m, which achieves a coupling efficiency of 70% (1.5dB) at the 1.55&#x03BC;m telecommunication wavelength.},
  Doi                      = {10.1364/OE.18.013173},
  Keywords                 = {Surface plasmons
Plasmonics},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-18-12-13173}
}

@Article{Sorger2011,
  Title                    = {Strongly enhanced molecular fluorescence inside a nanoscale waveguide gap},
  Author                   = {Sorger, V. J. and Pholchai, N. and Cubukcu, E. and Oulton, R. F. and Kolchin, P. and Borschel, C. and Gnauck, M. and Ronning, C. and Zhang, X.},
  Journal                  = {Nano Lett},
  Year                     = {2011},
  Number                   = {11},
  Pages                    = {4907-11},
  Volume                   = {11},

  Abstract                 = {We experimentally demonstrate dramatically enhanced light-matter interaction for molecules placed inside the nanometer scale gap of a plasmonic waveguide. We observe spontaneous emission rate enhancements of up to about 60 times due to strong optical localization in two dimensions. This rate enhancement is a nonresonant nature of the plasmonic waveguide under study overcoming the fundamental bandwidth limitation of conventional devices. Moreover, we show that about 85% of molecular emission couples into the waveguide highlighting the dominance of the nanoscale optical mode in competing with quenching processes. Such optics at molecular length scales paves the way toward integrated on-chip photon source, rapid transfer of quantum information, and efficient light extraction for solid-state-lighting devices.},
  Doi                      = {10.1021/nl202825s},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Fluorescent Dyes/*chemistry
Lighting/*methods
Materials Testing
Nanostructures/*chemistry/ultrastructure
Particle Size
Surface Plasmon Resonance/*methods},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/21978206}
}

@Article{Sorger2011a,
  Title                    = {Experimental demonstration of low-loss optical waveguiding at deep sub-wavelength scales},
  Author                   = {Sorger, Volker J. and Ye, Ziliang and Oulton, Rupert F. and Wang, Yuan and Bartal, Guy and Yin, Xiaobo and Zhang, Xiang},
  Journal                  = {Nature Communications},
  Year                     = {2011},
  Pages                    = {331},
  Volume                   = {2},

  Doi                      = {10.1038/ncomms1315},
  ISSN                     = {2041-1723},
  Type                     = {Journal Article}
}

@Article{Splendiani2010,
  Title                    = {Emerging Photoluminescence in Monolayer MoS2},
  Author                   = {Splendiani, Andrea and Sun, Liang and Zhang, Yuanbo and Li, Tianshu and Kim, Jonghwan and Chim, Chi-Yung and Galli, Giulia and Wang, Feng},
  Journal                  = {Nano Letters},
  Year                     = {2010},
  Number                   = {4},
  Pages                    = {1271-1275},
  Volume                   = {10},

  Doi                      = {10.1021/nl903868w},
  Eprint                   = { 
 http://dx.doi.org/10.1021/nl903868w
 
},
  Owner                    = {Toan},
  Timestamp                = {2015.04.09},
  Url                      = { 
 http://dx.doi.org/10.1021/nl903868w
 
}
}

@Article{Srituravanich2008,
  Title                    = {Flying plasmonic lens in the near field for high-speed nanolithography},
  Author                   = {Srituravanich, W. and Pan, L. and Wang, Y. and Sun, C. and Bogy, D. B. and Zhang, X.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2008},
  Number                   = {12},
  Pages                    = {733-7},
  Volume                   = {3},

  Abstract                 = {The commercialization of nanoscale devices requires the development of high-throughput nanofabrication technologies that allow frequent design changes. Maskless nanolithography, including electron-beam and scanning-probe lithography, offers the desired flexibility but is limited by low throughput. Here, we report a new low-cost, high-throughput approach to maskless nanolithography that uses an array of plasmonic lenses that 'flies' above the surface to be patterned, concentrating short-wavelength surface plasmons into sub-100 nm spots. However, these nanoscale spots are only formed in the near field, which makes it very difficult to scan the array above the surface at high speed. To overcome this problem we have designed a self-spacing air bearing that can fly the array just 20 nm above a disk that is spinning at speeds of between 4 and 12 m s(-1), and have experimentally demonstrated patterning with a linewidth of 80 nm. This low-cost nanofabrication scheme has the potential to achieve throughputs that are two to five orders of magnitude higher than other maskless techniques.},
  Doi                      = {10.1038/nnano.2008.303},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {Nanostructures
Nanotechnology/*instrumentation/methods
Optics and Photonics
Surface Plasmon Resonance/*methods},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/19057593}
}

@Article{Srivastava2010,
  Title                    = {Light-Controlled Self-Assembly of Semiconductor Nanoparticles into Twisted Ribbons},
  Author                   = {Srivastava, Sudhanshu and Santos, Aaron and Critchley, Kevin and Kim, Ki-Sub and Podsiadlo, Paul and Sun, Kai and Lee, Jaebeom and Xu, Chuanlai and Lilly, G. Daniel and Glotzer, Sharon C. and Kotov, Nicholas A.},
  Journal                  = {Science},
  Year                     = {2010},
  Number                   = {5971},
  Pages                    = {1355-1359},
  Volume                   = {327},

  Abstract                 = {The collective properties of nanoparticles manifest in their ability to self-organize into complex microscale structures. Slow oxidation of tellurium ions in cadmium telluride (CdTe) nanoparticles results in the assembly of 1- to 4-micrometer-long flat ribbons made of several layers of individual cadmium sulfide (CdS)/CdTe nanocrystals. Twisting of the ribbons with an equal distribution of left and right helices was induced by illumination with visible light. The pitch lengths (250 to 1500 nanometers) varied with illumination dose, and the twisting was associated with the relief of mechanical shear stress in assembled ribbons caused by photooxidation of CdS. Unusual shapes of multiparticle assemblies, such as ellipsoidal clouds, dog-bone agglomerates, and ribbon bunches, were observed as intermediate stages. Computer simulations revealed that the balance between attraction and electrostatic repulsion determines the resulting geometry and dimensionality of the nanoparticle assemblies.},
  Doi                      = {10.1126/science.1177218},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000275418700035}
}

@Article{Srivastava2010a,
  Title                    = {Light-Controlled Self-Assembly of Semiconductor Nanoparticles into Twisted Ribbons},
  Author                   = {Srivastava, Sudhanshu and Santos, Aaron and Critchley, Kevin and Kim, Ki-Sub and Podsiadlo, Paul and Sun, Kai and Lee, Jaebeom and Xu, Chuanlai and Lilly, G. Daniel and Glotzer, Sharon C. and Kotov, Nicholas A.},
  Journal                  = {Science},
  Year                     = {2010},
  Number                   = {5971},
  Pages                    = {1355-1359},
  Volume                   = {327},

  Abstract                 = {The collective properties of nanoparticles manifest in their ability to self-organize into complex microscale structures. Slow oxidation of tellurium ions in cadmium telluride (CdTe) nanoparticles results in the assembly of 1- to 4-micrometer-long flat ribbons made of several layers of individual cadmium sulfide (CdS)/CdTe nanocrystals. Twisting of the ribbons with an equal distribution of left and right helices was induced by illumination with visible light. The pitch lengths (250 to 1500 nanometers) varied with illumination dose, and the twisting was associated with the relief of mechanical shear stress in assembled ribbons caused by photooxidation of CdS. Unusual shapes of multiparticle assemblies, such as ellipsoidal clouds, dog-bone agglomerates, and ribbon bunches, were observed as intermediate stages. Computer simulations revealed that the balance between attraction and electrostatic repulsion determines the resulting geometry and dimensionality of the nanoparticle assemblies.},
  Doi                      = {10.1126/science.1177218},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000275418700035}
}

@Article{Staudacher2013,
  Title                    = {Nuclear Magnetic Resonance Spectroscopy on a (5-Nanometer)3 Sample Volume},
  Author                   = {Staudacher, T. and Shi, F. and Pezzagna, S. and Meijer, J. and Du, J. and Meriles, C. A. and Reinhard, F. and Wrachtrup, J.},
  Journal                  = {Science},
  Year                     = {2013},
  Number                   = {6119},
  Pages                    = {561-563},
  Volume                   = {339},

  Abstract                 = {Application of nuclear magnetic resonance (NMR) spectroscopy to nanoscale samples has remained an elusive goal, achieved only with great experimental effort at subkelvin temperatures. We demonstrated detection of NMR signals from a (5-nanometer)3 voxel of various fluid and solid organic samples under ambient conditions. We used an atomic-size magnetic field sensor, a single nitrogen-vacancy defect center, embedded ~7 nanometers under the surface of a bulk diamond to record NMR spectra of various samples placed on the diamond surface. Its detection volume consisted of only 104 nuclear spins with a net magnetization of only 102 statistically polarized spins.},
  Doi                      = {10.1126/science.1231675},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/339/6119/561.abstract}
}

@Article{Steckel2006,
  Title                    = {Color-Saturated Green-Emitting QD-LEDs},
  Author                   = {Steckel, Jonathan S. and Snee, Preston and Coe-Sullivan, Seth and Zimmer, John P. and Halpert, Jonathan E. and Anikeeva, Polina and Kim, Lee-Ann and Bulovic, Vladimir and Bawendi, Moungi G.},
  Journal                  = {Angewandte Chemie International Edition},
  Year                     = {2006},
  Number                   = {35},
  Pages                    = {5796-5799},
  Volume                   = {45},

  Doi                      = {10.1002/anie.200600317},
  ISSN                     = {1521-3773},
  Keywords                 = {light-emitting devices
nanocrystals
quantum dots
semiconductors},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/anie.200600317}
}

@Article{Steeds2009,
  Title                    = {Photoluminescence study of the carbon antisite-vacancy pair in 4H - and 6H-SiC},
  Author                   = {Steeds, J. W.},
  Journal                  = {Physical Review B},
  Year                     = {2009},
  Number                   = {24},
  Volume                   = {80},

  Doi                      = {10.1103/PhysRevB.80.245202},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{Stockman2004,
  Title                    = {Nanofocusing of Optical Energy in Tapered Plasmonic Waveguides},
  Author                   = {Stockman, Mark},
  Journal                  = {Physical Review Letters},
  Year                     = {2004},
  Number                   = {13},
  Volume                   = {93},

  Doi                      = {10.1103/PhysRevLett.93.137404},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Stranahan2010,
  Title                    = {Super-resolution optical imaging of single-molecule SERS hot spots},
  Author                   = {Stranahan, S. M. and Willets, K. A.},
  Journal                  = {Nano Lett},
  Year                     = {2010},
  Number                   = {9},
  Pages                    = {3777-84},
  Volume                   = {10},

  Abstract                 = {We present the first super-resolution optical images of single-molecule surface-enhanced Raman scattering (SM-SERS) hot spots, using super-resolution imaging as a powerful new tool for understanding the interaction between single molecules and nanoparticle hot spots. Using point spread function fitting, we map the centroid position of SM-SERS with +/-10 nm resolution, revealing a spatial relationship between the SM-SERS centroid position and the highest SERS intensity. We are also able to measure the unique position of the SM-SERS centroid relative to the centroid associated with nanoparticle photoluminescence, which allows us to speculate on the presence of multiple hot spots within a single diffraction-limited spot. These measurements allow us to follow dynamic movement of the SM-SERS centroid position over time as it samples different locations in space and explores regions larger than the expected size of a SM-SERS hot spot. We have proposed that the movement of the SERS centroid is due to diffusion of a single molecule on the surface of the nanoparticle, which leads to changes in coupling between the scattering dipole and the optical near field of the nanoparticle.},
  Doi                      = {10.1021/nl102559d},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Keywords                 = {Diffusion
Scattering, Radiation
Spectrum Analysis, Raman/*methods},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20718441}
}

@Article{Suhling2005,
  Title                    = {Time-resolved fluorescence microscopy},
  Author                   = {Suhling, K. and French, P. M. W. and Phillips, D.},
  Journal                  = {Photochemical \& Photobiological Sciences},
  Year                     = {2005},
  Number                   = {1},
  Pages                    = {13-22},
  Volume                   = {4},

  Doi                      = {10.1039/b412924p},
  Owner                    = {Toan},
  Pm                       = {15616687},
  Sn                       = {1474-905X},
  Tc                       = {268},
  Timestamp                = {2015.04.10},
  Ut                       = {WOS:000225889800002},
  Z8                       = {4},
  Z9                       = {273},
  Zb                       = {113},
  Zs                       = {0}
}

@Article{Sun2012,
  Title                    = {Bright infrared quantum-dot light-emitting diodes through inter-dot spacing control},
  Author                   = {Sun, L. and Choi, J. J. and Stachnik, D. and Bartnik, A. C. and Hyun, B. R. and Malliaras, G. G. and Hanrath, T. and Wise, F. W.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2012},
  Number                   = {6},
  Pages                    = {369-73},
  Volume                   = {7},

  Abstract                 = {Infrared light-emitting diodes are currently fabricated from direct-gap semiconductors using epitaxy, which makes them expensive and difficult to integrate with other materials. Light-emitting diodes based on colloidal semiconductor quantum dots, on the other hand, can be solution-processed at low cost, and can be directly integrated with silicon. However, so far, exciton dissociation and recombination have not been well controlled in these devices, and this has limited their performance. Here, by tuning the distance between adjacent PbS quantum dots, we fabricate thin-film quantum-dot light-emitting diodes that operate at infrared wavelengths with radiances (6.4 W sr(-1) m(-2)) eight times higher and external quantum efficiencies (2.0%) two times higher than the highest values previously reported. The distance between adjacent dots is tuned over a range of 1.3 nm by varying the lengths of the linker molecules from three to eight CH(2) groups, which allows us to achieve the optimum balance between charge injection and radiative exciton recombination. The electroluminescent powers of the best devices are comparable to those produced by commercial InGaAsP light-emitting diodes. By varying the size of the quantum dots, we can tune the emission wavelengths between 800 and 1,850 nm.},
  Doi                      = {10.1038/nnano.2012.63},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {*Infrared Rays
*Quantum Dots
*Semiconductors},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22562037}
}

@Article{Sun2007,
  Title                    = {Bright, multicoloured light-emitting diodes based on quantum dots},
  Author                   = {Sun, Qingjiang and Wang, Y. Andrew and Li, Lin Song and Wang, Daoyuan and Zhu, Ting and Xu, Jian and Yang, Chunhe and Li, Yongfang},
  Journal                  = {Nature Photonics},
  Year                     = {2007},
  Number                   = {12},
  Pages                    = {717-722},
  Volume                   = {1},

  Doi                      = {10.1038/nphoton.2007.226},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Susumu2007,
  Title                    = {Enhancing the Stability and Biological Functionalities of Quantum Dots via Compact Multifunctional Ligands},
  Author                   = {Susumu, Kimihiro and Uyeda, H. Tetsuo and Medintz, Igor L. and Pons, Thomas and Delehanty, James B. and Mattoussi, Hedi},
  Journal                  = {Journal of the American Chemical Society},
  Year                     = {2007},
  Number                   = {45},
  Pages                    = {13987-13996},
  Volume                   = {129},

  Doi                      = {10.1021/ja0749744},
  ISSN                     = {0002-7863},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/ja0749744}
}

@Article{Talapin2009,
  Title                    = {Prospects of Colloidal Nanocrystals for Electronic and Optoelectronic Applications},
  Author                   = {Talapin, Dmitri V. and Lee, Jong-Soo and Kovalenko, Maksym V. and Shevchenko, Elena V.},
  Journal                  = {Chemical Reviews},
  Year                     = {2009},
  Number                   = {1},
  Pages                    = {389-458},
  Volume                   = {110},

  Doi                      = {10.1021/cr900137k},
  ISSN                     = {0009-2665},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/cr900137k}
}

@Article{Tame2013,
  Title                    = {Quantum plasmonics},
  Author                   = {Tame, M. S. and McEnery, K. R. and Ã–zdemir, Åž K. and Lee, J. and Maier, S. A. and Kim, M. S.},
  Journal                  = {Nature Physics},
  Year                     = {2013},
  Number                   = {6},
  Pages                    = {329-340},
  Volume                   = {9},

  Doi                      = {10.1038/nphys2615},
  ISSN                     = {1745-2473
1745-2481},
  Type                     = {Journal Article}
}

@Article{Tan2014,
  Title                    = {Quantum Plasmon Resonances Controlled by Molecular Tunnel Junctions},
  Author                   = {Tan, Shu Fen and Wu, Lin and Yang, Joel K. W. and Bai, Ping and Bosman, Michel and Nijhuis, Christian A.},
  Journal                  = {Science},
  Year                     = {2014},
  Number                   = {6178},
  Pages                    = {1496-1499},
  Volume                   = {343},

  Abstract                 = {Quantum tunneling between two plasmonic resonators links nonlinear quantum optics with terahertz nanoelectronics. We describe the direct observation of and control over quantum plasmon resonances at length scales in the range 0.4 to 1.3 nanometers across molecular tunnel junctions made of two plasmonic resonators bridged by self-assembled monolayers (SAMs). The tunnel barrier width and height are controlled by the properties of the molecules. Using electron energy-loss spectroscopy, we directly observe a plasmon mode, the tunneling charge transfer plasmon, whose frequency (ranging from 140 to 245 terahertz) is dependent on the molecules bridging the gaps.},
  Doi                      = {10.1126/science.1248797},
  ISSN                     = {0036-8075},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000333471000043}
}

@Article{Tanaka2003,
  Title                    = {Simulations of nanometric optical circuits based on surface plasmon polariton gap waveguide},
  Author                   = {Tanaka, Kazuo and Tanaka, Masahiro},
  Journal                  = {Applied Physics Letters},
  Year                     = {2003},
  Number                   = {8},
  Pages                    = {1158},
  Volume                   = {82},

  Doi                      = {10.1063/1.1557323},
  ISSN                     = {00036951},
  Type                     = {Journal Article}
}

@Article{Tang2014,
  Title                    = {Tuning band gaps of BN nanosheets and nanoribbons via interfacial dihalogen bonding and external electric field},
  Author                   = {Tang, Q. and Bao, J. and Li, Y. and Zhou, Z. and Chen, Z.},
  Journal                  = {Nanoscale},
  Year                     = {2014},
  Number                   = {15},
  Pages                    = {8624-34},
  Volume                   = {6},

  Abstract                 = {Density functional theory computations with dispersion corrections (DFT-D) were performed to investigate the dihalogen interactions and their effect on the electronic band structures of halogenated (fluorinated and chlorinated) BN bilayers and aligned halogen-passivated zigzag BN nanoribbons (BNNRs). Our results reveal the presence of considerable homo-halogen (FF and ClCl) interactions in bilayer fluoro (chloro)-BN sheets and the aligned F (Cl)-ZBNNRs, as well as substantial hetero-halogen (FCl) interactions in hybrid fluoro-BN/chloro-BN bilayer and F-Cl-ZBNNRs. The existence of interfacial dihalogen interactions leads to significant band-gap modifications for the studied BN nanosystems. Compared with the individual fluoro (chloro)-BN monolayers or pristine BNNRs, the gap reduction in bilayer fluoro-BN (B-FF-N array), hybrid fluoro-BN/chloro-BN bilayer (N-FCl-N array), aligned Cl-ZBNNRs (B-ClCl-N alignment), and hybrid F-Cl-ZBNNRs (B-FCl-N alignment) is mainly due to interfacial polarizations, while the gap narrowing in bilayer chloro-BN (N-ClCl-N array) is ascribed to the interfacial nearly-free-electron states. Moreover, the binding strengths and electronic properties of the interactive BN nanosheets and nanoribbons can be controlled by applying an external electric field, and extensive modulation from large-gap to medium-gap semiconductors, or even metals can be realized by adjusting the direction and strength of the applied electric field. This interesting strategy for band gap control based on weak interactions offers unique opportunities for developing BN nanoscale electronic devices.},
  Doi                      = {10.1039/c4nr00008k},
  ISSN                     = {2040-3372 (Electronic)
2040-3364 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24824079}
}

@Article{Tanuma2014,
  Title                    = {Three-dimensional imaging of extended defects in 4H-SiC by optical second-harmonic generation and two-photon-excited photoluminescence},
  Author                   = {Tanuma, Ryohei and Tsuchida, Hidekazu},
  Journal                  = {Applied Physics Express},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {021304},
  Volume                   = {7},

  Doi                      = {10.7567/apex.7.021304},
  ISSN                     = {1882-0778
1882-0786},
  Type                     = {Journal Article}
}

@Article{Tartakovskii2001,
  Title                    = {Stimulated Polariton Scattering in Semiconductor Microcavities: New Physics and Potential Applications},
  Author                   = {Tartakovskii, A. I. and Skolnick, M. S. and Krizhanovskii, D. N. and Kulakovskii, V. D. and Stevenson, R. M. and ButtÃ©, R. and Baumberg, J. J. and Whittaker, D. M. and Roberts, J. S.},
  Journal                  = {Advanced Materials},
  Year                     = {2001},
  Number                   = {22},
  Pages                    = {1725-1730},
  Volume                   = {13},

  Abstract                 = {Stimulated polariton scattering in semiconductor microcavities is reported. The phenomena arise from the bosonic character of the coupled excitonâ€“photon modes of the system. The ability to manipulate and control the polariton dispersions in microcavities is shown to be a key factor underlying the new observations. The potential of such phenomena to form the basis of a new type of coherent light source (â€œpolaritonâ€? lasers) and highly efficient optical parametric oscillators is discussed.},
  Doi                      = {10.1002/1521-4095(200111)13:22<1725::AID-ADMA1725>3.0.CO;2-Z},
  ISSN                     = {1521-4095},
  Keywords                 = {Microcavities
Polariton scattering
Semiconductors},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/1521-4095(200111)13:22<1725::AID-ADMA1725>3.0.CO;2-Z}
}

@Article{Taylor2008,
  Title                    = {High-sensitivity diamond magnetometer with nanoscale resolution},
  Author                   = {Taylor, J. M. and Cappellaro, P. and Childress, L. and Jiang, L. and Budker, D. and Hemmer, P. R. and Yacoby, A. and Walsworth, R. and Lukin, M. D.},
  Journal                  = {Nature Physics},
  Year                     = {2008},
  Number                   = {10},
  Pages                    = {810-816},
  Volume                   = {4},

  Doi                      = {10.1038/nphys1075},
  ISSN                     = {1745-2473
1745-2481},
  Type                     = {Journal Article}
}

@Article{Teii2012,
  Title                    = {Low threshold field emission from high-quality cubic boron nitride films},
  Author                   = {Teii, Kungen and Matsumoto, Seiichiro},
  Journal                  = {Journal of Applied Physics},
  Year                     = {2012},
  Number                   = {9},
  Pages                    = {093728},
  Volume                   = {111},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.4711093},
  Keywords                 = {field emission
visible spectra
electrical conductivity
semiconductor thin films
plasma CVD
semiconductor growth
X-ray diffraction
surface roughness
III-V semiconductors
wide band gap semiconductors
Raman spectra
boron compounds
ultraviolet spectra
X-ray photoelectron spectra},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/jap/111/9/10.1063/1.4711093}
}

@Article{Teissier2014,
  Title                    = {Strain Coupling of a Nitrogen-Vacancy Center Spin to a Diamond Mechanical Oscillator},
  Author                   = {Teissier, J. and Barfuss, A. and Appel, P. and Neu, E. and Maletinsky, P.},
  Journal                  = {Physical Review Letters},
  Year                     = {2014},
  Number                   = {2},
  Volume                   = {113},

  Doi                      = {10.1103/PhysRevLett.113.020503},
  ISSN                     = {0031-9007
1079-7114},
  Type                     = {Journal Article}
}

@Article{Temnov2012,
  Title                    = {Ultrafast acousto-magneto-plasmonics},
  Author                   = {Temnov, Vasily V.},
  Journal                  = {Nature Photonics},
  Year                     = {2012},
  Number                   = {11},
  Pages                    = {728-736},
  Volume                   = {6},

  Doi                      = {10.1038/nphoton.2012.220},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Temnov2010,
  Title                    = {Active magneto-plasmonics in hybrid metalâ€“ferromagnet structures},
  Author                   = {Temnov, Vasily V. and Armelles, Gaspar and Woggon, Ulrike and Guzatov, Dmitry and Cebollada, Alfonso and Garcia-Martin, Antonio and Garcia-Martin, Jose-Miguel and Thomay, Tim and Leitenstorfer, Alfred and Bratschitsch, Rudolf},
  Journal                  = {Nature Photonics},
  Year                     = {2010},
  Number                   = {2},
  Pages                    = {107-111},
  Volume                   = {4},

  Doi                      = {10.1038/nphoton.2009.265},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Tews2004,
  Title                    = {Electronic structure and transport properties of quantum dots},
  Author                   = {Tews, M.},
  Journal                  = {Annalen der Physik},
  Year                     = {2004},
  Number                   = {5},
  Pages                    = {249-304},
  Volume                   = {13},

  Doi                      = {10.1002/andp.200410076},
  ISSN                     = {0003-3804
1521-3889},
  Type                     = {Journal Article}
}

@Article{Togan2010,
  Title                    = {Quantum entanglement between an optical photon and a solid-state spin qubit},
  Author                   = {Togan, E. and Chu, Y. and Trifonov, A. S. and Jiang, L. and Maze, J. and Childress, L. and Dutt, M. V. and Sorensen, A. S. and Hemmer, P. R. and Zibrov, A. S. and Lukin, M. D.},
  Journal                  = {Nature},
  Year                     = {2010},
  Number                   = {7307},
  Pages                    = {730-4},
  Volume                   = {466},

  Abstract                 = {Quantum entanglement is among the most fascinating aspects of quantum theory. Entangled optical photons are now widely used for fundamental tests of quantum mechanics and applications such as quantum cryptography. Several recent experiments demonstrated entanglement of optical photons with trapped ions, atoms and atomic ensembles, which are then used to connect remote long-term memory nodes in distributed quantum networks. Here we realize quantum entanglement between the polarization of a single optical photon and a solid-state qubit associated with the single electronic spin of a nitrogen vacancy centre in diamond. Our experimental entanglement verification uses the quantum eraser technique, and demonstrates that a high degree of control over interactions between a solid-state qubit and the quantum light field can be achieved. The reported entanglement source can be used in studies of fundamental quantum phenomena and provides a key building block for the solid-state realization of quantum optical networks.},
  Doi                      = {10.1038/nature09256},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20686569}
}

@Article{Tokushima2000,
  Title                    = {Lightwave propagation through a 120 degrees sharply bent single-line-defect photonic crystal waveguide},
  Author                   = {Tokushima, M. and Kosaka, H. and Tomita, A. and Yamada, H.},
  Journal                  = {Applied Physics Letters},
  Year                     = {2000},
  Number                   = {8},
  Pages                    = {952-954},
  Volume                   = {76},

  Abstract                 = {We have demonstrated 1.55 mu m wavelength lightwave propagation through a 120 degrees sharply bent waveguide formed in a triangular-lattice two-dimensional photonic crystal (2D PC). Such propagation has not previously been experimentally confirmed. The photonic crystal was fabricated in a silicon-on-insulator (SOI) wafer with the top silicon layer of the wafer used as a core layer. A 877-mu m-long single-line-defect waveguide was formed in the PC with a sharp 120 degrees bend near the middle of the waveguide. A tapered-hemispherical-end fiber was coupled to the input end of the waveguide for the light input, and the output from the other end of the waveguide was directly observed by scanning its near-field profile with another tapered-hemispherical-end fiber. (C) 2000 American Institute of Physics. [S0003-6951(00)01208-0].},
  Doi                      = {10.1063/1.125902},
  ISSN                     = {0003-6951},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000085343700004}
}

@Article{Tong2004,
  Title                    = {Single-mode guiding properties of subwavelength-diameter silica and silicon wire waveguides},
  Author                   = {Tong, L. M. and Lou, J. Y. and Mazur, E.},
  Journal                  = {Optics Express},
  Year                     = {2004},
  Number                   = {6},
  Pages                    = {1025-1035},
  Volume                   = {12},

  Abstract                 = {Single-mode optical wave guiding properties of silica and silicon subwavelength-diameter wires are studied with exact solutions of Maxwell's equations. Single mode conditions, modal fields, power distribution, group velocities and waveguide dispersions are studied. It shows that air-clad subwavelength-diameter wires have interesting properties such as tight-confinement ability, enhanced evanescent fields and large waveguide dispersions that are very promising for developing future microphotonic devices with subwavelength-width structures. (C) 2004 Optical Society of America.},
  Doi                      = {10.1364/opex.12.001025},
  ISSN                     = {1094-4087},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000220594800008}
}

@Article{Toyli2012,
  Title                    = {Measurement and Control of Single Nitrogen-Vacancy Center Spins above 600Â K},
  Author                   = {Toyli, D. M. and Christle, D. J. and Alkauskas, A. and Buckley, B. B. and Van de Walle, C. G. and Awschalom, D. D.},
  Journal                  = {Physical Review X},
  Year                     = {2012},
  Number                   = {3},
  Volume                   = {2},

  Doi                      = {10.1103/PhysRevX.2.031001},
  ISSN                     = {2160-3308},
  Type                     = {Journal Article}
}

@Article{Umeda2007,
  Title                    = {Identification of positively charged carbon antisite-vacancy pairs in 4H-SiC},
  Author                   = {Umeda, T. and Ishoya, J. and Ohshima, T. and Morishita, N. and Itoh, H. and Gali, A.},
  Journal                  = {Physical Review B},
  Year                     = {2007},
  Number                   = {24},
  Volume                   = {75},

  Abstract                 = {An antisite-vacancy pair and a monovacancy are a set of fundamental stable and/or metastable defects in compound semiconductors. Theory predicted that carbon antisite-vacancy pairs would be much more stable in p-type SiC than silicon vacancies and that they would be a common defect. However, no experimental evidence has yet supported this prediction. We reexamine electron-irradiated p-type 4H-SiC and identify the positively charged carbon antisite-vacancy pairs (CSiVC+) by means of electron paramagnetic resonance and ab initio calculations. We compare them with other coexisting defects such as carbon vacancy (V-C) and divacancy (VSiVC) and show that CSiVC and V-C are very similar in terms of thermal stability and electronic levels.},
  Doi                      = {10.1103/PhysRevB.75.245202},
  ISSN                     = {1098-0121},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000247625000055}
}

@Article{Umeda2006,
  Title                    = {Identification of the carbon antisite-vacancy pair in 4H-SiC},
  Author                   = {Umeda, T. and Son, N. T. and Isoya, J. and Janzen, E. and Ohshima, T. and Morishita, N. and Itoh, H. and Gali, A. and Bockstedte, M.},
  Journal                  = {Physical Review Letters},
  Year                     = {2006},
  Number                   = {14},
  Volume                   = {96},

  Abstract                 = {The metastability of vacancies was theoretically predicted for several compound semiconductors alongside their transformation into the antisite-vacancy pair counterpart; however, no experiment to date has unambiguously confirmed the existence of antisite-vacancy pairs. Using electron paramagnetic resonance and first principles calculations we identify the SI5 center as the carbon antisite-vacancy pair in the negative charge state (CSiVC-) in 4H-SiC. We suggest that this defect is a strong carrier-compensating center in n-type or high-purity semi-insulating SiC.},
  Doi                      = {10.1103/PhysRevLett.96.145501},
  ISSN                     = {0031-9007},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000236797200038}
}

@Article{Urena2012,
  Title                    = {Excitation enhancement of a quantum dot coupled to a plasmonic antenna},
  Author                   = {Urena, E. B. and Kreuzer, M. P. and Itzhakov, S. and Rigneault, H. and Quidant, R. and Oron, D. and Wenger, J.},
  Journal                  = {Adv Mater},
  Year                     = {2012},
  Number                   = {44},
  Pages                    = {OP314-20},
  Volume                   = {24},

  Abstract                 = {Plasmonic antennas are key elements to control the luminescence of quantum emitters. However, the antenna's influence is often hidden by quenching losses. Here, the luminescence of a quantum dot coupled to a gold dimer antenna is investigated. Detailed analysis of the multiply excited states quantifies the antenna's influence on the excitation intensity and the luminescence quantum yield separately.},
  Doi                      = {10.1002/adma.201202783},
  ISSN                     = {1521-4095 (Electronic)
0935-9648 (Linking)},
  Keywords                 = {Computer Simulation
Gold/*chemistry
Light
Lighting/*methods
Luminescent Measurements/*methods
Metal Nanoparticles/*chemistry
*Models, Chemical
*Quantum Dots
Scattering, Radiation
Surface Plasmon Resonance/*methods},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23027548}
}

@Article{Vahala2003,
  Title                    = {Optical microcavities},
  Author                   = {Vahala, Kerry J.},
  Journal                  = {Nature},
  Year                     = {2003},
  Number                   = {6950},
  Pages                    = {839-846},
  Volume                   = {424},

  ISSN                     = {0028-0836},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nature01939}
}

@Article{Valentine2008,
  Title                    = {Three-dimensional optical metamaterial with a negative refractive index},
  Author                   = {Valentine, J. and Zhang, S. and Zentgraf, T. and Ulin-Avila, E. and Genov, D. A. and Bartal, G. and Zhang, X.},
  Journal                  = {Nature},
  Year                     = {2008},
  Number                   = {7211},
  Pages                    = {376-9},
  Volume                   = {455},

  Abstract                 = {Metamaterials are artificially engineered structures that have properties, such as a negative refractive index, not attainable with naturally occurring materials. Negative-index metamaterials (NIMs) were first demonstrated for microwave frequencies, but it has been challenging to design NIMs for optical frequencies and they have so far been limited to optically thin samples because of significant fabrication challenges and strong energy dissipation in metals. Such thin structures are analogous to a monolayer of atoms, making it difficult to assign bulk properties such as the index of refraction. Negative refraction of surface plasmons was recently demonstrated but was confined to a two-dimensional waveguide. Three-dimensional (3D) optical metamaterials have come into focus recently, including the realization of negative refraction by using layered semiconductor metamaterials and a 3D magnetic metamaterial in the infrared frequencies; however, neither of these had a negative index of refraction. Here we report a 3D optical metamaterial having negative refractive index with a very high figure of merit of 3.5 (that is, low loss). This metamaterial is made of cascaded 'fishnet' structures, with a negative index existing over a broad spectral range. Moreover, it can readily be probed from free space, making it functional for optical devices. We construct a prism made of this optical NIM to demonstrate negative refractive index at optical frequencies, resulting unambiguously from the negative phase evolution of the wave propagating inside the metamaterial. Bulk optical metamaterials open up prospects for studies of 3D optical effects and applications associated with NIMs and zero-index materials such as reversed Doppler effect, superlenses, optical tunnelling devices, compact resonators and highly directional sources.},
  Doi                      = {10.1038/nature07247},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/18690249}
}

@Article{Verhagen2006,
  Title                    = {Enhanced Nonlinear Optical Effects with a Tapered Plasmonic Waveguide},
  Author                   = {Verhagen, Ewold and Kuipers, Laurens and Polman, Albert},
  Journal                  = {Nano Letters},
  Year                     = {2006},
  Number                   = {2},
  Pages                    = {334-337},
  Volume                   = {7},

  Doi                      = {10.1021/nl062440f},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl062440f}
}

@Article{Veronis2007,
  Title                    = {Theoretical investigation of compact couplers between dielectric slabwaveguides and two-dimensional metal-dielectric-metal plasmonicwaveguides},
  Author                   = {Veronis, Georgios and Fan, Shanhui},
  Journal                  = {Optics Express},
  Year                     = {2007},
  Number                   = {3},
  Pages                    = {1211-1221},
  Volume                   = {15},

  Abstract                 = {We theoretically investigate the properties of compact couplers between high-index contrast dielectric slab waveguides and two-dimensional metal-dielectric-metal subwavelength plasmonic waveguides. We show that a coupler created by simply placing a dielectric waveguide terminated flat at the exit end of a plasmonic waveguide can be designed to have a transmission efficiency of ~70% at the optical communicationwavelength. We also show that the transmission efficiency of the couplers can be further increased by using optimized multisection tapers. In both cases the transmission response is broadband. In addition, we investigate the properties of a Fabry-Perot structure in which light is coupled in and out of a plasmonic waveguide sandwiched between dielectric waveguides. Finally, we discuss potential fabrication processes for structures that demonstrate the predicted effects.},
  Doi                      = {10.1364/OE.15.001211},
  Keywords                 = {Guided waves
Integrated optics devices
Surface plasmons},
  Type                     = {Journal Article},
  Url                      = {http://www.opticsexpress.org/abstract.cfm?URI=oe-15-3-1211}
}

@Article{Vlasov2014,
  Title                    = {Molecular-sized fluorescent nanodiamonds},
  Author                   = {Vlasov, Igor I. and Shiryaev, Andrey A. and Rendler, Torsten and Steinert, Steffen and Lee, Sang-Yun and Antonov, Denis and VÃ¶rÃ¶s, MÃ¡rton and Jelezko, Fedor and Fisenko, Anatolii V. and Semjonova, Lubov F. and Biskupek, Johannes and Kaiser, Ute and Lebedev, Oleg I. and Sildos, Ilmo and Hemmer, Philip R. and Konov, Vitaly I. and Gali, Adam and Wrachtrup, JÃ¶rg},
  Journal                  = {Nature Nanotechnology},
  Year                     = {2014},
  Number                   = {1},
  Pages                    = {54-58},
  Volume                   = {9},

  Abstract                 = {Doping of carbon nanoparticles with impurity atoms is central to their application. However, doping has proven elusive for very small carbon nanoparticles because of their limited availability and a lack of fundamental understanding of impurity stability in such nanostructures. Here, we show that isolated diamond nanoparticles as small as 1.6 nm, comprising only âˆ¼400 carbon atoms, are capable of housing stable photoluminescent colour centres, namely the silicon vacancy (SiV). Surprisingly, fluorescence from SiVs is stable over time, and few or only single colour centres are found per nanocrystal. We also observe size-dependent SiV emission supported by quantum-chemical simulation of SiV energy levels in small nanodiamonds. Our work opens the way to investigating the physics and chemistry of molecular-sized cubic carbon clusters and promises the application of ultrasmall non-perturbative fluorescent nanoparticles as markers in microscopy and sensing. [ABSTRACT FROM AUTHOR]
Copyright of Nature Nanotechnology is the property of Nature Publishing Group and its content may not be copied or emailed to multiple sites or posted to a listserv without the copyright holder's express written permission. However, users may print, download, or email articles for individual use. This abstract may be abridged. No warranty is given about the accuracy of the copy. Users should refer to the original published version of the material for the full abstract. (Copyright applies to all Abstracts.)},
  Doi                      = {10.1038/nnano.2013.255},
  ISSN                     = {17483387},
  Keywords                 = {MOLECULAR size
FLUORESCENCE
NANODIAMONDS
DOPING agents (Chemistry)
CARBON nanotubes
PHOTOLUMINESCENCE
MICROSCOPY},
  Type                     = {Journal Article},
  Url                      = {https://www.lib.uts.edu.au/goto?url=http://search.ebscohost.com/login.aspx?direct=true&db=a9h&AN=93463799&site=ehost-live}
}

@Article{Voss2007,
  Title                    = {High-Order Waveguide Modes in ZnO Nanowires},
  Author                   = {Voss, Tobias and Svacha, Geoffry T. and Mazur, Eric and MÃ¼ller, Sven and Ronning, Carsten and Konjhodzic, Denan and Marlow, Frank},
  Journal                  = {Nano Letters},
  Year                     = {2007},
  Number                   = {12},
  Pages                    = {3675-3680},
  Volume                   = {7},

  Doi                      = {10.1021/nl071958w},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl071958w}
}

@Article{Wallraff2004,
  Title                    = {Strong coupling of a single photon to a superconducting qubit using circuit quantum electrodynamics},
  Author                   = {Wallraff, A. and Schuster, D. I. and Blais, A. and Frunzio, L. and Huang, R. and Majer, J. and Kumar, S. and Girvin, S. M. and Schoelkopf, R. J.},
  Journal                  = {Nature},
  Year                     = {2004},
  Number                   = {7005},
  Pages                    = {162-7},
  Volume                   = {431},

  Abstract                 = {The interaction of matter and light is one of the fundamental processes occurring in nature, and its most elementary form is realized when a single atom interacts with a single photon. Reaching this regime has been a major focus of research in atomic physics and quantum optics for several decades and has generated the field of cavity quantum electrodynamics. Here we perform an experiment in which a superconducting two-level system, playing the role of an artificial atom, is coupled to an on-chip cavity consisting of a superconducting transmission line resonator. We show that the strong coupling regime can be attained in a solid-state system, and we experimentally observe the coherent interaction of a superconducting two-level system with a single microwave photon. The concept of circuit quantum electrodynamics opens many new possibilities for studying the strong interaction of light and matter. This system can also be exploited for quantum information processing and quantum communication and may lead to new approaches for single photon generation and detection.},
  Doi                      = {10.1038/nature02851},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/15356625}
}

@Article{Wallraff2004a,
  Title                    = {Strong coupling of a single photon to a superconducting qubit using circuit quantum electrodynamics},
  Author                   = {Wallraff, A. and Schuster, D. I. and Blais, A. and Frunzio, L. and Huang, R. S. and Majer, J. and Kumar, S. and Girvin, S. M. and Schoelkopf, R. J.},
  Journal                  = {Nature},
  Year                     = {2004},
  Number                   = {7005},
  Pages                    = {162-167},
  Volume                   = {431},

  ISSN                     = {0028-0836},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nature02851}
}

@Article{Wang2009,
  Title                    = {Annealing effects on the morphology and luminescence of cubic boron nitride based ceramics},
  Author                   = {Wang, P. F. and Li, Zh H. and Zhang, B. and Gao, K. and Zhu, Y. M.},
  Journal                  = {Solid State Sciences},
  Year                     = {2009},
  Number                   = {12},
  Pages                    = {2162-2166},
  Volume                   = {11},

  Abstract                 = {Cubic boron nitride based ceramics with silicon were sintered at 1350 Â°C under a pressure of 5.0 GPa. The effects of post-annealing on grain morphology, surface morphology, and photoluminescence of Siâ€“cBN ceramics were investigated by scanning electron microscope and room temperature photoluminescence measurements. The results showed that the annealing treatment had great influence on cBN grain morphology, rather than the surface morphology. The luminescence intensity increased with annealing temperature and annealing time. The void-net structure formed by continuous distribution of SiOx particulate on the ceramic surface resulted in the emission band peaking at about 701.2 nm, and the tense passivation of Si by SiOx led to the peak's low intensity. The near ultraviolet emission band peaking at about 317 nm was attributed to the oxygen vacancies formed in cBN grain surface, caused by the scavenging of oxygen from the cBN grain surface by the added Si.},
  Doi                      = {http://dx.doi.org/10.1016/j.solidstatesciences.2009.08.010},
  ISSN                     = {1293-2558},
  Keywords                 = {Annealing
Microstructure
Luminescence
Cubic boron nitride},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S1293255809002933}
}

@Article{Wang2012,
  Title                    = {Electronics and optoelectronics of two-dimensional transition metal dichalcogenides},
  Author                   = {Wang, Q. H. and Kalantar-Zadeh, K. and Kis, A. and Coleman, J. N. and Strano, M. S.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2012},
  Number                   = {11},
  Pages                    = {699-712},
  Volume                   = {7},

  Abstract                 = {The remarkable properties of graphene have renewed interest in inorganic, two-dimensional materials with unique electronic and optical attributes. Transition metal dichalcogenides (TMDCs) are layered materials with strong in-plane bonding and weak out-of-plane interactions enabling exfoliation into two-dimensional layers of single unit cell thickness. Although TMDCs have been studied for decades, recent advances in nanoscale materials characterization and device fabrication have opened up new opportunities for two-dimensional layers of thin TMDCs in nanoelectronics and optoelectronics. TMDCs such as MoS(2), MoSe(2), WS(2) and WSe(2) have sizable bandgaps that change from indirect to direct in single layers, allowing applications such as transistors, photodetectors and electroluminescent devices. We review the historical development of TMDCs, methods for preparing atomically thin layers, their electronic and optical properties, and prospects for future advances in electronics and optoelectronics.},
  Doi                      = {10.1038/nnano.2012.193},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {Chalcogens/*chemistry
Electronics/*instrumentation
Equipment Design
Models, Molecular
Optics and Photonics/*instrumentation
Semiconductors/*instrumentation
Transition Elements/*chemistry},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23132225}
}

@Article{Wang2014,
  Title                    = {Tunable magnetic and electronic properties of BN nanosheets with triangular defects: a first-principles study},
  Author                   = {Wang, Y. and Ding, Y.},
  Journal                  = {J Phys Condens Matter},
  Year                     = {2014},
  Number                   = {43},
  Pages                    = {435302},
  Volume                   = {26},

  Abstract                 = {Experimentally, vacancy defects are commonly observed in BN nanosheets, expecially nitrogen-terminated triangular defects. Based on first-principles calculations, we systematically investigate the magnetic and electronic properties of BN nanosheets with these triangular vacancies (referred to as Vi(i = 1 - 4) defects with i representing the number of N atoms on each side of the triangle). It is found that the Vi defects bring diverse magnetic states into BN sheets, which are ferrimagnetic for V1, nonmagnetic for V2, ferrimagnetic for V3 and antiferromagnetic for V4 defects. When the isotropic strains are applied, the ferrimagnetic state is sustained for V1 defect, whereas the V2 defect undergoes a nonmagnetic to antiferromagnetic transition and the V3, V4 defects experience an abrupt change in the absolute magnetic moments under small strains, which are originated from the N-N bond breaking at these defects. Different from the BN nanoribbons, the antiparallel coupling is more favorable for the N atoms at the edges of triangular defects. Due to the triangular defects, the band gaps of BN sheets are reduced substantially, which could be further modulated by the strains. When the defective BN sheets serve as a substrate for graphene, the V1, V3 and V4 defects in BN would induce p-type doping in the graphene sheet. Interestingly, when the V2 defect is embedded in BN sheets, the doping behavior of graphene can be well-controlled by the strain, which is charge neutral at the strain-free state and p-type doped under strains. Our studies demonstrate that the rich magnetic and electronic properties of BN sheets with triangular defects enable the system's potential applications in nanodevices.},
  Doi                      = {10.1088/0953-8984/26/43/435302},
  ISSN                     = {1361-648X (Electronic)
0953-8984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25299579}
}

@Article{Wang2013,
  Title                    = {Structural, Electronic, and Magnetic Properties of the Semifluorinated Boron Nitride Bilayer: A First-Principles Study},
  Author                   = {Wang, Yanli and Ding, Yi},
  Journal                  = {The Journal of Physical Chemistry C},
  Year                     = {2013},
  Number                   = {6},
  Pages                    = {3114-3121},
  Volume                   = {117},

  Doi                      = {10.1021/jp311189a},
  ISSN                     = {1932-7447
1932-7455},
  Type                     = {Journal Article}
}

@Article{Wang2015,
  Title                    = {Plasmon Resonances of Highly Doped Two-Dimensional MoS2},
  Author                   = {Wang, Y. and Ou, J. Z. and Chrimes, A. F. and Carey, B. J. and Daeneke, T. and Alsaif, M. M. and Mortazavi, M. and Zhuiykov, S. and Medhekar, N. and Bhaskaran, M. and Friend, J. R. and Strano, M. S. and Kalantar-Zadeh, K.},
  Journal                  = {Nano Lett},
  Year                     = {2015},
  Number                   = {2},
  Pages                    = {883-90},
  Volume                   = {15},

  Abstract                 = {The exhibition of plasmon resonances in two-dimensional (2D) semiconductor compounds is desirable for many applications. Here, by electrochemically intercalating lithium into 2D molybdenum disulfide (MoS2) nanoflakes, plasmon resonances in the visible and near UV wavelength ranges are achieved. These plasmon resonances are controlled by the high doping level of the nanoflakes after the intercalation, producing two distinct resonance peak areas based on the crystal arrangements. The system is also benchmarked for biosensing using bovine serum albumin. This work provides a foundation for developing future 2D MoS2 based biological and optical units.},
  Doi                      = {10.1021/nl503563g},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25562610}
}

@Article{Warburton2013,
  Title                    = {Single spins in self-assembled quantum dots},
  Author                   = {Warburton, R. J.},
  Journal                  = {Nat Mater},
  Year                     = {2013},
  Number                   = {6},
  Pages                    = {483-93},
  Volume                   = {12},

  Abstract                 = {Self-assembled quantum dots have excellent photonic properties. For instance, a single quantum dot is a high-brightness, narrow-linewidth source of single photons. Furthermore, the environment of a single quantum dot can be tailored relatively easily using semiconductor heterostructure and post-growth processing techniques, enabling electrical control of the quantum dot charge and control over the photonic modes with which the quantum dot interacts. A single electron or hole trapped inside a quantum dot has spintronics applications. Although the spin dephasing is rather rapid, a single spin can be manipulated using optical techniques on subnanosecond timescales. Optical experiments are also providing new insights into old issues, such as the central spin problem. This Review provides a snapshot of this active field, with some indications for the future. It covers the basic materials and optical properties of single quantum dots, techniques for initializing, manipulating and reading out single spin qubits, and the mechanisms that limit the electron-spin and hole-spin coherence.},
  Doi                      = {10.1038/nmat3585},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23695745}
}

@Article{Warren2012,
  Title                    = {Plasmoelectronics: coupling plasmonic excitation with electron flow},
  Author                   = {Warren, S. C. and Walker, D. A. and Grzybowski, B. A.},
  Journal                  = {Langmuir},
  Year                     = {2012},
  Number                   = {24},
  Pages                    = {9093-102},
  Volume                   = {28},

  Abstract                 = {Explorations of the coupling of light and charge via localized surface plasmons have led to the discovery that plasmonic excitation can influence macroscopic flows of charge and, conversely, that charging events can change the plasmonic excitation. We discuss recent theory and experiments in the emerging field of plasmoelectronics, with particular emphasis on the application of these materials to challenges in nanotechnology, energy use, and sensing.},
  Doi                      = {10.1021/la300377j},
  ISSN                     = {1520-5827 (Electronic)
0743-7463 (Linking)},
  Keywords                 = {Electronics
*Electrons
*Surface Plasmon Resonance},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22385329}
}

@Article{Watanabe2011,
  Title                    = {Hexagonal Boron Nitride as a New Ultraviolet Luminescent Material and Its Application},
  Author                   = {Watanabe, Kenji and Taniguchi, Takashi},
  Journal                  = {International Journal of Applied Ceramic Technology},
  Year                     = {2011},
  Number                   = {5},
  Pages                    = {977-989},
  Volume                   = {8},

  Abstract                 = {Hexagonal boron nitride (hBN), which is conventionally used as one of the best-known heat-resistant materials due to its high thermal and chemical stability, has recently been found as a highly luminous material in the far-ultraviolet (FUV) region. This paper reviews the recent studies of hBN growth, optical properties, and device application development. In the case of highly pure crystals of hBN grown by the solvent growth method, the electronic excitation states near the band gap are governed by optically allowed exciton effects, which originate from the Jahnâ€“Teller effect on the exciton series. The excitonic luminescence bands are utilized for an FUV plane light-emitting device excited by field emitters to take advantage of the highly luminous character.},
  Doi                      = {10.1111/j.1744-7402.2011.02626.x},
  ISSN                     = {1744-7402},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1111/j.1744-7402.2011.02626.x}
}

@Article{Watanabe2004,
  Title                    = {Direct-bandgap properties and evidence for ultraviolet lasing of hexagonal boron nitride single crystal},
  Author                   = {Watanabe, K. and Taniguchi, T. and Kanda, H.},
  Journal                  = {Nat. Mater.},
  Year                     = {2004},
  Number                   = {6},
  Pages                    = {404-9},
  Volume                   = {3},

  Abstract                 = {The demand for compact ultraviolet laser devices is increasing, as they are essential in applications such as optical storage, photocatalysis, sterilization, ophthalmic surgery and nanosurgery. Many researchers are devoting considerable effort to finding materials with larger bandgaps than that of GaN. Here we show that hexagonal boron nitride (hBN) is a promising material for such laser devices because it has a direct bandgap in the ultraviolet region. We obtained a pure hBN single crystal under high-pressure and high-temperature conditions, which shows a dominant luminescence peak and a series of s-like exciton absorption bands around 215 nm, proving it to be a direct-bandgap material. Evidence for room-temperature ultraviolet lasing at 215 nm by accelerated electron excitation is provided by the enhancement and narrowing of the longitudinal mode, threshold behaviour of the excitation current dependence of the emission intensity, and a far-field pattern of the transverse mode.},
  Doi                      = {10.1038/nmat1134},
  ISSN                     = {1476-1122 (Print)
1476-1122 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/15156198}
}

@Article{Watanabe2006,
  Title                    = {Band-edge luminescence of deformed hexagonal boron nitride single crystals},
  Author                   = {Watanabe, Kenji and Taniguchi, Takashi and Kuroda, Takashi and Kanda, Hisao},
  Journal                  = {Diamond and Related Materials},
  Year                     = {2006},
  Number                   = {11â€“12},
  Pages                    = {1891-1893},
  Volume                   = {15},

  Abstract                 = {We studied deformation effects on band-edge luminescence of pure hexagonal boron nitride single crystals. After simple deformation of the single crystals at room temperature, the band-edge luminescence showed a dramatic change, originating from stacking disorder, in the peak wavelength. It changed from 215Â nm in a free exciton band to 227Â nm in a bound exciton band. This 227-nm bound exciton luminescence has a fast radiative decay time (below a few ns).},
  Doi                      = {http://dx.doi.org/10.1016/j.diamond.2006.06.014},
  ISSN                     = {0925-9635},
  Keywords                 = {Hexagonal boron nitride (hBN)
Optical properties
Exciton
Luminescence},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0925963506002226}
}

@Article{Wee2007,
  Title                    = {Two-photon Excited Fluorescence of Nitrogen-Vacancy Centers in Proton-Irradiated Type Ib Diamondâ€ },
  Author                   = {Wee, Tse-Luen and Tzeng, Yan-Kai and Han, Chau-Chung and Chang, Huan-Cheng and Fann, Wunshain and Hsu, Jui-Hung and Chen, Kuan-Ming and Yu, Yueh-Chung},
  Journal                  = {The Journal of Physical Chemistry A},
  Year                     = {2007},
  Number                   = {38},
  Pages                    = {9379-9386},
  Volume                   = {111},

  Doi                      = {10.1021/jp073938o},
  ISSN                     = {1089-5639},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/jp073938o}
}

@Article{Wei1999,
  Title                    = {Observation of the dynamic Stark effect on electromagnetically induced transparency},
  Author                   = {Wei, Changjiang and Manson, Neil},
  Journal                  = {Physical Review A},
  Year                     = {1999},
  Number                   = {3},
  Pages                    = {2540-2546},
  Volume                   = {60},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevA.60.2540}
}

@Article{Wei2009,
  Title                    = {Propagating Surface Plasmon Induced Photon Emission from Quantum Dots},
  Author                   = {Wei, Hong and Ratchford, Daniel and Li, Xiaoqin and Xu, Hongxing and Shih, Chih-Kang},
  Journal                  = {Nano Letters},
  Year                     = {2009},
  Number                   = {12},
  Pages                    = {4168-4171},
  Volume                   = {9},

  Doi                      = {10.1021/nl9023897},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl9023897}
}

@Article{Wei2014,
  Title                    = {Directionally-Controlled Periodic Collimated Beams of Surface Plasmon Polaritons on Metal Film in Ag Nanowire/AlO/Ag Film Composite Structure},
  Author                   = {Wei, H. and Tian, X. and Pan, D. and Chen, L. and Jia, Z. and Xu, H.},
  Journal                  = {Nano Lett},
  Year                     = {2014},

  Abstract                 = {Plasmonics holds promise for the realization of miniaturized photonic devices and circuits in which light can be confined and controlled at the nanoscale using surface plasmon polaritons (SPPs), surface waves of collective oscillations of electrons at a metal/dielectric interface. However, realizing plasmonic applications fundamentally requires the ability to guide and transfer SPPs in different plasmonic structures. Here the generation and control of periodic collimated SPP-beams are reported in composite structures of silver nanowire on silver film with a dielectric spacer layer between them. It is revealed that the collimated beams on the silver film originate from the interference between film-SPPs generated by two SPP modes on the nanowire. The direction of the collimated beams can be readily tuned by changing the thickness of the dielectric spacer. These findings demonstrate the transfer of nanowire SPPs to film SPPs and offer a new approach to generate nondiffracting SPP-beams, which could facilitate the design and development of complex plasmonic systems for device applications and enable the tailoring of SPP radiation and SPP-matter interactions.},
  Doi                      = {10.1021/nl504018q},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25514318}
}

@Article{Wei2015,
  Title                    = {Comparative fracture toughness of multilayer graphenes and boronitrenes},
  Author                   = {Wei, X. and Xiao, S. and Li, F. and Tang, D. M. and Chen, Q. and Bando, Y. and Golberg, D.},
  Journal                  = {Nano Lett},
  Year                     = {2015},
  Number                   = {1},
  Pages                    = {689-94},
  Volume                   = {15},

  Abstract                 = {We report the comparative in situ fracture toughness testing on single-edge V/U-notched multilayer graphenes and boronitrenes in a high-resolution transmission electron microscope (HRTEM). The nanostructures of notch tips and fracture edges of the tested specimens are unambiguously resolved using HRTEM. By analyzing the notch tip stresses using finite element method, the fracture toughness of multilayer graphenes and boronitrenes is determined to be 12.0 +/- 3.9 and 5.5 +/- 0.7 MPa radicalm, respectively, taking into account the notch tip blunting effects.},
  Doi                      = {10.1021/nl5042066},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25555238}
}

@Article{Wiederhecker2009,
  Title                    = {Controlling photonic structures using optical forces},
  Author                   = {Wiederhecker, G. S. and Chen, L. and Gondarenko, A. and Lipson, M.},
  Journal                  = {Nature},
  Year                     = {2009},
  Number                   = {7273},
  Pages                    = {633-6},
  Volume                   = {462},

  Abstract                 = {The use of optical forces to manipulate small objects is well known. Applications include the manipulation of living cells by optical tweezers and optical cooling in atomic physics. The miniaturization of optical systems (to the micro and nanoscale) has resulted in very compliant systems with masses of the order of nanograms, rendering them susceptible to optical forces. Optical forces have been exploited to demonstrate chaotic quivering of microcavities, optical cooling of mechanical modes, actuation of a tapered-fibre waveguide and excitation of the mechanical modes of silicon nano-beams. Despite recent progress in this field, it is challenging to manipulate the optical response of photonic structures using optical forces; this is because of the large forces that are required to induce appreciable changes in the geometry of the structure. Here we implement a resonant structure whose optical response can be efficiently statically controlled using relatively weak attractive and repulsive optical forces. We demonstrate a static mechanical deformation of up to 20 nanometres in a silicon nitride structure, using three milliwatts of continuous optical power. Because of the sensitivity of the optical response to this deformation, such optically induced static displacement introduces resonance shifts spanning 80 times the intrinsic resonance linewidth.},
  Doi                      = {10.1038/nature08584},
  ISSN                     = {1476-4687 (Electronic)
0028-0836 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/19915549}
}

@Article{Wilson2003,
  Title                    = {Perturbing an electromagnetic induced transparency within an inhomogeneously broadened transition},
  Author                   = {Wilson, E. and Manson, N. and Wei, C.},
  Journal                  = {Physical Review A},
  Year                     = {2003},
  Number                   = {2},
  Pages                    = {023812},
  Volume                   = {67},

  Type                     = {Journal Article},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevA.67.023812}
}

@Article{Wrachtrup1993,
  Title                    = {Optical detection of magnetic resonance in a single molecule},
  Author                   = {Wrachtrup, J. and von Borczyskowski, C. and Bernard, J. and Orritt, M. and Brown, R.},
  Journal                  = {Nature},
  Year                     = {1993},
  Number                   = {6426},
  Pages                    = {244-245},
  Volume                   = {363},

  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/363244a0}
}

@Article{Wrachtrup2013,
  Title                    = {Nitrogen-vacancy centers close to surfaces},
  Author                   = {Wrachtrup, JÃ¶rg and Jelezko, Fedor and Grotz, Bernhard and McGuinness, Liam},
  Journal                  = {MRS Bulletin},
  Year                     = {2013},
  Number                   = {02},
  Pages                    = {149-154},
  Volume                   = {38},

  Doi                      = {doi:10.1557/mrs.2013.22},
  ISSN                     = {1938-1425},
  Keywords                 = {Electron spin resonance, defects, diamond, devices, sensor},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1557/mrs.2013.22}
}

@Article{Wu2004,
  Title                    = {Raman Spectroscopy and Time-Resolved Photoluminescence of BN and BxCyNz Nanotubes},
  Author                   = {Wu, J. and Han, Wei-Qiang and Walukiewicz, W. and Ager, J. W. and Shan, W. and Haller, E. E. and Zettl, A.},
  Journal                  = {Nano Letters},
  Year                     = {2004},
  Number                   = {4},
  Pages                    = {647-650},
  Volume                   = {4},

  Abstract                 = {We report Raman and time-resolved photoluminescence spectroscopic studies of multiwalled BN and BxCyNz nanotubes. The Raman spectroscopy shows that the as-grown BxCyNz nanotubes are radially phase separated into BN shells and carbon shells. The photoluminescence decay process is characterized by two time constants that are attributed to intra- and inter-BN sheet charge recombination, respectively. A comparison of the photoluminescence of BN nanotubes to that of hexagonal BN is consistent with the existence of a spatially indirect band gap in multiwalled BN nanotubes as predicted by theory.},
  Doi                      = {10.1021/nl049862e},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl049862e}
}

@Article{Wu2014,
  Title                    = {Probing subdiffraction limit separations with plasmon coupling microscopy: concepts and applications},
  Author                   = {Wu, L. and Reinhard, B. M.},
  Journal                  = {Chem Soc Rev},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {3884-97},
  Volume                   = {43},

  Abstract                 = {Due to their advantageous material properties, noble metal nanoparticles are versatile tools in biosensing and imaging. A characteristic feature of gold and silver nanoparticles is their ability to sustain localized surface plasmons that provide both large optical cross-sections and extraordinary photophysical stability. Plasmon coupling microscopy takes advantage of the beneficial optical properties and utilizes electromagnetic near-field coupling between individual noble metal nanoparticle labels to resolve subdiffraction limit separations in an all-optical fashion. This Tutorial provides an introduction into the physical concepts underlying distance dependent plasmon coupling, discusses potential experimental implementation of plasmon coupling microscopy, and reviews applications in the area of biosensing and imaging.},
  Doi                      = {10.1039/c3cs60340g},
  ISSN                     = {1460-4744 (Electronic)
0306-0012 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24390574}
}

@Article{Wu2015,
  Title                    = {Monolayer semiconductor nanocavity lasers with ultralow thresholds},
  Author                   = {Wu, Sanfeng and Buckley, Sonia and Schaibley, John R. and Feng, Liefeng and Yan, Jiaqiang and Mandrus, David G. and Hatami, Fariba and Yao, Wang and Vuckovic, Jelena and Majumdar, Arka and Xu, Xiaodong},
  Journal                  = {Nature},
  Year                     = {2015},
  Number                   = {7545},
  Pages                    = {69--72},
  Volume                   = {520},

  ISSN                     = {0028-0836},
  Owner                    = {Toan},
  Timestamp                = {2015.04.09},
  Url                      = {http://dx.doi.org/10.1038/nature14290}
}

@Article{Wurtz2011,
  Title                    = {Designed ultrafast optical nonlinearity in a plasmonic nanorod metamaterial enhanced by nonlocality},
  Author                   = {Wurtz, G. A. and Pollard, R. and Hendren, W. and Wiederrecht, G. P. and Gosztola, D. J. and Podolskiy, V. A. and Zayats, A. V.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2011},
  Number                   = {2},
  Pages                    = {107-11},
  Volume                   = {6},

  Abstract                 = {All-optical signal processing enables modulation and transmission speeds not achievable using electronics alone. However, its practical applications are limited by the inherently weak nonlinear effects that govern photon-photon interactions in conventional materials, particularly at high switching rates. Here, we show that the recently discovered nonlocal optical behaviour of plasmonic nanorod metamaterials enables an enhanced, ultrafast, nonlinear optical response. We observe a large (80%) change of transmission through a subwavelength thick slab of metamaterial subjected to a low control light fluence of 7 mJ cm(-2), with switching frequencies in the terahertz range. We show that both the response time and the nonlinearity can be engineered by appropriate design of the metamaterial nanostructure. The use of nonlocality to enhance the nonlinear optical response of metamaterials, demonstrated here in plasmonic nanorod composites, could lead to ultrafast, low-power all-optical information processing in subwavelength-scale devices.},
  Doi                      = {10.1038/nnano.2010.278},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Keywords                 = {Computer Simulation
Light
Manufactured Materials
Nanotubes/*chemistry
Nonlinear Dynamics
Scattering, Radiation
Surface Plasmon Resonance/*instrumentation/*methods},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/21258335}
}

@Article{Xia2014,
  Title                    = {Two-dimensional material nanophotonics},
  Author                   = {Xia, Fengnian and Wang, Han and Xiao, Di and Dubey, Madan and Ramasubramaniam, Ashwin},
  Journal                  = {Nature Photonics},
  Year                     = {2014},
  Number                   = {12},
  Pages                    = {899-907},
  Volume                   = {8},

  Doi                      = {10.1038/nphoton.2014.271},
  ISSN                     = {1749-4885
1749-4893},
  Type                     = {Journal Article}
}

@Article{Xie1994,
  Title                    = {Probing Single Molecule Dynamics},
  Author                   = {Xie, X. Sunney and Dunn, Robert C.},
  Journal                  = {Science},
  Year                     = {1994},
  Number                   = {5170},
  Pages                    = {361-364},
  Volume                   = {265},

  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/265/5170/361.abstractN2 - The room temperature dynamics of single sulforhodamine 101 molecules dispersed on a glass surface are investigated on two different time scales with near-field optics. On the 10-2- to 102-second time scale, intensity fluctuations in the emission from single molecules are examined with polarization measurements, providing insight into their spectroscopic properties. On the nanosecond time scale, the fluorescence lifetimes of single molecules are measured, and their excited-state energy transfer to the aluminum coating of the near-field probe is characterized. A movie of the time-resolved emission demonstrates the feasibility of fluorescence lifetime imaging with single molecule sensitivity, picosecond temporal resolution, and a spatial resolving power beyond the diffraction limit.}
}

@Article{Xing2013,
  Title                    = {Essential Differences of Organic Films at the Molecular Level via Vacuum Deposition and Solution Processes for Organic Light-Emitting Diodes},
  Author                   = {Xing, Xing and Zhong, Luwei and Zhang, Lipei and Chen, Zhijian and Qu, Bo and Chen, Erqiang and Xiao, Lixin and Gong, Qihuang},
  Journal                  = {The Journal of Physical Chemistry C},
  Year                     = {2013},
  Number                   = {48},
  Pages                    = {25405-25408},
  Volume                   = {117},

  Doi                      = {10.1021/jp410547w},
  ISSN                     = {1932-7447
1932-7455},
  Type                     = {Journal Article}
}

@Article{Xu2014,
  Title                    = {Surface-Plasmon-Mediated Programmable Optical Nanofabrication of an Oriented Silver Nanoplate},
  Author                   = {Xu, Bin-Bin and Wang, Lei and Ma, Zhuo-Chen and Zhang, Ran and Chen, Qi-Dai and Lv, Chao and Han, Bing and Xiao, Xin-Ze and Zhang, Xu-Lin and Zhang, Yong-Lai and Ueno, Kosei and Misawa, Hiroaki and Sun, Hong-Bo},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {7},
  Pages                    = {6682-6692},
  Volume                   = {8},

  Doi                      = {10.1021/nn5029345},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn5029345}
}

@Article{Xu2013a,
  Title                    = {Graphene-Like Two-Dimensional Materials},
  Author                   = {Xu, Mingsheng and Liang, Tao and Shi, Minmin and Chen, Hongzheng},
  Journal                  = {Chemical Reviews},
  Year                     = {2013},
  Number                   = {5},
  Pages                    = {3766-3798},
  Volume                   = {113},

  Owner                    = {Toan},
  Timestamp                = {2015.04.08}
}

@Article{Xu2013,
  Title                    = {Synthesis and optical properties of cadmium selenide quantum dots for white light-emitting diode application},
  Author                   = {Xu, Xianmei and Wang, Yilin and Gule, Teri and Luo, Qiang and Zhou, Liya and Gong, Fuzhong},
  Journal                  = {Materials Research Bulletin},
  Year                     = {2013},
  Number                   = {3},
  Pages                    = {983-987},
  Volume                   = {48},

  Doi                      = {10.1016/j.materresbull.2012.11.093},
  ISSN                     = {00255408},
  Type                     = {Journal Article}
}

@Article{Xu2014a,
  Title                    = {One-dimensional surface phonon polaritons in boron nitride nanotubes},
  Author                   = {Xu, Xiaoji G. and Ghamsari, Behnood G. and Jiang, Jian-Hua and Gilburd, Leonid and Andreev, Gregory O. and Zhi, Chunyi and Bando, Yoshio and Golberg, Dmitri and Berini, Pierre and Walker, Gilbert C.},
  Journal                  = {Nat. Commun.},
  Year                     = {2014},
  Pages                    = {4782--},
  Volume                   = {5},

  Abstract                 = {Surface polaritons, which are electromagnetic waves coupled to material charge oscillations, have enabled applications in concentrating, guiding and harvesting optical energy below the diffraction limit. Surface plasmon polaritons involve oscillations of electrons and are accessible in noble metals at visible and near-infrared wavelengths, whereas surface phonon polaritons (SPhPs) rely on phonon resonances in polar materials, and are active in the mid-infrared. Noble metal surface plasmon polaritons have limited applications in the mid-infrared. SPhPs at flat interfaces normally possess long polariton wavelengths and provide modest field confinement/enhancement. Here we demonstrate propagating SPhPs in a one-dimensional material consisting of a boron nitride nanotube at mid-infrared wavelengths. The observed SPhP exhibits high field confinement and enhancement, and a very high effective index (neff~70). We show that the modal and propagation length characteristics of the SPhPs may be controlled through the nanotube size and the supporting substrates, enabling mid-infrared applications.},
  Comment                  = {Supplementary information available for this article at http://www.nature.com/ncomms/2014/140826/ncomms5782/suppinfo/ncomms5782_S1.html},
  Owner                    = {Toan},
  Timestamp                = {2015.04.09},
  Url                      = {http://dx.doi.org/10.1038/ncomms5782}
}

@Article{Yan2012,
  Title                    = {Optical modulation based on direct photon-plasmon coupling in organic/metal nanowire heterojunctions},
  Author                   = {Yan, Y. and Zhang, C. and Zheng, J. Y. and Yao, J. and Zhao, Y. S.},
  Journal                  = {Adv Mater},
  Year                     = {2012},
  Number                   = {42},
  Pages                    = {5681-6},
  Volume                   = {24},

  Abstract                 = {Surface plasmon polaritons (SPPs) can be launched with an organic nanowire that serves as both light source and dielectric waveguide in a single organic/metal nanowire heterojunction. Efficient modulation of the output signals from the silver tip can be achieved via the alternation of incident polarizations, which is further used to design and realize prototypical photonic-plasmonic logic devices. These findings are essential for incorporating plasmonic waveguides as practical components into hybrid high-capacity photonic circuits.},
  Doi                      = {10.1002/adma.201202698},
  ISSN                     = {1521-4095 (Electronic)
0935-9648 (Linking)},
  Keywords                 = {Anthracenes/chemistry
Metals/*chemistry
Nanowires/*chemistry
Organic Chemicals/*chemistry
Photons
Surface Plasmon Resonance},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22907883}
}

@Article{Yang2005,
  Title                    = {Wet synthesis of nearly monodisperse CdSe nanoparticles at room temperature},
  Author                   = {Yang, Yu Jun and Xiang, Bao Jian},
  Journal                  = {Journal of Crystal Growth},
  Year                     = {2005},
  Number                   = {3â€“4},
  Pages                    = {453-458},
  Volume                   = {284},

  Abstract                 = {A facile aqueous route to synthesize CdSe nanoparticles at room temperature has been developed. With poly(vinylpyrrolidone) (PVP) as capping agent, nearly monodisperse CdSe nanoparticles were prepared by 10 min of reaction between CdCl2 and Na2SeSO3 in the presence of thioglycerol. Thioglycerol (TG) was found to not only act as the complexant but also to effectively catalyze the reaction between CdCl2 and Na2SeSO3. The product was characterized with UVâ€“vis absorption spectroscopy, photoluminescence spectroscopy, powder X-ray diffraction and transmission electron microscopy.},
  Doi                      = {http://dx.doi.org/10.1016/j.jcrysgro.2005.07.038},
  ISSN                     = {0022-0248},
  Keywords                 = {A1. Characterization
A1. Crystal morphology
A2. Growth from solutions
B1. Nanomaterials
B2. Semiconducting IIâ€“VI materials},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0022024805009097}
}

@Article{Yao2012,
  Title                    = {Scalable architecture for a room temperature solid-state quantum information processor},
  Author                   = {Yao, N. Y. and Jiang, L. and Gorshkov, A. V. and Maurer, P. C. and Giedke, G. and Cirac, J. I. and Lukin, M. D.},
  Journal                  = {Nat Commun},
  Year                     = {2012},
  Pages                    = {800},
  Volume                   = {3},

  Abstract                 = {The realization of a scalable quantum information processor has emerged over the past decade as one of the central challenges at the interface of fundamental science and engineering. Here we propose and analyse an architecture for a scalable, solid-state quantum information processor capable of operating at room temperature. Our approach is based on recent experimental advances involving nitrogen-vacancy colour centres in diamond. In particular, we demonstrate that the multiple challenges associated with operation at ambient temperature, individual addressing at the nanoscale, strong qubit coupling, robustness against disorder and low decoherence rates can be simultaneously achieved under realistic, experimentally relevant conditions. The architecture uses a novel approach to quantum information transfer and includes a hierarchy of control at successive length scales. Moreover, it alleviates the stringent constraints currently limiting the realization of scalable quantum processors and will provide fundamental insights into the physics of non-equilibrium many-body quantum systems.},
  Doi                      = {10.1038/ncomms1788},
  ISSN                     = {2041-1723 (Electronic)
2041-1723 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22531185}
}

@Article{Yao2012a,
  Title                    = {Large-scale production of two-dimensional nanosheets},
  Author                   = {Yao, Yagang and Lin, Ziyin and Li, Zhuo and Song, Xiaojuan and Moon, Kyoung-Sik and Wong, Ching-ping},
  Journal                  = {Journal of Materials Chemistry},
  Year                     = {2012},
  Number                   = {27},
  Pages                    = {13494},
  Volume                   = {22},

  Doi                      = {10.1039/c2jm30587a},
  ISSN                     = {0959-9428
1364-5501},
  Type                     = {Journal Article}
}

@Article{Yin2003,
  Title                    = {Novel Route to Cubic Boron Nitride Dendritic Nanostructures under Electron Beam Irradiation},
  Author                   = {Yin, L. W. and Li, M. S. and Liu, Y. X. and Xu, B. and Sui, J. L. and Qi, Y. X.},
  Journal                  = {Advanced Materials},
  Year                     = {2003},
  Number                   = {9},
  Pages                    = {720-723},
  Volume                   = {15},

  Doi                      = {10.1002/adma.200304674},
  ISSN                     = {1521-4095},
  Keywords                 = {Boron nitride
Dendrites
Electron beam irradiation
Nanostructures},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1002/adma.200304674}
}

@Article{Yoo2013,
  Title                    = {Metal-lined semiconductor nanotubes for surface plasmon-mediated luminescence enhancement},
  Author                   = {Yoo, J. and Ma, X. and Tang, W. and Yi, G. C.},
  Journal                  = {Nano Lett},
  Year                     = {2013},
  Number                   = {5},
  Pages                    = {2134-40},
  Volume                   = {13},

  Abstract                 = {Highly efficient solid-state light-emitting devices require semiconductor architectures equipped with high quantum efficiency and integratability on conductive substrates. Surface plasmon (SP)-mediated luminescence enhancement has been considered as one of the most promising solutions, because SP resonance can greatly improve the radiative recombination rate and be achieved using metal entities compatible with the electrode fabrication process. Nevertheless, metal/semiconductor heterostructures have had several fabrication-compatible issues due to metal as a potential contaminant of the semiconductor. We present here a simple fabrication scheme for a metal-lined semiconductor nanotube heterostructure, in which a metal layer is selectively formed on the inner wall of the semiconductor nanotube. The Ag-lining process in a ZnO nanotube resulted in 7.5-fold enhancement of the photoluminescence intensity at 11 K. This SP fabrication technique looks promising for highly efficient solid-state lighting based on semiconductor nanostructures without detrimental effects.},
  Doi                      = {10.1021/nl400547z},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23573911}
}

@Article{Yu2006,
  Title                    = {Morphology dependence of cathodoluminescence from cubic boron nitride films deposited by chemical vapor deposition},
  Author                   = {Yu, J. and Ong, H. C. and Wong, K. Y. and Lau, W. M. and Matsumoto, S.},
  Journal                  = {Journal of Applied Physics},
  Year                     = {2006},
  Number                   = {12},
  Pages                    = {124915},
  Volume                   = {99},

  Doi                      = {doi:http://dx.doi.org/10.1063/1.2205356},
  Keywords                 = {cathodoluminescence
semiconductor thin films
chemical vapour deposition
III-V semiconductors
Raman spectra
wide band gap semiconductors
chemical analysis
surface structure
boron compounds
semiconductor growth},
  Type                     = {Journal Article},
  Url                      = {http://scitation.aip.org/content/aip/journal/jap/99/12/10.1063/1.2205356}
}

@Article{Yu2006a,
  Title                    = {Thermal Stability of Cubic Boron Nitride Films Deposited by Chemical Vapor Deposition},
  Author                   = {Yu, J. and Zheng, Z. and Ong, H. C. and Wong, K. Y. and Matsumoto, S. and Lau, W. M.},
  Journal                  = {The Journal of Physical Chemistry B},
  Year                     = {2006},
  Number                   = {42},
  Pages                    = {21073-21076},
  Volume                   = {110},

  Abstract                 = {Thermal stability of well-crystallized cubic boron nitride (cBN) films grown by chemical vapor deposition has been investigated by cathodoluminescence (CL), Raman spectroscopy, and scanning electron microscopy (SEM) with the cBN films annealed at various temperatures up to 1300 Â°C. The crystallinity of the cBN films further improves, as indicated by a reduction of the relevant Raman line width, when the annealing temperature exceeds 1100 Â°C. Structural damage or amorphization was observed on the grain boundaries of the cBN crystals when annealing temperature reaches 1300 Â°C. The CL spectra are found to be unchanged up to 1100 Â°C after annealing at 500 Â°C, showing the stability of the cBN films in electronic properties up to this temperature. New features were observed in the CL spectra when annealing temperature reaches 1200?1300 Â°C.},
  Doi                      = {10.1021/jp0610766},
  ISSN                     = {1520-6106},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/jp0610766}
}

@Article{Yu2014,
  Title                    = {Hot-electron-transfer enhancement for the efficient energy conversion of visible light},
  Author                   = {Yu, S. and Kim, Y. H. and Lee, S. Y. and Song, H. D. and Yi, J.},
  Journal                  = {Angew Chem Int Ed Engl},
  Year                     = {2014},
  Number                   = {42},
  Pages                    = {11203-7},
  Volume                   = {53},

  Abstract                 = {Great strides have been made in enhancing solar energy conversion by utilizing plasmonic nanostructures in semiconductors. However, current generation with plasmonic nanostructures is still somewhat inefficient owing to the ultrafast decay of plasmon-induced hot electrons. It is now shown that the ultrafast decay of hot electrons across Au nanoparticles can be significantly reduced by strong coupling with CdS quantum dots and by a Schottky junction with perovskite SrTiO3 nanoparticles. The designed plasmonic nanostructure with three distinct components enables a hot-electron-assisted energy cascade for electron transfer, CdS-->Au-->SrTiO3, as demonstrated by steady-state and time-resolved photoluminescence spectroscopy. Consequently, hot-electron transfer enabled the efficient production of H2 from water as well as significant electron harvesting under irradiation with visible light of various wavelengths. These findings provide a new approach for overcoming the low efficiency that is typically associated with plasmonic nanostructures.},
  Doi                      = {10.1002/anie.201405598},
  ISSN                     = {1521-3773 (Electronic)
1433-7851 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25169852}
}

@Article{Yu2005,
  Title                    = {Bright Fluorescent Nanodiamonds:â€‰ No Photobleaching and Low Cytotoxicity},
  Author                   = {Yu, Shu-Jung and Kang, Ming-Wei and Chang, Huan-Cheng and Chen, Kuan-Ming and Yu, Yueh-Chung},
  Journal                  = {Journal of the American Chemical Society},
  Year                     = {2005},
  Number                   = {50},
  Pages                    = {17604-17605},
  Volume                   = {127},

  Doi                      = {10.1021/ja0567081},
  ISSN                     = {0002-7863},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/ja0567081}
}

@Article{Yuan2002,
  Title                    = {Electrically Driven Single-Photon Source},
  Author                   = {Yuan, Zhiliang and Kardynal, Beata E. and Stevenson, R. Mark and Shields, Andrew J. and Lobo, Charlene J. and Cooper, Ken and Beattie, Neil S. and Ritchie, David A. and Pepper, Michael},
  Journal                  = {Science},
  Year                     = {2002},
  Number                   = {5552},
  Pages                    = {102-105},
  Volume                   = {295},

  Abstract                 = {Electroluminescence from a single quantum dot within the intrinsic region of a p-i-n junction is shown to act as an electrically driven single-photon source. At low injection currents, the dot electroluminescence spectrum reveals a single sharp line due to exciton recombination, while another line due to the biexciton emerges at higher currents. The second-order correlation function of the diode displays anti-bunching under a continuous drive current. Single-photon emission is stimulated by subnanosecond voltage pulses. These results suggest that semiconductor technology can be used to mass-produce a single-photon source for applications in quantum information technology.},
  Doi                      = {10.1126/science.1066790},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencemag.org/content/295/5552/102.abstract}
}

@Article{Zachreson2014,
  Title                    = {Electron beam controlled restructuring of luminescence centers in polycrystalline diamond},
  Author                   = {Zachreson, C. and Martin, A. A. and Aharonovich, I. and Toth, M.},
  Journal                  = {ACS Appl Mater Interfaces},
  Year                     = {2014},
  Number                   = {13},
  Pages                    = {10367-72},
  Volume                   = {6},

  Abstract                 = {Color centers in diamond are becoming prime candidates for applications in photonics and sensing. In this work we study the time evolution of cathodoluminescence (CL) emissions from color centers in a polycrystalline diamond film under electron irradiation. We demonstrate room-temperature activation of several luminescence centers through a thermal mechanism that is catalyzed by an electron beam. CL activation kinetics were measured in realtime and are discussed in the context of electron induced dehydrogenation of nitrogen-vacancy-hydrogen clusters and dislocation defects. Our results also show that (unintentional) electron beam induced chemical etching can take place during CL analysis of diamond. The etching is caused by residual H2O molecules present in high vacuum CL systems.},
  Doi                      = {10.1021/am501865t},
  ISSN                     = {1944-8252 (Electronic)
1944-8244 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24932526}
}

@Article{Zayats2003,
  Title                    = {Near-field photonics: surface plasmon polaritons and localized surface plasmons},
  Author                   = {Zayats, A. V. and Smolyaninov, II},
  Journal                  = {Journal of Optics a-Pure and Applied Optics},
  Year                     = {2003},
  Number                   = {4},
  Pages                    = {S16-S50},
  Volume                   = {5},

  Abstract                 = {Surface plasmon polaritons and localized surface plasmons are discussed in the context of photonic applications. Near-field imaging of scattering, reflection, interference and localization of surface polaritons is reviewed, and approaches for the implementation of elements of surface polariton optics are presented. Surface plasmon polaritonic crystals and their role in the determination of optical properties of periodically nanostructured metal films are described. Non-linear effects related to surface polaritons and localized surface plasmons allowing control of optical properties of nanostructured metal films with light are discussed. Surface plasmon optics opens up numerous possibilities for application of these intrinsically two-dimensional excitations in passive and active devices of all-optical integrated circuits.},
  Doi                      = {10.1088/1464-4258/5/4/353},
  ISSN                     = {1464-4258},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000184571900026}
}

@Article{Zeng2012,
  Title                    = {Valley polarization in MoS2 monolayers by optical pumping},
  Author                   = {Zeng, Hualing and Dai, Junfeng and Yao, Wang and Xiao, Di and Cui, Xiaodong},
  Journal                  = {Nat. Nanotechnol.},
  Year                     = {2012},
  Number                   = {8},
  Pages                    = {490-493},
  Volume                   = {7},

  Doi                      = {http://www.nature.com/nnano/journal/v7/n8/abs/nnano.2012.95.html},
  ISSN                     = {1748-3387},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1038/nnano.2012.95}
}

@Article{Zeng2012a,
  Title                    = {Electronic structures and transport properties of fluorinated boron nitride nanoribbons},
  Author                   = {Zeng, J. and Chen, K. Q. and Sun, C. Q.},
  Journal                  = {Phys Chem Chem Phys},
  Year                     = {2012},
  Number                   = {22},
  Pages                    = {8032-7},
  Volume                   = {14},

  Abstract                 = {By applying the nonequilibrium Green's functions and the density-functional theory, we investigate the electronic structures and transport properties of fluorinated zigzag-edged boron nitride nanoribbons. The results show that the transition between half-metal and semiconductor in zigzag-edged boron nitride nanoribbons can be realized by fluorination at different sites or by the change of the fluorination level. Moreover, the negative differential resistance and varistor-type behaviors can also be observed in such fluorinated zigzag-edged boron nitride nanoribbon devices. Therefore, the fluorination of zigzag-edged boron nitride nanoribbons will provide the possibilities for a multifunctional molecular device design.},
  Doi                      = {10.1039/c2cp23937j},
  ISSN                     = {1463-9084 (Electronic)
1463-9076 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/22555657}
}

@Article{Zeng2011,
  Title                    = {Single-Layer Semiconducting Nanosheets: High-Yield Preparation and Device Fabrication},
  Author                   = {Zeng, Zhiyuan and Yin, Zongyou and Huang, Xiao and Li, Hai and He, Qiyuan and Lu, Gang and Boey, Freddy and Zhang, Hua},
  Journal                  = {Angew. Chem. Int. Ed.},
  Year                     = {2011},
  Number                   = {47},
  Pages                    = {11093--11097},
  Volume                   = {50},

  Doi                      = {10.1002/anie.201106004},
  Oi                       = {Lu, Gang/0000-0003-1722-0176; Li, Hai/0000-0002-9659-1153; He,EOLEOLQiyuan/0000-0001-9083-8285},
  Owner                    = {Toan},
  Pm                       = {22021163},
  Ri                       = {Zhang, Hua/A-1302-2009; Lu, Gang/A-1893-2011; Yin, Zongyou/A-2383-2012; Li, Hai/E-7555-2011; Huang, Xiao/B-7720-2014; He, Qiyuan/J-1505-2014},
  Sn                       = {1433-7851},
  Tc                       = {266},
  Timestamp                = {2015.04.09},
  Ut                       = {WOS:000297467100007},
  Z8                       = {7},
  Z9                       = {267},
  Zb                       = {25},
  Zs                       = {0}
}

@Article{Zhang2014,
  Title                    = {Silicon-vacancy color centers in nanodiamonds: cathodoluminescence imaging markers in the near infrared},
  Author                   = {Zhang, H. and Aharonovich, I. and Glenn, D. R. and Schalek, R. and Magyar, A. P. and Lichtman, J. W. and Hu, E. L. and Walsworth, R. L.},
  Journal                  = {Small},
  Year                     = {2014},
  Number                   = {10},
  Pages                    = {1908-13},
  Volume                   = {10},

  Doi                      = {10.1002/smll.201303582},
  ISSN                     = {1613-6829 (Electronic)
1613-6810 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/24596272}
}

@Article{Zhang2011,
  Title                    = {Photonic crystal disk lasers},
  Author                   = {Zhang, Yinan and Hamsen, Christoph and Choy, Jennifer T. and Huang, Yong and Ryou, Jae-Hyun and Dupuis, Russell D. and Loncar, Marko},
  Journal                  = {Optics Letters},
  Year                     = {2011},
  Number                   = {14},
  Pages                    = {2704-2706},
  Volume                   = {36},

  Abstract                 = {A novel type of nanolasers, which combines the advantages of photonic crystal lasers and microdisk lasers, has been demonstrated based on InAlGaAs/InGaAs quantum wells using pulsed optical pumping at room temperature. It incorporates the properties of small footprint, small mode volume, and submilliwatt threshold, and favors vertical emission. We believe that this type of laser acts as a promising candidate for highly-integrated on-chip nanolasers in applications for signal processing and index sensing. (C) 2011 Optical Society of America},
  ISSN                     = {0146-9592},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000293347000035}
}

@Article{Zhang2014a,
  Title                    = {Dendritic, Transferable, Strictly Monolayer MoS2 Flakes Synthesized on SrTiO3 Single Crystals for Efficient Electrocatalytic Applications},
  Author                   = {Zhang, Yu and Ji, Qingqing and Han, Gao-Feng and Ju, Jing and Shi, Jianping and Ma, Donglin and Sun, Jingyu and Zhang, Yanshuo and Li, Minjie and Lang, Xing-You and Zhang, Yanfeng and Liu, Zhongfan},
  Journal                  = {ACS Nano},
  Year                     = {2014},
  Number                   = {8},
  Pages                    = {8617-8624},
  Volume                   = {8},

  Abstract                 = {Controllable synthesis of macroscopically uniform, high-quality monolayer MoS2 is crucial for harnessing its great potential in optoelectronics, electrocatalysis, and energy storage. To date, triangular MoS2 single crystals or their polycrystalline aggregates have been synthesized on insulating substrates of SiO2/Si, mica, sapphire, etc., via portable chemical vapor deposition methods. Herein, we report a controllable synthesis of dendritic, strictly monolayer MoS2 flakes possessing tunable degrees of fractal shape on a specific insulator, SrTiO3. Interestingly, the dendritic monolayer MoS2, characterized by abundant edges, can be transferred intact onto Au foil electrodes and serve as ideal electrocatalysts for hydrogen evolution reaction, reflected by a rather low Tafel slope of ?73 mV/decade among CVD-grown two-dimensional MoS2 flakes. In addition, we reveal that centimeter-scale uniform, strictly monolayer MoS2 films consisting of relatively compact domains can also be obtained, offering insights into promising applications such as flexible energy conversion/harvesting and optoelectronics.},
  Doi                      = {10.1021/nn503412w},
  ISSN                     = {1936-0851},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nn503412w}
}

@Article{Zhang2014b,
  Title                    = {Plasmonic hybridization induced trapping and manipulation of a single Au nanowire on a metallic surface},
  Author                   = {Zhang, Y. and Wang, J. and Shen, J. and Man, Z. and Shi, W. and Min, C. and Yuan, G. and Zhu, S. and Urbach, H. P. and Yuan, X.},
  Journal                  = {Nano Lett},
  Year                     = {2014},
  Number                   = {11},
  Pages                    = {6430-6},
  Volume                   = {14},

  Abstract                 = {Hybridization in the narrow gaps between the surface plasmon polaritons (SPPs) along a metal surface and the localized surface plasmons on metallic nano-objects strongly enhance the electromagnetic field. Here, we employ plasmonic hybridization to achieve dynamic trapping and manipulation of a single metallic nanowire on a flat metal surface. We reveal that the plasmonic hybridization achieved by exciting plasmonic tweezers with a linearly polarized laser beam could induce strong trapping forces and large rotational torques on a single metallic nanowire. The position and orientation of the nanowire could dynamically be controlled by the hybridization-enhanced nonisotropic electric field in the gap. Experimental results further verify that a single Au nanowire could robustly be trapped at the center of an excited SPP field by the induced forces and then rotated by the torques. Finally, a plasmonic swallow tail structure is built to demonstrate its potential in the fabrication of lab-on-a-chip plasmonic devices.},
  Doi                      = {10.1021/nl502975k},
  ISSN                     = {1530-6992 (Electronic)
1530-6984 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/25302534}
}

@Article{Zhang2014c,
  Title                    = {Spintronic and electronic properties of a positively charged NBVN center in hexagonal boron nitride monolayer},
  Author                   = {Zhang, Y. G. and Cheng, G. D. and Peng, W. and Tang, Z.},
  Journal                  = {Computational Materials Science},
  Year                     = {2014},
  Pages                    = {316-319},
  Volume                   = {95},

  Doi                      = {10.1016/j.commatsci.2014.08.003},
  ISSN                     = {09270256},
  Type                     = {Journal Article}
}

@Article{Zhang2011a,
  Title                    = {Fluorinating hexagonal boron nitride into diamond-like nanofilms with tunable band gap and ferromagnetism},
  Author                   = {Zhang, Z. and Zeng, X. C. and Guo, W.},
  Journal                  = {J Am Chem Soc},
  Year                     = {2011},
  Number                   = {37},
  Pages                    = {14831-8},
  Volume                   = {133},

  Abstract                 = {Cubic boron nitride (c-BN) possesses a number of extreme properties rivaling or surpassing those of diamond. Especially, owing to the high chemical stability, c-BN is desired for fabricating electronic devices that can stand up to harsh environments. However, realization of c-BN-based functional devices is still a challenging task due largely to the subtlety in the preparation of high-quality c-BN films with uniform thickness and controllable properties. Here, we present a simple synthetic strategy by surface fluorination of few-layered hexagonal boron nitride (h-BN) sheets to produce thermodynamically favorable F-terminated c-BN nanofilms with an embedded N-N bond layer and strong inbuilt electric polarization. Due to these specific features, the fluorinated c-BN nanofilms have controllable band gap by thickness or inbuilt and applied electric fields. Especially, the produced nanofilms can be tuned into substantial ferromagnetism through electron doping within a reasonable level. The electron-doping-induced deformation ratio of the c-BN nanofilms is found to be 1 order of magnitude higher than those of carbon nanotubes and graphene. At sufficient high doping levels, the nanofilm can be cleaved peculiarly along the N-N bond layer into diamond-like BN films. As the proposed synthesis strategy of the fluorinated c-BN nanofilms is well within the reach of current technologies, our results represent an extremely cost-effective approach for producing high-quality c-BN nanofilms with tunable electronic, magnetic, and electromechanical properties for versatile applications.},
  Doi                      = {10.1021/ja206703x},
  ISSN                     = {1520-5126 (Electronic)
0002-7863 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/21834534}
}

@Article{Zhang2011b,
  Title                    = {Fluorinating Hexagonal Boron Nitride/Graphene Multilayers into Hybrid Diamondlike Nanofilms with Tunable Energy Gap},
  Author                   = {Zhang, Zhuhua and Zeng, Xiao Cheng and Guo, Wanlin},
  Journal                  = {The Journal of Physical Chemistry C},
  Year                     = {2011},
  Number                   = {44},
  Pages                    = {21678-21684},
  Volume                   = {115},

  Doi                      = {10.1021/jp207175u},
  ISSN                     = {1932-7447
1932-7455},
  Type                     = {Journal Article}
}

@Article{Zhao2015,
  Title                    = {Electrically driven plasmon mediated energy transfer between ZnO microwires and Au nanoparticles},
  Author                   = {Zhao, Bin and Jiang, Ming-Ming and Zhao, Dong-Xu and Li, Yang and Wang, Fei and Shen, De-Zhen},
  Journal                  = {Nanoscale},
  Year                     = {2015},
  Number                   = {3},
  Pages                    = {1081-1089},
  Volume                   = {7},

  Abstract                 = {Electrically driven energy transfer between the surface defect states of ZnO quadrilateral microwires (MWs) and localized surface plasmon polaritons has been realized by means of introducing Au nanoparticles (NPs). An electroluminescence device with green emission using ZnO quadrilateral MWs, was fabricated. Once the Au NPs are sputtered on the surfaces of the ZnO MWs, the electroluminescence of the ZnO MWs will shift from green to red. Meanwhile, dual emissions were observed by means of sputtering Au NPs on a single ZnO MW periodically. Due to the Au NPs, electrically driven plasmon mediated energy transfer can achieve the modulation of amplifying, or quenching the surface defect emission. The relevant dynamic process of the surface plasmon mode mediated energy transfer was investigated. This new energy transfer method potentially offers an approach of modification and recombination of the surface defect state excitations of wide bandgap semiconductor materials.},
  Doi                      = {10.1039/C4NR05369A},
  ISSN                     = {2040-3364},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1039/C4NR05369A}
}

@Article{Zhao2006,
  Title                    = {Efficient CdSe/CdS Quantum Dot Light-Emitting Diodes Using a Thermally Polymerized Hole Transport Layer},
  Author                   = {Zhao, Jialong and Bardecker, Julie A. and Munro, Andrea M. and Liu, Michelle S. and Niu, Yuhua and Ding, I. Kang and Luo, Jingdong and Chen, Baoquan and Jen, Alex K. Y. and Ginger, David S.},
  Journal                  = {Nano Letters},
  Year                     = {2006},
  Number                   = {3},
  Pages                    = {463-467},
  Volume                   = {6},

  Abstract                 = {We report multilayer nanocrystal quantum dot light-emitting diodes (QD-LEDs) fabricated by spin-coating a monolayer of colloidal CdSe/CdS nanocrystals on top of thermally polymerized solvent-resistant hole-transport layers (HTLs). We obtain high-quality QD layers of controlled thickness (down to submonolayer) simply by spin-coating QD solutions directly onto the HTL. The resulting QD-LEDs exhibit narrow (?30 nm, fwhm) electroluminescence from the QDs with virtually no emission from the organic matrix at any voltage. Using multiple spin-on HTLs improves the external quantum efficiency of the QD-LEDs to ?0.8% at a brightness of 100 cd/m2 (with a maximum brightness over 1000 cd/m2). We conclude that QD-LEDs could be made more efficient by further optimization of the organic semiconductors.},
  Doi                      = {10.1021/nl052417e},
  ISSN                     = {1530-6984},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/nl052417e}
}

@Article{Zhao2008,
  Title                    = {Facile preparation of low cytotoxicity fluorescent carbon nanocrystals by electrooxidation of graphite},
  Author                   = {Zhao, Q. L. and Zhang, Z. L. and Huang, B. H. and Peng, J. and Zhang, M. and Pang, D. W.},
  Journal                  = {Chem Commun (Camb)},
  Year                     = {2008},
  Number                   = {41},
  Pages                    = {5116-8},

  Abstract                 = {A simple and facile method was developed to prepare fluorescent carbon nanocrystals (CNCs) with low cytotoxicity and no photobleaching, by electrooxidation of graphite in aqueous solution.},
  Doi                      = {10.1039/b812420e},
  ISSN                     = {1359-7345 (Print)
1359-7345 (Linking)},
  Keywords                 = {Animals
Cell Line
Cell Survival/drug effects
Dogs
Electrochemistry
Fluorescent Dyes/*chemical synthesis/*toxicity
Graphite/*chemistry
Hydrogen-Ion Concentration
Nanoparticles/*chemistry/*toxicity
Oxidation-Reduction
Solutions
Spectrophotometry, Ultraviolet},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/18956040}
}

@Article{Zheng2009,
  Title                    = {Electrochemiluminescence of Water-Soluble Carbon Nanocrystals Released Electrochemically from Graphite},
  Author                   = {Zheng, Liyan and Chi, Yuwu and Dong, Yongqing and Lin, Jianpeng and Wang, Binbin},
  Journal                  = {Journal of the American Chemical Society},
  Year                     = {2009},
  Number                   = {13},
  Pages                    = {4564-4565},
  Volume                   = {131},

  Doi                      = {10.1021/ja809073f},
  ISSN                     = {0002-7863},
  Type                     = {Journal Article},
  Url                      = {http://dx.doi.org/10.1021/ja809073f}
}

@Article{Zhigadlo2014,
  Title                    = {Crystal growth of hexagonal boron nitride (hBN) from Mg-B-N solvent system under high pressure},
  Author                   = {Zhigadlo, N. D.},
  Journal                  = {Journal of Crystal Growth},
  Year                     = {2014},
  Pages                    = {308-311},
  Volume                   = {402},

  Abstract                 = {Transparent and colorless hexagonal boron nitride (hBN) single crystals were grown from the Mg-B-N system using high-pressure-high-temperature cubic anvil technique. By varying the synthesis conditions we could determine the sequence of phase transformations occurring in the Mg-B-N system, construct the pressure-temperature (P-T) phase diagram and discuss the possible growth mechanism. The largest plate-like-shaped hBN crystals with sizes up to 25 mm in length and up to 10 pm in thickness were grown at 30 kbar and 1900-2100 degrees C. The hBN crystals exhibited strong, narrow diffraction peaks typical of wellordered stacking crystal planes, with the c-axis perpendicular to the crystal face. A characteristic Raman peak observed at 1367 cm with a full width at half maximum o18 cm(-1) corresponds to the E-2g vibration mode and indicates the high purity and order of hBN crystals grown by this method. From the practical point of view this work can stimulate further explorations of the Mg-B-N solvent system to obtain isotopically-enriched h(10)BN crystals, which can act as a key element in solid-state neutron detector devices. (C) 2014 Elsevier B.V. All rights reserved},
  Doi                      = {10.1016/j.jcrysgro.2014.06.038},
  ISSN                     = {0022-0248},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000340002400049}
}

@Article{Zhong2014,
  Title                    = {A facile route to high-purity BN nanoplates with ultraviolet cathodoluminescence emissions at room temperature},
  Author                   = {Zhong, Bo and Zhao, Guoliang and Huang, Xiaoxiao and Zhang, Xiaodong and Chen, Jingwei and Ren, Hangjuan and Wen, Guangwu},
  Journal                  = {Materials Research Bulletin},
  Year                     = {2014},
  Number                   = {0},
  Pages                    = {190-195},
  Volume                   = {53},

  Abstract                 = {We present a novel and notably simple approach to fabricate BN nanoplates in large scale employing ammonia borane as a single-source precursor. The structure and chemical composition of the as-synthesized products are extensively characterized by X-ray diffraction (XRD), scanning electron microscopy (SEM), high-resolution transmission electron microscopy (HRTEM) and electron energy-loss spectroscopy (EELS). XRD analysis indicates that the products are hexagonal BN crystal. SEM images confirm that the BN nanoplates have an average diameter of about 200 nm and thickness of tens of nanometers. HRTEM results illustrate the BN nanoplates to be single-crystals. EELS result suggests the nanoplates are composed of boron and nitride elements. The formation mechanism of the BN nanoplates has been elucidated based on our experimental observations, and a growth model has been proposed accordingly. Cathodoluminescence spectroscopic analysis is performed and strong ultraviolet (UV) emissions are detected. Our method provides a simple route towards the large-scale fabrication of high-quality BN nanoplates, for which various promising applications such as compact UV emitters can be envisioned.},
  Doi                      = {http://dx.doi.org/10.1016/j.materresbull.2014.02.016},
  ISSN                     = {0025-5408},
  Keywords                 = {Boron nitride nanoplates
Ammonia borane
Growth mechanism
Cathodoluminescence performance},
  Type                     = {Journal Article},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0025540814000968}
}

@Article{Zhou2013,
  Title                    = {Lasing action in strongly coupled plasmonic nanocavity arrays},
  Author                   = {Zhou, W. and Dridi, M. and Suh, J. Y. and Kim, C. H. and Co, D. T. and Wasielewski, M. R. and Schatz, G. C. and Odom, T. W.},
  Journal                  = {Nat Nanotechnol},
  Year                     = {2013},
  Number                   = {7},
  Pages                    = {506-11},
  Volume                   = {8},

  Abstract                 = {Periodic dielectric structures are typically integrated with a planar waveguide to create photonic band-edge modes for feedback in one-dimensional distributed feedback lasers and two-dimensional photonic-crystal lasers. Although photonic band-edge lasers are widely used in optics and biological applications, drawbacks include low modulation speeds and diffraction-limited mode confinement. In contrast, plasmonic nanolasers can support ultrafast dynamics and ultrasmall mode volumes. However, because of the large momentum mismatch between their nanolocalized lasing fields and free-space light, they suffer from large radiative losses and lack beam directionality. Here, we report lasing action from band-edge lattice plasmons in arrays of plasmonic nanocavities in a homogeneous dielectric environment. We find that optically pumped, two-dimensional arrays of plasmonic Au or Ag nanoparticles surrounded by an organic gain medium show directional beam emission (divergence angle <1.5 degrees and linewidth <1.3 nm) characteristic of lasing action in the far-field, and behave as arrays of nanoscale light sources in the near-field. Using a semi-quantum electromagnetic approach to simulate the active optical responses, we show that lasing is achieved through stimulated energy transfer from the gain to the band-edge lattice plasmons in the deep subwavelength vicinity of the individual nanoparticles. Using femtosecond-transient absorption spectroscopy, we verified that lattice plasmons in plasmonic nanoparticle arrays could reach a 200-fold enhancement of the spontaneous emission rate of the dye because of their large local density of optical states.},
  Doi                      = {10.1038/nnano.2013.99},
  ISSN                     = {1748-3395 (Electronic)
1748-3387 (Linking)},
  Type                     = {Journal Article},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/23770807}
}

@Article{Zhu2009,
  Title                    = {Theortical calculation of enhancement factor of third-order nonlinear susceptibility in gold nanowire and nanotube},
  Author                   = {Zhu, Jian and Huang, Xia and Li, Jian-Jun and Zhao, Jun-Wu},
  Journal                  = {Journal of Optoelectronics and Advanced Materials},
  Year                     = {2009},
  Number                   = {1},
  Pages                    = {56-61},
  Volume                   = {11},

  Abstract                 = {The third-order nonlinear optical properties in gold nanowire and nanotube were theoretical studied by using quasi-static approximation. The enhancement factor patterns of the third-order nonlinear optical susceptibility in both gold nanowire and nanotube are anisotropic. For gold nanowire and the symmetric mode of nanotube, the "hot spots" of positive or negative nonlinear enhancement factors occur close to the poles of the wire or tube along the incident polarization direction. Whereas for antisymmetric mode of nanotube, the "hot spots" of positive or negative nonlinear enhancement factors occur within the gold tube and locate close to the poles of the tube along or perpendicular to the incident polarization direction. These calculation results show that the pattern of the third-order nonlinear enhancement factor is controlled by the fluctuation in surface electrons and the distribution of local electric field. These tunable third-order nonlinear optical characteristic will help us to select the best morphology of gold nanotube for the fabrication of smart optical nano-sensors.},
  ISSN                     = {1454-4164},
  Type                     = {Journal Article},
  Url                      = {<Go to ISI>://WOS:000263377300007}
}

@Article{Zia2006,
  Title                    = {Near-field characterization of guided polariton propagation and cutoff in surface plasmon waveguides},
  Author                   = {Zia, Rashid and Schuller, Jon and Brongersma, Mark},
  Journal                  = {Physical Review B},
  Year                     = {2006},
  Number                   = {16},
  Volume                   = {74},

  Doi                      = {10.1103/PhysRevB.74.165415},
  ISSN                     = {1098-0121
1550-235X},
  Type                     = {Journal Article}
}

@Article{OptMag,
  Title                    = {[Thesis]Optical Magnetometry with Nitrogen-Vacancy Centers in Diamond},

  Type                     = {Journal Article}
}


